ReZone: Disarming TrustZone with TEE Privilege Reduction

In TrustZone-assisted TEEs, the trusted OS has unrestricted access to both secure and normal world memory. Unfortunately, this architectural limitation has opened an aisle of exploration for attackers, which have demonstrated how to leverage a chain of exploits to hijack the trusted OS and gain full control of the system, targeting (i) the rich execution environment (REE), (ii) all trusted applications (TAs), and (iii) the secure monitor. In this paper, we propose ReZone. The main novelty behind ReZone design relies on leveraging TrustZone-agnostic hardware primitives available on commercially off-the-shelf (COTS) platforms to restrict the privileges of the trusted OS. With ReZone, a monolithic TEE is restructured and partitioned into multiple sandboxed domains named zones, which have only access to private resources. We have fully implemented ReZone for the i.MX 8MQuad EVK and integrated it with Android OS and OP-TEE. We extensively evaluated ReZone using microbenchmarks and real-world applications. ReZone can sustain popular applications like DRM-protected video encoding with acceptable performance overheads. We have surveyed 80 CVE vulnerability reports and estimate that ReZone could mitigate 86.84% of them.

==> Table-mechanism_implementation.tex <==
\begin{table}[htb]
\begin{tabular}{p{2.8cm}p{2.4cm}p{2.4cm}}
& iMX8QM
& iMX8M                   \\ \hline

CPU inaccessible memory                            
& Yes: Partition containing the AP clusters can be restricted from accessing memory regions                     
& Yes: a differente processor can use the RDC to create memory regions inaccessible to AP cores \\ \hline

Cluster private memory                             
& Yes: A partition can cover a single cluster, so that each cluster is running its own parititions
& Yes, in theory, but the platform only has one cluster             \\ \hline

Monitor private memory                             
& Through proposed scheme \ref{sec:scheme}
& Through proposed scheme \ref{sec:scheme}\\ \hline

Normal world memory inaccessible from secure world 
& Only by suspending all cores from running normal world software, we could then grey-out (by the memory regions from the partition) the normal world memory so that the trusted OS could not access it
& Only by suspending all cores from running normal world software, we could then grey-out (by marking memory as inaccessible to both worlds using TZASC) the normal world memory so that the trusted OS could not access it \\ \bottomrule
\end{tabular}
\end{table}

==> TableCVEanalysis-5column.tex <==
{\if10 %5 column


{    \newcommand{\Y}{\checkmark}
    \newcommand{\Par}{\LEFTcircle}
    \newcommand{\N}{---}
    \newcommand{\II}{?}
    \newcommand{\NA}{N/A}
\begin{table*}[!t]
\centering
\scalebox{0.65}{
\begin{minipage}{1.05\textwidth}
    %\scriptsize
    \centering
    % \setlength{\tabcolsep}{2pt}
    \setlength{\tabcolsep}{3pt}
    %\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{|ccc|ccc|ccc|ccc|ccc|}
    \hline
    CVE & C & & CVE & C & & CVE & C & & CVE & C & & CVE & C & \\ \hline
    \cveshort{2014-9979} & TO & \Y & \cveshort{2017-6292} & TO & \Y & \cveshort{2017-18315} & TO & \Y & \cveshort{2017-18317} & TA & \II & \cveshort{2016-2432} & TO/TA & \Y \\
    \cveshort{2015-8999} & TO & \Y & \cveshort{2017-6294} & TO & \Y & \cveshort{2018-3588} & TO & \Y & \cveshort{2018-5210} & TA & \Y & \cveshort{2016-10297} & TO/TA & \Y \\
    \cveshort{2015-9070} & TO & \Y & \cveshort{2017-8274} & TO & \Y & \cveshort{2018-5870} & TO & \Y & \cveshort{2018-5885} & TA & \Y & \cveshort{2017-6289} & TO/TA & \Y \\
    \cveshort{2015-9071} & TO & \Y & \cveshort{2017-11010} & TO & \Y & \cveshort{2016-10239} & TO & \Y & \cveshort{2014-9932} & TO/TA & \Y & \cveshort{2017-14913} & TO/TA & \Y \\
    \cveshort{2015-9072} & TO & \Y & \cveshort{2017-11011} & TO & \Y & \cveshort{2018-11950} & TO & \Y & \cveshort{2014-9935} & TO/TA & \Y & \cveshort{2017-18293} & TO/TA & \Y \\
    \cveshort{2015-9073} & TO & \Y & \cveshort{2017-14912} & TO & \Y & \cveshort{2015-4422} & TA & \Y & \cveshort{2014-9936} & TO/TA & \Y & \cveshort{2017-18296} & TO/TA & \II \\
    \cveshort{2015-9108} & TO & \Y & \cveshort{2017-14916} & TO & \Y & \cveshort{2015-6639} & TA & \Y & \cveshort{2014-9937} & TO/TA & \Y & \cveshort{2017-18297} & TO/TA & \Y \\
    \cveshort{2015-9112} & TO & \Y & \cveshort{2017-14917} & TO & \Y & \cveshort{2015-6647} & TA & \Y & \cveshort{2014-9945} & TO/TA & \Y & \cveshort{2017-18298} & TO/TA & \Y \\
    \cveshort{2015-9113} & TO & \Y & \cveshort{2017-17176} & TO & \Y & \cveshort{2015-9000} & TA & \Y & \cveshort{2014-9948} & TO/TA & \Y & \cveshort{2018-5866} & TO/TA & \Y \\
    \cveshort{2015-9198} & TO & \Y & \cveshort{2017-18071} & TO & \Y & \cveshort{2015-9002} & TA & \Y & \cveshort{2014-9949} & TO/TA & \Y & \cveshort{2017-18282} & HW & \N \\
    \cveshort{2015-9199} & TO & \N & \cveshort{2017-18128} & TO & \N & \cveshort{2015-9162} & TA & \Y & \cveshort{2015-8995} & TO/TA & \Y & \cveshort{2015-9003} & CI & \N \\
    \cveshort{2015-9200} & TO & \Y & \cveshort{2017-18129} & TO & \Y & \cveshort{2015-9174} & TA & \Y & \cveshort{2015-8996} & TO/TA & \Y & \cveshort{2016-10398} & CI & \N \\
    \cveshort{2016-2431} & TO & \Y & \cveshort{2017-18132} & TO & \Y & \cveshort{2015-9183} & TA & \Y & \cveshort{2015-8997} & TO/TA & \Y & \cveshort{2017-14907} & CI & \N \\
    \cveshort{2016-10238} & TO & \Y & \cveshort{2017-18133} & TO & \Y & \cveshort{2017-6293} & TA & \Y & \cveshort{2015-8998} & TO/TA & \Y & \cveshort{2017-18146} & CI & \N \\
    \cveshort{2016-10432} & TO & \Y & \cveshort{2017-18311} & TO & \Y & \cveshort{2017-18310} & TA & \N & \cveshort{2015-9005} & TO/TA & \Y & \cveshort{2016-10458} & BL & \N \\
    \cveshort{2017-6290} & TO & \Y & \cveshort{2017-18314} & TO & \II & \cveshort{2017-18312} & TA & \II & \cveshort{2015-9007} & TO/TA & \Y & \cveshort{2017-14911} & BL & \N \\
    \hline 
\end{tabular} 

\end{minipage}
%\hfill
\begin{minipage}{\textwidth}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{c|cc|c}
    \multicolumn{1}{c}{ } & \multicolumn{2}{c}{In Scope?} & \\
    \cmidrule(lr){2-3}
    \multicolumn{1}{c}{ } & \multicolumn{1}{c}{Y} & \multicolumn{1}{c}{N} & Total \\ \hline
    TO/TA & 21 & & 21 \\
    TO & 34 & 2 & 36 \\
    TA & 11 & 1 & 12 \\
    HW & & 1 & 1 \\
    CI & & 4 & 4 \\
    BL & & 2 & 2 \\ \hline
    Total & 66 & 10 & 76 \\
    Rel. & 86.84\% & 13.16\% & \\ \hline
    \end{tabular} 
    \vspace{-0.1cm}
\end{minipage}
}
\caption{\small Mitigation analysis of CVEs with critical CVSS scores: CVEs in scope (\Y), out of scope (\N), insufficient information (\II).} \label{tab:security-table}
\vspace{-0.5cm}
\end{table*}

\else


\begin{table*}[!t]

\centering
%\scriptsize
\newcommand{\Y}{\checkmark}
\newcommand{\Par}{\LEFTcircle}
\newcommand{\N}{---}
\newcommand{\II}{?}
\newcommand{\NA}{N/A}
% \setlength{\tabcolsep}{2pt}
\scalebox{0.65}{
\setlength{\tabcolsep}{3pt}
%\renewcommand{\arraystretch}{1.3}

\begin{tabular}{|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|} \hline
CVE & C & & CVE & C & & CVE & C & & CVE & C & & CVE & C & &CVE & C & &CVE & C & &CVE & C &  \\ \hline
\cveshort{2014-9979} & TO & \Y & \cveshort{2015-9199} & TO & \N & \cveshort{2017-11011} & TO & \Y & \cveshort{2017-18311} & TO & \Y & \cveshort{2015-9000} & TA & \Y & \cveshort{2018-5885} & TA & \Y & \cveshort{2015-8997} & TO/TA & \Y & \cveshort{2017-18297} & TO/TA & \Y \\
\cveshort{2015-8999} & TO & \Y & \cveshort{2015-9200} & TO & \Y & \cveshort{2017-14912} & TO & \Y & \cveshort{2017-18314} & TO & \II & \cveshort{2015-9002} & TA & \Y & \cveshort{2014-9932} & TO/TA & \Y & \cveshort{2015-8998} & TO/TA & \Y & \cveshort{2017-18298} & TO/TA & \Y \\
\cveshort{2015-9070} & TO & \Y & \cveshort{2016-2431} & TO & \Y & \cveshort{2017-14916} & TO & \Y & \cveshort{2017-18315} & TO & \Y & \cveshort{2015-9162} & TA & \Y & \cveshort{2014-9935} & TO/TA & \Y & \cveshort{2015-9005} & TO/TA & \Y & \cveshort{2018-5866} & TO/TA & \Y \\
\cveshort{2015-9071} & TO & \Y & \cveshort{2016-10238} & TO & \Y & \cveshort{2017-14917} & TO & \Y & \cveshort{2018-3588} & TO & \Y & \cveshort{2015-9174} & TA & \Y & \cveshort{2014-9936} & TO/TA & \Y & \cveshort{2015-9007} & TO/TA & \Y & \cveshort{2017-18282} & HW & \N \\
\cveshort{2015-9072} & TO & \Y & \cveshort{2016-10432} & TO & \Y & \cveshort{2017-17176} & TO & \Y & \cveshort{2018-5870} & TO & \Y & \cveshort{2015-9183} & TA & \Y & \cveshort{2014-9937} & TO/TA & \Y & \cveshort{2016-2432} & TO/TA & \Y & \cveshort{2015-9003} & CI & \N \\
\cveshort{2015-9073} & TO & \Y & \cveshort{2017-6290} & TO & \Y & \cveshort{2017-18071} & TO & \Y & \cveshort{2016-10239} & TO & \Y & \cveshort{2017-6293} & TA & \Y & \cveshort{2014-9945} & TO/TA & \Y & \cveshort{2016-10297} & TO/TA & \Y & \cveshort{2016-10398} & CI & \N \\
\cveshort{2015-9108} & TO & \Y & \cveshort{2017-6292} & TO & \Y & \cveshort{2017-18128} & TO & \N & \cveshort{2018-11950} & TO & \Y & \cveshort{2017-18310} & TA & \N & \cveshort{2014-9948} & TO/TA & \Y & \cveshort{2017-6289} & TO/TA & \Y & \cveshort{2017-14907} & CI & \N \\
\cveshort{2015-9112} & TO & \Y & \cveshort{2017-6294} & TO & \Y & \cveshort{2017-18129} & TO & \Y & \cveshort{2015-4422} & TA & \Y & \cveshort{2017-18312} & TA & \II & \cveshort{2014-9949} & TO/TA & \Y & \cveshort{2017-14913} & TO/TA & \Y & \cveshort{2017-18146} & CI & \N \\
\cveshort{2015-9113} & TO & \Y & \cveshort{2017-8274} & TO & \Y & \cveshort{2017-18132} & TO & \Y & \cveshort{2015-6639} & TA & \Y & \cveshort{2017-18317} & TA & \II & \cveshort{2015-8995} & TO/TA & \Y & \cveshort{2017-18293} & TO/TA & \Y & \cveshort{2016-10458} & BL & \N \\
\cveshort{2015-9198} & TO & \Y & \cveshort{2017-11010} & TO & \Y & \cveshort{2017-18133} & TO & \Y & \cveshort{2015-6647} & TA & \Y & \cveshort{2018-5210} & TA & \Y & \cveshort{2015-8996} & TO/TA & \Y & \cveshort{2017-18296} & TO/TA & \II & \cveshort{2017-14911} & BL & \N \\

\hline
\end{tabular} 
}

\vspace{0.2cm}

\renewcommand{\arraystretch}{1.1}
\scalebox{0.69}{
\begin{tabular}{ccccccc|cc}
In Scope? & TO/TA & TO & TA & HW & CI & BL & Total & Percentage \\
\hline
Y & 21  & 34    & 11    &   &   &   & 66 & 86.84\% \\
N &     & 2     & 1     & 1 & 4 & 2 & 10 & 13.16\% \\
\hline
Total & 21 & 36 & 12 & 1 & 4 & 2 & 76 & \\ 
\hline
\end{tabular} 
}
\vspace{-0.1cm}
\caption{\small Mitigation analysis of CVEs with critical CVSS scores: CVEs in scope (\Y), out of scope (\N), insufficient information (\II).} \label{tab:security-table}
\vspace{-0.5cm}
\end{table*}
}
}
\fi

==> TableResearchComparisoinTCB_seperate.tex <==
\if11

\begin{table*}[t]
        \begin{minipage}{0.65\textwidth}
            \centering
            \newcommand{\Y}{\checkmark}
            \newcommand{\Par}{\LEFTcircle}
            \newcommand{\N}{---}
            \newcommand{\II}{???}
            \newcommand{\NA}{N/A}
            % \setlength{\tabcolsep}{2pt}
            \scalebox{0.60}{
            \setlength{\tabcolsep}{2pt}
            \renewcommand{\arraystretch}{1.2}
            \begin{tabular}{c|ccc|ccc|cc|ccc}
            & \multicolumn{3}{|c}{\makecell{Security \\ (Can defend against)}} & \multicolumn{3}{|c}{ \makecell{Scalability \\ (Does not depend on)}} & \multicolumn{2}{|c}{\makecell{Programming \\ (Unmod. Code)}} & \multicolumn{3}{|c}{\makecell{Performance \\ (Sources of Overhead)}} \\
            \hline
            System & \makecell{TOS→NW \\ (P1)} & \makecell{TOS→Mon \\ (P2)} & \makecell{TOS$_1$→TOS$_2$ \\ (P3)} & PPC & ACU & \makecell{Non-COTS \\ Features} & Runtime & API & S2-TLB & \makecell{Micro. Arch. \\ Maintenance} & \makecell{Trap \& \\ Emul.} \\
            \hline
            %Typical TZ TEE & \bad & \bad & NA & \good & \good & \good & \good & \good & \good & \good & \good \\
            PrivateZone \cite{Jang2018} & \bad & \bad & \good & \bad & \good & \good & \bad & \bad & \bad & \bad & \good \\
            OSP \cite{Cho2016} & \bad & \bad & \good & \bad & \good & \good & \bad & \bad & \bad & \bad & \good \\
            vTZ \cite{Hua2017} & \bad & \good & \half & \bad & \good & \good & \good & \good & \bad & \good & \bad \\
            Sanctuary \cite{Brasser2019} & \bad & \bad & \good & \good & \good & \bad & \bad & \bad & \good & \bad & \good \\
            TrustICE \cite{Sun2015} & \bad & \bad & \good & \good & \good & \good & \bad & \bad & \good & \bad & \good \\
            TEEv \cite{Li2019} & \half & \half & \good & \good & \good & \good & \bad & \good & \good & \good & \bad \\
            PrOS \cite{Kwon19} & \bad & \half & \good & \bad & \good & \good & \bad & \good & \good & \good & \bad \\ 
            \textbf{\project} & \good & \good & \good & \bad & \bad & \good & \good & \good & \good & \bad & \good \\ 
                \bottomrule
            \end{tabular}
            }
            \caption{\small Analysis of \project and similar systems. \good\xspace indicates that the system fares positively, \bad\xspace that it fares negatively.}
            \end{minipage}
            \hfill
            \begin{minipage}{0.33\textwidth}
            \centering
            \setlength{\tabcolsep}{3pt}
            \renewcommand{\arraystretch}{1.5}
            \scalebox{0.6}{%
            \begin{tabular}{c|cccc}
            & Monitor & trustedOS & \makecell{Add. \\ LoC} & \makecell{Total \\ kLoC} \\ \midrule
            Vanilla TZ TEE & TF-A & OPTEE & - & 254.7 \\
            PrivateZone \cite{Jang2018} & TF-A* & OPTEE & libprivexec & 259.9 \\
            OSP \cite{Cho2016} & TF-A* & OPTEE & NW Hyp & 255.5 \\
            vTZ \cite{Hua2017} & 2,000 & - & & 2.0* \\
            Sanctuary \cite{Brasser2019} & TF-A* & OPTEE* & TA 2x & 256.0 \\
            TrustICE \cite{Sun2015} & TF-A* & OPTEE & - & 255.0 \\
            TEEv \cite{Li2019} & TF-A* & - & TEE-Visor & 28.8 \\
            PrOS \cite{Kwon19} & TF-A* & - & PVisor & 27.6 \\
            \textbf{\project} & \textbf{TF-A}* & - & gatekeeper & \textbf{30} \\ 
            \bottomrule
            \end{tabular}  
            }
            \vspace{-0.1cm}
            \caption{\small SLOC of the TCB for a Vanilla TZ TEE, \project, and similar systems.}
             \vspace{-0.5cm}
            \label{tab:tcb_comparison}
        \end{minipage}
    \end{table*}

\else 

\begin{table*}[t]\centering
%\scriptsize
\newcommand{\Y}{\checkmark}
\newcommand{\Par}{\LEFTcircle}
\newcommand{\N}{---}
\newcommand{\II}{???}
\newcommand{\NA}{N/A}
% \setlength{\tabcolsep}{2pt}
\scalebox{0.75}{
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|ccc|ccc|cc|ccc}
& \multicolumn{3}{|c}{\makecell{Security \\ (Can defend against)}} & \multicolumn{3}{|c}{ \makecell{Scalability \\ (Does not depend on)}} & \multicolumn{2}{|c}{\makecell{Programming \\ (Unmod. Software)}} & \multicolumn{3}{|c}{\makecell{Performance \\ (Sources of Overhead)}} \\
\hline
System & \makecell{TOS→NW \\ (P1)} & \makecell{TOS→Mon \\ (P2)} & \makecell{TOS$_1$→TOS$_2$ \\ (P3)} & PPC & ACU & \makecell{Non-COTS \\ Features} & Runtime & API & S2-TLB & \makecell{Micro. Arch. \\ Maintenance} & \makecell{Trap and \\ Emulate} \\
\hline
%Typical TZ TEE & \bad & \bad & NA & \good & \good & \good & \good & \good & \good & \good & \good \\
PrivateZone \cite{Jang2018} & \bad & \bad & \good & \bad & \good & \good & \bad & \bad & \bad & \bad & \good \\
OSP \cite{Cho2016} & \bad & \bad & \good & \bad & \good & \good & \bad & \bad & \bad & \bad & \good \\
vTZ \cite{Hua2017} & \bad & \good & \half & \bad & \good & \good & \good & \good & \bad & \good & \bad \\
Sanctuary \cite{Brasser2019} & \bad & \bad & \good & \good & \good & \bad & \bad & \bad & \good & \bad & \good \\
TrustICE \cite{Sun2015} & \bad & \bad & \good & \good & \good & \good & \bad & \bad & \good & \bad & \good \\
TEEv \cite{Li2019} & \half & \half & \good & \good & \good & \good & \bad & \good & \good & \good & \bad \\
PrOS \cite{Kwon19} & \bad & \half & \good & \bad & \good & \good & \bad & \good & \good & \good & \bad \\ 
\textbf{\project} & \good & \good & \good & \bad & \bad & \good & \good & \good & \good & \bad & \good \\ 
    \bottomrule
\end{tabular}
}
\vspace{-0.1cm}
\caption{\small Analysis of \project and similar systems. \good\xspace indicates that the system fares positively, \bad\xspace that it fares negatively.}
\label{tab:sys_comparison}
\vspace{-0.5cm}
\end{table*}



\begin{table}[!t]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.5}
\centering
\scalebox{0.74}{%
\begin{tabular}{c|cccc}
& Monitor & trustedOS & \makecell{Add. \\ LoC} & \makecell{Total \\ kLoC} \\ \midrule
Vanilla TZ TEE & TF-A & OPTEE & - & 254.7 \\
PrivateZone \cite{Jang2018} & TF-A* & OPTEE & libprivexec & 259.9 \\
OSP \cite{Cho2016} & TF-A* & OPTEE & NW Hyp & 255.5 \\
vTZ \cite{Hua2017} & 2,000 & - & & 2.0* \\
Sanctuary \cite{Brasser2019} & TF-A* & OPTEE* & TA 2x & 256.0 \\
TrustICE \cite{Sun2015} & TF-A* & OPTEE & - & 255.0 \\
TEEv \cite{Li2019} & TF-A* & - & TEE-Visor & 28.8 \\
PrOS \cite{Kwon19} & TF-A* & - & PVisor & 27.6 \\
\textbf{\project} & \textbf{TF-A}* & - & gatekeeper & \textbf{30} \\ 
\bottomrule
\end{tabular}  
}
\vspace{-0.1cm}
\caption{\small SLOC of the TCB for a typical TrustZone-assisted TEE system, \project, and related work. The reference SLOC value for the TF-A secure monitor is 24,607 and OP-TEE kernel is 230,094.  }
 \vspace{-0.5cm}
\label{tab:tcb_comparison}
\end{table}
\fi

==> TableResearchComparison.tex <==
\begin{table*}[t]\centering
%\scriptsize
\newcommand{\Y}{\checkmark}
\newcommand{\Par}{\LEFTcircle}
\newcommand{\N}{---}
\newcommand{\II}{???}
\newcommand{\NA}{N/A}
% \setlength{\tabcolsep}{2pt}
\scalebox{0.75}{
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|ccc|ccc|cc|ccc}
& \multicolumn{3}{|c}{\makecell{Security \\ (Can defend against)}} & \multicolumn{3}{|c}{ \makecell{Scalability \\ (Does not depend on)}} & \multicolumn{2}{|c}{\makecell{Programming \\ (Unmod. Software)}} & \multicolumn{3}{|c}{\makecell{Performance \\ (Sources of Overhead)}} \\
\hline
System & \makecell{TOS→NW \\ (P1)} & \makecell{TOS→Mon \\ (P2)} & \makecell{TOS$_1$→TOS$_2$ \\ (P3)} & PPC & ACU & \makecell{Non-COTS \\ Features} & Runtime & API & S2-TLB & \makecell{Micro. Arch. \\ Maintenance} & \makecell{Trap and \\ Emulate} \\
\hline
%Typical TZ TEE & \bad & \bad & NA & \good & \good & \good & \good & \good & \good & \good & \good \\
PrivateZone \cite{Jang2018} & \bad & \bad & \good & \bad & \good & \good & \bad & \bad & \bad & \bad & \good \\
OSP \cite{Cho2016} & \bad & \bad & \good & \bad & \good & \good & \bad & \bad & \bad & \bad & \good \\
vTZ \cite{Hua2017} & \bad & \good & \half & \bad & \good & \good & \good & \good & \bad & \good & \bad \\
Sanctuary \cite{Brasser2019} & \bad & \bad & \good & \good & \good & \bad & \bad & \bad & \good & \bad & \good \\
TrustICE \cite{Sun2015} & \bad & \bad & \good & \good & \good & \good & \bad & \bad & \good & \bad & \good \\
TEEv \cite{Li2019} & \bad & \bad & \good & \good & \good & \good & \bad & \good & \good & \good & \bad \\
PrOS \cite{Kwon19} & \bad & \bad & \good & \bad & \good & \good & \bad & \good & \good & \good & \bad \\ 
\textbf{\project} & \good & \good & \good & \bad & \bad & \good & \good & \good & \good & \bad & \good \\ 
    \bottomrule
\end{tabular}
}
\vspace{-0.1cm}
\caption{\small Analysis of \project and similar systems. \good\xspace indicates that the system fares positively, \bad\xspace that it fares negatively.}
\label{tab:sys_comparison}
\vspace{-0.5cm}
\end{table*}



==> TableTCBComparison.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.5}
\centering
\scalebox{0.74}{%
\begin{tabular}{c|cccc}
& Monitor & trustedOS & \makecell{Add. \\ LoC} & \makecell{Total \\ kLoC} \\ \midrule
Vanilla TZ TEE & TF-A & OPTEE & - & 254.7 \\
PrivateZone \cite{Jang2018} & TF-A* & OPTEE & libprivexec & 259.9 \\
OSP \cite{Cho2016} & TF-A* & OPTEE & NW Hyp & 255.5 \\
vTZ \cite{Hua2017} & 2,000 & - & & 2.0* \\
Sanctuary \cite{Brasser2019} & TF-A* & OPTEE* & TA 2x & 256.0 \\
TrustICE \cite{Sun2015} & TF-A* & OPTEE & - & 255.0 \\
TEEv \cite{Li2019} & TF-A* & - & TEE-Visor & 28.8 \\
PrOS \cite{Kwon19} & TF-A* & - & PVisor & 27.6 \\
\textbf{\project} & \textbf{TF-A}* & - & gatekeeper & \textbf{30} \\ 
\bottomrule
\end{tabular}  
}
\vspace{-0.1cm}
\caption{\small SLOC of the TCB for a typical TrustZone-assisted TEE system, \project, and related work. The reference SLOC value for the TF-A secure monitor is 24,607 and OP-TEE kernel is 230,094.  }
 \vspace{-0.5cm}
\label{tab:tcb_comparison}
\end{table}

==> backups/back-20220205-intro.tex <==
%=======================================================================
%> [INTRO]
%=======================================================================	
\section{Introduction}

Arm TrustZone~\cite{Pinto2019, Pinto2019_2} is a technology embedded into Arm processors presently found in billions of mobile phones and embedded devices, such as car infotainment systems and SmartTVs. Vendors and Original Equipment Manufacturers (OEM) rely on TrustZone for deploying Trusted Execution Environments (TEEs), which protect the execution of sensitive programs named Trusted Applications (TAs).  Some TAs implement kernel-level services of the operating system (OS); for example, for user authentication or file disk encryption~\cite{androidwhitepaper}. Other TAs implement shared user-level functionality, e.g., DRM media decoders~\cite{TZVideoPath} or online banking services~\cite{trustonicBanking}. TEEs themselves consist of a trusted software stack offering API and runtime support for hosting TAs. TEEs such as Qualcomm's QSEE and OP-TEE protect the confidentiality and integrity of TAs' memory state, thereby ensuring it cannot be inspected or tampered with by a potentially compromised OS.

To protect the TAs, TEEs leverage mechanisms provided by TrustZone. In Armv7-A/Armv8-A, this technology provides two execution environments named \textit{normal world} and \textit{secure world}\footnote{As per Arm's recent documentation~\cite{tzarmv8a}, \textit{secure world} can be referred to as \textit{trusted world}; we adopt the previous and more familiar terminology~\cite{Pinto2019}.}. The normal world runs a rich software stack, named Rich Execution Environment (REE), comprised of full-blown OS and applications; it is generally considered untrusted. The secure world runs a smaller software stack consisting of TEE and TAs. TrustZone enforces system-wide isolation between worlds and provides controlled entry points for world switching whenever the REE invokes TAs' services.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/intro-trustzone.pdf}
    \vspace{-0.3cm}
    \caption{\small Privilege escalation attack in a TrustZone-assisted TEE: (1) hijack a user-level TA, e.g., exploiting vulnerability in the Widevine TA (CVE-2015-6639)~\cite{gb-exploit4}, (2) hijack the trusted OS, e.g., exploiting vulnerability in syscall interface of Qualcomm's QSEOS (CVE-2016-2431)~\cite{gb-exploit5}. Once in control of the trusted OS, other attacks can be launched: (a) control the rich OS, e.g., backdoor in the Linux kernel~\cite{gb-exploit6}, (b) control a kernel-level TA, e.g., to extract full disk encryption keys of Android's KeyMaster service~\cite{gb-keymaster}, or (c) control the secure monitor, e.g., to unbrick the device bootloader~\cite{gb-bootloader}.}
    \label{fig:intro_trustzone}
    \vspace{-0.5cm}
\end{figure}

However, a fundamental limitation of the TrustZone security architecture is that the trusted OS -- i.e., one of TEE's core components -- runs with an excess of privileges, exposing the entire system to catastrophic privilege escalation attacks if the trusted OS gets compromised. Figure~\ref{fig:intro_trustzone} illustrates how these attacks can be launched. It shows the TEE stack, consisting of the \textit{secure monitor} and \textit{trusted OS}. The secure monitor runs in EL3 -- the most privileged exception level -- and provides essential mechanisms for world switching and platform management. The trusted OS runs in S.EL1 -- i.e., secure kernel mode -- and implements memory management, scheduling, IPC, and common services for TAs. TAs run in unprivileged S.EL0 -- i.e., secure user mode. TAs are directly exposed to malicious requests coming from normal world applications. If a TA's control flow gets hijacked as a result of exploiting a software vulnerability (1), the attacker can control that TA. If the attacker can further hijack the trusted OS by exploiting another vulnerability (2), he can gain full control of the system, including: the REE in the normal world (a), all the TAs (b), and the secure monitor (c). This level of control is possible because S.EL1 gives full permission to access and reconfigure both secure and non-secure memory regions.
%
\rev{These problems mostly carryover to Armv8.4 and onward, with S-EL2 having the same privileges as S-EL1 up until Armv8.4. Armv9 is also susceptible to some of these problems, although to a lesser a extent. Because \project offers guarantees that the new architectures do not, it can be used to complement them.}

Unfortunately, numerous devices today face serious risks of being compromised by attacks of this nature. In the past, security researchers have demonstrated how these attacks can be mounted as described above, escalating privileges from NS.EL0 into S.EL1 by chaining two exploits: first, targeting a vulnerable DRM TA~\cite{gb-exploit4}, and then a vulnerability in the system call interface of the trusted OS~\cite{gb-exploit5}. Once in control of the trusted OS, it was possible to (a) plant a backdoor in Linux kernel~\cite{gb-exploit6}, (b) retrieve cryptographic keys from Android's KeyMaster~\cite{gb-exploit4}, or (c) disable trusted boot protections~\cite{gb-bootloader}. Notably, recent studies~\cite{Cerdeira2020} have shown that commercial TEE systems have plenty and serious vulnerabilities, most of them affecting user-level TAs and trusted OS. This suggests that the current attack surface for TEE systems is seriously enlarged.

Despite the abundant research on TrustZone security~\cite{Pinto2019,Cerdeira2020}, there is a lack of practical system defenses if the trusted OS is hijacked. TEE systems like Sanctuary~\cite{Brasser2019} aim to reduce the attack surface of the trusted OS by relocating TAs onto user-level enclaves in the normal world. However, due to portability reasons, vendors and OEMs continue deploying TAs in commercial TEEs, therefore exposing many devices to potential attacks. Another approach is to confine the TEE stack inside a secure world sandbox, e.g., by leveraging same privilege isolation~\cite{Kwon19,Li2019} or hardware virtualization~\cite{hafnium}. Same privilege isolation uses binary instrumentation to sanitize dangerous instructions of the trusted OS. Unfortunately, if the control flow of the trusted OS is hijacked at runtime, an attacker can still execute arbitrary secure memory accesses. Hardware virtualization can help create sandboxed environments using virtual machines. However, virtualization support for the secure world (S.EL2) is fairly recent, i.e., in Armv8.4-A. As a result, it cannot be used in many devices today.

This paper presents \project, a new security architecture that can effectively counter ongoing privilege escalation attacks by reducing the privileges of a potentially compromised trusted OS. \rev{Following previous works~\cite{Kwon19, Li2019}, and Arm's new architectures~\cite{armv84sel2,armv9realms},} this is achieved by creating \textit{zones}, i.e., sandboxed domains inside the secure world. Zones have access only to private memory regions, and provide an execution environment for untrusted S.EL$_\textrm{1/0}$ code, i.e., trusted OS and TAs. \project restricts the memory access privileges of the code running inside a zone, preventing it from arbitrarily accessing memory allocated for: (a) the normal world REE, (b) other zones, and (c) the secure monitor. %The only way for a given zone to communicate with an external memory protection domain is through mutually shared memory regions. 
With \project, a typical monolithic TEE can then be restructured and partitioned into multiple zones. For instance, Figure~\ref{fig:intro_rezone} depicts a setup featuring two zones -- 1 and 2 -- each of them runs a trusted OS instance as in a library OS. Then, user-level TAs and kernel-level TAs run in independent zones. With this configuration, an attacker hijacking the trusted OS in zone 1 (as explained in Figure~\ref{fig:intro_trustzone}), will not be able to further escalate its privileges beyond its sandbox. To give vendors and OEMs maximal flexibility, \project allows the creation of additional zones, and using different trusted OSes inside different zones.

A central novelty of \project's design is that we take advantage of a TrustZone-agnostic resource controller available in modern SoCs to restrict the privileges of S.EL1 (trusted OS) code. Existing systems such as Sanctuary~\cite{Brasser2019} have already leveraged the TrustZone Address Space Controller (TZASC) for protecting user-level enclaves in the normal world. For example, TZC-400 features the possibility to specify access permissions to various physical memory regions, including the ability to prevent secure world code from accessing predefined regions of secure world memory. However, S.EL1 code can still revert these permissions, rendering the TZASC insufficient for zone isolation. Instead, we use a TrustZone-agnostic resource controller that allows specific bus masters to control memory access permissions. An example is the Resource Domain Controller (RDC), existing in iMX8MQ and iMX8QM SoCs. In \project, we harness this feature and reserve a low-end microcontroller also available in the SoC to control how these permissions are set, effectively creating private memory regions for each zone. RDC and microcontroller can then be used as building blocks for restricting the memory access privileges of a (potentially compromised) trusted OS, and enforce strong zone isolation.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/intro-rezone.pdf}
    \vspace{-0.3cm}
    \caption{\small \project setup enforcing TEE privilege reduction: after compromising user-level TA$_\textrm{U}$ and trusted OS in zone 1, an attacker cannot escalate privileges to (a) rich OS, (b) kernel-level TA$_\textrm{K}$ in zone 2, or (c) secure monitor.}
    % \vspace{-0.2cm}
    \label{fig:intro_rezone}
    \vspace{-0.5cm}
\end{figure}

Based on this insight, we have built \project. Our system includes multiple non-trivial optimizations and fine-grained mechanisms to guarantee system-wide security (e.g., avoiding cache-based attacks based on cached content available for EL3 and S.EL1 code). To make our design generally applicable to various hardware platforms, we specify the general properties of SoCs that satisfy \project's requirements. We have fully implemented a \project prototype for the i.MX 8MQuad EVK, and integrated it with Android OS as REE and with OP-TEE as TEE. Our code will be open sourced.

We evaluated \project using microbenchmarks and real-world applications. Our evaluation shows that despite the existence of non-negligible performance overhead in microbenchmark programs, \project does not sensibly degrade the performance of applications such as crypto wallets or DRM media decoders. The DRM application, which requires frequent transitions between the normal world and the zone, preserves its ability to replay video at high frame rates. 
%The overall performance of the system is only mildly affected ($<$0.04\% slowdown). 
We have surveyed 80 CVE vulnerability reports and estimate that \project can thwart 87\% of potential privilege escalation attacks arising from exploiting these bugs.


==> backups/back-20220205-sec2.tex <==
%=======================================================================
%> [BACKGROUND]
%=======================================================================	
\section{Background and Motivation}

\subsection{Standard TrustZone Mechanisms}

We focus on TrustZone for Armv8-A architectures. TrustZone enables CPU cores to operate in one of two states: \textit{secure} and \textit{non-secure}. At exception levels EL0 and EL1, a processor core can execute in either of these states. For instance, the processor is in non-secure exception level 1 (NS.EL1) when running REE kernel code, and in secure EL1 (S.EL1) if executing the trusted OS. EL3 is always in secure state. To change security states, the execution must pass through EL3.

TrustZone extends the memory system by means of an additional bit called \textit{NS bit} that accompanies the address of memory and peripherals (see Figure~\ref{fig:RZ_HW}). This bit creates independent physical address spaces for normal world and secure world. Software running in the normal world can only make \textit{non-secure accesses} to physical memory because the core always tags the bus NS bit to 1 in any memory transaction generated by the normal world. Software running in the secure world usually makes only \textit{secure accesses} (i.e., NS=0), but can also make non-secure accesses (NS=1) for specific memory mappings using the NS flags in its page table entries. The processor maintains separate virtual address spaces for the secure and non-secure states. Trusted OS (or the secure monitor) can map virtual addresses to non-secure physical addresses by setting to 1 the NS bit in its page table entries. In non-secure state, that bit is ignored: the virtual address will always be translated to non-secure physical address (NS=0).

TrustZone-aware memory controllers are usually configured to assign non-secure/secure physical address spaces to different physical memory regions. In the Arm architecture, the TZASC enforces physical memory protection by allowing the partitioning of external memory on secure and non-secure regions. (The TZPC performs a similar function for peripherals.) To date, Arm has released two TZASC versions: Arm CoreLink TZC-380 and TZC-400. They share similar high-level features, i.e., the ability to configure access permissions for memory regions (contiguous address space areas).

\subsection{The Excess of Privileges of the Trusted OS}
\label{sec:challenge}

The TrustZone mechanisms described above were designed under the assumption that the S.EL1 (trusted OS) and EL3 (secure monitor) are trusted. However, if the trusted OS is hijacked, the attacks described in Figure~\ref{fig:intro_trustzone} can be trivially mounted. For illustration purposes, suppose that the physical memory addresses PA$_\textrm{OS}$, PA$_\textrm{TK}$, and PA$_\textrm{SM}$ are allocated to the rich OS, TA$_\textrm{K}$, and secure monitor, respectively. The attacker could mount said attacks by creating virtual address mappings in the S.EL1 page tables as indicated below, and use the virtual addresses VA$_i$ to access (read/write) the memory pages of the rich OS, TA$_\textrm{K}$, or secure monitor. Notation VA$\rightarrow\langle$PA, NS$\rangle$ denotes a page table entry translating virtual address VA to the physical address PA and associated NS bit value:

\noindent VA$_\textrm{OS}\rightarrow\langle$PA$_\textrm{OS}$, 1$\rangle$, VA$_\textrm{TK}\rightarrow\langle$PA$_\textrm{TK}$, 0$\rangle$, VA$_\textrm{SM}\rightarrow\langle$PA$_\textrm{SM}$, 0$\rangle$

\if10 %usenix subtmited
Simply put, the ability of the trusted OS to establish these mappings on its own address space enables it to access any system component, including the monitor. This means that a compromised trusted OS can take over every part of the system. For this reason, we argue that reducing the memory access privileges of S.EL1 code can significantly lower the impact of vulnerability exploits targeting the trusted OS. % as has been proposed in previous works~\cite{Li2019, Kwon19, Jang2018}.
\else %usenix revision
\rev{Simply put, \emph{the secure monitor cannot interfere with a trusted OS's ability to establish these mappings on the S-EL1 address space, which enables it to access any system component, including the monitor, TZASC, and all other software and hardware components}. This means that a compromised trusted OS can take over every part of the system. For this reason, we argue that reducing the memory access privileges of S.EL1 code can significantly lower the impact of vulnerability exploits targeting the trusted OS. % as has been proposed in previous works~\cite{Li2019, Kwon19, Jang2018}.
}
\fi

\rev{Arm's new architecture releases starting from Armv8.4, seem to solve this problem by introducing a trusted hypervisor. However, and even though the hypervisor adds a new layer fof defence, the security of the system relies on the trusted hypervisor. In Armv8.4 both normal world and the monitor can be attacked by a malicious trusted hypervisor as there's no isolation between these privilege levels. Effectively S-EL2 inherits all the priveleges of S-EL1 from the previous generation. Further, even though Armv9 brings protection to EL3, effectively protecting the secure monitor, a malicious hypervisor can still compromise the normal world.}

\input{TableCOTS}

%\subsection{Platform Model for Sandboxing the Trusted OS}\label{sec:plat_req}
\subsection{Platform Model}
\label{sec:plat_req}

Reducing the privileges of S.EL1 code so as to prevent unauthorized memory accesses is not straightforward using standard TrustZone mechanisms alone. Even though TZASC controllers such as TZC-380 and the TZC-400 can restrict memory accesses, since S.EL1 has the privilege to reconfigure the TZASC, the trusted OS can always override any permissions for blocking the trusted OS's access to certain memory regions. Also, TZASC does not distinguish between privilege levels, thus secure monitor (VA$_\textrm{SM}$) and TAs (VA$_\textrm{TK}$) memory cannot be restricted.

\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/rezone-hw.pdf}
    \vspace{-0.4cm}
    \caption{\small Hardware platform featuring TrustZone: \project-enabling hardware components are highlighted. These are the ACU and the PPC. PPC is configured by the bus master MID$_\textrm{1}$ (ACU). These configurations determine which access permissions are granted to a given MID for a specific physical memory region.}
    \label{fig:RZ_HW}
    \vspace{-0.2cm}
\end{figure}

Given the limitations of vanilla TrustZone mechanisms, we propose to leverage complementary, TrustZone-agnostic hardware features available in modern platforms for preventing illegal memory accesses potentially performed by untrusted S.EL1 code. These features consist of three hardware primitives that we require to be offered by the underlying platform.

\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
\item \textit{Platform Partition Controller (PPC):} Consists of a memory and peripheral protection controller that can restrict physical accesses to a given resource, i.e., memory or peripheral (see Figure~\ref{fig:RZ_HW}). On the iMX8MQ SoC, the PPC is implemented by the RDC peripheral. We characterize the PPC by having four main properties. It must be capable of: (a) intercepting all physical requests regardless of both the NS bit signal injected into the system bus and the configurations of the TZASC, (b) setting fine-grained access control attributes (e.g., RO, RW) for configurable memory regions; (c) differentiating between multiple bus masters, and (d) protecting memory-mapped input/output (MMIO) regions, including the PPC's memory-mapped registers. Importantly, (c) and (d) help to ensure that the PPC's configurations cannot be arbitrarily changed by (untrusted) S.EL1 code executed by the processor. Intuitively, to provide this guarantee in the setup illustrated in Figure~\ref{fig:RZ_HW}, the PPC would not allow the bus master identified with MID$_\textrm{0}$ -- i.e., the processor cluster -- to arbitrarily change the PPC configurations. Instead, as explained next, it is the bus master identified with MID$_\textrm{1}$ that will have that privilege.


%Property (a) ensures that we can block arbitrary memory accesses from S.EL1 without the concern of being overridden by the TZASC, and (b) gives flexibility to configure access permissions differently for various memory regions. Properties (c) and (d) allow restricting which bus masters are authorized for changing the configurations of the PPC. Importantly, this feature helps to ensure that the PPC's configurations cannot be arbitrarily changed by (untrusted) S.EL1 code executed by the processor. Intuitively, to provide this guarantee in the setup illustrated in Figure~\ref{fig:RZ_HW}, the PPC would not allow the bus master identified with MID$_\textrm{0}$ -- i.e., the processor cluster -- to arbitrarily change the PPC configurations. Instead, as explained next, it is the bus master identified with MID$_\textrm{1}$ that will have that privilege.

\item \textit{Auxiliary Control Unit (ACU):} This is an independent processor core, distinct from the main application processors. ACUs are small microcontrollers like Cortex-M4 added for housekeeping purposes. 
%Typically, these cores are added for housekeeping purposes and implemented as small microcontrollers (e.g., Cortex-M4). 
For example, Figure~\ref{fig:RZ_HW}, the ACU is identified by MID$_\textrm{1}$. The ACU coordinates the configuration of memory access permissions in the PPC, ensuring that the main processor cores cannot tamper with the PPC permissions. %The ACU executes a piece of trusted code responsible for implementing this coordination protocol.

\item \textit{Secure boot:} %This last building block aims to guarantee that the management core is in full control of the system's PPC and ACU. 
Secure boot validates the integrity and authenticity of the firmware, ensuring that the ACU has been securely bootstrapped and fully controls the PPC.
\end{enumerate}


%\subsection{PPC and ACU in COTS Platforms}\label{sec:PPC_ACU_COTS}

\subsection{Hardware Support on COTS Platforms}\label{sec:PPC_ACU_COTS}

\if10 %before revision
These primitives are readily available in several SoCs, for instance on iMX8MQ and iMX8QM SoCs, which we use for building \project. In these SoCs, the PPC and the ACU are implemented, respectively, by a hardware controller named Resource Domain Controller (RDC) and a Cortex-M4 processor. 
%Given that we have abstractly modeled the platform primitives presented above, 
Our defense mechanisms can further be ported to other platforms beyond the iMX8 SoC family. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol}. Also, a wide-range of Qualcomm Snapdragon family SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu, xpucves}. Both fulfill all PPC's requirements. All NXP's iMX8, Xilinx's Zynq and Qualcomm's Snapdragon SoCs deployments span a wide range of edge computing settings (e.g. automotive)~\cite{qc_report, nxp_report, xilinx_report}. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also fill the same role. ACUs are also a clear trend in modern SoCs, which tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}. 
\fi

\if10 % first revision iteration
\rev{The PPC and ACU primitives are readily available in several SoCs, see \autoref{tab:rezone-cots}, for instance on iMX8MQ SoC, which we use for building \project. In this SoC, the PPC and the ACU are implemented, respectively, by a hardware controller named Resource Domain Controller (RDC) and a Cortex-M4 processor.
%Given that we have abstractly modeled the platform primitives presented above, 
Our defense mechanisms can further be ported to other platforms beyond the iMX8 SoC family, and besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that can also fill the same role. The information gathered in this section was derived from looking at device trees, u-boot and TF-A source code, publicly available documentation such as reference manuals, and CVEs. CVEs helped us identified that Qualcomm platforms feature the XPU.}


\rev{As for specific platforms, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol}. Also, a wide-range of Qualcomm Snapdragon family SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu, xpucves} and SMMU. All these fulfill PPC's requirements, see ($\S \ref{sec:plat_req})$. The combination of NXP's iMX8, Xilinx's Zynq and Qualcomm's Snapdragon SoCs deployments span a wide range of edge computing settings (e.g. automotive)~\cite{qc_report, nxp_report, xilinx_report}. Nonetheless, other platforms that can support ReZone include Nvidia Tegra X1 and X2, and Xavier platforms, as well as Socionext SC2A11 and the Broadcom Stingray. Not all current platform can support ReZone though. Examples are Samsung Mediatek and Hisilicon platforms, which don't feature platform wide SMMUs, rather, they feature peripheral specific MMUs, usually for the purposes of media processing.}

\rev{In \autoref{tab:rezone-cots} the "Can Support \project" column values mean the following. "No" means that the platform does not support \project, "Unlikely" means that although there are PPC like mechanisms it is unlikely that they can be used on the CPU itself. "Likely" means that there is a PPC mechanism that is likely to apply to the CPU. Both these values suffer from lack of information, meaning that we don't have enough information to arrive at a definitive conclusion. "Yes" means that there is enough information available to conclude that ReZone can be used in the platform.}

\rev{ACUs are a clear trend in modern SoCs, which tend to include an increasing number of companion processing units for power management and security operations~\cite{armscp}. All analyzed platforms feature, in some form, an ACU. Recent Qualcomm platforms feature a Security Computing Unit (SCU), recent Samsung platforms feature an integrated, or embedded, secure element iSE/eSE, Mediatek features a power management IC, Socionext SC2A11, UltraScale+ MPSoc and the rest feature a variety of auxiliary units that can be reprogrammed to serve as ReZone's ACU.}
\fi

\if0 % second revision iteration
% para saber se a solucao que estamos a propor pode ser aplicada em larga escala, temos que saber se as plataforms COTS tem os componentes hw necessários para dar suporte a PPC e ACU, especialmente
% para fazer essa analise, dado que essa informacao nao está facil de forma acessivel, fizemos um estudo que consiste em aanlizar o suporte kernel, CVEs, etc para saber: 1) que componentes é que têm papel semelhante a PPC e ACU, e 2) que plataformas é que têm esses compoennts
% com base no nosso estudo, temos as principais resultados na tabela:
\rev{We first identified the the presence of a PPC, and an ACU in our development board, the i.MX8MQ. 
To access if readily available COTS platforms can support \project, we must identify the presence of the necessary mechanisms in a variety of platforms from different vendors. Given that this information is not easily accessible, we perform a study where we analyzed kernel, bootloader, and secure monitor support for these mechanisms. In particular, for Qualcomm platforms we looked at Linux 5.16 for SD855~\footnote{https://gitlab.com/sm8150-mainline/linux}, which luckily includes information about recent and past platforms. For Hisilicon we looked at the Huawei Mate 40 Pro Linux kernel code~\footnote{https://consumer.huawei.com/en/opensource/}. For Mediatek 1200 we looked at the OnePlus Nord 2 Linux kernel source~\footnote{https://github.com/OnePlusOSS/android\_kernel\_oneplus\_mt6893.git}. For the Samsung platforms we looked at the Exynos version of the S20, and S21 Linux kernel source code~\footnote{https://opensource.samsung.com/main}. For information about other platforms we analyzed TF-A~\footnote{https://git.trustedfirmware.org/TF-A/trusted-firmware-a.git/ v2.4} and U-boot source code~\footnote{https://github.com/u-boot/u-boot v2022.01}.
Further we've analyzed publicly available documentation such as reference manuals~\footnote{https://developer.nvidia.com/embedded/downloads}~\footnote{https://www.xilinx.com/support/documentation/user\_guides/ug1085-zynq-ultrascale-trm.pdf}, when available, and CVEs. CVEs were useful in identifying that many Qualcomm platforms feature an PPC like mechanism called XPU. This analysis demonstrated that there are other mechanisms which have the necessary PPC properties, and that there commonly are ACUs in COTS platforms. The main findings are presented in \autoref{tab:rezone-cots}.}

% agora explicar os componentes alternativos que fazem as vezes de PPC
\rev{At first, it may seem that TZASC fits the requirements for a PPC. However, a TZASC only protects memory regions, and so misses PPC requirement d). Additionally, only TZASC-400 can differentiate between bus masters, a highly specific hardware component not widely deployed to the best of our knowledge. In fact, looking at the latest TF-A release only two platforms support TZASC-400: NXP's lx2160a and ls1028a. To control access to peripherals another TrustZone component is needed, the TZPC. The available documentation shows, however, that the TZPC cannot distinguish between multiple bus masters nor prevent accesses to itself, missing PPC requirements c) and d).}

\rev{The mechanisms that we identified that can be used as a PPC are the SMMU, the XPU, the RDC, and the XMPU in conjunction with the XPPU. The SMMU is a relatively standard component, which enables, among other things, fine-grained restrictions on bus master accesses to resources at a system bus level. However, there are custom implementations of SMMUs that are designed to only interpose accesses of specific bus masters, for example media processing hardware. Such is the case of the Mediatek 1200, and the Kirin 9000. Platforms can feature multiple SMMUs, and they can server various bus masters. Nonetheless, in the case of the Samsung Platforms not enough information is available to ascertain that these SMMUs cannot be used to filter CPU accesses. The XPU~\cite{qualcommxpu}, is a Qualcomm hardware component which fills the PPC requirements, and the same is true for the XMPU and XPPU, which restrict accesses to memory and peripherals respectively~\cite{xilinxisol}. In general we observe that recent platforms are more likely to feature PPC-like mechanisms.}


% depois os componentes alternativos que fazem as vezes de ACU
\rev{ACUs are a clear trend in modern SoCs, which tend to include an increasing number of companion processing units for power management and security operations~\cite{armscp}. The ACUs on the platforms we analyzed are varied. Qualcomm, Samsung and NXP's iMX8QM feature security co-processors, namely the Secure Processing Unit (SPU)~\cite{SPU2019}, integrated/embedded Secure Element (iSE and eSE), and the System Controller Unit (SCU). Otherwise, platforms can feature programmable micro-processors, as in the case of the iMX8MQ. Although Mediatek features a System Control Processor (SCP), the component is likely too restrictive to host the gatekeeper, in particular because the interface is a set of well defined MMIO registers and not a mailbox interface as the other ACUs we analyzed. The rest of the ACUs all serve the same generic purpose, i.e., to abstract platform management operations, e.g., coordinating platform low power states.}

% depois um apanhado geral das placas que têm estes componentes com sugestão de haver uma trend que só vai fazer com que isto prolifere ainda mais
\fi


\nuno{The primitives presented above are readily available on iMX8MQ and iMX8QM SoCs, the first of which we use for building \project. In these SoCs, PPC and ACU are implemented, respectively, by a hardware controller named Resource Domain Controller (RDC) and a Cortex-M4 processor. To further assess if \project can be applied at a large scale, we need to determine if a variety of commercial-off-the-shelf (COTS) platforms are equipped with hardware components that can play the role of PPC and ACU. To this end, we analyzed 17 popular SoC platforms from nine different vendors. We based our study on several sources. In some cases, we consulted publicly available SoC reference manuals. In others, we inspected the source code of the Linux kernel, bootloader, and secure monitor looking for PPC/ACU driver support. CVEs were also useful for identifying a PPC-like mechanism on Qualcomm SoCs. Our main findings are presented in \autoref{tab:rezone-cots}.}

%%NS> important sentnce: This analysis demonstrated that there are other mechanisms which have the necessary PPC properties, and that there commonly are ACUs in COTS platforms.

% agora explicar os componentes alternativos que fazem as vezes de PPC
\mypara{PPC hardware candidates:} \nuno{Apart from the RDC, we identified several other components that can be used as PPC: SMMU, XPU, and XMPU in conjunction with XPPU. The SMMU is a relatively standard hardware component that enables, among other things, to enforce fine-grained restrictions on bus master accesses to resources at a system bus level. All of our studied platforms by Nvidia, Qualcomm, and Broadcom include a full-fledged SMMU. However, some custom SMMU implementations are designed to only interpose accesses of specific bus masters, e.g., media processing hardware. Such is the case of Mediatek 1200 and Kirin 9000. Samsung Exynos 900/2100 include dedicated SMMUs for specific peripherals. However, due to the lack of available information, we cannot ascertain that these SMMUs can also filter CPU accesses. The XPU~\cite{qualcommxpu} is a Qualcomm hardware component that entirely fills the PPC requirements. The same is true for Xilinx's XMPU and XPPU, which restrict accesses to memory and peripherals respectively~\cite{xilinxisol}. In general we observe that recent platforms are more likely to feature PPC-like mechanisms\footnote{Note that, at a first glance, it may seem that TZASC fits all the PPC requirements enumerated in Section~\ref{sec:plat_req}. However, a TZASC only protects memory regions. Therefore, it misses the PPC requirement (d). Additionally, only TZASC-400 can differentiate between bus masters, a highly specific hardware component not widely deployed, to the best of our knowledge. In fact, looking at the latest TF-A release only two platforms support TZASC-400: NXP's lx2160a and ls1028a. To control access to peripherals another TrustZone component is needed, the TZPC. The available documentation shows, however, that the TZPC cannot distinguish between multiple bus masters nor prevent accesses to itself, missing PPC requirements (c) and (d).}.}


% depois os componentes alternativos que fazem as vezes de ACU
\mypara{ACU hardware candidates:}
\nuno{On the platforms that we analyzed, we identified various ACU candidates. Qualcomm, Samsung, and NXP's iMX8QM are shipped with security co-processors: Secure Processing Unit (SPU)~\cite{SPU2019}, integrated/embedded Secure Element (iSE and eSE), and System Controller Unit (SCU). All other surveyed platforms incorporate programmable micro-processors that are generally reserved for platform management purposes, e.g., coordinating platform low power states. With one exception, all these micro-processors can be used as a full-fledged ACU. Although Mediatek's SoC features a System Control Processor (SCP), this platform is likely too restrictive to host \project, because the SCP interface is based on MMIO registers and not a mailbox interface as the other ACUs we analyzed. In summary, our findings are consistent with Arm's reports~\cite{armscp}, which point to a clear trend in modern SoCs to include companion processing units for power management and security operations.
}

\mypara{Platform support for \project:} \nuno{From our analysis, we found that 13 SoCs have suitable PPC and ACU hardware, which make the deployment of \project possible on devices featuring these platforms. In contrast, the SoCs from Mediatek and HiSilicon lack at least one of the required PPC or ACU mechanisms to accommodate \project. In the case of Samsung's SoCs, we miss important information to issue a final judgment. Notably, most of the analyzed Qualcomm platforms are compatible with \project, which means that our system can potentially be deployed on many commodity mobile devices.}

%\rev{On the mobile platforms we analyzed, only Qualcomm, featuring a PPC, can support \project. From the information we gathered,  However, Qualcomm platforms going back at least to 2018 can support it as well. Taking into account the large number of sold Qualcomm SoCs~\footnote{https://www.counterpointresearch.com/smartphone-soc-shipments-q3-2021/}, \project could potentially be deployed on a significant number of mobile platforms.}

%% (SPU)~\cite{SPU2019}

%These primitives are currently available, e.g., on iMX8MQ and iMX8QM SoCs, and we use them for building \project.
%\mypara{\sugg{Available hardware to implement \project.}} 
%We have abstractly modeled the PPC so that \project can be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol}. Also, a wide-range of Qualcomm Snapdragon family SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu, xpucves}. Both fulfill all PPC requirements. 
%All NXP's iMX8, Xilinx Zynq and Qualcomm's Snapdragon SoCs deployments span a wide range of edge computing settings such as the automotive industry~\cite{}. Furthermore, Qualcomm is one of the major players in the mobile market~\cite{qc_marketshare}.
%Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. ACUs are also a clear trend in modern SoCs, which tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}.

%To implement \project, we leveraged an OEM-specific platform partition controller, i.e., NXP's RDC. However, in \ref{sec:plat_req}, 
% We have abstractly modeled the PPC so that \project can be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol} while Qualcomm Snapdragon SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu}. Both fulfill all PPC requirements. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. ACUs are also a clear trend in modern SoCs, which %due to the hardware complexity 
% tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}.
% }
%\sugg{TODO: estimar quantas plataformas destas existem no mundo real e segmentos de mercado.}


==> backups/back-20220205-sec7.tex <==
\if0

\rev{TrustZone-based TEEs have been the target of multiples attacks, which exploit software flaws to obtain privileged execution, extract secrets, or twarth security functionality. In \project we propose to achieve three main security properties: (P1) monitor protection, (P2) normal world protection, (P3) allow for multiple TEEs. These properties are \project's invariants, and in this section we address how they are upheld by our implementation, and how the invariants themselves minimize the impact of attacks.}

\mypara{Monitor Protection (P1)} \rev{In deployments before Armv8.4 or without S-EL2, the trusted OS has full access to all resources including the secure monitor code and memory regions. This allows a malicious Trusted OS to compromise the monitor, the highest privilege code in the system. Protection of monitor memory is achieved by marking most of monitor memory as inaccessible leaving accessible only a small region of code, to allow for safely switching in and out of Trusted OS execution. Additionally due to the limitations of using a core external control mechanisms, to prevent TEE from accessing normal world memory we must suspend all co-located cluster cores when executing a TEE.}

\mypara{Normal World Protection (P2)} \rev{In typical deployments, the Trusted OS has full access to the normal world memory. By guaranteeing that S-EL1 cannot access normal world memory with the exception of explicitly assigned shared memory, a malicious Trusted OS cannot directly compromise the normal world software. In \project only resources that a TEE can access are made available to each TEE. For the same reasons mentioned in P1, it is necessary to suspend all co-located cluster cores, while the TEE is executing.}

\mypara{Multiple TEEs (P3)} \rev{Allowing for multiple TEEs enables use cases where TAs can trust less in each other, specially if they are from different developers. This is achieved by running TAs, or groups of TAs, in different TEEs. This is important because malicious TAs can escalate privileges and attack other TAs within the TEE. Creating multiple TEEs is achieved by allowing access to resource of a particular TEE to only that specific TEE. Thus, different TEEs cannot access each-other's resources and are hence protected from each other's attacks.}
\newline

\rev{We next analyze how three representative real-world attacks would fare in a system deployed with \project.}

\mypara{Attack 1.} \rev{An attacker compromises a system TA through the trusted OS, by first obtaining execution privileges in the trusted OS~\cite{BreakFDE,shen-trustedcore}. This can be used to thwart security functionality. For example, an attacker can obtain the secret key used to encrypt the file system~\cite{BreakFDE} or effectively compromise the fingerprint authentication mechanism~\cite{shen-trustedcore}.
%The secret key is encrypted by the user password, however it is possible to bruteforce the password on a powerful PC.
%
Because \project allows for the secure deployment of multiple OSes (P3), it is possible to prevent a compromised component from zone$_{1}$ from directly obtaining secrets from other zones. Securely developing zone$_{1}$ is easier than doing the some for a single TEE domain hosting all TAs. Thus, by using \project to allow more than one TEE to execute in the secure world, a vulnerability in one zone can not be used to obtain secrets from another.}
 
\mypara{Attack 2.} \rev{By leveraging a TA's access to normal world memory, it is possible to access all memory in the normal world~\cite{gb-exploit6, Aravind2017}. This is possible because the trusted OS can map the normal world physical memory at will, and in certain scenarios can map this memory unto a TAs address space. With access to normal world memory an attacker can compromise the Linux kernel, for example by creating a back door within seldom used kernel modules. This gives the attacker arbitrary code execution at kernel level of privilege. 
%
In \project we restrict the normal world memory accessible to a trusted OS (P2), and only allow predetermined memory regions to be used as shared memory. This prevents an attacker in the TEE from compromising the normal world, as it can no longer access its code or memory regions.
%Fixing the shared memory space makes it possible for secure monitor to enforce secure-world zones. This comes at the cost of not being able to use dynamic shared memory which in certain scenarios can reduce performance due to forcing additional copies of memory.
}
\if10
\mypara{Attack 3.} \rev{An attacker can highjacking the control flow of a Trusted OS to compromise it~\cite{gb-exploit4}. In particular the attacker might leverage the presence of privileged operations, for example in the case for Armv7-A or Armv8-A\_aarch32 the DACR registers, which when set to zero disable MMU based memory protection and access any resource int the system.
%
In \project, we use platform-level access control mechanisms to enforce zone access permissions to memory. Even with access to privileged instructions in the trusted OS, an attacker can not modified these policies, and is thus still confined to the specified zone. This ensures that even a fully compromised trusted OS cannot access resources other than ones that it was explicitly allowed to access (P1, P2, P3).}
\fi

\mypara{Attack 3.} \rev{In Samsung platforms secure drivers are highly privilege components. By compromising a TA, researchers have show that it is possible to exploit a flaw in a secure driver~\cite{BreakingArmTZ}. Secure drivers have access to mmap, which allows them to map physical memory. The Secure Monitor can then be mapped by the now malicious secure driver. An attacker can modify EL3 code, for example the SMC handler, allowing them to obtain EL3 execution privileges. Because \project ensures that S.EL1 cannot access the secure monitor memory (P1), \project effectively prevents this type of privilege escalation attacks.}
\newline

\rev{\project effectively mitigates against a wide range of powerful privilege escalation attacks, improving the security of both the normal world, secure monitor, and TAs.}

\fi

\if0
\subsection{Attack Mitigation}
TrustZone-based TEEs have been the target of multiples attacks, which exploit software flaws to obtain privileged execution, extract secrets, or twarth security functionality. We next analyze how these attacks would fare in a system deployed with \project.

\mypara{Attack 1. } By compromising a TA, it is possible to exploit a flaw in a secure driver~\cite{BreakingArmTZ, DeepDive}. Secure drivers have access to mmap, which allows them to map physical memory. The Secure Monitor can then be mapped by the now malicious secure driver, and the attacker can do anything on the platform, including exposing secrets. A master key is one of such secrets. In the Samsung ..., the master key is used by the drcrypto driver for cryptographic operations.
There are two ways in which the master key can be obtained: a) obtaining access to EL3 memory and reading the master key location, b) or via an SMC to the secure monitor.

\mypara{Mitigation 1. } \project mitigates against obtaining the Master Key by preventing the trusted OS from accessing monitor memory. Because malicious software can longer map the Secure Monitor it can no longer obtain the master key directly. This solves problem 1.a). However, the attacker can still obtain the master key through a Secure Monitor Call (SMC), problem 1.b). To mitigate this, with \project, we argue for implementing cryptographic primitives requiring platform keys, and other system critical features, in a separate zone which will not reveal the key being used. 

\mypara{Attack 2.} An attacker can compromise a system TA through the trusted OS, by first obtaining execution privileges in the trusted OS~\cite{BreakFDE,shen-trustedcore}. This can be used to thwart security functionality. For example, an attacker can obtain the secret key used to encrypt the file system~\cite{BreakFDE} or effectively compromise the fingerprint authentication mechanism~\cite{shen-trustedcore}. 
%The secret key is encrypted by the user password, however it is possible to bruteforce the password on a powerful PC. 

\mypara{Mitigation 2.} \project allows for the secure deployment of multiple OSes. It is possible to prevent a compromised component from zone$_{1}$ from obtaining secrets from other zones, provided that zone$_{1}$ is bug free. Securely developing zone$_{1}$ is easier than doing the some for a single TEE domain hosting all TAs. Thus, by using \project to allow more than one TEE to execute in the secure world, a vulnerability in one zone can not be used to obtain secrets from another.
 
\mypara{Attack 3.} By leveraging a TA's access to normal world memory, it is possible to access all memory in the normal world~\cite{gb-exploit6, Aravind2017}. This is possible because the trusted OS can map the normal world physical memory at will, and in certain scenarios can map this memory unto a TAs address space. With access to normal world memory an attacker can compromise the Linux kernel, for example by creating a back door within seldom used kernel modules. This gives the attacker arbitrary code execution at kernel level of privilege.

\mypara{Mitigation 3.} In \project we can restrict the normal world memory accessible to a trusted OS. This requires knowledge of what memory is dedicated for sharing memory between the TEE and REE, however, on some platforms TF~-~A already supports modifying an in-memory device tree. This means that TF-A can specify to the kernel which memory is available for sharing information between worlds. Fixing the shared memory space makes it possible for secure monitor to enforce secure-world zones, although, at a cost of not supporting dynamic shared memory, which allows a normal world process to mark part of its memory as shareable with the TEE.

\mypara{Attack 4.} Code reuse attacks. An attacker can leverage control highjacking to compromise the trusted OS~\cite{gb-exploit4}. In particular the attacker might leverage the presence of privileged operations, for example in the case for Armv7-A or Armv8-A\_aarch32 the DACR registers, which when set to zero disable MMU based memory protection.

\mypara{Mitigation 4.} In \project, we use platform level access control mechanisms to enforce zone access permissions to memory. Even with access to privileged instructions in the trusted OS, an attacker can not modified these policies, and thus is confined to the specified sandbox. 
\fi

==> backups/back-20220209-sec8.tex <==
\subsection{\project and Armv8.4 S.EL2}
\label{sec:sel2}

\nuno{So far, we have mainly discussed the design and implementation of \project targeting platforms compliant with the Armv8-A architecture prior to the release of the Armv8.4 and the introduction of the secure hypervisor mode (S.EL2). Below, we explain why the secure hypervisor cannot fix the fundamental problem of the excess of privileges within the secure world and how \project can still be leveraged in Armv8.4 platforms to provide additional security guarantees.}
%and provide additional security guarantees


\nuno{The Armv8.4-A added support for EL2 in the secure state. This additional privilege level introduces hardware virtualization in the secure world, aiming at providing multiple TEE support while guaranteeing hardware-enforced isolation between multiple trusted OS and the normal world. From a high-level perspective, S.EL2 seems to provide similar security properties as \project's, i.e., the protection of the monitor (P1), the protection of the normal world (P2), and the protection of multiple trusted OSes or co-located environments (P3) (see $\S\ref{sec:sec_analysis}$).
While the introduction of S.EL2 seems promising, we argue that the fundamental problem of violation of the principle of the least privilege of TrustZone is not entirely fixed. Despite the isolation enforced around the trusted OSes, P1 and P2 are not fully met, as both monitor and the normal world can be accessed by the secure hypervisor. Simply put, \emph{the secure monitor cannot prevent the secure hypervisor from mapping memory regions arbitrarily into the S.EL2 and S.EL1 address space}. With a compromised secure hypervisor an attacker can do the same damage as it could do with a compromised trusted OS, i.e., it can fully compromise the system. For instance, Hafnium, the Arm reference implementation for the secure hypervisor features over 20 KSLoC, which directly contribute to enlarge the TCB of the system. Thus, we argue that \project can still be leveraged  to isolate the secure hypervisor, thus fully guaranteeing P1 and P2 security properties. From a technical point of view, we do not envision any outstanding implementation challenge; in fact, we believe the trampoline logic would be simplified, because all the logic related to multiple zones would be naturally managed by the secure hypervisor. The \project trampoline would just enforce boundaries around the single S.EL2 component, (similar to a current design with a single zone), and interpose in any context-switch entry and exit.} 

%In addition, the inclusion ... enlarge the TCB when compared to \project, by requiring yet another privileged software component to manage VMs.
%maintains the traditional TrustZone model and only slightly modifies it to achieve its security properties, while only marginally increasing the TCB.

%\rev{Although S-EL2 can be used to implement the same properties as ReZone, the degree to which they are enforced is not the same. In particular, P1 and P2 are still not fully assured as both monitor and the normal world can be accessed by the secure hypervisor. With the feature-creep observed in the last few years for Trusted OSes~\cite{}, which resulted in increased TCBs, it would not be unexpected that serious vulnerabilities also affect the new software layer. With a compromised secure hypervisor an attacker can do the same damage as it could with a compromised trusted OS in previous generations, i.e., it can fully compromise the system.}

%\nuno{In summary, \project offers a practical and general solution to fix the problem of excess of privileges within the secure world, that can be applied not only to restrict the privileges of the trusted OS on platforms prior to Armv8.4, but also to restrict the privileges of the secure hypervisor when available.}



%This allows it to maintain a minimal and immutable TCB.
% Arm foresees these to be developed to the highest standards of software engineering to achieve minimal, correct and impervious implementations. However, one cannot completely rely on this, as it was also the initial promise of TrustZone software itself. The evolution of requirements and services will likely bloat both software stacks.
%from all others, in particular, 
%: non-secure/normal, secure, monitor and realm~\cite{armv9realms}.


% NS> old text from sec 2 that might be useful here
%\rev{Arm's new architecture releases starting from Armv8.4, seem to solve this problem by introducing a trusted hypervisor. However, and even though the hypervisor adds a new layer fof defence, the security of the system relies on the trusted hypervisor. In Armv8.4 both normal world and the monitor can be attacked by a malicious trusted hypervisor as there's no isolation between these privilege levels. Effectively S-EL2 inherits all the priveleges of S-EL1 from the previous generation. Further, even though Armv9 brings protection to EL3, effectively protecting the secure monitor, a malicious hypervisor can still compromise the normal world.}

\subsection{\project and Armv9 CCA}
\label{sec:cca}

\nuno{Recently, with the release of the Armv9, Arm introduced the Confidential Computing Architecture (CCA). In CCA, Arm CPUs are augmented with the Real Management Extension (RME), which introduces two additional worlds: realm world and root world. 
The root world is dedicated to EL3 and, notably, cannot be accessed by other worlds privileged levels (EL2, EL1, and EL0). In contrast, the normal world still can be accessed from any other world, in particular the secure and realm worlds. The realm world is essentially a symmetric duplicate of the secure world, thus it cannot be accessed by the secure world and vice-versa. This architectural change addresses the security property P1 and acknowledges that Arm has already recognized one major architectural flaw we address with our work. CCA also achieves property P3, given that the S.EL2 can virtualize S.EL1. Notwithstanding, despite the undeniable architectural security improvements over former Cortex-A architectures, we argue that \project can still be leveraged in CCA to provide the security guarantees required by property P2. In CCA, as in Armv8.4, the normal world still needs to trust the secure world hypervisor. Thus, CCA suffers from part of the issues discussed above.}
% a feature that is on par, security-wise, with \project's protection of monitor memory from lower privilege levels. This effectively achieves property P1, (see $\S\ref{sec:sec_analysis}$), and it does so to a higher degree than S-EL2 alone, due to not depending on a trusted hypervisor. 
%Additionally, the introduction of the realm world enables the deployment of TA functionality to this world, minimizing the secure world TCB. 

\nuno{The security enhancements advocated by Arm's CCA are still yet to materialize, and historically take years to do so. Notwithstanding, it should be noted that the \emph{Real Management Extension is an optional feature starting from Armv9.2 \cite{armv9arm}}. This means that it remains questionable the widespread availability of RME from OEMs and the effective deployability in SoCs targeting the mobile and other embedded segments (e.g., automotive). Competitive architectures provide similar features in server class hardware only~\cite{SEV2019, inteltdx}. \rev{In addition, as of today, the only announced mobile SoCs featuring Armv9 feature Armv9.0
\cite{mobilev9}, and thus no RME.}
Similarly, the announced server chip supporting Armv9, i.e., Marvell Octeon 10
\cite{marvellv9}, is based on the Neoverse N2\cite{neoversen2}, which features also Armv9.0. Without RME, which adds root world and realm world, there is no protection for monitor mode~\cite{norealmnoroot}, and thus the provided security features are the same as the ones discussed in Armv8.4.}

%If platforms continue to add PPC-like mechanisms, as we expect they will, before Arm CCA reaches mainstream adoption, \project will be able to provide unparalleled security guarantees on a wide range of devices.


%While in this architecture, the secure world is targeted to deploy static security services and firmware, the realm world is meant to host dynamically instantiated realms that contain either full-blown OSes or small TA unikernels.

%=======================================================================
%> [DISCUSSION]
%=======================================================================
\subsection{Discussion}
\label{sec:discussion}


%\st{\mypara{Available hardware to implement \project.}  %To implement \project, we leveraged an OEM-specific platform partition controller, i.e., NXP's RDC. However, in \ref{sec:plat_req},  We have abstractly modeled the PPC so that \project can be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol} while Qualcomm Snapdragon SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu}. Both fulfill all PPC requirements. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. ACUs are also a clear trend in modern SoCs, which %due to the hardware complexity  tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}.}
\if0
\subsection{Deployment In Other Platforms}\label{sec:otherplat}
\mypara{Xilinx Protection Units.} Xilinx has also developed and included in their Zynq UltraScale+ MPSoC portfolio a set of protection units complementary to TrustZone~\cite{}. The Xilinx memory protection unit (XMPU) and the Xilinx peripheral protection unit (XPPU) are system-level controllers that verify if a particular bus master is explicitly allowed to access a specific address (memories and peripherals). There are a total of eight XMPUs for protecting transactions into the DDR, the OCM, and the interconnect (e.g., SATA and PCIe). There is one XPPU, which allows for protecting peripherals, message buffers, and inter-subsystem communication channels. A master ID list is used to define the masters that are allowed to access peripherals. Similarly to the i.MX8 families, in Zynq UltraScale+ devices the quad Cortex-A53 cluster has the same master ID for all of its cores, making it impossible to use the XMPU and XPPU to create security domains per core.
\fi

%\jose{is it necessary to mention management cores?} \sugg{as we are pressed for space, I dont' think it's worth it really. Maybe say somehting like, platform mangement cores are already present in various platforms to perform, power mangement or serving as a senser hub, In \project we require a dedic/ate security one (qualcomm has one in their latest flagships)}

%\mypara{System/OTA updates.}
%\project does not impose any limitation or changes in the platform update mechanism. The OEM must provide a secure boot process that allows for the authentication and deployment of secure world software. 

%During the secure boot, the bootloader will authenticate images and boot the system. The updated binary shall contain updated zone images and an updated resource allocation policy list per zone.

%\mypara{Performance vs. security trade-off.}  %To guarantee the correct sandboxing of zones, \project requires extreme measures, i.e., on a world-switch, a core must flush the full cache hierarchy and halt the other cores from the cluster. As shown in $\S$\ref{sec:eval}, although, at the micro view, there are a non-negligible overhead, from a macro perspective, real-world applications does not impact the user experience. 
%These performance impact might still be further minimized. 
%To further reduce the performance overheads of \project, we propose to explore several ideas. 

%%%\project's mechanisms induce non-negligible overheads and has limitations concerning simultaneous trusted OS calls. Although we consider that this is not a major issue for the standard behaviour of real-world TAs (and the performance overhead results observed in section \ref{sec:eval}),  we believe there is still room for optimizations. 

\if10 %before revision
\mypara{Performance optimizations.} To further reduce \project's performance overheads, there is still room for optimizations. 
For example, \project can benefit from multi-cluster platforms, where one cluster might continue executing in the normal world while the other runs a zone. Also, batching of a zone's invocations would amortize the costs of world-switching. %On the other hand, \project can contain or even fully mitigate critical attacks (see $\S$ \ref{sec:security_analysis}). % In essence, we believe \project is trading a small decrease in performance for huge security benefits. 
%\sugg{On deployments where the same trusted OS is deployed in multiple zones, common memory regions (e.g., OS page tables and code) can be shared between zones.}
\fi

\mypara{ReZone limitations and potential optimizations.} \nuno{ReZone has two fundamental limitations. The first limitation (a) is related to the fact that only a single TA can run simultaneously per cluster, due to the lack of propagation of the core ID to the bus (see $\S\ref{sec:cross_interference}$) . Naturally, this can impose concurrency limitations on TA execution and lead to punctual starvation (i.e., DoS)  of TAs. Notwithstanding, TrustZone-assisted TEEs do not provide availability guarantees. The second limitation (b) is related to performance, i.e., frequent invocation of (small duration) TAs may lead to non-negligible performance overhead, due to the very high number of world-switch calls. To address these two fundamental limitations, we propose two optimizations, respectively. Multi-core platforms typically provide multi-cluster configurations. Thus, to overcome the single TA execution issue (a), we propose the implementation of a fair-cluster scheduling policy, which manages and balances TA execution across multiple clusters. This optimization would allow running, concurrently, as many TAs as the number of available clusters. Finally, to alleviate the performance overhead for (b), we suggest the implementation of a seamless batching mechanism, responsible for batching multiple requests from the rich OS and issue secure world calls upon set of a well-defined threshold. This would reduce significantly the number of transitions between worlds, and consequently the number and impact of microarchitectural maintenance operations, boosting performance.}
%and unbounded worst-case execution time (WCET)
%the PCC not being able to differentiate between accesses from different cores, thus cores must be idle while executing a zone
%There are two main performance bottlenecks in \project. The first is that the normal world cannot execute while a trusted OS is executing. The only way we can address this is by leveraging multiple clusters in multi-cluster platforms. In this scenario one cluster would continue executing in the normal world while the other would run a zone. The second bottleneck is that, frequent calls to a zone that perform little work, will have higher incurred overheads than more spaced out invocations that do more work. With this insight, it is possible to optimize secure world workloads creating a batching mechanism to allow batching of a zone's invocations. This would amortize the costs of world-switching, mostly in cases requiring frequent fast calls.

%{\color{orange} ... Starting from ArmV8.4, TrustZone features a secure world hypervisor designed to provide different execution environments within the secure world itself, and which will also enable the protection of normal world, and monitor memory. However, platforms featuring the new architecture are not yet widespread, meaning that there is a lack hardware solutions for achieving the goals we propose. Additionally \project can be applied to already existing platforms which meet the necessary hardware requirements as discussed in ($\S$\ref{sec:plat_req}) ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... }

\if10 % Before revision
\mypara{Appropriation of PPC and ACU.}  By using the platform's PPC and ACU to implement \project, one may wonder if this appropriation will not disrupt the functionality of the system in case these components are used for other purposes. From our experience with the i.MX8 platform, \project caused no disruptions to REE/TEE system and applications. As long as the \project security is preserved, PPC and ACU can be shared with other services, e.g., being able to run additional code on the Cortex-M4 (i.e., the ACU), or use a spare security domain in the RDC (i.e., the PPC) for other purposes.
\fi

\mypara{ReZone appropriation of PPC/ACU.} \nuno{We believe ReZone can leverage the platform's PPC and ACU without jeopardizing the utilization of these components for their intended purposes and legacy use cases. In particular, we believe it is possible to share these hardware components while guaranteeing \project security properties, e.g., using a spare security domain in the PPC or enabling the co-existence of the gatekeeper code with other critical or non-critical functionalities already embedded in the ACU. There are multiple classes of works in the literature that provide strong isolation for software running in microcontrollers \cite{Kwon2019,Pinto2019_2,Hassaan2019,Pinto2020,Grisafi22}. Different solutions provide different trade-offs between code size, performance, power consumption, and security, but, modern low-end TEEs, such as MultiZone \cite{Pinto2020}, leverage minimal hardware primitives ready-available in almost all Arm Cortex-M microcontrollers to provide high performance, robust, lightweight enclaves. }
%By using the platform's PPC and ACU to implement \project, one may wonder if this appropriation will not disrupt the functionality of the system in case these components are used for other purposes. As long as the \project security is preserved, PPC and ACU can be shared with other services, e.g., use a spare security domain in the RDC (i.e., the PPC), or being able to run additional code on the Cortex-M4 (i.e., the ACU) for other purposes. In cases where the available ACU performs non-critical work, it is necessary to allow the secure co-existence between the non-critical functionality, and the gatekeeper code. There are multiple ways this could be achieved, from using small operating systems that support hardware enforced isolation such as FreeRTOS, to using software based isolation techniques~\cite{ammar2019s} if it does not. Although this could have some impact on the performance of the ACU, depending on the ACU's workloads, we believe the improved security guarantees to the system as a whole are worth the cost.


%\sugg{In \project we change the security semantics of the platform, in particular we use secrets to disallow unintended reconfiguration of the PPC, while still allowing the PPC unlocking mechanism to be available to the Trusted OS. To enable this we take advantage of an ACU and a PPC present in our test platform, a Cortex-M4 processor and a RDC from NXP. Our use of these components somewhat limits how they can be used for other purposes. We required the Cortex-M4 to run the gatekeeper code, however this functionality can be implemented alongside other features by means of a embedded OS, for example~\cite{uCOSII, Garlati2020}, at the cost of lowering overall security by increasing the system TCB. A second caveat, is due to our use of the RDC, which poses more significant limitations. We make use of three of the four available domains that are possible to be created by the RDC. Still, it is possible to make use of the forth domain to establish an additional partition at a platform level.}

%\mypara{\project semantics.}  \sugg{In \project we change the security semantics of the platform, in particular we use secrets to disallow unintended reconfiguration of the PPC, while still allowing the PPC unlocking mechanism to be available to the Trusted OS. To enable this we take advantage of an ACU and a PPC present in our test platform, a Cortex-M4 processor and a RDC from NXP. Our use of these components somewhat limits how they can be used for other purposes. We required the Cortex-M4 to run the gatekeeper code, however this functionality can be implemented alongside other features by means of a embedded OS, for example~\cite{uCOSII, Garlati2020}, at the cost of lowering overall security by increasing the system TCB. A second caveat, is due to our use of the RDC, which poses more significant limitations. We make use of three of the four available domains that are possible to be created by the RDC. Still, it is possible to make use of the forth domain to establish an additional partition at a platform level.}

\mypara{ReZone PPC/ACU and TZASC.}
\nuno{\project still leverages the TZASC to protect the secure world from normal world accesses, such as in vanilla TrustZone deployments. It would be possible to design \project to not use the TZASC, but this would create additional limitations. It should be noted that without the TZASC, CPU accesses cannot be differentiated from secure and non-secure. Thus, it would be required to sandbox the normal world exactly as ReZone sandboxes zones, i.e., it would be necessary to perform additional operations (e.g., cross-core synchronization, cluster suspension, cache maintenance operations, etc) to the normal world, with the restriction on lack of concurrency with the monitor. The notable exception is related to the TLB maintenance, which would not be necessary given the existence of independent TLB entries for the normal world (that are not shared). In summary, leveraging the TZASC in tandem with the PPC/ACU creates several performance optimizations while providing security guarantees between the normal world and the zones.}
%TZASC
%1. Recapitular pk TZASC nao pode ser usado com PPC
%2. Reforçar que usar um PPC e ignorar o TZASC tras problemas
%3. Reeiterar que a sinergia dos dois, permite reduzir overhead

\mypara{Arm SMMU as ReZone PPC.}
% The Arm SMMU is an IOMMU architecture that can translate an input address to an output address based on address mapping and memory attributes (i.e., translation tables). The main requirement for an IOMMU to be used as a PPC is the possibility of performing address translation functions for multiple masters, in particular the CPU. The Arm SMMU architecture, in its different versions, i.e., Arm SMMUv1, SMMUv2, SMMUv3, can fully provide such a feature. 
%in the overall ReZone architecture and execution flow,
\nuno{To leverage an SMMU as the ReZone PPC, we envision minor changes in the execution flow while entering (EL3$\rightarrow$S.EL1) and exiting (S.EL1$\rightarrow$EL3) a zone. In doing so, we expect modifications in two architectural components: (i) the trampoline and (ii) the ACU. For the trampoline, we expect minor changes to the dynamic access control configuration code (see $\S\ref{sec:dynamic-conf}$), i.e., the trampoline must explicitly create page tables that enforce the required access permissions for each zone, instead of configuring permissions directly through memory-mapped registers. The trampoline must also perform the invalidation of the SMMU TLB, to ensure the configured page tables enter in effect. Finally, for the ACU, the main change encompasses the explicit view of the page tables (created by the trampoline) and the update of these page tables to prevent CPUs from accessing both the page tables and the SMMU itself. If the CPU could access the SMMU, or its page tables, a zone could undo the established access control policy and fully compromise the system. The aforementioned modifications encompass modifications while entering a zone. Similar (inverse) operations need to be performed at the zone exit. }
%We believe the remaining operations performed during a context-switch (Figure \ref{fig:scr_ctx_hw}) are kept intact.
%We have mentioned above that an SMMU can be used as a PPC. An SMMU is an hardware component that can translate and filter accesses to the system bus. Specifically, this is achieved by translation tables that specify the translation, and access policy properties. One fundamental characteristic of a system that uses the SMMU for this end is that the SMMU must be able to also translate CPU accesses, which is not a given, in particular in system that feature custom SMMUs. Assuming that an SMMU can indeed translate CPU accesses, the process to use it as a PPC in \project is as follows. The trampoline would be responsible for correctly configuring memory accesses, the same as before, however instead of configuring resources by configuring registers and specifying start and end addresses for memory regions, the trampoline would establish translation tables, which can simple translate to the physical address space, and configure the appropriate memory attributes. The ACU would also need to implement some awareness of the page table and its configuration, as it would need to configure the SMMU to always allow the ACU to access the SMMU, and to allow/disallow the CPUs, and other bus masters, from accessing the SMMU (including the page tables). With this primitives in place, the process is the same as before. The trampoline makes an authenticated request to the ACU, and the ACU configures the SMMU to allow the trampoline to configure it as necessary. After, the trampoline will make another request the ACU, which will maintain the configured access policies, and update the translation table to prevent access the SMMU by other system entities.


==> backups/back-20220210-sec8.1.tex <==

\subsection{\project and Related Systems} \label{subsec:related-systems}
\nuno{Next, we compare \project to systems which share similar design goals and we evaluate them on five key dimensions: security guarantees, scalability, programming overheads, performance, and TCB (Table \ref{tab:tcb_comparison}). We selected seven systems as the best representative of the identified classes of solutions, i.e., (i) multiple environments on the normal world using virtualization (vTZ, PrOS, PrivateZone), (ii) normal world enclaves using the TZASC (Sanctuary, TrustICE), and (iii) secure world enclaves using same privilege isolation (TEEv, PrOS).}
\nuno{vTZ, OSP, and PrivateZone leverage the virtualization extensions available in the normal world to create multiple isolated environments. vTZ virtualizes the full TrustZone infrastructure, enabling the execution of full-fledged trusted OSes in the normal world, while OSP and PrivateZone provide a custom runtime environment per TA. A key aspect of vTZ is the dependency on binary instrumentation to remove privileged memory management instructions from the normal world hypervisor. TrustICE and Sanctuary leverage the TZASC to create enclaves within the normal world. Enclaves are isolated and cannot access the REE, but the trusted OS still has full access to the system. TrustICE has multi-core limitations while Sanctuary depends on features not available in any COTS hardware release to date. 
TEEv and PrOS use same privilege isolation to run a secure hypervisor on the secure world, due to the lack of secure virtualization (S.EL2). TEEv also depends on a privilege TEE to manage accesses to trusted hardware and cryptographic keys. Both solutions require binary instrumentation of the trusted OSes to guarantee isolation between the trusted OSes and the hypervisor.}




\if\comptcb
\else
\input{TableTCBComparison}
\fi

\mypara{Security.}
\nuno{To assess the security, we took into account the threat model and the security properties defined in section $\S\ref{sec:threat_model}$: (P1) protection of the normal world \emph{(TOS→NW)}; (P2) protection of the secure-monitor \emph{(TOS→Mon.)}; and, (P3) protection of co-located zones/environments \emph{(TOS$_1$→TOS$_2$)}. \project can offer stronger security guarantees when compared to other systems. When compared to TEEv, \project provides hardware-enforced protection to guarantee P1 and P2, while TEEv relies on same privilege isolation techniques (binary instrumentation). Thus TEEV (and PrOS) do not allow the trusted OS to run arbitrary code in the S.EL1 mode.}
%Although vTZ features the ability to execute multiple trusted OSes, for a normal world VM there exists only one trusted OS instance. Thus isolation is guaranteed between trusted OSes but not in the context of a single normal world VM.

\mypara{Scalability.}
\nuno{To understand the scalability of the different systems across COTS platforms, we assessed the dependency of these systems on specific hardware components and features. The majority of the systems depend on a PPC, in particular from an SMMU to restrict and manage accesses from other system bus masters~\cite{Hua2017,Cho2016,Jang2018,Kwon19}. \project also depends from an ACU, which, per the Arm's reports~\cite{armscp}, is a clear trend in COTS SoCs. Although Sanctuary~\cite{Brasser2019} does not depend from a PPC and ACU, the system relies on the unrealistic assumption that the core ID is propagated to the bus, i.e., this solution is not practical for real-world platforms.}

%\project relies on common, though not ubiquitous, components. This enables \project to be deployed in COTS platforms. The same is not true for Sanctuary~\cite{Brasser2019}, which requires modifications to the inner-workings of the caches, which the authors achieve by modifying the CPU hardware in an emulator. Most other works share \project's requirement for PPC-like mechanisms (e.g., an SMMU), with \project additionally requiring an ACU.
%Notwithstanding, ACUs are common enough to be widely available. For an analysis on platforms that can support \project, please refer to $\S\ref{sec:PPC_ACU_COTS}$.}

\mypara{Programming Overheads.}
\nuno{We defined programming overheads as necessary modifications, imposed by the systems, to the TrustZone related APIs (e.g., Global Platform) and/or runtime components, i.e., trusted OS and normal world software. \project does not require modifications to runtime components and APIs. Thus, \project can be fully leveraged with existing secure and world software stacks, including normal world and secure hypervisors. Related work typically requires modifications or instrumentation of the trusted OS ~\cite{Li2019, Brasser2019} or the normal world hypervisor~\cite{Hua2017}, implementation of custom drivers to provide communication facilities to enclaves \cite{Jang2018, Cho2016, Brasser2019, Sun2015, Kwon19}, or appropriation of specific privileged modes (e.g., NS.EL2).}

\mypara{Performance Overhead.}
%Due to the lack of a standardized benchmark suite for TEEs, researches evaluate their system's performance using a variety of custom TAs, real world cases, and synthetic benchmarks. This makes a quantitative comparison between systems unreliable. Instead, we analyze the main source of performance overheads for each system. \project does not use virtualization hardware thus it is not affected by stage-2 TLB misses. However, \project does perform significant micro-architectural maintenance operations. These operations force data to be written to main memory, and thus are slow. Cells marked with "*" on this column identify systems that although their original implementation does not feature maintenance operations, the security they provide is compromised because of it~\cite{Brasser2019, Sun2015}, due to cache-in-the-middle attacks~\cite{wang2020cache}. Thus, we considered that a correct implementation of these systems would perform these operations. \project is not affected by trap and emulation, as this is used by the systems applying privilege isolation techniques \cite{Hua2017, Li2019, Kwon19}. }
\nuno{
We analysed the related work and we concluded that other systems are closed source, do not target the same hardware platform, do not feature the same CPU and the microarchiteture (e.g., caches and TLB size), the CPUs do not run at the same frequency, and do not evaluate the same benchmarks or real-world applications. Obviously, all these aspects are key to establish a quantitative performance comparison. Thus, we focused on a qualitative evaluation of the key operations that may impact the performance overhead of the systems, in particular, TLB misses due to using stage-2 virtualization \emph{(S2-TLB)}, micro-architectural maintenance operations, and trap and emulation. For \project, micro-architectural maintenance operations are the most relevant source of overhead. These operations may force data to be frequently written to main memory, thus having a considerable impact on the execution of the system. \project does not leverage any hardware virtualization support, thus it is not affected by stage-2 TLB misses. \project also does not required trap and emulation.}
%Cells marked with "*" on this column identify systems that although their original implementation does not feature maintenance operations, the security they provide is compromised because of it~\cite{Brasser2019, Sun2015}, due to cache-in-the-middle attacks~\cite{wang2020cache}. Thus, we considered that a correct implementation of these systems would perform these operations.



\mypara{Trusted Computing Base.}
\label{sec:eval_tcb}
%\footnote{\rev{We use the term TCB to refer to the system software components that if compromised or malicious can attack other parts of the system, e.g, by accessing or manipulating victim's code and data. In \project we are concerned about the TCB from the point of view of both the normal world and monitor; a malicious S-EL1 can attack both.}}
%\footnote{\rev{Shall we add here a small definition on what we undertand as TCB?!}}
\nuno{Lastly, we assess the TCB size of each system. We collect information about the TCB from the original papers and added the reference sizes for TF-A (24,607 SLOC) and OP-TEE (230,094 SLOC). SLOC values were computed using the SLOCCount tool. Modifications to the software components are marked with "$^+$".
In \project, the trusted OS is not part of the system TCB. The security of the system, i.e., the normal world and secure monitor, is no longer vulnerable to a compromised trusted OS. \project adds a total of 5345 SLOC, encompassing trampoline code (1523 SLOC) and the gatekeeper (3,822 SLOC). The gatekeeper leverages ready available board support package (BSP) code; an optimized assembly implementation would reduce this number to a few hundred SLOC.
vTZ has the smallest TCB, since it does not rely on a trusted OS and implements a custom (and minimalist) monitor. We argue this is not realistic, because deployed systems in mobile and embedded industries rely on the TF-A to provide low-level platform management features, in particular, the Power State Coordination Interface (PSCI). Thus, we mark vTZ SLOC with "*", because, in practice, these features would be implemented in EL3, increasing the SLOC count.}
%, although the system may still depend on the functionality provided by a trusted OS (e.g., fingerprint authentication)




==> backups/main-body-back-220203.tex <==
%=======================================================================
%> [INTRO]
%=======================================================================	
\section{Introduction}

Arm TrustZone~\cite{Pinto2019, Pinto2019_2} is a technology embedded into Arm processors presently found in billions of mobile phones and embedded devices, such as car infotainment systems and SmartTVs. Vendors and Original Equipment Manufacturers (OEM) rely on TrustZone for deploying Trusted Execution Environments (TEEs), which protect the execution of sensitive programs named Trusted Applications (TAs).  Some TAs implement kernel-level services of the operating system (OS); for example, for user authentication or file disk encryption~\cite{androidwhitepaper}. Other TAs implement shared user-level functionality, e.g., DRM media decoders~\cite{TZVideoPath} or online banking services~\cite{trustonicBanking}. TEEs themselves consist of a trusted software stack offering API and runtime support for hosting TAs. TEEs such as Qualcomm's QSEE and OP-TEE protect the confidentiality and integrity of TAs' memory state, thereby ensuring it cannot be inspected or tampered with by a potentially compromised OS.

To protect the TAs, TEEs leverage mechanisms provided by TrustZone. In Armv7-A/Armv8-A, this technology provides two execution environments named \textit{normal world} and \textit{secure world}\footnote{As per Arm's recent documentation~\cite{tzarmv8a}, \textit{secure world} can be referred to as \textit{trusted world}; we adopt the previous and more familiar terminology~\cite{Pinto2019}.}. The normal world runs a rich software stack, named Rich Execution Environment (REE), comprised of full-blown OS and applications; it is generally considered untrusted. The secure world runs a smaller software stack consisting of TEE and TAs. TrustZone enforces system-wide isolation between worlds and provides controlled entry points for world switching whenever the REE invokes TAs' services.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/intro-trustzone.pdf}
    \vspace{-0.3cm}
    \caption{\small Privilege escalation attack in a TrustZone-assisted TEE: (1) hijack a user-level TA, e.g., exploiting vulnerability in the Widevine TA (CVE-2015-6639)~\cite{gb-exploit4}, (2) hijack the trusted OS, e.g., exploiting vulnerability in syscall interface of Qualcomm's QSEOS (CVE-2016-2431)~\cite{gb-exploit5}. Once in control of the trusted OS, other attacks can be launched: (a) control the rich OS, e.g., backdoor in the Linux kernel~\cite{gb-exploit6}, (b) control a kernel-level TA, e.g., to extract full disk encryption keys of Android's KeyMaster service~\cite{gb-keymaster}, or (c) control the secure monitor, e.g., to unbrick the device bootloader~\cite{gb-bootloader}.}
    \label{fig:intro_trustzone}
    \vspace{-0.5cm}
\end{figure}

However, a fundamental limitation of the TrustZone security architecture is that the trusted OS -- i.e., one of TEE's core components -- runs with an excess of privileges, exposing the entire system to catastrophic privilege escalation attacks if the trusted OS gets compromised. Figure~\ref{fig:intro_trustzone} illustrates how these attacks can be launched. It shows the TEE stack, consisting of the \textit{secure monitor} and \textit{trusted OS}. The secure monitor runs in EL3 -- the most privileged exception level -- and provides essential mechanisms for world switching and platform management. The trusted OS runs in S.EL1 -- i.e., secure kernel mode -- and implements memory management, scheduling, IPC, and common services for TAs. TAs run in unprivileged S.EL0 -- i.e., secure user mode. TAs are directly exposed to malicious requests coming from normal world applications. If a TA's control flow gets hijacked as a result of exploiting a software vulnerability (1), the attacker can control that TA. If the attacker can further hijack the trusted OS by exploiting another vulnerability (2), he can gain full control of the system, including: the REE in the normal world (a), all the TAs (b), and the secure monitor (c). This level of control is possible because S.EL1 gives full permission to access and reconfigure both secure and non-secure memory regions.
%
\rev{Even in newer Arm releases, starting from Armv8.4 and including Armv9, the problems are not all solved. In Armv8.4 Arm introduced S-EL2, a level privelege designed to host a trusted hypervisor that can potential address some of these issues. However the monitor and normal world are not protected from the hypervisor itself. As such the trusted hypervisor, if compromised, can launch the same attacks as S-EL1 could in previous generations. In Armv9, Arm introduce new access control mechanisms that bring definitive protection to the secure monitor, but still the normal world security is still subject to a trusted hypervisor.}

Unfortunately, numerous devices today face serious risks of being compromised by attacks of this nature. In the past, security researchers have demonstrated how these attacks can be mounted as described above, escalating privileges from NS.EL0 into S.EL1 by chaining two exploits: first, targeting a vulnerable DRM TA~\cite{gb-exploit4}, and then a vulnerability in the system call interface of the trusted OS~\cite{gb-exploit5}. Once in control of the trusted OS, it was possible to (a) plant a backdoor in Linux kernel~\cite{gb-exploit6}, (b) retrieve cryptographic keys from Android's KeyMaster~\cite{gb-exploit4}, or (c) disable trusted boot protections~\cite{gb-bootloader}. Notably, recent studies~\cite{Cerdeira2020} have shown that commercial TEE systems have plenty and serious vulnerabilities, most of them affecting user-level TAs and trusted OS. This suggests that the current attack surface for TEE systems is seriously enlarged.

Despite the abundant research on TrustZone security~\cite{Pinto2019,Cerdeira2020}, there is a lack of practical system defenses if the trusted OS is hijacked. TEE systems like Sanctuary~\cite{Brasser2019} aim to reduce the attack surface of the trusted OS by relocating TAs onto user-level enclaves in the normal world. However, due to portability reasons, vendors and OEMs continue deploying TAs in commercial TEEs, therefore exposing many devices to potential attacks. Another approach is to confine the TEE stack inside a secure world sandbox, e.g., by leveraging same privilege isolation~\cite{Kwon19,Li2019} or hardware virtualization~\cite{hafnium}. Same privilege isolation uses binary instrumentation to sanitize dangerous instructions of the trusted OS. Unfortunately, if the control flow of the trusted OS is hijacked at runtime, an attacker can still execute arbitrary secure memory accesses. Hardware virtualization can help create sandboxed environments using virtual machines. However, virtualization support for the secure world (S.EL2) is fairly recent, i.e., in Armv8.4-A. As a result, it cannot be used in many devices today.

This paper presents \project, a new security architecture that can effectively counter ongoing privilege escalation attacks by reducing the privileges of a potentially compromised trusted OS. This is achieved by creating \textit{zones}, i.e., sandboxed domains inside the secure world. Zones have access only to private memory regions, and provide an execution environment for untrusted S.EL$_\textrm{1/0}$ code, i.e., trusted OS and TAs. \project restricts the memory access privileges of the code running inside a zone, preventing it from arbitrarily accessing memory allocated for: (a) the normal world REE, (b) other zones, and (c) the secure monitor. %The only way for a given zone to communicate with an external memory protection domain is through mutually shared memory regions. 
With \project, a typical monolithic TEE can then be restructured and partitioned into multiple zones. For instance, Figure~\ref{fig:intro_rezone} depicts a setup featuring two zones -- 1 and 2 -- each of them runs a trusted OS instance as in a library OS. Then, user-level TAs and kernel-level TAs run in independent zones. With this configuration, an attacker hijacking the trusted OS in zone 1 (as explained in Figure~\ref{fig:intro_trustzone}), will not be able to further escalate its privileges beyond its sandbox. To give vendors and OEMs maximal flexibility, \project allows the creation of additional zones, and using different trusted OSes inside different zones.

A central novelty of \project's design is that we take advantage of a TrustZone-agnostic resource controller available in modern SoCs to restrict the privileges of S.EL1 (trusted OS) code. Existing systems such as Sanctuary~\cite{Brasser2019} have already leveraged the TrustZone Address Space Controller (TZASC) for protecting user-level enclaves in the normal world. For example, TZC-400 features the possibility to specify access permissions to various physical memory regions, including the ability to prevent secure world code from accessing predefined regions of secure world memory. However, S.EL1 code can still revert these permissions, rendering the TZASC insufficient for zone isolation. Instead, we use a TrustZone-agnostic resource controller that allows specific bus masters to control memory access permissions. An example is the Resource Domain Controller (RDC), existing in iMX8MQ and iMX8QM SoCs. In \project, we harness this feature and reserve a low-end microcontroller also available in the SoC to control how these permissions are set, effectively creating private memory regions for each zone. RDC and microcontroller can then be used as building blocks for restricting the memory access privileges of a (potentially compromised) trusted OS, and enforce strong zone isolation.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/intro-rezone.pdf}
    \vspace{-0.3cm}
    \caption{\small \project setup enforcing TEE privilege reduction: after compromising user-level TA$_\textrm{U}$ and trusted OS in zone 1, an attacker cannot escalate privileges to (a) rich OS, (b) kernel-level TA$_\textrm{K}$ in zone 2, or (c) secure monitor.}
    % \vspace{-0.2cm}
    \label{fig:intro_rezone}
    \vspace{-0.5cm}
\end{figure}

Based on this insight, we have built \project. Our system includes multiple non-trivial optimizations and fine-grained mechanisms to guarantee system-wide security (e.g., avoiding cache-based attacks based on cached content available for EL3 and S.EL1 code). To make our design generally applicable to various hardware platforms, we specify the general properties of SoCs that satisfy \project's requirements. We have fully implemented a \project prototype for the i.MX 8MQuad EVK, and integrated it with Android OS as REE and with OP-TEE as TEE. Our code will be open sourced.

We evaluated \project using microbenchmarks and real-world applications. Our evaluation shows that despite the existence of non-negligible performance overhead in microbenchmark programs, \project does not sensibly degrade the performance of applications such as crypto wallets or DRM media decoders. The DRM application, which requires frequent transitions between the normal world and the zone, preserves its ability to replay video at high frame rates. 
%The overall performance of the system is only mildly affected ($<$0.04\% slowdown). 
We have surveyed 80 CVE vulnerability reports and estimate that \project can thwart 87\% of potential privilege escalation attacks arising from exploiting these bugs.


%=======================================================================
%> [BACKGROUND]
%=======================================================================	
\section{Background and Motivation}

\subsection{Standard TrustZone Mechanisms}

We focus on TrustZone for Armv8-A architectures. TrustZone enables CPU cores to operate in one of two states: \textit{secure} and \textit{non-secure}. At exception levels EL0 and EL1, a processor core can execute in either of these states. For instance, the processor is in non-secure exception level 1 (NS.EL1) when running REE kernel code, and in secure EL1 (S.EL1) if executing the trusted OS. EL3 is always in secure state. To change security states, the execution must pass through EL3.

TrustZone extends the memory system by means of an additional bit called \textit{NS bit} that accompanies the address of memory and peripherals (see Figure~\ref{fig:RZ_HW}). This bit creates independent physical address spaces for normal world and secure world. Software running in the normal world can only make \textit{non-secure accesses} to physical memory because the core always tags the bus NS bit to 1 in any memory transaction generated by the normal world. Software running in the secure world usually makes only \textit{secure accesses} (i.e., NS=0), but can also make non-secure accesses (NS=1) for specific memory mappings using the NS flags in its page table entries. The processor maintains separate virtual address spaces for the secure and non-secure states. %Moreover, within the secure state, the processor maintains separate translation regimes for EL3 and S.EL1. 
Trusted OS (or the secure monitor) can map virtual addresses to non-secure physical addresses by setting to 1 the NS bit in its page table entries. In non-secure state, that bit is ignored: the virtual address will always be translated to non-secure physical address (NS=0).

\if0
The NS bit of the translated physical memory address is also propagated onto the data cache tags. 
Issuing a non-secure access to cached data marked as secure causes a cache miss. Accessing cached %non-secure or secure 
memory in secure state may or may not cause a hit depending on the translated NS bit value.
%, i.e., it does not use a NS.EL1 translation while in secure state, or a S.EL1 translation while in non-secure state. 
\fi

TrustZone-aware memory controllers are usually configured to assign non-secure/secure physical address spaces to different physical memory regions. %Typically, the non-secure address space is assigned to a subset of the existing physical memory. Instead, the secure address space covers all existing physical memory, including the regions mapped to non-secure address space. 
In the Arm architecture, the TZASC enforces physical memory protection by allowing the partitioning of external memory on secure and non-secure regions. (The TZPC performs a similar function for peripherals.) To date, Arm has released two TZASC versions: Arm CoreLink TZC-380 and TZC-400. They share similar high-level features, i.e., the ability to configure access permissions for memory regions (contiguous address space areas).

\subsection{The Excess of Privileges of the Trusted OS}
\label{sec:challenge}

The TrustZone mechanisms described above were designed under the assumption that the S.EL1 (trusted OS) and EL3 (secure monitor) are trusted. However, if the trusted OS is hijacked, the attacks described in Figure~\ref{fig:intro_trustzone} can be trivially mounted. For illustration purposes, suppose that the physical memory addresses PA$_\textrm{OS}$, PA$_\textrm{TK}$, and PA$_\textrm{SM}$ are allocated to the rich OS, TA$_\textrm{K}$, and secure monitor, respectively. The attacker could mount said attacks by creating virtual address mappings in the S.EL1 page tables as indicated below, and use the virtual addresses VA$_i$ to access (read/write) the memory pages of the rich OS, TA$_\textrm{K}$, or secure monitor. Notation VA$\rightarrow\langle$PA, NS$\rangle$ denotes a page table entry translating virtual address VA to the physical address PA and associated NS bit value:

\noindent VA$_\textrm{OS}\rightarrow\langle$PA$_\textrm{OS}$, 1$\rangle$, VA$_\textrm{TK}\rightarrow\langle$PA$_\textrm{TK}$, 0$\rangle$, VA$_\textrm{SM}\rightarrow\langle$PA$_\textrm{SM}$, 0$\rangle$

Simply put, the ability of the trusted OS to establish these mappings on its own address space enables it to access any system component, including the monitor. This means that a compromised trusted OS can take over every part of the system. For this reason, we argue that reducing the memory access privileges of S.EL1 code can significantly lower the impact of vulnerability exploits targeting the trusted OS. % as has been proposed in previous works~\cite{Li2019, Kwon19, Jang2018}.

\rev{\david{Está demasiado parecido à introdução, mas não sei que mais dizer} Arm's new architecture releases starting from Armv8.4, seem to solve this problem by introducing a trusted hypervisor. However, and even though the hypervisor adds a new layer fof defence, the security of the system relies on the trusted hypervisor. In Armv8.4 both normal world and the monitor can be attacked by a malicious trusted hypervisor as there's no isolation between these privilege levels. Effectively S-EL2 inherits all the priveleges of S-EL1 from the previous generation. Further, even though Armv9 brings protection to EL3, effectively protecting the secure monitor, a malicious hypervisor can still compromise the normal world.}

%\subsection{Platform Model for Sandboxing the Trusted OS}\label{sec:plat_req}
\subsection{Platform Model}\label{sec:plat_req}

\if10 % Anterior
Reducing the privileges of S.EL1 code so as to prevent unauthorized memory accesses is not straightforward using standard TrustZone mechanisms alone. Even though TZASC controllers such as TZC-380 and the TZC-400 can restrict memory accesses, since S.EL1 has the privilege to reconfigure the TZASC, the trusted OS can always override any permissions for blocking the trusted OS's access to certain memory regions. Also for this reason access to the secure monitor (VA$_\textrm{SM}$) and TAs (VA$_\textrm{TK}$) cannot be restricted, added to the fact that trusted OS and secure monitor enjoy the highest privileges to read/write secure and non-secure memory.
\else % Minha proposta
Reducing the privileges of S.EL1 code so as to prevent unauthorized memory accesses is not straightforward using standard TrustZone mechanisms alone. Even though TZASC controllers such as TZC-380 and the TZC-400 can restrict memory accesses, since S.EL1 has the privilege to reconfigure the TZASC, the trusted OS can always override any permissions for blocking the trusted OS's access to certain memory regions. Also, TZASC does not distinguish between privilege levels, thus secure monitor (VA$_\textrm{SM}$) and TAs (VA$_\textrm{TK}$) memory cannot be restricted.
\fi


\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/rezone-hw.pdf}
    \vspace{-0.4cm}
    \caption{\small Hardware platform featuring TrustZone: \project-enabling hardware components are highlighted. These are the ACU and the PPC. PPC is configured by the bus master MID$_\textrm{1}$ (ACU). These configurations %are written in MMIO regions of the PPC, and 
    determine which access permissions are granted to a given MID for a specific physical memory region.}
    \label{fig:RZ_HW}
    \vspace{-0.2cm}
\end{figure}

Given the limitations of vanilla TrustZone mechanisms, we propose to leverage complementary, TrustZone-agnostic hardware features available in modern platforms for preventing illegal memory accesses potentially performed by untrusted S.EL1 code. These features consist of three hardware primitives that we require to be offered by the underlying platform.

\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
\item \textit{Platform Partition Controller (PPC):} Consists of a memory and peripheral protection controller that can restrict physical accesses to a given resource, i.e., memory or peripheral (see Figure~\ref{fig:RZ_HW}). On the iMX8MQ SoC, the PPC is implemented by the RDC peripheral. We characterize the PPC by having four main properties. It must be capable of: (a) intercepting all physical requests regardless of both the NS bit signal injected into the system bus and the configurations of the TZASC, (b) setting fine-grained access control attributes (e.g., RO, RW) for configurable memory regions; (c) differentiating between multiple bus masters, and (d) protecting memory-mapped input/output (MMIO) regions, including the PPC's memory-mapped registers. Importantly, (c) and (d) help to ensure that the PPC's configurations cannot be arbitrarily changed by (untrusted) S.EL1 code executed by the processor. Intuitively, to provide this guarantee in the setup illustrated in Figure~\ref{fig:RZ_HW}, the PPC would not allow the bus master identified with MID$_\textrm{0}$ -- i.e., the processor cluster -- to arbitrarily change the PPC configurations. Instead, as explained next, it is the bus master identified with MID$_\textrm{1}$ that will have that privilege.


%Property (a) ensures that we can block arbitrary memory accesses from S.EL1 without the concern of being overridden by the TZASC, and (b) gives flexibility to configure access permissions differently for various memory regions. Properties (c) and (d) allow restricting which bus masters are authorized for changing the configurations of the PPC. Importantly, this feature helps to ensure that the PPC's configurations cannot be arbitrarily changed by (untrusted) S.EL1 code executed by the processor. Intuitively, to provide this guarantee in the setup illustrated in Figure~\ref{fig:RZ_HW}, the PPC would not allow the bus master identified with MID$_\textrm{0}$ -- i.e., the processor cluster -- to arbitrarily change the PPC configurations. Instead, as explained next, it is the bus master identified with MID$_\textrm{1}$ that will have that privilege.

\item \textit{Auxiliary Control Unit (ACU):} This is an independent processor core, distinct from the main application processors. ACUs are small microcontrollers like Cortex-M4 added for housekeeping purposes. 
%Typically, these cores are added for housekeeping purposes and implemented as small microcontrollers (e.g., Cortex-M4). 
For example, Figure~\ref{fig:RZ_HW}, the ACU is identified by MID$_\textrm{1}$. The ACU coordinates the configuration of memory access permissions in the PPC, ensuring that the main processor cores cannot tamper with the PPC permissions. %The ACU executes a piece of trusted code responsible for implementing this coordination protocol.

\item \textit{Secure boot:} %This last building block aims to guarantee that the management core is in full control of the system's PPC and ACU. 
Secure boot validates the integrity and authenticity of the firmware, ensuring that the ACU has been securely bootstrapped and fully controls the PPC.
\end{enumerate}

\subsection{PPC and ACU in COTS Platforms}\label{sec:PPC_ACU_COTS}

\if10 %before revision
These primitives are readily available in several SoCs, for instance on iMX8MQ and iMX8QM SoCs, which we use for building \project. In these SoCs, the PPC and the ACU are implemented, respectively, by a hardware controller named Resource Domain Controller (RDC) and a Cortex-M4 processor. 
%Given that we have abstractly modeled the platform primitives presented above, 
Our defense mechanisms can further be ported to other platforms beyond the iMX8 SoC family. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol}. Also, a wide-range of Qualcomm Snapdragon family SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu, xpucves}. Both fulfill all PPC's requirements. All NXP's iMX8, Xilinx's Zynq and Qualcomm's Snapdragon SoCs deployments span a wide range of edge computing settings (e.g. automotive)~\cite{qc_report, nxp_report, xilinx_report}. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also fill the same role. ACUs are also a clear trend in modern SoCs, which tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}. 
\fi

\rev{The PPC and ACU primitives are readily available in several SoCs, see \autoref{tab:rezone-cots}, for instance on iMX8MQ SoC, which we use for building \project. In this SoC, the PPC and the ACU are implemented, respectively, by a hardware controller named Resource Domain Controller (RDC) and a Cortex-M4 processor.
%Given that we have abstractly modeled the platform primitives presented above, 
Our defense mechanisms can further be ported to other platforms beyond the iMX8 SoC family, and besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that can also fill the same role. The information gathered in this section was derived from looking at device trees, u-boot and TF-A source code, publicly available documentation such as reference manuals, and CVEs. CVEs helped us identified that Qualcomm platforms feature the XPU.}

\rev{At first, it may seem that TZASC fits the requirements for a PPC. However, a TZASC only protects memory regions, and so misses PPC requirement d). Additionally, only TZASC-400 can differentiate between bus masters, a highly specific hardware component not widely deployed to the best of our knowledge. In fact, looking at the latest TF-A release only two platforms support TZASC-400: NXP's lx2160a and ls1028a. To control access to peripherals another TrustZone component is needed, the TZPC. The available documentation shows, however, that the TZPC cannot distinguish between multiple bus masters nor prevent accesses to itself, missing PPC requirements c) and d).}

\rev{As for specific platforms, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol}. Also, a wide-range of Qualcomm Snapdragon family SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu, xpucves} and SMMU. All these fulfill PPC's requirements, see ($\S \ref{sec:plat_req})$. The combination of NXP's iMX8, Xilinx's Zynq and Qualcomm's Snapdragon SoCs deployments span a wide range of edge computing settings (e.g. automotive)~\cite{qc_report, nxp_report, xilinx_report}. Nonetheless, other platforms that can support ReZone include Nvidia Tegra X1 and X2, and Xavier platforms, as well as Socionext SC2A11 and the Broadcom Stingray. Not all current platform can support ReZone though. Examples are Samsung Mediatek and Hisilicon platforms, which don't feature platform wide SMMUs, rather, they feature peripheral specific MMUs, usually for the purposes of media processing.}

\rev{In \autoref{tab:rezone-cots} the "Can Support \project" column values mean the following. "No" means that the platform does not support \project, "Unlikely" means that although there are PPC like mechanisms it is unlikely that they can be used on the CPU itself. "Likely" means that there is a PPC mechanism that is likely to apply to the CPU. Both these values suffer from lack of information, meaning that we don't have enough information to arrive at a definitive conclusion. "Yes" means that there is enough information available to conclude that ReZone can be used in the platform.}

\rev{ACUs are a clear trend in modern SoCs, which tend to include an increasing number of companion processing units for power management and security operations~\cite{armscp}. All analyzed platforms feature, in some form, an ACU. Recent Qualcomm platforms feature a Security Computing Unit (SCU), recent Samsung platforms feature an integrated, or embedded, secure element iSE/eSE, Mediatek features a power management IC, Socionext SC2A11, UltraScale+ MPSoc and the rest feature a variety of auxiliary units that can be reprogrammed to serve as ReZone's ACU.}


%These primitives are currently available, e.g., on iMX8MQ and iMX8QM SoCs, and we use them for building \project.
%\mypara{\sugg{Available hardware to implement \project.}} 
%We have abstractly modeled the PPC so that \project can be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol}. Also, a wide-range of Qualcomm Snapdragon family SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu, xpucves}. Both fulfill all PPC requirements. 
%All NXP's iMX8, Xilinx Zynq and Qualcomm's Snapdragon SoCs deployments span a wide range of edge computing settings such as the automotive industry~\cite{}. Furthermore, Qualcomm is one of the major players in the mobile market~\cite{qc_marketshare}.
%Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. ACUs are also a clear trend in modern SoCs, which tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}.

%To implement \project, we leveraged an OEM-specific platform partition controller, i.e., NXP's RDC. However, in \ref{sec:plat_req}, 
% We have abstractly modeled the PPC so that \project can be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol} while Qualcomm Snapdragon SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu}. Both fulfill all PPC requirements. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. ACUs are also a clear trend in modern SoCs, which %due to the hardware complexity 
% tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}.
% }
%\sugg{TODO: estimar quantas plataformas destas existem no mundo real e segmentos de mercado.}


\input{TableCOTS}

%=======================================================================
%> [Goals and Threat Model]
%=======================================================================	
\section{Design Goals and Threat Model}

\subsection{Design Goals}

We aim to design a security architecture that leverages the primitives presented above to create secure world sandboxes. We refer to these sandboxes as \textit{secure world zones}, or simply \textit{zones}. A zone is meant to host a partitioned TEE stack running at S.EL$_\textrm{1/0}$, i.e., trusted OS and TA software (see Figure~\ref{fig:intro_rezone}). Since multiple zones $z_i$ can co-exist within the secure world, we use the superscript notation S.EL$^i_\textrm{1/1}$ to identify zone $i$. More concretely, we strive to attain four subgoals:

\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
\item \textit{Reduce the privileges of the trusted OS:} %In contrast to vanilla TrustZone platforms where S.EL1 code has unrestricted access to secure and non-secure memory regions, our goal is to sandbox trusted OS code preventing it from accessing outside the memory regions reserved for its particular zone. 
As depicted in Figure~\ref{fig:intro_rezone}, zones must thwart the escalation of privileges of an attacker from the trusted OS to other memory regions of the system. To this end, a zone $z_i$ is expected to enforce three security properties: (P1) protection of the secure-monitor, i.e., EL3 code, (P2) protection of the normal world, i.e., software running at NS.EL$_\textrm{1/0}$, and (P3) protection of co-located zones, i.e., software running at S.EL$^j_\textrm{1/0}$, where $i\ne{j}$.

\item \textit{Depend on a small TCB:} In traditional TEE stacks, both the trusted OS and monitor are considered trusted. In our case, the trusted OS is no longer part of the TCB. To implement zones in the secure world, we will rely on the secure monitor as root of trust, and incorporate as little additional code as possible into the TCB, e.g., for managing PPC and ACU.

\item \textit{Maintain TEE software portability:} There is a lot of legacy TEE and TA software. Vendors and OEMs should easily be able to port preexisting TEE/TA stacks into zone-based environments, requiring minimal to no changes in the code.

\item \textit{Offer a good performance/security trade-off:} The overheads incurred by our solution should not significantly slow down typical real-world TrustZone-based TEE workloads. In other words, we are willing to trade some loss of performance, as long as the performance degradation is not detrimental to the user experience, for improved security guarantees.
\end{enumerate}


\subsection{Threat Model}\label{sec:threat_model}

The attacker's main goal is to subvert the security properties of zones (i.e., P1-3 described above in subgoal 1). We assume the adversary has already compromised the trusted OS of a given zone $z_i$, and aims to escape it (see Figure~\ref{fig:intro_rezone}). %As represented in Figure~\ref{fig:intro_rezone}, the attacker may have hijacked the control flow of  $z_i$'s trusted OS through a chain of vulnerability exploits targeting a TA and then the trusted OS itself. It is also possible that the attacker may have exploited a vulnerability directly in the trusted OS through the normal world interface. Once inside $z_i$,
Running in S.EL1$^i$, the attacker may attempt to access (read/write) external memory addresses outside the $z_i$'s private memory % by crafting page tables and issuing memory requests accordingly 
($\S$\ref{sec:challenge}). These access requests may target i) the physical address space of the victim at NS.EL$_\textrm{1/0}$, EL3, or S.EL$^j_\textrm{1/0}$, or ii) the PPC or memory regions used by the ACU. In the first case, the objective is to override the PPC's memory-mapped registers containing the permissions that forbid access to the victim's memory regions. In the second case, the idea is to subvert the ACU's behavior, e.g., causing the ACU to hand over the control of the PPC to the processor core executing the attacker's code. This would indirectly allow the attacker to disable the PPC's restrictions. The attacker may also leverage the effect of caches to read or write cached memory cells for which S.EL1$^i$ does not currently have permissions.
 
In this work, we do not consider software attacks exploiting vulnerabilities in the secure monitor or in the ACU software. We assume that these components are correct and belong to the system's TCB. The platform's secure boot initializes the system to a known state. We do not consider physical attacks that tamper with hardware, e.g., fault injection. Our solution has the side-effect of providing cache side-channel protection between zones. However, microarchitectural side-channels are out of the scope of our work. Similar to a typical TrustZone deployment, we do not consider denial-of-service (DoS) attacks including those caused, for example, by a malicious trusted OS not relinquishing control to the normal world.


%=======================================================================
%> [DESIGN]
%=======================================================================	
\section{Design}
\label{sec:overview}

Figure~\ref{fig:rezone_arch} represents the architecture of \project. Hardware-wise, our system relies on a typical TrustZone-enabled platform. For controlling memory access permissions, in addition to a TZASC controller, \project relies on a PPC hardware component. The PPC is dynamically configured to block secure world accesses from the processor based on the processor's bus master ID (MID$_\texttt{0}$). The PPC can be reconfigured only by a bus master, predefined at bootstrapping time. In \project, this bus master is the ACU (MID$_\texttt{1}$). ACU and processor can communicate with each other efficiently using a message queue (MQ) implemented by a hardware peripheral.

Software-wise, \project comprises the \textit{secure monitor} and the \textit{gatekeeper}. The former consists of standard secure monitor software (e.g., implemented by Arm Trusted Firmware) augmented with a \project-specific sub-component named \textit{trampoline}. The secure monitor (and trampoline) run on the main processor core and the gatekeeper on the ACU; the PPC protects their private memory regions, which store security-sensitive context information. Taken together, trampoline and gatekeeper manage the execution of zones in the system. They ensure that each zone can access only a private physical memory address space assigned to the zone, and take care of all context-switching tasks involving zone entering and exiting operations. These operations occur when an REE application makes a call to a zone's guest TA (\textit{zone entry}), and the TA returns the results of the call (\textit{zone exit}). REE and zone can share data through a shared memory region. \project's software components are shipped with the platform firmware. When the system bootstraps, the firmware configures the memory layout and statically creates one or multiple zones indicating the composition of their respective software stacks, i.e., trusted OS and TAs. Next, we explain our design decisions and how the system works. We refer the reader to Figure~\ref{fig:HZ-exec-model}.

\subsection{Memory Partitioning and Permissions}
\label{sec:memory_restrictions}

The starting point in \project is to partition the physical memory layout into regions, allocating these regions to different protection domains of the system, and specifying regions' memory access permissions accordingly. In doing this, we are primarily concerned about restricting secure world accesses when the processor runs zone code, i.e., S.EL$_\textrm{1/0}$. The final memory layout and access permissions are depicted in Figure~\ref{fig:HZ-exec-model}. We progressively explain these regions and permissions, beginning with a vanilla TrustZone-enabled platform, and then extending it with \project's protections.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/rezone-arch.pdf}
    \vspace{-0.4cm}
    \caption{\small \project architecture: Its software components are colored in dark shade and consist of secure monitor (which includes the trampoline) and gatekeeper. Secure monitor runs on the main processor cores; gatekeeper runs on the ACU. \project software controls memory accesses via the PPC.}
    \label{fig:rezone_arch}
    \vspace{-0.5cm}
\end{figure}

\begin{figure*}[!ht]
    \centering
        \includegraphics[width=0.95\linewidth]{images/rezone-execution.pdf}
    \vspace{-0.4cm}
    \caption{\small \project execution model, memory access permissions, and memory layout: \project ensures that the code running inside zone 1 -- i.e., at S.EL$_\textrm{1/0}$ -- can only access zone 1's private memory region (M$_\textrm{Z1}$). This protection is achieved by reconfiguring the PPC to restrict the processor's access permissions when entering zone 1 (steps 3\&4), and reverting these configurations when exiting zone 1 (steps 5\&6). %The PPC is used only to restrict the secure accesses.
    }
    \label{fig:HZ-exec-model}
    \vspace{-0.4cm}
\end{figure*}

Just like in a typical TrustZone setup, in \project, the normal world includes regions for the REE OS (M$_\texttt{REE}$) and shared memory (M$_\texttt{SH}$). The secure world has independent regions for the TEE software. The TZASC is then configured to prevent the normal world software from accessing secure world regions. The first line in the permissions table (see Figure~\ref{fig:HZ-exec-model}) shows how the normal world has only read/write access permissions to normal world memory regions.

Then, we further separate the secure world memory into independent regions for the secure monitor and for each zone $i$, e.g., zone 1 (M$_\texttt{Z1}$). We need to ensure that the secure monitor software (EL3) has full access permissions, but the code running at S.EL$_\textrm{1/0}$ is confined to (i) the zone's private memory M$_\texttt{Z1}$ and (ii) the REE shared memory for TA calls. To this end, we leverage the PPC to restrict secure world accesses. However, given that the PPC cannot distinguish secure accesses coming from EL3 or from S.EL$_\textrm{1/0}$ code, these permissions need to be dynamically changed by the monitor when entering a zone (i.e., reprogramming the PPC to remove \texttt{RW} access permissions to M$_\texttt{REE}$ and to secure world memory as per line three in the permissions table) and when leaving a zone (i.e., reverting to the permissions in line two of the table).

However, a difficulty arises when exiting a zone. If the S.EL1 code running inside a zone is wholly prevented from accessing the secure monitor memory, this protection will still be in place by the time the zone's trusted OS traps into EL3; consequently, the secure monitor will be blocked by PCC resulting in memory access aborts and a system crash. To solve this problem, we create a dedicated secure memory region containing code and data that are necessary only to facilitate this transition securely. This code is part of the trampoline, which still belongs to the secure monitor because it runs in EL3. We then segregate a region of the trampoline's memory (M$_\texttt{T}$) from the rest of the secure monitor memory (M$_\texttt{M}$) because these regions need to be configured with different memory access permissions. M$_\texttt{M}$ is always denied access from S.EL$_\textrm{1/0}$. In contrast, M$_\texttt{T}$ is marked read-only by the PPC, therefore, allowing the processor to both execute trampoline code from M$_\texttt{T}$ and load context data also from M$_\texttt{T}$ while still running in S.EL1. The trampoline code will then engage the ACU to remove the PPC memory access restrictions to M$_\texttt{M}$, thus allowing the secure monitor to freely run at S.EL3 and restore the normal world execution. These reasons justify the PPC permissions in the last two rows of the table in Figure~\ref{fig:HZ-exec-model}.


\subsection{Securing the PPC Memory Permissions }
\label{sec:PPC_memory_restrictions}

To guarantee the enforcement of the memory access permissions as described above, the PPC must be (re)configured exclusively by a trusted component. In \project, this component is the gatekeeper/ACU ensemble. We configure the PPC so that only the ACU is authorized to perform this operation. Since the PPC can differentiate requests based on the bus master ID, we program the PPC to accept configuration requests only by a bus master identified with the ACU's MID. Requests originating from other bus masters, e.g., the processor, will be denied. The ACU runs the gatekeeper code and dynamically updates the PPC permissions when entering or leaving a zone by serving the specific requests sent by the trampoline, e.g., to enable M$_\textrm{M}$ \texttt{RW} permissions at zone exits.

\project also needs to defend against a potential attack. Processor and ACU communicate via a message queue unit (MQ in Figure~\ref{fig:rezone_arch}) which is agnostic to the current exception level of the processor. %Therefore, when the processor sends a permission reconfiguration request via the MQ to the ACU, the gatekeeper cannot distinguish whether this request was generated by trusted EL3 code or by untrusted S.EL1 code. 
As a result, an attacker running at S.EL1 in a zone could craft a request to disable the memory access restrictions enforced by the PPC. To thwart this threat, the gatekeeper must foretell that this request is malicious and therefore refuse it. To this end, trampoline in EL3 and gatekeeper share a secret token that is initialized at boot time and copied to their private address space. This token is then used by the trampoline for authenticating PPC reconfiguration requests sent to the gatekeeper. Since the secret token is not accessible at S.EL1, an attacker can no longer spoof legitimate requests, making the system robust against these attacks.


%\subsection{Preventing Cross-zone Interference at the Processor Level}
\subsection{Preventing Cross-zone Interference}
\label{sec:cross_interference}

The mechanisms discussed so far secure all memory transactions observed outside the processor cluster according to the permissions matrix in Figure~\ref{fig:HZ-exec-model}. These mechanisms require additional measures to safeguard against potential attacks within the processor itself. We address two concrete concerns.

First, the PPC acts only at the system bus level. Therefore, its memory access protections do not extend to the internal caches of the processor cluster. For this reason, if the caches contain data that a given zone is not authorized to read or write, if the core enters that particular zone, this content will be accessible to that zone, which constitutes a security violation. To prevent these problems, the cache hierarchy of the core executing the zone is flushed by the trampoline.

Second, the PPC cannot differentiate between individual cores within a cluster, because the PPC observes requests as being from a single bus master: the cluster's shared cache. As a result, \project's memory restrictions enforced by the PPC are collectively applied across all cores of the same cluster. However, blocking access to the normal world memory when a core enters a zone will also prevent other co-located cluster cores from accessing normal world memory, which may lead to crashes if they are currently executing REE code. To prevent this problem, upon zone entry, \project must halt other co-located cluster cores running in the normal world until the core exits the zone. Despite the non-negligible performance overheads potentially introduced by these measures, our experiments show that these overheads can be tolerated due to the infrequent TEE invocation patterns and short TA execution times inside the secure world (see $\S$\ref{sec:eval}), essentially trading some performance degradation for increased TEE security.


\subsection{Zone Entry and Exit Workflows}
\label{sec:key_mechanism}

The protection mechanisms described above act together whenever an REE application invokes a TA hosted in a zone. %This invocation triggers \project's world-switch mechanisms responsible for entering and leaving a zone (see \autoref{fig:HZ-exec-model}).

A zone entry begins when the normal-world OS issues a request through the invocation of the \texttt{smc} instruction (1), causing the execution to be handed over to the secure monitor. If the request needs to be handled by the trusted OS, \project will first differentiate to which zone the requests to that particular TA have been statically assigned. Then, it forwards the request to the respective zone, i.e., zone 1 in Figure~\ref{fig:HZ-exec-model}. For this, the secure monitor starts by notifying all other cores in that cluster. The other cores will then enter an idle state. The trampoline first flushes the core's and shared cache content and then continues by issuing a request (2) to the gatekeeper to configure the PPC to block access of the application core. To authenticate the request as coming from the secure monitor processor mode, the gatekeeper expects to receive the secret token, which was handed to the monitor during boot. After a successful reply from the gatekeeper (3), the trampoline will then (4) jump to the trusted OS.

A zone exit occurs once the trusted OS returns execution to the secure monitor (5). At this point, the trampoline issues a new request to the gatekeeper (6) to unblock secure memory accesses from the core. The gatekeeper ensures this by reconfiguring the PPC to disable the zone's protection policies, i.e., granting \texttt{RW} for all memory regions. The secure monitor will then (7) resume execution, notify other cluster cores to, finally, return to the normal world context (8) executing under traditional TrustZone restrictions enforced by the TZASC.


\newcounter{problem}
\newenvironment{problem}[1]{\refstepcounter{problem}\par\medskip
   \textbf{Problem~\theproblem. #1: } \rmfamily}{\medskip}
   
%=======================================================================
%> [IMPLEMENTATION]
%=======================================================================	
\section{Implementation}
\label{sec:impl}

%We implemented a full-fledged prototype of \project on a real-world hardware platform. Next, we present the most interesting implementation challenges and conclude with an overview of our software prototype.
%sugg{we don't introduce other sections}


%\subsection{Hardware Specification and Security Configurations}
%\label{imp:hw_sec}

The implementation of \project is tightly dependent on the targeted hardware. We used the i.MX 8MQuad Evaluation Kit (EVK), which features an i.MX8MQ SoC by NXP. This SoC is powered by (i) one cluster of four Cortex-A53 application processors (@1.5 GHz) and (ii) one microcontroller, a Cortex-M4 (@266 MHz). The Cortex-A53 cluster has 32KiB level-1 (L1) instruction and data caches per core and a shared 2MiB level-2 (L2) cache. The Cortex-M4 has a 16KiB instruction cache and a 16KiB unified cache.

We use the Cortex-M4 to act as \project's ACU, and an SoC-embedded controller named RDC to play the role of PPC. This controller %is present in the i.MX family and 
enables fine-grained control of access permissions %in platforms with multiple bus masters. This PPC offers this service 
through the creation of security domains. There are at most four domains, each identified by an ID (DID$_i$). A domain represents a collection of platform resources (e.g., memory regions, peripherals), and it is tagged with a set of per-resource access permissions (e.g., read/write, read-only). Bus masters, such as the processor cluster, microcontroller, DMA, etc., can be associated with one or multiple domains. A bus master in DID$_i$ can only access a resource, if the resource is also associated with the bus master's DID$_i$, and its access privileges will be determined by the permissions of DID$_i$.

Based on the security domain scheme provided by this PPC, we use the following insight to implement the memory partitioning and access permissions described in $\S$~\ref{sec:memory_restrictions}. %To create domains, assign/remove resources and/or bus masters to domains, and set permissions, it is necessary to configure PPC's registers. 
Since the PPC is itself a platform resource, we need to reserve a domain (e.g., DID$_1$) with full read/write permissions to the PPC's registers, and associate the ACU as the single bus master to DID$_1$. Doing that, we guarantee no other bus master in the system will be able to tamper with PPC's security permissions. If DID$_1$ can be specified on the system prior to any tampering from an adversary, we ensure that the ACU remains in full and exclusive control of the PPC. To achieve this, we can rely on the secure boot to run a customized initialization routine (i.e., gatekeeper code) that will fully initialize the ACU before starting the zones' trusted OSes. 
%This initialization will be performed by the gatekeeper code that will then set up DID$_1$ and other necessary domains in the PPC.

Our implementation configures two security domains when booting the system: DID$_\textrm{0}$, and DID$_\textrm{1}$. DID$_\textrm{0}$ contains all memory (and other) resources exposed to the cluster. DID$_\textrm{1}$ mainly contains the PPC and the gatekeeper's private memory region. The processor is associated with DID$_\textrm{0}$, and the ACU to DID$_\textrm{1}$. %This configuration ensures that the software running on the processor has no privilege to read or write neither ACU's private memory nor the PPC's configurations. 
As a result, only the ACU can reconfigure the PPC as per the access permission matrix depicted in Figure~\ref{fig:HZ-exec-model} (last two rows). In the i.MX 8M family, Cortex-A clusters are assigned a unique master ID. This means that DID$_\textrm{0}$'s permissions apply indistinguishably to every Cortex-A53 core of the cluster.

We need to establish a secure channel between the cluster and ACU. Upon zone entry/exit events, they exchange message requests (reconfiguration) via the platform's MQ (see Figure~\ref{fig:rezone_arch}). In the i.MX8MQ SoC, the MQ is composed of MU\_A and MU\_B. The PPC is configured to assign MU\_A exclusively to DID$_\textrm{0}$, and MU\_B to DID$_\textrm{1}$, ensuring that only the processor and ACU can communicate with each other through the local MU interfaces. To authenticate the requests sent by the processor, trampoline and gatekeeper share a secret token. 
%Given that trampoline's memory is set as read-only for untrusted S.EL1 code (see the permissions table in Figure~\ref{fig:HZ-exec-model}), the trampoline cannot store the token in memory, otherwise it could be read by a compromised trusted OS.
To preserve the secrecy of the token, the trampoline stores it in the \texttt{TPIDR\_EL3} 64-bit register, which is exclusively available to EL3 code (not even S.EL1 code can read this register) leaving the attacker a 1 in $2^{64}$ chance of guessing its value correctly. The token is randomly generated at boot time.

Given that the ACU runs at a clock speed 5.6$\times$ slower than the cluster, we implemented an optimization to offload workload from the gatekeeper (ACU) to the trampoline (cluster). We observed that the reconfiguration of the PPC's permissions DDI$_\textrm{0}$ resources become slower as the number of resources grows. To shift most work to the trampoline, the gatekeeper temporarily associates the PPC to DDI$_\textrm{0}$, allowing the trampoline to update PPC's permissions on the gatekeeper's behalf. Once finished, gatekeeper removes PPC from DDI$_\textrm{0}$, reacquiring its former condition of sole guardian of the PPC.

%Next, we present the most interesting implementation challenges and conclude with an overview of our software prototype.

%\subsection{Cross-core Synchronization When Running Inside a Zone}
\subsection{Cross-core Synchronization}
\label{sec:synch}

%When one core enters a zone and executes the trusted OS, given that the PPC removes access of the whole cluster to several memory regions (e.g., normal world memory), we must take care to prevent situations where the software running on another core would execute while the first core is still running inside the zone. Otherwise, a second core would simply crash as it cannot access neither the data nor the code from blocked memory regions. 

While one core is in a zone (secure world), the PPC blocks access from the whole cluster to several memory regions (e.g., normal world memory). Thus, specific actions need to be taken into account to prevent other cores from hanging and crashing. Below are the instances where such scenarios might occur (for the sake of simplicity we consider only two cores):

\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
    \item\label{sync1} Two cores $c_1$ and $c_2$ execute secure monitor code at EL3, and $c_1$ issues a zone entry, requesting a shift to S.EL1 while $c_2$ still runs at EL3. This can be a problem because if $c_1$'s request is attended without proper synchronization, $c_2$ will not be able to keep accessing monitor memory.
    
    \item\label{sync2} One core ($c_1$) is executing the trusted OS at S.EL1 while another ($c_2$) is sleeping. Meanwhile, the sleeping core $c_2$ awakens into monitor code (e.g. due to an interrupt). Again this is a problem because $c_2$ will not be able to access monitor memory while $c_1$ executes the trusted OS.
    
    \item\label{sync3} Two cores $c_1$ and $c_2$ are executing normal world code, and $c_2$ requires a service from a TA hosted inside a zone. This is a problem because, when $c_2$ enters the zone, $c_1$ will be denied access to normal world memory.
\end{enumerate}

We solve this problem by synchronizing the cores using spin locks and IPI interrupts. To address scenario \ref{sync1}, the monitor tracks which cores are currently executing the secure monitor. If a core intends to enter a zone, they all wait on a barrier when leaving EL3. At that point, $c_2$ sits on a spin lock while $c_1$ is allowed to jump into the trusted OS. Once $c_1$ concludes the zone call and returns to EL3, $c_2$ can continue. We solve scenario \ref{sync2} by waking the core $c_2$ into a trampoline's read-only memory region (not-writable by the running trusted OS) and waiting for the trusted OS in $c_1$ to cease execution by using a spin lock (\texttt{rz\_lock}). 
To solve scenario \ref{sync3}, we use an IPI interrupt and a spin lock (\texttt{rz\_lock}). First, when $c_1$ issues a request from normal world to enter a zone, it traps into the monitor (EL3) where it fires an IPI interrupt and grabs the \texttt{rz\_lock}. The goal of this interrupt is to notify other cores (i.e., $c_2$) that $c_1$ wishes to enter a zone. Core $c_2$ is then interrupted and jumps into trampoline code, an exception handler running in EL3, where it unlocks $c_1$ letting it continue to enter the zone; $c_2$ now waits on the spin lock until $c_1$ exits the zone, allowing $c_2$ to resume its execution in the normal world.


%\subsection{Microarchitectural Maintenance in EL3-S.EL1 Switches}
\subsection{Microarchitectural Maintenance }
%\subsection{Microarchitectural Maintenance \rev{and Access Control Configuration}}


\if10 % before revision
Triggered by a zone entry/exit event, context switching between EL3-S.EL1 requires the trampoline to coordinate not only the PPC reconfiguration and cross-core synchronization, but also important cleanup tasks (see Figure~\ref{fig:scr_ctx_hw}). Having extensively discussed operations C and D above, we now focus on microarchitectural maintenance that needs to be performed.
\fi

\rev{Triggered by a zone entry/exit event, context switching between EL3-S.EL1 requires the trampoline to perform fundamental cleanup tasks (see Figure~\ref{fig:scr_ctx_hw}). }
When entering a zone (EL3$\rightarrow$S.EL1), the trampoline running on the core needs to ensure that the trusted OS (after the switch is finished) cannot access resources outside of the zone. After taking all measures to prevent interference from other cores ($\S$\ref{sec:synch}), the trampoline needs to invalidate the L1 instruction and data caches and the shared L2 cache (A). Unless this operation is performed, data or instructions left in the cached will be accessible to the trusted OS, thus violating zone isolation. %, therefore violation the isolation properties of a zone's sandbox. 
Also, right before jumping into the trusted OS, the trampoline disables SMP coherency. Recall that at this point, all other cores in the cluster are suspended. Each core has data and instruction in its own L1 caches. With SMP coherency enabled, a request to access cached data would cause the coherency protocol to fetch the data from another core's L1, resulting in a cache hit; thus, data could be accessed by the present core, violating the zone's isolation properties. %Disabling SMP coherency prevents this problem. Without support to disable SMP coherency, we would need to flush the L1 caches of all other cores as part of synchronization to ensure that cached data on other cores is not accessible to them.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/hw-arch/rezone-ContextSwitch.pdf}
    \vspace{-0.4cm}
    \caption{\small Context-switch between EL3-S.EL1 requires microarchitectural maintenance operations (A, B, E). Entering a zone (EL3$\rightarrow$S.EL1) requires A, B, C, D and E. Exiting a zone (S.EL1$\rightarrow$EL3) requires C, D, E and F.}
    \label{fig:scr_ctx_hw}
	\vspace{-0.5cm}
\end{figure}

In addition to cache maintenance, when switching between the trusted OSes of different zones, the trampoline needs to perform TLB maintenance (i.e., TLB invalidation) for the current core (B). The main reason is not due to concerns about violation of zone isolation, as this is already enforced by the PPC by setting each zone's memory region to be private. However, given that (i) the TLB for S.EL1 is shared by the trusted OSes of active zones, and (ii) the TLB has no way to tell which of the cached page table entries belong to each zone  (unless a TLB invalidation is performed), a TLB lookup by the trusted OS could translate into a physical address that belongs to another zone, thus causing unexpected faults. As an optimization, we perform TLB maintenance only when switching between different trusted OSes, % if the last invoked trusted OS is different from the one currently executing. 
%Therefore, in practice, TLB invalidation is only necessary when switching between zones 
and it does not affect TLB entries of the REE OS. With all microarchitectural maintenance done, the trampoline will restore the general-purpose register state and exit to the trusted OS.

\subsection{\rev{Dynamic Access Control Configuration}}
\rev{At the center of context operation between EL3-S.EL1 is the PPC reconfiguration. The PPC is reconfigured after performing micro-architectural maintenance, as doing so before would prevent normal and monitor memory from being written back to main memory. To reconfigure the PPC, the first thing to do is to obtain access to it. This is done by sending a request to the ACU with the secret token to authenticate the trampoline. The ACU will then allow the application cores to access the PPC. At this point only the trampoline is executing, and thus, only it can access the PPC. The trampoline can then perform the necessary configurations, while taking into account that only the specific Trusted OS resources, as well as trampoline code, and a dedicate shared memory region to allow communication between the normal-world and the trustedOS, should be accessible. In our PoC the resource configurations for each Trusted OS are hardcoded inline, but in a real-world release other more flexible mechanisms can be used. After the reconfiguration is performed the trampoline will send another request to the ACU. This time the ACU will configure the PPC so as to prevent access to it other than by the ACU itself. At this point the ACU will reply to the trampoline, and control can be safely handled to the TrustedOS.}

\subsection{Handling Exceptions at S.EL1 Exits}

In contrast to zone entries, exiting a zone by returning from S.EL1 to EL3 no longer requires steps A and B shown in Figure~\ref{fig:scr_ctx_hw}. However, we need special precautions in dealing with exceptions from S.EL1. Two problems may arise:

\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
    \vspace{-0.2cm}
    \item\label{prob1} \textit{TLB-miss:} Upon entering the vector table to handle an S.EL1 exception in EL3, if the TLB misses a page table entry that maps to the memory region of the exception handler, then the MMU must perform a page table walk. As the caches have been flushed before entering S.EL1, this operation will trigger an access to main memory to load the page table entry. However, since the EL3 page tables are stored in the secure monitor's memory region, whose access by EL3 code is still blocked by the PPC at this stage (recall only the trampoline memory is marked read-only), the code for handling the exception cannot be loaded and the system will hang.
    
    \item\label{prob2} \textit{EL3 code injection from S.EL1}: From 1) it follows that the code on the EL3 vector table must be marked as read-only by the PPC, allowing also the trusted OS to read the handler code from memory. However, since the vector table code will be cached in the L1/L2 caches, write operations are still permitted to cache lines tagged as secure, as long as they do not reach the main memory (note the PPC acts only at the bus level). An attacker with S.EL1 privileges can use this feature to modify the exception handler code to its advantage, e.g., by modifying the SMC handler, an SMC call can trigger the secure monitor to load malware from the cache.
\end{enumerate}

To solve both problems, we disable the MMU for EL3 code (F in Figure~\ref{fig:scr_ctx_hw}). We do this in the last steps of exiting from EL3 to S.EL1 when entering a zone. Note that this measure only applies to the MMU for EL3 code: we do not disable the MMU for S.EL1 code. %This separation is possible because EL3 and S.EL1 have different address spaces and can be disabled/enabled individually. %Given that the virtual memory addresses are identity-mapped to physical addresses in the secure monitor, disabling the MMU will not disrupt the secure monitor execution. 
This solves problem 1, as from that point on, memory accesses at EL3 will not be subject to MMU translation; thus, no page table accesses are needed, and the exception handler can then be executed. Disabling the MMU will also disable L1 and L2 caches for EL3 address spaces, and this will partially solve problem 2 as the exception handling code will always be fetched from main memory. This memory is protected read-only by the PPC, hence no modifications will be possible; however, this solution does not entirely solve the whole problem. Note that during the switch from EL3 to S.EL1, after flushing all caches, the trampoline still executes with caches enabled. This will inevitably leave some traces of trampoline data and instructions in the caches, which a malicious trusted OS can try to leverage for an attack by modifying them locally while running in S.EL1 as described above. To clean up potentially tampered cache content and avoid these attacks, we invalidate on-cache trampoline-related memory when the exception handler in EL3 is executed on an S.EL1 exit (E in Figure~\ref{fig:scr_ctx_hw}). After this cache management operation completes, the exception can be handled securely.

%%
%% NS: BACKUP => don't delete yet
%%

\if0
\mypara{Multi Cluster Scenario}\label{sec:mult}
%Our test platforms provide the necessary mechanisms for deploying a system with multiple TEEs. \nuno{TEE software, each one inside an IEE, right?} To implement multiple TEEs in the platform featuring a single cluster, the iMX8MQ, it's necessary to make only the current TEE's program memory available to EL-1. This is achieved in a similar way that secure-monitor program memory is protected; the RDC is used to prevent access to the required memory regions (i.e. other TEEs). When handling trusted service requests the secure-monitor will enable, by interacting with the micro-controller, only the required TEE to execute the service. Figure \ref{fig:multi-tee-same-cluster} illustrates the process. 
%
To implement multiple TEEs in the platform featuring more than one cluster, in addition to the techniques mentioned above, we can also leverage the fact that memory access policies can be defined per cluster. This enables simultaneously running one TEE per cluster while benefiting from mutual isolation. There are many ways to employ this idea, one might be to have as many TEEs as clusters, and statically assign a TEE per cluster. This allows for a straightforward implementation of protection mechanisms, while allowing multiple TEEs to serve trusted service requests parallel to each other. More complex implementations might optimize TEE distribution base on available clusters, to run any TEE on any cluster while clusters are available to execute as many trusted services concurrently as possible.
Given that it's possible to run different TEEs on different clusters, one problem arises. Which TEE should run an each cluster. Nowadays it is common for CPUs to be implemented in a BIG.little configuration. So it is intuitive to assign performance sensitive workloads to high performance cores. System designers may define what services are to run on each cluster as to provide the best user experience. \sugg{These points could go to the design}

\fi


\subsection{Software Implementation}
\label{imp:sw}

The \project software is a firmware bundle based on TF-A (v2.0). TF-A implements basic bootstrapping and secure monitor functionality. We modified TF-A to incorporate the trampoline, encompassing 303 and 1220 SLOC of C and assembly code, respectively. We also used the TF-A to bootstrap the gatekeeper. The gatekeeper is implemented as a bare-metal application that runs on the Cortex-M4. It was written in 417 SLOC of C code and packaged with essential drivers to interface with the RDC. The system image was compiled with the GNU Arm toolchain for the A-profile Architecture (v9.2.1) and GNU Arm Embedded Toolchain (v9.3.1).
%, and the final bootable image was produced with the imx-mkimage (branch imx\_5.4.3\_2.0.0).

We also changed the TF-A's context management routines and data structures to support two zones, each running a trusted OS instance based on OP-TEE (v3.7.0). To run OP-TEE inside a zone, no intrusive modifications were necessary; we have disabled only the support for dynamic shared memory. We create the second OP-TEE instance in a different address space and updated the values of SMC IDs to be uniquely attributed to each OP-TEE instance. We created two full-blown stack builds featuring different REE: one running the Linux kernel (5.4.24) and the second the Android OS (AOSP 10.0). It was not necessary to modify REE code to support \project; however, since we added support to run multiple trusted OSes, we added drivers to interface with both of them. We also duplicated the OP-TEE Linux kernel driver and modified the SMC\_IDs used to make calls to the second OP-TEE instance. There are two tee-supplicant services, one for each OP-TEE.


%=======================================================================
%> [EVALUATION]
%=======================================================================
%\newpage
\section{Performance Evaluation}
\label{sec:eval}


We evaluated \project using the i.MX8 platform and software described in $\S$\ref{sec:impl}. On the i.MX8 platform, all cores, i.e., the Cortex-A53 APU cluster (4x) and the Cortex-M4, were running. Our performance evaluation covers three vectors:

%focused on microbenchmarks ($\S$\ref{sec:eval_micro}) and real-world applications ($\S$\ref{sec:eval_TAs}). 


%\noindent \textit{Workloads:} 
\mypara{1. Microbenchmarks:}
%To evaluate the performance overhead of \project from a micro benchmarking perspective, 
We evaluate the performance overheads at increasing levels of REE-TA interaction. Firstly, we measure the \textit{world switch time}, i.e. the time to transition from normal world to the first instruction of the trusted OS. %since executing the SMC instruction in the normal world until starting the first instruction of the trusted OS in S.EL1. (NS.EL1 $\rightarrow$ S.EL1). 
Secondly, we measure the \textit{round-trip execution time of the GlobalPlatform TEE Client API} (v1.0), i.e., the standard API for an REE application to interact with the TEE. We tested 9 APIs. Lastly, we gauge the \textit{execution time of OP-TEE xtest}, a suite of regression tests provided by OP-TEE to verify the correct implementation of the trusted OS and related APIs. % (e.g., trusted OS core features and cryptographic operations).
The suite has a total of 95 tests, grouped into nine groups. The suite also has seven benchmarks to assess the performance of cryptographic- and storage-related operations.

\if  0
\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
  \vspace{-0.1cm}
    \item \textit{World switch}: First, we measure the time since executing the SMC instruction in the normal world until starting the first instruction of the trusted OS in S.EL1. (NS.EL1 $\rightarrow$ S.EL1).
    
    \item \textit{GlobalPlatform API call}: Then we measure the round-trip execution time of the GlobalPlatform TEE Client API (v1.0), which is the standard API for an REE application to interact with the TEE. We tested 9 APIs.

    \item \textit{OP-TEE xtest suite}: Lastly, we gauge the execution time of xtest, a suite of regression tests provided by OP-TEE to verify the correct implementation of the trusted OS and related APIs, i.e., trusted OS core features, cryptographic operations, etc. 
    The suite has a total of 95 tests, grouped into nine groups. The suite also has seven benchmarks to assess the performance of cryptographic- and storage-related operations. 
\end{enumerate}
\fi

\mypara{2. Real-world applications:} %We also assessed the performance of real-world applications. To this end, 
We evaluated two TAs: a Bitcoin wallet and a DRM player service. The open-source Bitcoin wallet TA~\cite{bitcoinwallet} provides services, e.g., for creation and deletion of a master key, access the mnemonic for a master key, sign a transaction, and get the address of the wallet. The DRM player service is implemented with the open-source OP-TEE Clearkey plugin~\cite{opteeclearkey} and the media player ExoPlayer~\cite{exoplayer}. This service approximates to a security level 2 (L2) DRM compatible setup~\cite{widevinelevels}, where video content is split into subsamples and decrypted within the TEE, but processed in the normal world. The L2 DRM configuration represents the worst-case scenario for performance since the process is split among the two worlds. %To evaluate the performance of this service, 
We measured the (i) execution time for decrypting one subsample for three different resolutions and frame rates and (ii) the time elapsed between decoded content.  

\if 0
\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
    \item \textit{Bitcoin wallet}: The open-source Bitcoin wallet TA~\cite{bitcoinwallet} provides a set of services, e.g., for creation and deletion of a master key, access the mnemonic for a master key, sign a transaction, and get the address of the wallet.
    \item \textit{DRM player service:} It is implemented with the open-source OP-TEE Clearkey plugin~\cite{opteeclearkey} and the media player ExoPlayer~\cite{exoplayer}. This service approximates to a security level 2 (L2) DRM compatible setup~\cite{widevinelevels}, where video content is split into subsamples and decrypted within the TEE, but processed in the normal world. The L2 DRM configuration translates the worst-case scenario for performance since the process is split among the two worlds. To evaluate the performance of this service, we measured the (i) execution time for decrypting one subsample for three different resolutions and frame rates and (ii) the time elapsed between decoded content. 
\end{enumerate}
\fi

\mypara{3. Impact to REE performance:} %Lastly, to understand the impact of \project on the overall REE execution time, 
We used PCMark for Android benchmark (v3.0), which assesses the performance of smartphones by testing everyday activities. The suite consists of five real applications (e.g., web browsing, data and video editing) and it does not invoke secure world functionality.
The benchmark provides an overall score (Work 3.0) translating the performance of the whole system into a quantifiable scoring system: a higher score indicating better performance.

\mypara\textit{Timing and sampling methodology:} To measure the world switch time, we used the AArch64 generic timer, a 64-bit cycle counter running at 8.33MHz. To measure the execution time of both the GlobalPlatform API and the xtext suite, we used the Linux time API with the CLOCK\_REALTIME parameter enabled. To measure the Bitcoin wallet execution time we used the Linux time utility. For the DRM service, we used (i) the Linux time API for the subsamples decryption and (ii) the Java System.nanoTime for the processing.

\noindent \textit{Testbed configurations:} Excepting world switch measurements, for all other experiments, we compare three system configurations: (i) the standard OP-TEE deployment (No RZ); (ii) the \project deployment (RZ); and (iii) the \project deployment with no trusted OS preemption from the REE (RZ no IRQ). For all experiments, we collected 1000 samples, presenting the average value.
For microbenchmarks, we flush the caches at the end of each test. This reduces the hot-cache effect of the previous iteration and approximates a realistic TEE setup. Next, we present our main findings.



\if0
To evaluate the performance overhead at a micro perspective we measured: (i) the \textit{world switch time}, i.e., the amount of time since the SMC call in the normal world till the execution of the first instruction on the trusted OS (NS $\rightarrow$ S); (ii) the round-trip execution time of the \textit{GlobalPlatform client API}; and (iii) the execution time of \textit{xtest}, the OP-TEE sanity testsuite. OP-TEE provides a suite of regression tests, called xtest, to verify the correct implementation of the trusted OS and related APIs, i.e., trusted OS core features, cryptographic operations, secure storage, key management, etc. The suite encompasses a total of 95 test, grouped into nine groups. The suits also provides seven benchmarks aiming at assessing the performance of cryptographic- and storage-related operations (trusted storage, AES, SHA).  

To assess the performance of real world applications, we evaluated two different TAs: (i) a \textit{Bitcoin wallet}; and (ii) a \textit{DRM Player}. The open source Bitcoin wallet TA~\cite{bitcoinwallet} provides a set of services which includes the creation and deletion of a master key, access the mnemonic for a master key, sign a transaction, and get the address of the wallet. The DRM player service is implemented with the open source OP-TEE Clearkey plugin~\cite{opteeclearkey} and the media player ExoPlayer~\cite{exoplayer}. The service approximates to a security level 2 (L2) DRM compatible setup~\cite{widevinelevels}, where video content is split into subsamples and decrypted within the TEE, but processed/decoded in the normal world. The L2 DRM configuration translates the worst-case scenario for performance, since the process is split among the two worlds. To evaluate the DRM service performance we measured the (i) execution time for decrypting one subsample for three different resolutions and frame rates and (ii) the time elapsed between decoded content. 
% (\autoref{fig:drm_macro}, left) | (\autoref{fig:drm_macro}, right)
%We believe this two TAs are representative of completely different profiles with regard to the frequency the secure world is invoked. 
To measure the impact of \project on the overall normal world execution, we also ran the PCMark (v3.0) for Android benchmark. The benchmark is mainly used to measure the performance of smartphones and tablets, by using tests based on everyday activities. The suite consists of five real applications (e.g., web browsing, data and video editing), with the Work 3.0 benchmark translating the performance of the whole system. Running PCMark on a typical smartphone takes around 10 minutes. 

\noindent \textit{Timing mechanisms:} To measure the world switch time, we used the AArch64 generic timer, which features a 64-bit cycle counter running at 8.33MHz. To measure the execution time of both the GlobalPlatform API and the xtext suite, we used the Linux time API with the CLOCK\_REALTIME parameter enabled (i.e., Linux uses the AArch64 generic timer). To measure the Bitcoin wallet execution time we used the Linux time utility. For the DRM service we used (i) the Linux time API for the subsamples decryption and (ii) the Java System.nanoTime for the processing. For all experiments we collected 1000 samples, and present the geometric mean.
With the notable exception of the world switch time and the PCMark benchmark, for all experiments we compare three different system configurations: (i) the standard OP-TEE deployment (No RZ); (ii) the \project deployment (RZ); and (iii) the \project deployment with no trusted OS preemption from the REE (RZ no IRQ).
\fi


%We collected 1000 samples, while for each sample the APIs were invoked in sequence, following the order in which they are presented in \autoref{fig:api}. While calling the APIs in a particular order impose a cause-consequence effect at the microarchitecture (e.g., hot-cache), we believe this is the most realistic setup, per the standard behaviour of real-world applications. Between each collected sample, i.e., full execution of the nine APIs, we flush the microarchitectural state, so that there is no cumulative effect of the microarchitectural state between samples.



\subsection{Microbenchmarks}
\label{sec:eval_micro}

We identified two main factors impacting the performance overhead, i.e., (i) the number of trusted OS calls and (ii) the complexity/duration of the operation running in the secure world (mainly the logic of the TA). Workloads encompassing simple TA operations/logic with a higher number of world switches will translate into significant performance overhead. In contrast, workloads encompassing complex TA operations with small number of world switches will translate into negligible performance overhead. Multiple zones support has also a negligible impact on the overall performance of the system.


%\sugg{1) robusto; 2) alto a micro, menos a macro; 3) caches são a maior impacto na performance}
%\sugg{subcecçõa a methodology: micro usamos xx, macro xxx}
%\sugg{subsecão micro benchmakrs: }
%\sugg{subcecçõa b: main findings: messages 1 para por message}


\mypara{World switch time.}
The world switch time increased from an average of 5.7 to 74.9 microseconds, i.e., 13x. This increase is the cumulative penalty of: (i) the additional \project trampoline and gatekeeper execution time; (ii) the cluster-MCU requests; (ii) the penalty of running a portion of the trampoline with caches disabled; and finally, (iii) the time of the cache maintenance operations. Despite the high overhead of raw world switches, they often translate into relatively small slowdowns in real-world TEE usage scenarios (see $\S\ref{sec:eval_TAs}$).

%Although a 13x penalty may suggest a prohibitive performance cost for a system, we will see, that the \project overhead gets considerably smaller (till the point of becoming negligible) when seen from a macro perspective. 

%At the end of each iteration, we flush the caches, so that each sample does not translate the hot-cache effect of the previous running.
%; and finally, (iv) the cold cache effect on the trusted OS while fetching the first instructions

\if0
The results are presented in \autoref{tab:ctx}.
%
%
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{ccc}
& Time & Overhead\\
\toprule
No \project & 85.49us & - \\
\project & 420.86us & 4.92x \\
\bottomrule
\end{tabular} 
\caption{\small Context-switch overhead with \project}
\label{tab:ctx}
\end{table}
\fi

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/api_barchart.pdf}
    \vspace{-0.8cm}
    \if10
    \caption{\small \project overhead and time of GlobalPlatform API. }
    \else
    \caption{\small \rev{\project overhead, time, and normalized std. dev. of GlobalPlatform API. N=1000.}}
    \fi
    \vspace{-0.0em}
    \label{fig:api}
	\vspace{-0.5cm}
\end{figure}

\mypara{GlobalPlatform API.}
%The execution time accounts for the time spent since issuing the API call on the normal world client application till receiving the reply from the TA. This process includes a full round-trip world switch as well as the execution of the trusted OS and TA for handling the request. 
\autoref{fig:api} presents our main results. The geometric mean of the normalized performance overhead for the nine API benchmarks is 2.32x, i.e., a significant decrease comparing to the 13x overhead from the world switch. We can observe that the three APIs (i.e., \textit{OpenSession}, \textit{InvokeCommand}, and \textit{CloseSession}) that explicitly call the secure world have a larger penalty, ranging from 2.33x to 4.08x. The \textit{InvokeCommand} and \textit{CloseSession} APIs are the ones that take less time to execute, and thus the ones with the bigger overhead, due to the over-penalty of cache-related operations (see xtest evaluation). Third, from the remaining six APIs, three have almost no penalty. Notable exceptions encompass the two pairs of APIs for shared memory, i.e., \textit{AllocateSharedMemory} and \textit{RegisterSharedMemory}. This is related to the OP-TEE configuration which disables dynamic shared memory and thus implementations are identical. While calling these APIs, there is no switch to the secure world, and so code and data are already cached. The same happens on the release operation. Lastly, we can observe that the system configuration without preemption (RZ No IRQ) slightly decreases the overhead, reducing the geometric mean from 2.32x to 2.28x.


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/xtest_simple_barchart.pdf}
    \vspace{-0.8cm}
    \caption{\small Geometric mean of \project overhead for xtest. Unit tests (left) and benchmarks (right). Geometric mean is 1.71x.}
    \label{fig:xtest}
	\vspace{-0.5cm}
\end{figure}


\mypara{xtest suite.} \autoref{fig:xtest} presents a summarized view of the results, represented by the geometric mean of all tests for the same group. Unit tests are represented in nine groups on the left, while benchmarks are represented in three groups on the right. A detailed view of the results per test/benchmark can also be found in Appendix. %The first conclusion that can be taken is that geometric mean of the performance overhead for all tests and benchmarks is 1.71x. 
The group of tests that has a bigger impact is the TEE Internal API and Global Platform API, i.e., 2.96x and 2.37x, respectively. Note that this group of tests are the ones with smaller execution time and simpler secure world operations. Interestingly, the geometric mean of the performance overhead for the Global Platform API tests is very similar to the ones presented before. %The deviation can be justified by the higher number of APIs that are tested in xtest. 
On the other hand, tests such as mbed TLS and key derivation perform fewer but longer operations in the secure world. %This results in a smaller overall penalty. The network socket group leverages a normal world client application (i.e., tee-supplicant) to securely communicate through a socket. Naturally, these tests required a large number of world switches, from socket management to retrieving data. 
Since the execution time of the operations performed in the secure world is large, the performance overhead is relatively lower when compared to the TEE API groups. To complete, we tested a potential application-level optimization. %did an interesting experiment. 
Specifically, we modified one particular unit test (4007 symmetric) which consists of performing different symmetric encryption schemes (e.g., AES, DES) for incremental key sizes (e.g., 64-, 128-bit). The standard implementation has a total of 3978 secure world calls per run. We modified the implementation to perform all iterations in a single TA call. By simply batching all operations and processing them in a one-time operation, we reduced the number of calls to the secure world to 96 and were able to decrease the performance overhead from 3.6x to 1.08x.


\mypara{Multiple zones penalty.} To assess the performance penalty of supporting multiple zones, we built two specific test cases using xtest. The main difference, implementation-wise, to schedule a different zone, is the extra operation required to invalidate the TLB. Thus, in the first experiment, we measured the execution time of running xtest 4001 on trusted OS$_\textrm{2}$, while previously running also trusted OS$_\textrm{2}$. For the second test, we measured the execution time of running xtest 4001 on trusted OS$_\textrm{2}$, while previously running trusted OS$_\textrm{1}$. For the former, it takes, on average, 75.7ms to complete. For the latter, it takes, on average, 77.5ms to complete, i.e., a 1.8ms (2.6\%) increase.  




% linha a tracejado com a média
% máximo percentil 5\% 95\%
% Escala de 0% a 100%
% TODO: Expirementar as mesmas escalas




\subsection{Real-world Applications}
\label{sec:eval_TAs}

%When comparing the relative performance overheads of \project at a microbenchmarking scale with the results with Bitcoin wallet and DRM player, we observe dramatic improvements. 

%When analyzing the results with Bitcoin wallet and DRM player, 
Our findings suggest that \project will not significantly affect the user experience in real-world applications.

%Overall, the performance overhead of real-world applications and benchmarks is negligible and will not affect the user experience. 

In the case of the Bitcoin wallet, the geometric mean of the performance overhead is 1.50x for the vanilla \project implementation and 1.48x for a non-preemptible configuration (\autoref{fig:bitcoinwallet}). The most impacted wallet services are related to simple one-time operations. For instance, the absolute execution time of the operation checking if a master key exists is considerably smaller (11.9ms for the standard OP-TEE deployment) than the other services, and thus the penalty is higher. Notwithstanding, the results clearly demonstrate that the impact of \project in longer time-consuming operations, e.g., Bitcoin sign transaction (the one likely to be executed more frequently) is low (1.2x) and one order of magnitude smaller than the overhead observed in the raw world switch. 
%Furthermore, disabling the preemption on the trusted OS presents a marginal improvement.
%We narrowed our evaluation to the \textit{sign transaction} and \textit{get wallet address} services. ... , while services such as \textit{create master key} and \textit{delete master key} are seen as one-time operations

%     1 check key -> open secure storage -> will cause multiple calls to normal world as the OS accesses the ree fs
%     2 generate mnemonic/key -> generate mnemonic, store key in the ree fs (various calls to supplicant) 
%     3 generate mnemonic/key -> same as above, but mnemonic is an argument
%     4 delete mnemonic/key -> open object (ree fs), delete it (ree fs)
%     5 sign transaction -> get master key from ree fs, do many cryptographic operations
%     5 get address -> get master key from ree fs, derive public key (wallet address)
%     
%     every open, read, and close will invoke the normal world
%\sugg{command 1 being the simplest (and shortest running) is the most affected by \project. this command tries to open a file (holding the master key) from the REE, and thus will perform calls to the normal world. Similarly, command 4 is also a simple command which accesses the master key storage in the REE fs, and will delete it the key if it exists. By doing more work than command 1, the relative runtime execution of the command will have lower overheads. Other commands do significant amounts of cryptographic operations, and the penalties involved from context switching, and this cache maintenance, are less pronounced.}

%We use a previous implementation of a bitcoin wallet~\cite{bitcoinwallet} to be executed as a TA in a trusted OS. We measure the time to execute with the \emph{time} Linux utility, and observe the \emph{real time} component of the output. Overhead for TA operations goes up to 2.2x for the command that executes in least amount of time, however for other commands the overhead is smaller, as low as 1.2x. Overall, disabling interrupts in the trusted OS achieves modest performance improvements. The results are presented in \autoref{fig:bitcoinwallet}.

\if11
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/wallet_barchart.pdf}
    \vspace{-1.1cm}
    \if10
    \caption{\small Relative and absolute execution time for Bitcoin wallet.}
    \else
    \caption{\small \rev{Relative, absolute execution time, and normalized std. dev. for Bitcoin wallet. N=100.}}
    \fi
	%\vspace{-0.3cm}
    \label{fig:bitcoinwallet}
	\vspace{-0.5cm}
\end{figure}
\fi

Regarding the DRM player, \autoref{fig:drm_macro} plots our results. Overall, the geometric mean of the normalized performance overhead for the DRM subsample decryption is 1.64x. Intuitively, the higher the frame rate, the bigger the penalty, i.e., for the 1920x1080@60 configuration the expected performance penalty is 2x. \rev{Curiously, the higher framerate sample featured lower average frame sizes, causing frequent calls to smaller ammounts of work, which helps explain the higher overheads.} Second, the \project configuration without preemption (RZ No IRQ) slightly improves the performance of the decryption process, reducing the geometric mean of the normalized performance overhead to 1.4x. This benefit is also noticeable in the processing of the decoded frames and the rendering of the final image (\autoref{fig:drm_macro}, right). Third, although there is a slowdown in decryption, this penalty is in the order of 100 $\mu$seconds. Hence, it is not noticeable in the playback of the video and does not impact the user experience.

%{\color{orange}
%Although we observed 1.5x increase in subsample decryption times, this falls well bellow the ~16ms mark for 60fps content and 41ms for 24fps content.
%We also observe a slight improvement in performance, to around 1.4x, by disabling TEE interrupts. }

%{\color{orange}Although \project causes overheads in decrypting subsamples, the smooth playback of media is not compromised. In ExoPlayer, processing decoded frames for rendering the final image occurs at periodic intervals. We measure the time elapsed between decoded content. The results are presented in \autoref{fig:drm_macro}. Although the period between processing frames increases slightly the overhead is not perceptible to the end-user. Each subsample is decrypted individually, and due to the costs incurred by context switching, we believe that playing DRM content in a \project enabled system can be significantly optimized by increasing the number of subsamples decrypted per TEE call.}

%\sugg{geometric mean DRM subsample decryption: RZ: 1.64; RZ\_No\_IRQ: 1.43;}
%\sugg{geometric mean DRM elapsed time: RZ: 1.01; RZ\_No\_IRQ: 1.00}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\columnwidth]{images/benchmarks/drm_barchart.pdf}
    \includegraphics[width=0.49\columnwidth]{images/benchmarks/drm_macro_barchart.pdf}
    \vspace{-0.35cm}
    \caption{\small rev{Performance overhead, execution time, and normalized std. dev. for the DRM subsample decryption (left) and processing (right). N=1000, N=1000, N=400, for 1080@24, 1080@60, and 360@30 respectively.}
    }
    \label{fig:drm_macro}
    \vspace{-0.5cm}
\end{figure}

\if0 %sumited version
\subsection{Impact to the REE Performance}
\label{sec:eval_NW}

To measure the impact of \project on the overall REE execution time, we also executed the PCMark (v3.0) for the Android benchmark. This benchmark is mainly used to assess the performance of smartphones and tablets, by using tests based on everyday activities. The suite consists of five real applications (e.g., web browsing, data and video editing) \sugg{and it does not invoke the secure world}. 
\sugg{The benchmark provides an overal score (Work 3.0) translating the performance of the whole system into a quantifiable scoring system: a score with higher numbers indicating better performance. Running PCMark takes around 10 minutes.}
\st{It includes an additional benchmark (Work 3.0) translating the performance of the whole system into a quantifiable scoring system: a score with higher numbers indicating better performance. Running PCMark takes around 10 minutes. }


We compared five different system configurations: (i) the standard OP-TEE deployment, with no secure world calls while running PCMark (No RZ); (ii) the \project deployment, with no secure world calls while running PCMark (RZ); and the \project deployment with explicit secure world calls to a toy TA every (iii) one, (iv) ten, and (v) twenty seconds while running PCMark. The toy TA in the secure world performs a simple sum operation and returns to the normal world. The results are depicted in \autoref{fig:PCMarkv3}. In our tests, we can see that the penalty in the overall system performance is relatively low varying between 0.04\% and 0.99\%.


%{\color{orange}The final test result is represented by \emph{Work 3.0 performance score}. We perform measurements on a setup configured without \project, configured with \project without periodic invocation, configured with \project and with periodic invocations to a trusted OS in 1s, 10s, and 20s intervals. The more frequent the invocation to trusted OSes the more performance is affected, as can be observed in \autoref{fig:PCMarkv2}. However, \project does not significantly degrade performance of the normal world if a trusted OS is not invoked. }

%\sugg{PCMark Work 3.0, is a benchmark suite that performs tests that mimic common, everyday tasks. Instead of evaluating individual units, the result is a measurement of the performance of a device as a complete unit. The Work 3.0 Performance Score reflects this, as it uses web browsing, photo editing, video editing, data manipulation and writing scenarios to achieve a score of the system's performance.}

\if10
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/benchmarks/nw_barchart.pdf}
    \caption{\small \project normal world impact measured as impact on PCMark (v3.0) benchmark without invoking a trusted OS, and with periodic invocations in 1s, 10s, and 20s intervals.}
    \label{fig:PCMarkv3}
    \vspace{-0.5cm}
\end{figure}
\else
\begin{table}
\centering
\begin{tabular}{cccc}
\textbf{Configuration} & \textbf{Interval} & \textbf{Work 3.0 Score} & \textbf{Overhead} \\
\midrule
No RZ & - & 5020 & 0.00\% \\
RZ & - & 5018 & 0.04\% \\
RZ & 20s & 5018 & 0.04\% \\ 
RZ & 10s & 5002 & 0.36\% \\
RZ & 1s & 4971 & 0.99\% \\

\toprule
\end{tabular} 
    \caption{\small \project normal world impact measured as impact on PCMark (v3.0) benchmark without invoking a trusted OS, and with periodic invocations in 1s, 10s, and 20s intervals.}
  \vspace{-1.3em}
    \label{fig:PCMarkv3}
\end{table}
\fi

%\sugg{Use the Work 3.0 performance benchmark to test the performance of your device. This test takes around 10 minutes on a typical smartphone.}
\fi

\if10
\subsection{Impact to the REE Performance}
\else
\subsection{\rev{Impact to the REE Performance}}
\fi
\label{sec:eval_NW}

%To measure the impact of \project on the overall REE execution time, we also executed the PCMark (v3.0) for the Android benchmark. This benchmark is mainly used to assess the performance of smartphones and tablets, by using tests based on everyday activities. The suite consists of five real applications (e.g., web browsing, data and video editing) and it does not invoke secure world functionality.The benchmark provides an overall score (Work 3.0) translating the performance of the whole system into a quantifiable scoring system: a higher score indicating better performance.

We observed that the performance impact from \project on the REE is low, even when stressing secure world calls and the number of parallel calls from concurrent CPUs. 

First, we configured the REE to run the PCMark (in the quad-core configuration), while concurrently running a toy TA at different intervals (10, 100, and 1000 ms). The toy TA performs a simple sum operation and returns to the normal world. We compared with a system configuration running the vanilla OP-TEE and without calling the TA while running PCMark. \autoref{tab:pcmark}, on the left, presents the results. For reasonable intervals between the toy TA calls (1000 and 100) the performance penalty is low, 0.98\% to 6.20\%, respectively. When the interval is 10 ms (similar to a DRM workload), the impact is reasonable (13.47\%) and in the order of magnitude as the ones presented in $\S\ref{sec:eval_TAs}$. We then tried to understand the impact on the REE from having multiple CPUs issuing concurrent TA calls. To do that, we fixed the interval rate of calling the toy TA in 1000ms. \autoref{tab:pcmark}, on the right, depicts the results. The impact is low and proportional to the number of concurrent cores, achieving the largest penalty (4.08\%) when the four cores are issuing concurrent TA calls.  

%We compared different system configurations including single- and multi-core configurations. (i) the vanilla OP-TEE deployment, with no secure world calls while running PCMark (No RZ); and the \project deployment with explicit secure world calls to a toy TA every (ii) second, (iii) hundred milliseconds, and (iv) ten milliseconds while running PCMark concurrently. The toy TA performs a simple sum operation and returns to the normal world. The results are depicted in \autoref{tab:pcmark}. 

%In our tests, we observe up to 13.47\% impact on performance for scenarios of high-frequency calls to the secure world, which are expected of a typical DRM workload. On the other hand, for a burst of calls to the secure world, a scenario we consider unlikely to occur often, we observe an impact as high as 4.08\%, for a scenario were all CPU cores are called in a burst at 1 second intervals.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/benchmarks/pcmark.pdf}
%     \caption{\project normal world impact measured as impact on PCMark (v3.0) benchmark without invoking a trusted OS, and with periodic invocations at various intervals.}
%     \label{fig:PCMarkv3}
% \vspace{-0.5cm}
% \end{figure}
\input{TablePcmark}

%\sugg{Use the Work 3.0 performance benchmark to test the performance of your device. This test takes around 10 minutes on a typical smartphone.}

\if0
\subsection{\sugg{Multiple zones penalty}}
\label{sec:eval_mTEE}

%To understand the performance penalty of supporting multiple zones, we built two specific test case scenarios. The main difference, implementation-wise, in the trampoline, to schedule a different zone (i.e., trusted OS), is the extra operation required to invalidate the TLB. Thus, in the first case scenario, we measured the execution time of running xtest 4001 on trusted OS 2, while the previous running zone were also running trusted OS 2. In the second test case scenario, we measured the execution time since of running xtest 4001 on trusted OS 2, while the previous running zone were running trusted OS 1. To measure the execution time, we also used the Linux time API. We collected 1000 samples for each test case scenario. For the first test case scenario, it takes, on average, 75.7ms to complete. For the second test case scenario, it takes, on average, 77.5ms to complete, i.e., a 1.8ms (2.6\%) increase. Overall, we believe the extra penalty to provide multiple zones is really small and negligible for the overall performance of the system.     
\fi

\if0
\begin{verbatim}
    Ao termos multi-TEEs temos um factor extra de penalização de performance, TLBI invalidate.
    
    é necessário fazer TLBI quando executamos o TrustedOS 2 depois de ter executado o trusted OS 2 (isto porque fazemos TLBI quando sabemos que o último TEE a executar é diferente do que queremos executar a seguir)
    
    portanto temos dois cenários:
    1) TEE executa "sozinho", onde nõa haverá TLBI
    2) TEE é executado depois de outro (haverá um TLBI)
    
    portanto para avaliarmos fazemos
    Scenário 1:
        TOS2 -> executa uma TA (escolhemos o 4001, mas na verdade poderia ser outro exemplo qualquer)
    
    scenários 2:
        TOS1 -> xtest 1001 (isto chama só TOS, nãoi invoca TAs, na verdade não itneressa. o nosso interesse é que o próximo TOS seja diferente)
        TOS2 -> executa uma TA (escolhemos o 4001, mas na verdade poderia ser outro exemplo qualquer)
\end{verbatim}
\fi
 
%{\color{orange}To measure the impact multiple zones might have in performance, we compare two scenarios. In the first scenario we invoke trusted OS 2, we use xtest regression test 4001, which will invoke a TA to perform cryptographic operations. On scenario 2, we first invoke a simple operation on trusted OS1, before calling Truste OS2. This is done by invoking xtest regression test 1001, a simple test which only invokes the trusted OS. Invoking the trusted OS1 first will result in a TLBI being performed upon a call to trusted OS2. After trusted OS1 is invoked, we execute the same xtest test as in scenario 1, regression test 4001, on trusted OS2. 
%We observe an overhead of 2.6\% corresponding to an average of 1.8ms in a test which takes 77.5ms to execute without invalidating the TLB. We consider this overhead to be negligible, particularly in light of the overhead already incurred by the cache maintenance operations.}


%=======================================================================
%> [SECURITY ANALYSIS]
%=======================================================================

\section{Security Evaluation}\label{sec:security_analysis}
%In this section, we present our security analysis. We measure the TCB size and compare it to alternative solutions. We also survey 80 CVE vulnerability reports aiming at understanding the number of attacks \project could prevent. 


\if0
\subsection{Attack Mitigation}
TrustZone-based TEEs have been the target of multiples attacks, which exploit software flaws to obtain privileged execution, extract secrets, or twarth security functionality. We next analyze how these attacks would fare in a system deployed with \project.

\mypara{Attack 1. } By compromising a TA, it is possible to exploit a flaw in a secure driver~\cite{BreakingArmTZ, DeepDive}. Secure drivers have access to mmap, which allows them to map physical memory. The Secure Monitor can then be mapped by the now malicious secure driver, and the attacker can do anything on the platform, including exposing secrets. A master key is one of such secrets. In the Samsung ..., the master key is used by the drcrypto driver for cryptographic operations.
There are two ways in which the master key can be obtained: a) obtaining access to EL3 memory and reading the master key location, b) or via an SMC to the secure monitor.

\mypara{Mitigation 1. } \project mitigates against obtaining the Master Key by preventing the trusted OS from accessing monitor memory. Because malicious software can longer map the Secure Monitor it can no longer obtain the master key directly. This solves problem 1.a). However, the attacker can still obtain the master key through a Secure Monitor Call (SMC), problem 1.b). To mitigate this, with \project, we argue for implementing cryptographic primitives requiring platform keys, and other system critical features, in a separate zone which will not reveal the key being used. 

\mypara{Attack 2.} An attacker can compromise a system TA  through the trusted OS, by first obtaining execution privileges in the trusted OS~\cite{BreakFDE,shen-trustedcore}. This can be used to thwart security functionality. For example, an attacker can obtain the secret key used to encrypt the file system~\cite{BreakFDE} or effectively compromise the fingerprint authentication mechanism~\cite{shen-trustedcore}. 
%The secret key is encrypted by the user password, however it is possible to bruteforce the password on a powerful PC. 

\mypara{Mitigation 2.} \project allows for the secure deployment of multiple OSes. It is possible to prevent a compromised component from zone$_{1}$ from obtaining secrets from other zones, provided that zone$_{1}$ is bug free. Securely developing zone$_{1}$ is easier than doing the some for a single TEE domain hosting all TAs. Thus, by using \project to allow more than one TEE to execute in the secure world, a vulnerability in one zone can not be used to obtain secrets from another.
 
\mypara{Attack 3.} By leveraging a TA's access to normal world memory, it is possible to access all memory in the normal world~\cite{gb-exploit6, Aravind2017}. This is possible because the trusted OS can map the normal world physical memory at will, and in certain scenarios can map this memory unto a TAs address space. With access to normal world memory an attacker can compromise the Linux kernel, for example by creating a back door within seldom used kernel modules. This gives the attacker arbitrary code execution at kernel level of privilege.

\mypara{Mitigation 3.} In \project we can restrict the normal world memory accessible to a trusted OS. This requires knowledge of what memory is dedicated for sharing memory between the TEE and REE, however, on some platforms TF~-~A already supports modifying an in-memory device tree. This means that TF-A can specify to the kernel which memory is available for sharing information between worlds. Fixing the shared memory space makes it possible for secure monitor to enforce secure-world zones, although, at a cost of not supporting dynamic shared memory, which allows a normal world process to mark part of its memory as shareable with the TEE.

\mypara{Attack 4.} Code reuse attacks. An attacker can leverage control highjacking to compromise the trusted OS~\cite{gb-exploit4}. In particular the attacker might leverage the presence of privileged operations, for example in the case for Armv7-A or Armv8-A\_aarch32 the DACR registers, which when set to zero disable MMU based memory protection.

\mypara{Mitigation 4.} In \project, we use platform level access control mechanisms to enforce zone access permissions to memory. Even with access to privileged instructions in the trusted OS, an attacker can not modified these policies, and thus is confined to the specified sandbox. 
\fi

\subsection{Mitigation of Potential Attacks}
%\subsection{%Vulnerability Analysis}
% \sugg{Objectivo. Perceber como CVEs reais quais os ataques que podem ser mitigados}
% \sugg{Metodologia, 80 CVEs, critério usado para classificação, relacionar com os vetores de ataque. Se o exploit é mitigado ...}
% \sugg{takeways, main findings, insights - TOs, }
% \sugg{Component -> ataque vector}
% \sugg{bullet -> check - unknown}

%We also survey 80 CVE vulnerability reports aiming at understanding the number of attacks \project could prevent. 

Lastly, we aim to study how deploying \project in real-world systems could help 
mitigate privilege escalation attacks resulting from the exploitation of vulnerabilities located in TEEs. %various secure world components. %In particular, since \project can prevent lateral movement and privilege escalation inside zones, it can then prevent vulnerabilities in one zone from affecting other zones, the normal world, or the secure monitor.
%In particular, we wish to study the potential opportunities for compromising real-world TA or trusted OSes, leading to the privilege escalation indicated by steps 1 and 2 in Figure~\ref{fig:intro_rezone}.

As part of this study, we analyze a database of TEE-related CVEs provided by Cerdeira et al.~\cite{Cerdeira2020}. We have analyzed all 80 CVEs reported as critical and grouped them according to the affected component: trusted OS (TO), trusted application (TA), cryptographic implementation (CI), hardware issue (HW), and bootloader (BL). CVEs %Vulnerabilities that affect the TEE but 
that do not clearly identify the vulnerable component (i.e., trusted OS or TA) are labeled as TO/TA. %We consider a \project deployment where there is a trusted OS per TA (e.g., a library OS). %Note that, even if a vulnerability allows for complete compromise of the trusted functionality (e.g., obtaining pin unlocking data) a vulnerability is still considered mitigate since lateral movement and privilege escalation will not be possible. 
\autoref{tab:security-table} summarizes our analysis. Entries marked as \textit{sandboxed} refer to vulnerabilities that have the potential to be successfully exploited as indicated in Figure~\ref{fig:intro_rezone}, and lead to privilege escalation attacks that can be mitigated by \project. In total, we identified \rev{66} vulnerabilities that \project could help counter successful exploits of these bugs.
%could be used as stepping stone for TEE attacks. By ``zone-boxing'' the affected component, 

%\project can prevent full system compromise of 64 (86.5\%) vulnerability exploits of the analyzed critical vulnerabilities, by preventing vulnerabilities from reaching outside of their dedicate zone.
%Although \project cannot prevent vulnerabilities from occurring in TAs and in trusted OS, cannot protect against system miss-configurations, poor cryptographic implementations or defective bootloaders, 

\input{secure_analysis_table}

\mypara{Trusted OS and TA vulnerabilities.}
%trusted OS and Trusted TA vulnerabilities, are related in that often times a vulnerability in a TA can be leveraged to exploit vulnerabilities and flaws in the trusted OS~\cite{Cerdeira2020}. 
With \project, most analyzed vulnerabilities in the trusted OS and TAs can be sandboxed, i.e., cannot be used in privilege escalation attacks that target the normal world, the secure monitor, or other TAs. 
Notwithstanding, in some cases the attacker may be driven by a different goal. %'s goal is not necessarily to further escalate its privileges beyond the perimeter of the compromised TA itself. 
For instance, \cve{2018-5210} describes a vulnerability that allows an attacker to gain TEE privilege execution, which leads to retrieving device unlocking information at the TA level. This can then be used to obtain the device unlocking code. We consider this vulnerability sandboxed because an attacker cannot affect other system components. 
A second example is \cve{2017-18311}: a misconfiguration vulnerability where a custom implementation of a TrustZone controller allows other masters to escalate privileges. \project would not prevent this attack. However, our system could be extended to consider other bus masters in protecting normal and secure world software, considering the platform's PPC is flexible enough to do so.

\mypara{Other vulnerabilities.} 
\rev{
%\cve{2018-11950} pertains to the loading of unauthorized TAs into the TEE. We consider this vulnerability out of scope because \project does not interfere with TA loading process. However malicious TAs could compromise the security of the system, for example by having access to privileged system calls, and in that case the flaw is sandboxed. \david{sandboxed or not?}
\cve{2015-9199} is related to the dynamically marking memory as secure. In \project this functionally would only affect the established shared memory regions, thus this CVE does not apply to a \project enabled system. 
In \cve{2017-18310} a TA exposes too many services to the normal world, which may allow the normal world perform actions it shouldn't be able to. \project cannot control which operations are available to the normal world. 
\cve{2017-18128} is an issue with the configuration of an hardware component that can expose secret information. \project does not prevent the secure world from exposing secrets to other system entities (e.g., the normal world).
}
\cve{2017-18282} is a hardware issue where a hardware component can be manipulated by a malicious agent from the normal world into performing secure data accesses. These types of issues are not prevented by \project, as we only protect against secure accesses while the trusted OS is executing.
Cryptographic-related vulnerabilities such as \cve{2017-14911} are out of scope. \project relies on the correct implementation of cryptographic primitives and schemes. Bootloader-related vulnerabilities, \cve{2016-10458} for example, are also out of scope. \project relies on the platform's secure boot to correctly initialize the system.


%The bootloading stage occurs before the secure monitor starts execution. At this stage the CPU executes in the secure world and flaws at this point may enable attackers to load arbitrary code at the highest privilege level. We consider these types of problems out of the scope of \project as the mechanism used to load the runtime TCB are the root of all trust in the system.


%\mypara{2016-2431} This vulnerability refers to a lack of system calls parameter validation on the trusted OS. It assumes code execution privileges in a TA, and enables attackers to build read and write gadgets to the trusted OS. This vulnerability fits the attack scenario where an attacker gains trusted OS level privileges. With trusted OS level of privileges an attacker can access any memory and every resource available to the CPU. Although \project does not address the vulnerability directly is prevents a compromised trusted OS from attacking the normal world and the secure monitor, thus reducing the impact of this vulnerability.


% \sugg{TODO: escolher 4 ou 5 vulnerabilidades}
\if0
2016-2431	"The Qualcomm TrustZone component in Android before 2016-05-01 on Nexus 5, Nexus 6, Nexus 7 (2013), and Android One devices allows attackers to gain privileges via a crafted application, aka internal bug 249688009.

This vulnerability assumes code execution privileges in QSEE TA.
TrustZone kernel does not perform any validation on QSEE-supplied arguments (more specifically, it freely uses any given pointers), meaning that at the time all syscalls were vulnerable. Vulnerable syscalls allow for building read and write gadgets to the trusted OS.
"


2017-17176	The hardware security module of Mate 9 and Mate 9 Pro Huawei smart phones with the versions earlier before MHA-AL00BC00B156, versions earlier before MHA-CL00BC00B156, versions earlier before MHA-DL00BC00B156, versions earlier before MHA-TL00BC00B156, versions earlier before LON-AL00BC00B156, versions earlier before LON-CL00BC00B156, versions earlier before LON-DL00BC00B156, versions earlier before LON-TL00BC00B156 has a arbitrary memory read/write vulnerability due to the input parameters validation. An attacker with the root privilege of the Android system could exploit this vulnerability to read and write memory data anywhere or execute arbitrary code in the TrustZone.


2017-6294	"In Android before the 2018-06-05 security patch level, NVIDIA Tegra X1 TZ contains a possible out of bounds write due to missing bounds check which could lead to escalation of privilege from the kernel to the TZ. User interaction is not needed for exploitation. This issue is rated as high. Version: N/A. Android: A-69316825. Reference: N-CVE-2017-6294. 

NVIDIA TLK TrustZone OS contains a potential vulnerability in the logging driver where the software writes data after the end or before the beginning of the intended buffer, which may lead to arbitrary code execution, denial of service, or escalation of privileges. - buffer overflow may lead to arbitray code execution within the TEE"


2015-4422	"The TEEOS module of Huawei Mate 7 smartphone which is used to realize the function of fingerprint identification has an input check error, which enables the attackers with the root permission to modify kernel-mode memory data of TEEOS module, which could make system break down, TEEOS be tampered or malicious code execution. (Vulnerability ID: HWPSIRT-2015-03012)

There is a arbitrary memory read/write vulnerability in the hardware security module of some Huawei smart phones due to the input parameters validation. An attacker with the root privilege of the Android system could exploit this vulnerability to read and write memory data anywhere or execute arbitrary code in the TrustZone. (Vulnerability ID: HWPSIRT-2017-01060)
http://www.huawei.com/en/psirt/security-advisories/huawei-sa-20170306-01-smartphone-en - An attacker can write arbitrary code to TEE global task memory, this allows him to obtain execution wiithin the global task by provoking a crash and forcing code execution to an attacker controlled address
 - a system call vulnerability allows an attacker to arbitrarily write to any memory address within the TEE, which allows him for example to bypass security checks for accessing fingerprint images

Security Advisory - Arbitrary Memory Read Write Vulnerability in Huawei Smart Phones
"
\fi

\if0

\subsection{Attack Surface}
%\sugg{Mitigations are also attack surface}

The attack surface for a typical TrustZone assisted TEE system includes all the SMCs and interfaces the secure monitor, trusted OS and Trusted Applications provide to the normal world.

Attack surface becomes:
\begin{itemize}
    \item Guessing the authentication token
    \item Connection with the micro-controller
    \item SMC calls (calls to the monitor)
    \item Interfaces TAs provide
    \item trusted OS syscalls
\end{itemize}

\fi

\subsection{Security Analysis}\label{sec:sec_analysis}
\rev{TrustZone-based TEEs have been the target of multiples attacks, which exploit software flaws to obtain privileged execution, extract secrets, or twarth security functionality. In \project we propose to achieve three main security properties: (P1) monitor protection, (P2) normal world protection, (P3) allow for multiple TEEs. These properties are \project's invariants, and in this section we address how they are upheld by our implementation, and how the invariants themselves minimize the impact of attacks.}

\mypara{Monitor Protection (P1)} \rev{In deployments before Armv8.4 or without S-EL2, the trusted OS has full access to all resources including the secure monitor code and memory regions. This allows a malicious Trusted OS to compromise the monitor, the highest privilege code in the system. Protection of monitor memory is achieved by marking most of monitor memory as inaccessible leaving accessible only a small region of code, to allow for safely switching in and out of Trusted OS execution. Additionally due to the limitations of using a core external control mechanisms, to prevent TEE from accessing normal world memory we must suspend all co-located cluster cores when executing a TEE.}

\mypara{Normal World Protection (P2)} \rev{In typical deployments, the Trusted OS has full access to the normal world memory. By guaranteeing that S-EL1 cannot access normal world memory with the exception of explicitly assigned shared memory, a malicious Trusted OS cannot directly compromise the normal world software. In \project only resources that a TEE can access are made available to each TEE. For the same reasons mentioned in P1, it is necessary to suspend all co-located cluster cores, while the TEE is executing.}

\mypara{Multiple TEEs (P3)} \rev{Allowing for multiple TEEs enables use cases where TAs can trust less in each other, specially if they are from different developers. This is achieved by running TAs, or groups of TAs, in different TEEs. This is important because malicious TAs can escalate privileges and attack other TAs within the TEE. Creating multiple TEEs is achieved by allowing access to resource of a particular TEE to only that specific TEE. Thus, different TEEs cannot access each-other's resources and are hence protected from each other's attacks.}
\newline

\rev{We next analyze how three representative real-world attacks would fare in a system deployed with \project.}

\mypara{Attack 1.} \rev{An attacker compromises a system TA through the trusted OS, by first obtaining execution privileges in the trusted OS~\cite{BreakFDE,shen-trustedcore}. This can be used to thwart security functionality. For example, an attacker can obtain the secret key used to encrypt the file system~\cite{BreakFDE} or effectively compromise the fingerprint authentication mechanism~\cite{shen-trustedcore}.
%The secret key is encrypted by the user password, however it is possible to bruteforce the password on a powerful PC.
%
Because \project allows for the secure deployment of multiple OSes, it is possible to prevent a compromised component from zone$_{1}$ from directly obtaining secrets from other zones. Securely developing zone$_{1}$ is easier than doing the some for a single TEE domain hosting all TAs. Thus, by using \project to allow more than one TEE to execute in the secure world, a vulnerability in one zone can not be used to obtain secrets from another.}
 
\mypara{Attack 2.} \rev{By leveraging a TA's access to normal world memory, it is possible to access all memory in the normal world~\cite{gb-exploit6, Aravind2017}. This is possible because the trusted OS can map the normal world physical memory at will, and in certain scenarios can map this memory unto a TAs address space. With access to normal world memory an attacker can compromise the Linux kernel, for example by creating a back door within seldom used kernel modules. This gives the attacker arbitrary code execution at kernel level of privilege. 
%
In \project we restrict the normal world memory accessible to a trusted OS, and only allow predetermined memory regions to be used as shared memory. This requires knowledge of what memory is dedicated for sharing memory between the TEE and REE. This prevents an attacker in the TEE from compromising the normal world, as it can no longer access its code or memory regions.
%Fixing the shared memory space makes it possible for secure monitor to enforce secure-world zones. This comes at the cost of not being able to use dynamic shared memory which in certain scenarios can reduce performance due to forcing additional copies of memory.
}

\mypara{Attack 3.} \rev{An attacker can highjacking the control flow of a Trusted OS to compromise it~\cite{gb-exploit4}. In particular the attacker might leverage the presence of privileged operations, for example in the case for Armv7-A or Armv8-A\_aarch32 the DACR registers, which when set to zero disable MMU based memory protection.
%
In \project, we use platform-level access control mechanisms to enforce zone access permissions to memory. Even with access to privileged instructions in the trusted OS, an attacker can not modified these policies, and is thus still confined to the specified zone. This ensures that even a fully compromised trusted OS cannot access resources other than ones that it was explicitly allowed to access.}

%=======================================================================
%> [Comparison with other systems]
%=======================================================================
\section{\project in Perspective}
\subsection{\project and Related Systems}
\rev{To compare \project with other works, we've selected the works that more closely relate to ours and compare them in terms of relative performance to typical TrustZone deployment, programming overheads, scalability and TCB, see \autoref{tab:sys_comparison}. vTZ~\cite{Hua2017}, OSP~\cite{Cho2016}, and PrivateZone~\cite{Jang2018} leverage the virtualization extensions available in the normal world (NS.EL2) to create isolated environments, with vTZ running full-fledged trustedOSes in the normal world, while OSP and PrivateZone run their own runtime environment for each application.
TrustICE~\cite{Sun2015} and Sanctuary~\cite{Brasser2019} leverage the TZASC to create enclaves within the normal world. Enclaves are isolated and cannot access the REE, but the trusted OS running in the secure world still has full access to the system.
TEEv~\cite{Li2019} and PrOS~\cite{Kwon19} use same privilege isolation to secure a minimalist hypervisor from trustedOSes, due to the lack of hardware virtualization support in the secure world before Armv8.4-A. TEEv proposes an architecture where there's a more privilege TEE that manages the most critical resources such as trusted hardware are cryptographic keys. Both these solutions, and vTZ, rely on binary instrumentation for removing privilege memory management instructions.}

\mypara{Performance}
\rev{To compare performance overheads we select a real world use case presented in each system, as this is more indicative of the real impact each solution. By not providing a comparison between a workload implemented for both their proposed architecture and a typical scenario, PrivateZone~\cite{Jang2018}, Sanctuary~\cite{Brasser2019} and TrustICE~\cite{Sun2015} don't provide sufficient information to perform this analysis. Keep in mind that the implemented applications between the system are not the same and this only provides a rough estimate of the relative performance impact of each systems. For PrOS~\cite{Kwon19} we select the bitcoin wallet application, a relatively simple TA. This is the system that achieves the least overheads. The explanation for this is the straightforward implementation of the multiple environments. All TEEs feature the necessary resources to perform their operations, and there's no heavy architectural management operations. For TEEv~\cite{Li2019} we select the AliPay case, as it makes full use of the features they implement, including both the system TEE and another TEE in the workload. TEEv benefits from much of the same implementation aspect as PrOS, however there's a system TEE that manages critical aspect such as finger print hardware and key management. This results in increased number of context switches for the necessary requests to be fulfilled by the system TEE on behalf of other the TEEs.
For OSP~\cite{Cho2016} we selected the results for the encryption application for 100 KB using 4KB chunks. The overheads are explained by the dynamic activation of the hypervisor and related impacts such as TLB misses. For vTZ~\cite{Hua2017} we take the geometric mean of the performance results for four real applications. We select a single guest configuration as this is the most comparable scenario between the considered works. The overheads are caused by the cost of context switching operations which involve vTZ's secure world switching module. For \project we selected the bitcoin wallet application. \project demonstrates the higher performance penalties out of all the analyzed systems. As we've analyzed above, in $\S\ref{sec:eval}$, most overhead is due to the cache-maintenance operations. These operations force data to be written to main memory, and thus are quite slow and translate into higher overheads than other systems, however, as we've shown, user interactivity is not compromised for the workloads we've analyzed.}

\mypara{Programming Overheads}
\rev{
To analyze programming overheads we analyze the required changes for software to be adapted for each system. In all system we analyze if they required modification to the normal world, the Trusted OSes or the Trusted Applications to support each solution. The easiest system to develop for is vTZ~\cite{Hua2017} which does not require changes to both the normal world or the virtualized TrustZone, but may require the development of CIEEs to emulate TrustZone features. PrivateZone~\cite{Jang2018}, OSP~\cite{Cho2016}, Sanctuary~\cite{Brasser2019}, TrustICE~\cite{Sun2015}, and PrOS~\cite{Kwon19} required modification to the normal world kernel to support their respective environments. Additionally, PrivateZone, OSP, and Sanctuary require that applications be specifically developed for their isolated environments, as well. TEEv~\cite{Li2019} requires modifications to the booting process of each Trusted OS they host. \project requires no changes in the normal wold software aside from enabling the necessary TEE drivers (one per TEE instance) and slightly modifying them to conform the new SMC IDs. \project also only requires that TEEs be compiled to specific memory regions, which can be easily configured in configuration makefiles in OP-TEE.}

\mypara{COTS} \rev{From the system we analyzed, only Sanctuary~\cite{Brasser2019} is not deployable in COTS platforms. This is because allowing each core on a cluster to have its own ID requires modifications to the inner-workings of the caches, which the authors achieve by modifying the hardware in an emulator.  Other works leverage software techniques easily applicable in a wide range of platforms, or common hardware mechanisms such as normal world virtualization vTZ~\cite{Hua2017}, PrivateZone~\cite{Jang2018}, OSP~\cite{Cho2016}. To fully protect the environments, additional mechanisms (i.e., SMMU) may be necessary to protect against attacks (e.g., DMA), otherwise software techniques such as those employed by TEEv~\cite{Li2019} (e.g., front-end/back-end driver model) are required. However, because some mobile platforms do not feature SMMUs that can guarantee this isolation (some platforms have bus-master specific SMMUs, and not platform wide SMMUs), we score these systems with \half. \project requires a PPC and an ACU (note that a platform wide SMMU is a PPC) in the platform, thus cannot widely be adopted in COTS. Because of this we score \project with \half\xspace on this dimension. For an analysis on platforms that can support \project, please refer to $\S\ref{sec:PPC_ACU_COTS}$.}

\mypara{Scalability}
\rev{
We next analyze how scalable each system is, in regards to: how many environments or applications can deployed, if it can support multiple environments, and if those environments can be created dynamically.
Typical TZ TEEs feature a single TEE instance. Simultaneous execution of TAs on OPTEE is supported when executed on different cores.
PrivateZone~\cite{Jang2018}, OSP~\cite{Cho2016}, Sanctuary~\cite{Brasser2019}, feature the some overall scalability as they provide mechanisms to create isolated environments for single applications to execute protected from the normal world operating systems. They provide the ability to dynamically load any number of applications one at a time per core. vTZ~\cite{Hua2017} is only restricted by system memory in how many VMs, and vTZs, can be instantiated simultanously, and thus executing in parallel, otherwise TEEs in the vTZ feature the same scalability characteristics as the original TEEs. As for if vTZ supports dynamically creating new environments, we conclude that it can, because it is based on the Xen hypervisor which supports that feature.
TrustICE~\cite{Sun2015} allows for dynamically creating any number of protected applications, however it does not allow any concurrency. This is due to the use of a version of TZASC that cannot distinguish between core IDs. The CPU (even multiple clusters) are subject to the same memory protections and thus only one core can execute while the trusted application is active.
TEEv~\cite{Li2019} implementation is similar to \project in that multiple TEEs are configured at boot-time, however TEEv allows simultaneous execution of vTEEs in different cores. PrOS~\cite{Kwon19}, in regards to concurrency, does not impose restrictions. 
\project can feature multiple TEEs. In our implementation they are configured at boot time, but there are no restrictions limiting the implementation of dynamically instantiated TEEs. \project, however, does not allow the execution of more than one TA per cluster.
}

\mypara{TCB}
\label{sec:eval_tcb}
\rev{In this work we use TCB to mean parts of the system that if compromised/malicious can compromise other parts of the system, for example, by being able to arbitrary read/write memory of the victim component. In \project we are concerned about the TCB from the point of view of both the normal world and monitor; a malicious S-EL1 can attack both.} We measured \project's TCB size and compare it to alternative solutions. To assess the TCB size, we counted the number of source lines of code (SLOC) using the SLOCCount tool. We computed the TCB size of \project and of a vanilla OP-TEE, i.e., the TF-A and OP-TEE kernel. We also calculated the full TCB size of representative systems covering three classes of multi-environment isolation approaches: (i) normal world virtualization (NW-Virt), (ii) normal world enclaves (NW-E), and (iii) secure world same privilege isolation (SW-SPI). To calculate the full TCB size of these systems, we collected information about the TCB from the original papers and added up reference TCB sizes of TF-A or TF-A+OP-TEE kernel.     
%
%\project enables the creation Zones, sandboxes for trusted OSes running in S.EL1. With this, the runtime system TCB is reduced considerably, as a malicious trustedOS can no longer compromise the system.
%
From \autoref{tab:tcb_comparison}, we can draw three main conclusions. Firstly, \project reduces the TCB size of a typical TrustZone-assisted TEE system by 88.2\%, mainly due to the removal of the OP-TEE kernel as part of the TCB. Secondly, \project adds a total of 5345 SLOC to the privileged software, which includes the addition of the trampoline code (1523 SLOC) and the gatekeeper (3,822 SLOC). Although the gatekeeper code may seem large, it is a consequence of leveraging ready-available board support package (BSP) code. A clean-slate assembly implementation would reduce these numbers to a few hundred SLOC. Lastly, \project presents security advantages comparing to related work. For both the NW-Virt and NW-E class of solutions, \project presents a smaller TCB. \rev{The exception is vTZ. vTZ achieves such small TCB by only implementing a small number of features in monitor, thus not relying on ATF. However, vTZ target use case is server deployment. On mobile platforms, OEMs usually extend the ATF implemention with their own firmware features, thus it would not be realistic to remove ATF from the software stack.} Comparing to TEEv and PrOS, \project also presents non-intuitive security advantages: first, we highlight that a clean-slate implementation of the \project gatekeeper would push the \project TCB reduction to +90\%; second, the numbers presented in \autoref{tab:tcb_comparison} do not account either for (i) the manual engineering effort for removing privilege memory management instructions or (ii) the TCB of binary instrumentation tools used to automate such process (marked with an \textbf{*}); and third, the isolation imposed by \project in the secure world is hardware-enforced. \david{um dos reviewers não ficou convencido que isto era necessáriamente melhor. Para endereçarmos isso a única hipotese que vejo é retirar este último ponto.}

\if 0
\begin{enumerate}[wide, labelindent=0pt]
  \setlength\itemsep{0em}
    \vspace{-0.2cm}
    \item \project reduces the TCB size of a typical TrustZone-assisted TEE system by 88.2\%, mainly due to the removal of the OP-TEE kernel as part of the TCB. \newline
    \vspace{-0.5cm}
    
    \item \project adds a total of 5345 SLOC to the privileged software, which includes the addition of the trampoline code (1523 SLOC) and the gatekeeper (3,822 SLOC). Although the gatekeeper code may seem significantly large for the simplicity of the component, it is a consequence of leveraging ready-available board support package (BSP) code. A clean-slate assembly implementation (which we strive to implement in the future) would reduce these numbers to a few hundred SLOC. \newline
    
    \vspace{-0.5cm}
    \item \project presents security advantages comparing to related work. For both the NW-Virt and NW-E class of solutions, \project presents a smaller TCB. Comparing to TEEv and PrOS, \project also presents non-intuitive security advantages: first, we highlight that a clean-slate implementation of the \project gatekeeper would push the \project TCB reduction to +90\%; second, the numbers represented in \autoref{tab:tcb_comparison} does not account either for (i) the manual engineering effort for removing privilege memory management instructions or (ii) the TCB of binary instrumentation tools used to automate such process (marked with an \textbf{*}); and third, the isolation imposed by \project in the secure world is hardware-enforced.\newline
\end{enumerate}
\fi

% while TW-SIP solutions rely on software
%, which may be not intuitively gathered from \autoref{tab:tcb_comparison}

%, a feature-full open-source TrustedOS, with support for many different platforms, from the TCB. With \project we add 5,345 LoC, spanning both monitor (1523 LoC) and \project controller code (3,822 LoC), when compared against a typical secure monitor deployment. The \project controller large number of LoC is due to our use of readily available board support code, we could optimize the implementation, and due to its simplicity it could be coded in assembly. This would further reduce the TCB as measured in LoC, and make \project controller code formally verifiable.

%We compare \project with similar works that aim to reduce the system TCB, \autoref{tab:tcb_comparison}.
%\project demonstrates significantly reduced TCB as compared to most other works. Comparing to works with similar TCB size, \project makes stronger security guarantees, by not relying on software techniques to establish a sandbox. Instead, \project uses hardware mechanisms to establish zones.

\if10
\input{TableTCBComparison}
\fi

\input{TableResearchComparisonTCB}

%Additional privileged software includes additions to the secure monitor code and other software components; in the case of \project it includes the \project Trampoline and Gatekeeper code.
%NW-Virt: Normal World Virtualization; NW-E: Normal World Enclave; TW-SPI: Trusted World Same Privilege Isolation.
\subsection{\project and S-EL2} \label{sec:sel2}
\rev{
Until now we've talked about \project in the context of TrustZone pre-Armv8.4. Starting from Armv8.4 TrustZone suffered a few changes that we will address in this an the next section. In particular we'll address how these changes do not fully achieve \project guarantees, and how \project can complement the newer Arm CPUs featuring these changes.}


\rev{In Armv8.4 Arm introduced S-EL2. This additional privilege level can be used provide similar security properties to \project's, i.e., the protection of the REE (P2), and monitor (P1) from the trusted OS and multiple isolated trusted OSes support (P3) (see $\S\ref{sec:sec_analysis}$).
While the introduction of S-EL2 seems promising the approach can significantly enlarge the TCB when compared to \project, by requiring yet another privileged software component to manage VMs.
For reference, Hafnium, the reference implementation for the trusted hypervisor, features over XXX LoC.
\project maintains the traditional TrustZone model and only slightly modifies it to achieve its security properties, while only marginally increasing the TCB.}

\rev{Although S-EL2 can be used to implement the same properties as ReZone, the degree to which they are enforced is not the same. In particular, both monitor and the normal world are subject to the trusted hypervisor. With the feature-creep observed in the last few years for Trusted OSes~\cite{}, which resulted in increased TCBs, it would not be unexpected that serious vulnerabilities also affect the new software layer. With a compromised trusted hypervisor an attacker can do the same damage as it could with a compromised trusted OS in previous generations, i.e., it can fully compromise the system. \project can help bring additional security guarantees by effectively providing normal world and monitor protection, against other secure world components, in this case against a malicious trusted hypervisor. This way we argue that \project can complement deployments featuring a trusted hypervisor, especially in use cases requiring improved security guarantees.
%This allows it to maintain a minimal and immutable TCB.
% Arm foresees these to be developed to the highest standards of software engineering to achieve minimal, correct and impervious implementations. However, one cannot completely rely on this, as it was also the initial promise of TrustZone software itself. The evolution of requirements and services will likely bloat both software stacks.
%from all others, in particular, 
%: non-secure/normal, secure, monitor and realm~\cite{armv9realms}.
}

\subsection{\project and Arm CCA}
\rev{In Armv9, Arm introduced the Confidential Computing Architecture (CCA). In CCA, Arm CPUs with realm extensions feature 4 worlds, as opposed to 2 up until this point. The worlds are: root, secure, normal, and realm. 
The root world is dedicated to EL3, the secure world features S-EL2, S-EL1 and S-EL0 privilege levels (the same as before), normal world can be accessed from any other world, and realm world is protected from secure and normal world accesses. Notably, resources belonging to root world cannot be accessed by any other world, a feature that is on par, security wise, with \project's protection of monitor memory from lower privilege levels. This effectively achieves property P1, (see $\S\ref{sec:sec_analysis}$), and it does so to higher degree than S-EL2 alone, due to not depending on a trusted hypervisor. Naturally, Armv9 also achieves property P3, (see $\S\ref{sec:sec_analysis}$), given that the hypervisor can virtualize S-EL1 which allows for multiple TEEs to execute. Additionally, the introduction of the realm world allows for the deployment of TA functionality to this world, minimizing the secure world TCB. Although we consider this an improvement over the previous architectures, Armv9 does not yet fully achieve property P2, (see $\S\ref{sec:sec_analysis}$).}

\rev{
With CCA, as in Armv8.4, the normal world still needs to trust the hypervisor to correctly manage S-EL1 memory mappings. In \project the monitor guarantees that all resources accessible to lower privilege levels must be explicitly be allowed by itself, and thus prevents a malicious S-EL2 from compromising the normal world. To achieve similar properties, in CCA the secure world should not have automatic access to all normal world resources. The access control mechanisms introduced to support the CCA, should feature, in our view, an interface for the normal world to explicitly share memory with the secure world. This would allow the normal world to have control over which resources the secure world can access, and prevent malicious entities in the secure world from compromising the normal world, much like they are prevented from compromising the realm world. 
Otherwise, apart from monitor protection, CCA suffers from much of the same problems discusses above in $\S\ref{sec:sel2}$. We argue that \project can complement these improvements to the Arm architecture, especially in use cases requiring improved security guarantees for the normal world.
%While in this architecture, the secure world is targeted to deploy static security services and firmware, the realm world is meant to host dynamically instantiated realms that contain either full-blown OSes or small TA unikernels.
}


%=======================================================================
%> [DISCUSSION]
%=======================================================================
%\newpage
\section{Discussion}
\label{sec:discussion}


%\st{\mypara{Available hardware to implement \project.}  %To implement \project, we leveraged an OEM-specific platform partition controller, i.e., NXP's RDC. However, in \ref{sec:plat_req},  We have abstractly modeled the PPC so that \project can be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively)~\cite{xilinxisol} while Qualcomm Snapdragon SoCs feature the External Protection Unit (XPU)~\cite{qualcommxpu}. Both fulfill all PPC requirements. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. ACUs are also a clear trend in modern SoCs, which %due to the hardware complexity  tend to include an increasing number of ACUs for power management and security operations~\cite{armscp}.}
\if0
\subsection{Deployment In Other Platforms}\label{sec:otherplat}
\mypara{Xilinx Protection Units.} Xilinx has also developed and included in their Zynq UltraScale+ MPSoC portfolio a set of protection units complementary to TrustZone~\cite{}. The Xilinx memory protection unit (XMPU) and the Xilinx peripheral protection unit (XPPU) are system-level controllers that verify if a particular bus master is explicitly allowed to access a specific address (memories and peripherals). There are a total of eight XMPUs for protecting transactions into the DDR, the OCM, and the interconnect (e.g., SATA and PCIe). There is one XPPU, which allows for protecting peripherals, message buffers, and inter-subsystem communication channels. A master ID list is used to define the masters that are allowed to access peripherals. Similarly to the i.MX8 families, in Zynq UltraScale+ devices the quad Cortex-A53 cluster has the same master ID for all of its cores, making it impossible to use the XMPU and XPPU to create security domains per core.
\fi

%\jose{is it necessary to mention management cores?} \sugg{as we are pressed for space, I dont' think it's worth it really. Maybe say somehting like, platform mangement cores are already present in various platforms to perform, power mangement or serving as a senser hub, In \project we require a dedic/ate security one (qualcomm has one in their latest flagships)}

\mypara{System/OTA updates.}
\project does not impose any limitation or changes in the platform update mechanism. The OEM must provide a secure boot process that allows for the authentication and deployment of secure world software. %During the secure boot, the bootloader will authenticate images and boot the system. The updated binary shall contain updated zone images and an updated resource allocation policy list per zone.

%\mypara{Performance vs. security trade-off.}  %To guarantee the correct sandboxing of zones, \project requires extreme measures, i.e., on a world-switch, a core must flush the full cache hierarchy and halt the other cores from the cluster. As shown in $\S$\ref{sec:eval}, although, at the micro view, there are a non-negligible overhead, from a macro perspective, real-world applications does not impact the user experience. 
%These performance impact might still be further minimized. 
%To further reduce the performance overheads of \project, we propose to explore several ideas. 

%%%\project's mechanisms induce non-negligible overheads and has limitations concerning simultaneous trusted OS calls. Although we consider that this is not a major issue for the standard behaviour of real-world TAs (and the performance overhead results observed in section \ref{sec:eval}),  we believe there is still room for optimizations. 

\if10 %before revision
\mypara{Performance optimizations.} To further reduce \project's performance overheads, there is still room for optimizations. 
For example, \project can benefit from multi-cluster platforms, where one cluster might continue executing in the normal world while the other runs a zone. Also, batching of a zone's invocations would amortize the costs of world-switching. %On the other hand, \project can contain or even fully mitigate critical attacks (see $\S$ \ref{sec:security_analysis}). % In essence, we believe \project is trading a small decrease in performance for huge security benefits. 
%\sugg{On deployments where the same trusted OS is deployed in multiple zones, common memory regions (e.g., OS page tables and code) can be shared between zones.}
\fi

\mypara{Performance optimizations.} \rev{There are two main performance bottlenecks in \project. The first is that the normal world cannot execute while a trusted OS is executing. The only way we can address this is by leveraging multiple clusters in multi-cluster platforms. In this scenario one cluster would continue executing in the normal world while the other would run a zone. 
The second bottleneck is that, frequent calls to a zone that perform little work, will have higher incurred overheads than more spaced out invocations that do more work. With this insight, it is possible to optimize secure world workloads creating a batching mechanism to allow batching of a zone's invocations. This would amortize the costs of world-switching, mostly in cases requiring frequent fast calls.}

%{\color{orange} ... Starting from ArmV8.4, TrustZone features a secure world hypervisor designed to provide different execution environments within the secure world itself, and which will also enable the protection of normal world, and monitor memory. However, platforms featuring the new architecture are not yet widespread, meaning that there is a lack hardware solutions for achieving the goals we propose. Additionally \project can be applied to already existing platforms which meet the necessary hardware requirements as discussed in ($\S$\ref{sec:plat_req}) ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... }

\if10 % Before revision
\mypara{Appropriation of PPC and ACU.}  By using the platform's PPC and ACU to implement \project, one may wonder if this appropriation will not disrupt the functionality of the system in case these components are used for other purposes. From our experience with the i.MX8 platform, \project caused no disruptions to REE/TEE system and applications. As long as the \project security is preserved, PPC and ACU can be shared with other services, e.g., being able to run additional code on the Cortex-M4 (i.e., the ACU), or use a spare security domain in the RDC (i.e., the PPC) for other purposes.
\fi

\mypara{Appropriation of PPC and ACU.} \rev{By using the platform's PPC and ACU to implement \project, one may wonder if this appropriation will not disrupt the functionality of the system in case these components are used for other purposes. As long as the \project security is preserved, PPC and ACU can be shared with other services, e.g., use a spare security domain in the RDC (i.e., the PPC), or being able to run additional code on the Cortex-M4 (i.e., the ACU) for other purposes. In cases where the available ACU performs non-critical work, it is necessary to allow the secure co-existence between the non-critical functionality, and the gatekeeper code. There are multiple ways this could be achieved, from using small operating systems that support hardware enforced isolation such as FreeRTOS, to using software based isolation techniques~\cite{ammar2019s} if it does not. Although this could have some impact on the performance of the ACU, depending on the ACU's workloads, we believe the improved security guarantees to the system as a whole are worth the cost.}


%\sugg{In \project we change the security semantics of the platform, in particular we use secrets to disallow unintended reconfiguration of the PPC, while still allowing the PPC unlocking mechanism to be available to the Trusted OS. To enable this we take advantage of an ACU and a PPC present in our test platform, a Cortex-M4 processor and a RDC from NXP. Our use of these components somewhat limits how they can be used for other purposes. We required the Cortex-M4 to run the gatekeeper code, however this functionality can be implemented alongside other features by means of a embedded OS, for example~\cite{uCOSII, Garlati2020}, at the cost of lowering overall security by increasing the system TCB. A second caveat, is due to our use of the RDC, which poses more significant limitations. We make use of three of the four available domains that are possible to be created by the RDC. Still, it is possible to make use of the forth domain to establish an additional partition at a platform level.}

%\mypara{\project semantics.}  \sugg{In \project we change the security semantics of the platform, in particular we use secrets to disallow unintended reconfiguration of the PPC, while still allowing the PPC unlocking mechanism to be available to the Trusted OS. To enable this we take advantage of an ACU and a PPC present in our test platform, a Cortex-M4 processor and a RDC from NXP. Our use of these components somewhat limits how they can be used for other purposes. We required the Cortex-M4 to run the gatekeeper code, however this functionality can be implemented alongside other features by means of a embedded OS, for example~\cite{uCOSII, Garlati2020}, at the cost of lowering overall security by increasing the system TCB. A second caveat, is due to our use of the RDC, which poses more significant limitations. We make use of three of the four available domains that are possible to be created by the RDC. Still, it is possible to make use of the forth domain to establish an additional partition at a platform level.}

\mypara{PPC and TZASC}
\rev{In \project we still use TZASC to protect the secure world from normal world accesses, as in a typical TrustZone deployment. It would be possible to remove TZASC, however this would required us to perform the same operations we perform to sandbox S-EL1, but now applied to the normal world, and with the added restriction of not being able to execute monitor concurrently with the normal world. Note that without TZASC, CPU accesses cannot be differentiated from secure, and non-secure. Necessary operations include cross core synchronization, cluster suspension, cache maintenance operations, marking memory as unavailable (in this case secure world memory), and turning off the EL3 MMU, before entering the normal world. In summary everything we do to sandbox S-EL1 we would have to do also to sandbox the normal world, the exception being that no TLB maintenance is required given that in \project the normal world is a single execution environment, and thus TLB entries only belong to the normal world. Using TZASC allows ReZone to execute without additional overheads, improving performance, and complementing the security guarantees provided by \project's dynamic memory protection configuration.}

\mypara{\rev{SMMU as a PPC}}
\rev{
We have mentioned above that an SMMU can be used as a PPC. An SMMU is an hardware component that can translate and filter accesses to the system bus. Specifically, this is achieved by translation tables that specify the translation, and access policy properties. One fundamental characteristic of a system that uses the SMMU for this end is that the SMMU must be able to also translate CPU accesses, which is not a given, in particular in system that feature custom SMMUs. Assuming that an SMMU can indeed translate CPU accesses, the process to use it as a PPC in \project is as follows. The trampoline would be responsible for correctly configuring memory accesses, the same as before, however instead of configuring resources by configuring registers and specifying start and end addresses for memory regions, the trampoline would establish translation tables, which can simple translate to the physical address space, and configure the appropriate memory attributes. The ACU would also need to implement some awareness of the page table and its configuration, as it would need to configure the SMMU to always allow the ACU to access the SMMU, and to allow/disallow the CPUs, and other bus masters, from accessing the SMMU (including the page tables). With this primitives in place, the process is the same as before. The trampoline makes an authenticated request to the ACU, and the ACU configures the SMMU to allow the trampoline to configure it as necessary. After, the trampoline will make another request the ACU, which will maintain the configured access policies, and update the translation table to prevent access the SMMU by other system entities.
}

%=======================================================================
%> [RELATED WORK]
%=======================================================================
\section{Related Work}
\label{sec:related}
\david{Sugiro remover destas descriçoes os trabalhos que usamos na comparação, e dizer qualquer coisa como: "Here we present other related works, besides the ones already compared in section 8."}
Several security-oriented hardware architectures provide basic underlying primitives for the creation of TEE systems~\cite{Maene2018, Pinto2019, Cerdeira2020}. These technologies include \textit{CPU extensions}~\cite{Costan2016_2, Pinto2019, Costan2016}, separate \textit{co-processors}~\cite{Tarjei2016, SPU2019}, dedicated \textit{security chips}~\cite{TPM2019}, and \textit{secure virtualization}~\cite{SEV2019, armv9realms}. Recently, academia has been focused in exploring RISC-V to propose novel TEE hardware architectures~\cite{Nasahl2020, Bahmani2021}. In our work, we leverage COTS hardware primitives to provide augmented isolation within the TEE.

% proposes a secure TEE design strategy using a heterogeneous CPU architecture

%TyTAN~\cite{} and TrustLite~\cite{} are preeminent examples of hardware TEE architectures for resource-constrained embedded devices. 

%\par Contextualize TEE hardware with systems... In the following, we describe different approaches aiming at ... 

\mypara{Hardware-enforced TEE systems.} %There are a plethora of augmented TEE systems aiming at offering additional security guarantees. 
%A large body of work aims to improve the security of TEEs.
Komodo~\cite{Ferraiuolo2017} implements a small TEE monitor which provides sealed storage and remote attestation per the SGX specification. 
%TLR~\cite{Santos2014} and TrustShadow~\cite{Guan2017} implement
Lightweight secure world runtimes~\cite{Santos2014,Guan2017} aim at shielding security-critical applications from untrusted OSes. TrustICE~\cite{Sun2015} and Sanctuary~\cite{Brasser2019} leverage the TZASC to create enclaves within the normal world. Enclaves are isolated and cannot access the REE, but the trusted OS has full access to the system. TrustICE has multi-core limitations while Sanctuary depends on features not available in any COTS SoC release to date. 
A distinct line of work, e.g., LTZVisor~\cite{ltzvisor,ltzvisor-amp} and Voilá~\cite{voila}, have leveraged TrustZone hardware to virtualize system resources for a dual OS system configuration while addressing real-time guarantees. \project leverages hardware orthogonal to TrustZone to provide containerization for multiple trusted OSes, while providing the same availability and real-time guarantees as existing TrustZone-assisted TEEs. 
CaSe~\cite{Zhang2016_3} and SecTEE~\cite{Zhao2019} allow TAs to run entirely from the cache and on-chip memory, respectively. Keystone~\cite{Lee2020} and MultiZone~\cite{Garlati2020} leverage standard hardware primitives from the RISC-V ISA, i.e. physical memory protection (PMP), to isolate individual enclaves.  
%CaSe~\cite{Zhang2016_3} ensures that the TA state is encrypted while written back to the main memory. Ginseng~\cite{Yun2019} protects variables tagged as "sensitive", by allocating them on CPU registers and encrypting them before saving in memory.



\mypara{Virtualization-aided TEE systems.}
vTZ~\cite{Hua2017}, OSP~\cite{Cho2016}, and PrivateZone~\cite{Jang2018} leverage the virtualization extensions available in the normal world (NS.EL2) to create isolated environments. These approaches have some drawbacks, e.g., TCB augmentation, performance decrease \david{a reviewer noted that this is not true when compared to ReZone}, and intrusive design. With Armv8.4-A, Arm introduced the secure hypervisor mode (S.EL2) and Hafnium~\cite{hafnium}. Our solution does not rely on any hardware virtualization support and thus can be used in combination with existing hypervisors and legacy systems.
% OSP~\cite{Cho2016} tries to minimize the performance impact by activating the hypervisor on-demand.
%Overshadow~\cite{Xiaoxin2008}, Trustvisor~\cite{mccune2010trustvisor}, and Inktag~\cite{McCune2010} implement hypervisor-based security architectures for Intel and AMD. 
%In the context of TrustZone-based systems, 


\mypara{Same privilege isolation.} Same privilege or \textit{intra-level} isolation~\cite{Yeongpil2017} is a well-established software technique to harden monolithic OSes (e.g., \textit{nested kernel}~\cite{Dautenhahn2015}), hypervisors (e.g., \textit{Nexen}~\cite{Shi2017}), and TEEs~\cite{Li2019, Kwon19}, typically by interposing on all updates to virtual memory translations to assert protections on physical memory. TEEv~\cite{Li2019} and PrOS~\cite{Kwon19} use same privilege isolation to secure a minimalist hypervisor from trusted OSes, due to the lack of hardware virtualization support in the secure world before Armv8.4-A. Both solutions rely on manual engineering effort or binary instrumentation tools for removing privilege memory management instructions. 




%OSP~\cite{Cho2016}: Their work enables TAs to run on the normal world by using an hypervisor. 2 stage translation overheads are mitigated by only activating the hypervisor when TAs need to run. Our work does not require an hypervisor to be dedicated to the TAs, freeing that privilege level for other applications.

%TrustICE~\cite{Sun2015}: Their work enables TAs to run on the normal world by suspending the REE-OS on all cores while the TA is running. Non-running TAs are protected by marking their memory as secure. Biggest disadvantage is suspending the REE-OS to run TAs, our approach does not require this to provide multiple runtime environments.

%Sanctuary~\cite{sun2015trustice}: Their work enables TAs to run on the normal world by taking advantage of non-common platform features and hardware. Their work relies on each CPU core having its own master ID and this ID being used in bus accesses. It is unknown how widely available this feature realy is. For example the platform they use to test it, the hikey960 does not support it. Further it requires the presence of the TZC-400 which enables each core to have a differente view of what is normal-world memory. Wide use of the TZC unlikely. Going by the Arm-Trusted-Firmware repository, very few platforms actually use the TZC. Our solution is deployable to real world platforms.

%TEEv~\cite{Li2019}: Their work does not provide hardware enforced isolation, rather, it relies on same privilege isolation techniques, as such removing privileged instructions. With this they implement an hypervisor in EL1 to run multiple TEEs on the secure world. In our solution we only require trap and emulation techniques to protect the normal world, which is already "vulnerable" today. To protect environments between one another we achieve hardware enforced access control.

%PrOS~\cite{Kwon19}: Their work does not provide invariant isolation properties rather, they make calls to the monitor in a paravirtualizated-fashion. With this they implement an hypervisor in EL3 and are able to run multiple TEEs on sEL1. In our solution we only require trap and emulation techniques to protect the normal world, which is already "vulnerable" today. To protect environments between one another we achieve hardware enforced access control.

%vTZ~\cite{Hua2017}: Their work provides a TEE environment for each virtual machine, with aid of an hypervisor. They do this by emulating TrustZone features in software.




%=======================================================================	
%> [CONC]
%=======================================================================
\section{Conclusion}
\label{sec:conclusion}

With \project, we present a new security architecture that can reduce the privileges of a TrustZone-assisted TEE by leveraging hardware primitives available in modern hardware platforms. We have implemented and evaluated \project for the i.MX 8MQuad EVK and the results demonstrated that the performance of applications such as DRM is not significantly affected. We have also surveyed 80 CVE reports and estimate that \project could help mitigate 88\% of them.

%to restrict the privileges of the trusted OS
%creating sandboxed domains (\textit{zones}) inside the secure world. The key idea behind the \project design relies on

% %-------------------------------------------------------------------------------
% \section*{Acknowledgments}
% %-------------------------------------------------------------------------------
% 
% %We thank... David Cerdeira was supported by FCT grant SFRH/BD/146231/2019. - Algoritmi project reference: UIDB/00319/2020 -
% The USENIX latex style is old and very tired, which is why there's no \textbackslash{}acks command for you to use when acknowledging. Sorry.
% 
% %-------------------------------------------------------------------------------
% \section*{Availability}
% %-------------------------------------------------------------------------------
% 
% USENIX program committees give extra points to submissions that are backed by artifacts that are publicly available. If you made your code or data available, it's worth mentioning this fact in a dedicated section.
% 
% %-------------------------------------------------------------------------------
\newpage
\bibliographystyle{plain}
\bibliography{references.bib}

%\newpage
\section*{Appendix}

Figures \ref{img:appdx_1} to \ref{img:appdx_7} provide a fine-grain view of the results collected from the xtest suite. 

%... detail the overhead for each xtest test we execute to evaluate \project. Again, we advise the reader to not take this results at face value, as only the benchmark tests are intended to serve as benchmark. However the tests are useful in that they provide a diverse range of behaviors and workloads, and by analyzing them, they shed light on the impact of \project on various scenarios.

\label{sec:appdx}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/chart.pdf}
    \caption{OS core features xtest tests}
    \label{img:appdx_1}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/chart2.pdf}
    \caption{Network socket, key derivation and mbed TLS xtest tests}
     \label{img:appdx_2}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/chart4.pdf}
    \caption{Cryptographic algorithm xtest tests}
     \label{img:appdx_3}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/chart41.pdf}
    \caption{TEE Internal Arithmetic API, and Global Platform API xtest tests}
     \label{img:appdx_4}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/chart6.pdf}
    \caption{Storage xtest tests}
     \label{img:appdx_5}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/chart7.pdf}
    \caption{Shared memory xtest tests}
     \label{img:appdx_6}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.4]{images/chart_per_group/b.pdf}
    \caption{xtest benchmark suite}
     \label{img:appdx_7}
%\vspace{16.3cm}
\end{figure}



==> backups/main_body-23-jul.tex <==
%=======================================================================
%> [INTRO]
%=======================================================================	
\section{Introduction}

Arm TrustZone~\cite{Pinto2019} is a technology embedded into Arm processors. It is presently found in millions of mobile phones and low-end devices equipped with application processors, such as car infotainment systems and SmartTVs. Vendors and OEMs rely on TrustZone for deploying Trusted Execution Environments (TEEs), which protect the execution of sensitive programs named Trusted Applications (TAs). Some TAs implement kernel-level services of the operating system (OS); for example, Android OS is backed by dedicated TAs for user authentication purposes, key management, or file disk encryption~\cite{androidwhitepaper}. Other TAs implement user-level functionality that can be shared by several applications, e.g., DRM media decoders~\cite{TZVideoPath}, or online banking services~\cite{trustonicBanking}. TEEs themselves are rooted on TrustZone, and consist of a trusted software stack offering API and runtime support for the execution of TAs. TEEs such as OP-TEE and Qualcomm's QSEE ensure that the memory state of TAs cannot be inspected or tampered with by a potentially compromised OS (e.g., through a rootkit), thus offering strong confidentiality and integrity protections.

To protect the TAs, TEEs leverage central abstractions and hardware mechanisms provided by TrustZone. In Armv8-A, TrustZone provides two execution environments named \textit{normal world} and \textit{trusted world}\footnote{Normal and trusted world are also known as normal and secure world, respectively~\cite{Pinto2019}; we adopt the most recent terminology by Arm~\cite{tzarmv8a}.}. The normal world runs a rich software stack often named Rich Execution Environment (REE) comprised of full blown OS and applications; it is generally considered untrusted. The trusted world runs a smaller software stack consisting of TEE and TAs. TrustZone enforces system-wide isolation between worlds and provides controlled entry-points for world switching operations whenever the REE invokes services of TAs. In the Arm architecture, normal and trusted worlds map onto security states: \textit{non-secure} and \textit{secure}, respectively. At any given point in time, the processor runs in one of these states. Importantly, there are two physical address spaces -- \textit{non-secure} and \textit{secure} -- ensuring that software in non-secure state can only see non-secure resources (e.g., memory), but never secure resources. TEEs use this mechanism to shield the memory regions in the trusted world (including TAs' memory) from an untrusted OS running in normal world.

However, an important limitation of TrustZone is its lack of defenses against certain attacks to critical TEE components. To explain the nature and severity of these attacks, we depict the internals of a typical TEE stack in Figure~\ref{fig:intro_trustzone}. The TEE itself consists of two components: \textit{secure monitor} and \textit{trusted OS}. The secure monitor runs in EL3 -- i.e., the exception level granting highest system privileges -- and provides essential mechanisms for world switching and platform management. The trusted OS runs in S-EL1 -- i.e., kernel mode -- and implements memory management,  scheduling, IPC, and common services for TAs. TAs run in S-EL0 -- i.e., user mode -- and run with the least privileges of all. TAs are directly exposed to malicious requests coming from applications running in the normal world. If a TA gets hijacked as a result of exploiting a software vulnerability (1), the attacker can control that TA and even leak its secrets, but because the TA runs with S-EL0 privileges, the attacker will be restricted to accessing the memory address space of that particular TA, and to interfacing with the trusted OS through local system calls. However, if the attacker can further hijack the trusted OS by exploiting another vulnerability (2), he can immediately gain full control of the system, including: the REE in the normal world (a), all the TAs (b), and the secure monitor (c). This level of control is possible because S-EL1 gives full permission to access and reconfigure both secure and non-secure memory regions.

Unfortunately, many devices today face serious risks of being compromised by attacks of this nature. In the past, security researchers have demonstrated how these attacks can be mounted as described above, escalating privileges from N-EL0 into S-EL1 by chaining two exploits: first, targeting a vulnerable DRM TA~\cite{gb-exploit4}, and then a vulnerability in the system call interface of the trusted OS~\cite{gb-exploit5}. Once in control of the trusted OS, it was possible to install a backdoor in Linux kernel (a), retrieve decryption keys from Android's KeyMaster (b), or disable trusted boot protections (c). Notably, recent studies~\cite{Cerdeira2020} have shown that commercial TEE systems have numerous and serious vulnerabilities, most of them affecting user-level TAs and trusted OS software. This suggests that the current attack surface for TEE systems is seriously enlarged.

Despite the abundant research on TrustZone security~\cite{Pinto2019,Cerdeira2020}, not many systems can offer practical defenses when the trusted OS has been compromised. In one line of work, we find TEE systems like Sanctuary~\cite{Brasser2019} and others~\cite{Sun2015,Lee2020} that aim to reduce the attack surface of the trusted OS by relocating TAs onto user-level enclaves in the normal world. However, due to portability reasons, vendors and OEMs continue deploying TAs in commercially available TEEs, therefore exposing many devices to potential attacks. Another approach is to confine individual TEE stacks inside trusted world sandboxes, e.g., by leveraging a hardware virtualization~\cite{hafnium} or same-privilege isolation~\cite{Kwon19,Li2019}. However, although these sandboxing techniques can prevent a compromised trusted OS from further escalating privileges beyond its sandbox, they tend to depend on sizeable trusted computing bases, which may include a hypervisor or a binary instrumentation tool, respectively.

This paper presents \project, a new security architecture that can effectively counter ongoing privilege escalation attacks by reducing the privileges of a potentially compromised trusted OS. This is achieved by creating sandboxed domains named \textit{zones} inside the trusted world. Zones have access only to private memory regions, and provide an execution environment for untrusted S-EL1/S-EL0 code, i.e., trusted OS and TAs, respectively. \project restricts the memory access privileges of the code running inside a zone, preventing it from arbitrarily accessing memory allocated for: (a) the normal world REE, (b) other zones, and (c) the secure monitor. The only way for a given zone to communicate with an external memory protection domain is through mutually shared memory regions. With \project, a typical monolithic TEE can then be restructured and partitioned into multiple zones. For instance, Figure~\ref{fig:intro_rezone} depicts a setup featuring two zones -- U and Z -- each of them runs a trusted OS instance as in a libOS. Then, user-level TAs and kernel-level TAs run in independent zones. With this configuration, an attacker hijacking the trusted OS in zone U (as explained in Figure~\ref{fig:intro_trustzone}), will not be able to further escalate its privileges beyond its sandbox. To give vendors and OEMs maximal flexibility, \project allows the creation of additional zones, and using different trusted OSes inside different zones.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/intro-trustzone.pdf}
    \vspace{-0.2cm}
    \caption{Privilege escalation attack in a TrustZone-assisted TEE: (1) hijack a user-level TA, e.g., exploiting vulnerability in the Widevine TA (CVE-2015-6639)~\cite{gb-exploit4}, (2) hijack the trusted OS, e.g., exploiting vulnerability in syscall interface of Qualcomm's QSEOS (CVE-2016-2431)~\cite{gb-exploit5}. Once in control of the trusted OS, other attacks can be launched: (a) control the rich OS, e.g., by deploying a backdoor in the Linux kernel~\cite{gb-exploit6}, (b) control a kernel-level TA, e.g., to extract full disk encryption keys of Android's KeyMaster service~\cite{gb-keymaster}, or (c) control the secure monitor, e.g., to unblock the device bootloader~\cite{gb-bootloader}.}
    \label{fig:intro_trustzone}
%    \vspace{-0.2cm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/intro-rezone.pdf}
    \caption{\project setup enforcing TEE privilege reduction: after compromising user-level TA$_\textrm{U}$ and trusted OS in Zone U, an attacker cannot escalate privileges to (a) rich OS, (b) kernel-level TA$_\textrm{K}$ in Zone K, or (c) secure monitor.}
    \vspace{-0.2cm}
    \label{fig:intro_rezone}
    \vspace{-0.3cm}
\end{figure}

A central novelty of \project's design is that we take advantage of a TrustZone-agnostic address space controller available in modern platforms to restrict the privileges of S-EL1 (trusted OS) code. Existing systems such as Sanctuary~\cite{Brasser2019} have already leveraged a TrustZone address space controller named TZASC for protecting user-level enclaves in the normal world. TZASC controllers, such as the TZC-400, feature the possibility to specify access permissions to various physical memory regions, including the ability to prevent trusted world code from accessing normal world memory. However, these configurations can be reverted by S-EL1 code, rendering the TZASC ineffective for enforcing zone isolation. Instead, we use a TrustZone-agnostic address space controller that can allow only a specific bus master to reconfigure memory access permissions. An example of such a controller is the RDC, existing in iMX8MQ and iMX8QM boards. In \project, we harness this feature and reserve a low-end micro-controller available in the SoC to be exclusively responsible for setting these permissions, e.g., specifying the private memory regions of each zone. Given that the platform's main cores cannot override these permissions (not even when running in S-EL1), RDC and micro-controller can then be used as building blocks for restricting the memory access privileges of (a potentially compromised) trusted OS, and enforce strong zone isolation.

Based on this insight, we have built \project. Our system includes multiple non-trivial optimizations and mechanisms to manage the life-cycle of zones and guarantee system-wide security (e.g., avoiding cache-based data leaks). To make our design generally applicable to various hardware platforms, we specify the general properties of TrustZone-agnostic address space controllers that satisfy \project's requirements. We have fully implemented \project for the i.MX 8MQuad EVK, and integrated it with Android OS as REE and with OP-TEE as TEE. Our code will be made available open source.

We extensively evaluated \project using microbenchmarks and real-world applications. Our evaluation results show that despite the existence of non-negligible performance overheads in the microbenchmarks' programs, \project does not sensibly degrade the performance of real-world applications such as crypto wallets or DRM media decoders. Our DRM application, which requires frequent transitions between normal world and the enclosing zone, preserves its ability to replay video at high frame rates. The overall performance of the system is not affected. We have also surveyed Y CVE vulnerability reports and estimate that \project can thwart Z\% of potential privilege escalation attacks arising from from exploiting these bugs.

%% NS: BACKUP

%To begin their attack on the secure world, an attacker may start compromise a TA first. There are numerous reports on vulnerabilities in TAs (e.g.,~\cite{gb-exploit4}). These attacks depend on the software quality of the TAs, and as history tells us: writing bug free software is hard. After compromising a TA an attacker may try to compromise the Trusted OS, or the Trusted OS itself may have some vulnerability that may be exploited without exploiting a TA~\cite{shen-trustedcore}, and he may be successful. At this point, an attacker is in a high privileged position, as they can access any resource in the system. If not available to them until now, an attacker may create a backdoor in the normal-world kernel~\cite{gb-exploit6}. It's also possible to compromise TAs from the Trusted OS kernel~\cite{BreakFDE}. Additionally, an attacker may even compromise the secure monitor~\cite{DeepDive} giving them full control of the platform.

%Flow of attacks on TrustZone-based systems. Boomerang~\cite{Aravind2017}, QSEE Privilege Escalation and Exploit~\cite{gb-exploit4}, Exploiting TrustZone on Android~\cite{shen-trustedcore}, Breaking Android Full Disk Encryption~\cite{BreakFDE},  Hijacking the Linux Kernel from QSEE~\cite{gb-exploit6}, EL3 tour~\cite{EL3Tour}, A Deep Dive Into Samsung's TrustZone (Part 3)~\cite{DeepDive}, Breaking Samsung's Arm TrustZone~\cite{BreakingArmTZ}.

%=======================================================================
%> [BACKGROUND]
%=======================================================================	
\section{Background}

\subsection{Standard TrustZone Security Mechanisms}

We focus on TrustZone extensions for Armv7-A/Armv8-A architectures. TrustZone enables CPU cores to operate in one of two states: \textit{secure} and \textit{non-secure}. At exception levels EL0, EL1, and EL2, a processor core can execute in either of these states. For instance, the processor is in non-secure exception level 1 (N.EL1) when running REE kernel code, and in secure EL1 (S.EL1) for executing the trusted OS. The security state is controlled by the \texttt{SCR\_EL3.NS} bit in the processor. Regardless of the value of \texttt{SCR\_EL3.NS}, EL3 is always in secure state. To change security states, the execution must pass through EL3.

TrustZone extends the memory system by means of an additional bit called NS bit that accompanies the address of memory and peripherals (see Figure~\ref{fig:RZ_HW}). This additional bit gives independent physical address spaces for the normal world and for the secure world. Software running in the normal world can only make \textit{non-secure accesses} to physical memory because the core always sets the NS bit to 1 in any memory transaction generated by the normal world. Software running in the secure world usually makes only \textit{secure accesses} (i.e., NS=0), but can also make non-secure accesses (NS=1) for specific memory mappings using the NS flags in its page table entries. The processor maintains separate virtual address spaces for the secure and non-secure states. For instance, it does not use a NS.EL1 translation while in secure state, or a S.EL1 translation while in non-secure state. The page table entries contain an NS bit that allow the trusted OS (or the secure monitor) to map virtual addresses to non-secure physical addresses by setting NS to 1. In non-secure state, that bit is ignored: the virtual address will always be translated to non-secure physical address (NS=0). The NS bit of the translated physical memory address is propagated onto the data cache tags. Trying to perform a non-secure access to cached data marked as secure causes a cache miss. Accessing cached non-secure or secure memory in secure state causes a hit.

TrustZone-aware memory and address space controllers are usually configured to map non-secure/secure physical address spaces to different physical memory regions. Typically, the non-secure address space is mapped to a subset of the existing physical memory. In contrast, the secure address space covers the entire existing physical memory, including the regions that are mapped to non-secure address space. In the Arm architecture, the TZASC enforces physical memory protection by allowing the partitioning of external memory on secure and non-secure regions. To date, Arm has publicly released two TZASC specifications, i.e., the Arm CoreLink TZC-380 and TZC-400. Both controllers share similar high-level features, i.e., the ability to configure the security access permissions for memory regions (contiguous areas in the address space).

\subsection{The Excess of Privileges of the Trusted OS}
\label{sec:challenge}

The TrustZone mechanisms described above were designed under the assumption that the S.EL1 (trusted OS) and EL3 (secure monitor) are trusted. However, if the trusted OS is hijacked, the attacks described Figure~\ref{fig:intro_trustzone} can be trivially mounted. For illustration purposes, suppose that the physical memory addresses PA$_\textrm{OS}$, PA$_\textrm{TK}$, and PA$_\textrm{SM}$ are allocated to rich OS, TA$_\textrm{K}$, and secure monitor, respectively. The attacker could mount said attacks by creating virtual address mappings in the S.EL1 page tables as indicated bellow, and use the virtual addresses VA$_i$ to access (read/write) the memory pages of the rich OS, TA$_\textrm{K}$, or secure monitor. Notation VA$\rightarrow\langle$PA, NS$\rangle$ denotes a page table entry translating virtual address VA to the physical address PA and associated NS bit value:

\noindent VA$_\textrm{OS}\rightarrow\langle$PA$_\textrm{OS}$, 1$\rangle$, VA$_\textrm{TK}\rightarrow\langle$PA$_\textrm{TK}$, 0$\rangle$, VA$_\textrm{SM}\rightarrow\langle$PA$_\textrm{SM}$, 0$\rangle$

Preventing these memory accesses by reducing the privileges of S.EL1 code is currently not possible using standard TrustZone mechanisms. Even though TZASC controllers such as TZC-380 and TZC-400 include the ability to prevent secure accesses from accessing non-secure physical memory regions, trusted OSes can map memory as normal (VA$_\textrm{OS}$), enabling them to perform normal world accesses from secure world. Moreover, since S.EL1 software has the privilege to reconfigure the TZASC, the trusted OS can always override any permissions that might have been set by the secure monitor for blocking the trusted OS's access to certain memory regions. Access to the secure monitor (VA$_\textrm{SM}$) and TAs (VA$_\textrm{TK}$) can also not be restricted. In Armv7-A/Armv8-A, trusted OS and secure monitor enjoy the highest privileges with regard to read-write operations over secure and non-secure memory.


\subsection{Platform Model for Sandboxing the Trusted OS}\label{sec:plat_req}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/rezone-hw.pdf}
    \caption{Hardware platform featuring TrustZone: \project-enabling hardware components are highlighted. These are the PMC and the PPC. PPC is configured by the bus-master MID$_\textrm{1}$ (i.e., the PMC). These configurations are written in MMIO regions of the PPC, and determine which access permissions are granted to a given MID for a specific physical memory region.}
    \label{fig:RZ_HW}
    \vspace{-0.2cm}
\end{figure}

Given the limitations of vanilla TrustZone mechanisms, we propose to leverage complementary, TrustZone-agnostic hardware features available in modern platforms for preventing illegal memory accesses potentially performed by untrusted S.EL1 code. These features consist of three hardware primitives that we require to be offered by the underlying platform. These primitives are currently available, e.g., on iMX8MQ and iMX8QM boards, and we use them for building \project.

\begin{enumerate}[wide=0pt]
\item \vspace{3pt} \textbf{Platform partition controller (PPC):} Consists of a memory and peripheral protection controller that can restrict physical accesses to given resource, i.e., memory or peripheral (see Figure~\ref{fig:RZ_HW}). On the iMX8MQ board, the PPC is implemented by the RDC peripheral. We characterize the PPC by having four main properties. It must be capable of: (a) intercepting all physical requests regardless of the NS bit signal injected into the system bus and the configurations of the TZASC, (b) setting fine-grained access control attributes (e.g., RO, RW) for configurable memory regions; (c) differentiating between multiple bus-masters, and (d) protecting memory-mapped input/output (MMIO) regions, including the PPC's own memory-mapped registers. Property (a) ensures that we can block arbitrary memory accesses from S.EL3 without the concern of being overridden by the TZASC, and (b) gives us flexibility to configure access permissions differently for various memory regions. Properties (c) and (d) allow us to restrict which bus-masters are authorized for changing the configurations of the PPC. Importantly, this feature help us to ensure that the PPC's configurations cannot be arbitrarily changed by (untrusted) S.EL1 code executed by the processor. Intuitively, to provide this guarantee in the setup illustrated in Figure~\ref{fig:RZ_HW}, the PPC would not allow the bus master identified with MID$_\textrm{0}$ -- i.e., the processor cluster -- to arbitrarily change the PPC configurations. Instead, as explained next, it is the bus-master identified with MID$_\textrm{1}$ that will have that privilege.

\item \vspace{3pt} \textbf{Platform management core (PMC):} This is an independent processor, distinct from the main application processors. Typically, these cores are added for housekeeping purposes and implemented as small microcontrollers (e.g., Cortex-M4). For example, Figure~\ref{fig:RZ_HW}, the PMC is identified by MID$_\textrm{1}$. The PMC coordinates the configuration of memory access permissions in the PPC, ensuring that the main processor cores cannot tamper with the PPC permissions. The PMC executes a piece of trusted code responsible for implementing this coordination protocol.

\item \vspace{3pt} \textbf{Secure boot:} This last building block aims to guarantee that the management core is in full control of the system's PMC, while blocking the PMC's access to the main application cores. Secure boot validates the integrity and authenticity of the firmware, ensuring that the SMP has been properly bootstrapped into the trusted code referred above.

\end{enumerate}

%NS: BACKUP %These requirements are modeled on the platforms described in ($\S$\ref{sec:hwmp}) and ($\S$\ref{sec:otherplat}). Although we did not carry out an extensive survey, we believe many other current and future platforms will meet these requirements, especially those targeting the high-end embedded markets such as automotive. \sandro{We need to be more confident in this message.} \jose{need to discuss} %Also, there is an increasing trend to include similar mechanisms in mobile SoCs. For example, Qualcomm's SPU (secure processing unit)~\cite{Qualcomm2019} provides many, if not all, of the aforedescribed features.



%=======================================================================
%> [Goals and Threat Model]
%=======================================================================	
\section{Design Goals and Threat Model}

\subsection{Design Goals}

Our main objective is to design a security architecture that leverages the mechanisms presented above in order to enable the creation of sandboxed environments for the secure world in TrustZone platforms. We refer to these environments as secure world zones, or simply \textit{zones}, and they are meant to be used for hosting a partitioned TEE stack running at S.EL$_\textrm{0-1}$, i.e., trusted OS and TA software (see Figure~\ref{fig:intro_rezone}). Since multiple zones $z_i$ can co-exist within the secure world, we use the superscript notation S.EL$^i_\textrm{0-1}$ to identify the execution environment of zone $i$. More concretely, our design strives to attain four subgoals:

%With \project, we aim at building a novel design that improves the security guarantees of TrustZone based systems, by effectively reducing the secure world privileges and thus minimizing the system's Trusted Computing Base (TCB). This mechanism should be deployed in real world hardware platforms and shall incur acceptable overheads for typical TrustZone-based TEEs workloads. \project main goals can be summarized as follows:

\mypara{G1: Reduce the privileges of the trusted OS:} In contrast to vanilla TrustZone platforms where S.EL1 code has unrestricted access to to secure and non-secure memory regions, our goal is to sandbox trusted OS code preventing it from accessing outside the memory regions reserved for its particular zone. As depicted in Figure~\ref{fig:intro_rezone}, zones will be designed to thwart the escalation of privileges of an attacker from the trusted OS to other memory regions of the system. To this end, a zone $z_i$ is expected to enforce three security properties: (P1) \textit{protection of the secure-monitor}, i.e., software running at EL3, (P2) \textit{protection of the normal world}, i.e., software running at N.EL$_\textrm{0-1}$, and (P3) \textit{protection of co-located zones}, i.e., software running at S.EL$^j_\textrm{0-1}$ where $i\ne{j}$.

\mypara{G2: Depend on small TCB:} In traditional TEE stacks, both the trusted OS and monitor are considered trusted. In our case, the trusted OS is no longer part of the TCB. To implement zones in the secure world, we will rely on the secure monitor as root of trust, and incorporate as little additional code as possible into the TCB, e.g., for managing PPC and PMC. % Such code will be necessary, for instance, for managing the PPC and PMC hardware.

\mypara{G3: Maintain TEE software portability:} There is a lot of legacy TEE and TA software. Vendors and OEMs should easily be able to port preexisting TEE/TA stacks into zone-based environments, requiring minimal to no changes in the code.

\mypara{G4: Offer good performance/security trade-off:} The overheads incurred by our solution should not significantly slow down typical real-world TrustZone-based TEE workloads. In other words, we are willing to trade some loss of performance, as long as the performance degradation is not detrimental to the user experience, for improved security guarantees.


\subsection{Threat Model}\label{sec:threat_model}

The main goal of the attacker is to subvert the security properties of zones (P1-3). We assume the adversary has already compromised the trusted OS of a given zone $z_i$, and aims to escape it. As represented in Figure~\ref{fig:intro_rezone}, the attacker may have hijacked the control flow of  $z_i$'s trusted OS through a chain of vulnerability exploits in a TA and inside the trusted OS itself. It is also possible that the attacker may have exploited a vulnerability directly in the trusted OS through the normal world interface. Once inside $z_i$, running in S.EL1$^i$, the attacker may attempt to access (read/write) external memory addresses outside the $z_i$'s private memory by crafting page tables and issuing memory requests accordingly ($\S$\ref{sec:challenge}). These requests may be directed toward the physical address space of the victim at N.EL$_\textrm{0-1}$, EL3, or S.EL$^j_\textrm{0-1}$. These accesses may also be targeted to the memory regions used by the PPC or the PMC. In the first case, the objective is to override the PPC's memory-mapped registers containing the permissions that forbid access to the victim's memory regions. In the second case, the idea is to subvert the PMC's behavior, e.g., causing the PMC to hand over the control of the PPC to the processor core executing the attacker's code. This would indirectly allow the attacker to disable the PPC's restrictions. The attacker may also leverage the effect of caches to read or write cached memory cells for which S.EL1$^i$ does not currently have permissions.
 
In this work, the following attacks are out of scope. We do not consider software attacks exploiting vulnerabilities in the secure monitor or in the PMC software. We assume that these components are correct and belong to the system's TCB. The platform's secure boot initializes the system to a known state. We do not consider physical attacks that tamper with hardware, e.g., fault injection. Our solution has the side-effect of providing cache side-channel protection between zones, and between zones and normal world. However, micro-architectural side-channels are out of the scope of our work. Similarly to a typical TrustZone deployment, we do not consider DoS attacks including those caused, for example, by a malicious trusted OS not relinquishing control to the normal world.


%=======================================================================
%> [DESIGN]
%=======================================================================	
\section{Design}
\label{sec:overview}

This section presents \project, a security architecture that allows for the creation of zones in TrustZone's secure world. 

\subsection{Architecture}

Figure~\ref{fig:rezone_arch} represents the architecture of \project. Hardware wise, our system relies on a typical TrustZone-enabled platform. REE/TEE code runs on the main processor cores and accesses physical memory through the system bus. For controlling memory access permissions, in addition to a TZASC controller, \project relies on a PMC hardware component. The PMC is dynamically configured to restrict (e.g., block) secure accesses from the processor based on the processor's bus master ID (MID$_\texttt{0}$). The PMC can be reconfigured only by a bus master predefined during the system's bootstrapping phase. In \project, this bus master is the ACU (MID$_\texttt{1}$) which we also assume to be present on the platform. ACU and processor can communicate with each other efficiently using a message queue (MQ) implemented by a dedicated hardware peripheral.

Software wise, \project consists of two main components: the \textit{secure monitor} and the \textit{gatekeeper}. The former consists of standard secure monitor software (e.g., implemented by Arm Trusted Firmware) augmented with a \project-specific sub-component named \textit{trampoline}. The secure monitor (and trampoline) run on the main processor core and the gatekeeper on the ACU. These software components have their private memory regions protected by the PPC. These regions are used for storing security-sensitive context information. Taken together, trampoline and gatekeeper are responsible for managing the local execution of zones in the system. They ensure that each zone can access only a private physical memory address space assigned to the zone, and take care of all context-switching tasks involving zone entering and exiting operations. These operations occur, when a REE application makes a call to a zone's guest TA (\textit{zone entry}), and the TA returns the results of the call (\textit{zone exit}). During these operations, REE and zone can share data through a shared memory region. \project's software components are shipped with the platform firmware. When the system bootstraps, the firmware statically creates one or multiple zones indicating the composition of their respective software stacks, i.e., TOS and TAs software. The firmware also configures the memory layout and hardware components to ensure that \project runs in full control of the system.

To create sandboxed zone environments, the trampoline and gatekeeper work together to dynamically set up the system's memory access permissions through the PPC. In a nutshell, before entering a zone, they run a protocol to reconfigure the PPC to limit the access permissions of the processor to the memory resources of the zone in question. When exiting a zone, the inverse operation is executed. Next, we explain how the system is designed and how these operations work. We refer the reader to Figure~\ref{fig:HZ-exec-model} as we cover these issues.


\subsection{Memory Partitioning and Access Permissions}
\label{sec:memory_restrictions}

The starting point in \project design is to partition the physical memory layout into regions, allocating these regions to different protection domains of the system, and specifying regions' memory access permissions accordingly. In doing this, we are primarily concerned about restricting secure memory accesses when the processor runs zone code, i.e., S.EL$_\textrm{0/1}$. The final memory layout and access permissions are depicted in Figure~\ref{fig:HZ-exec-model}. We progressively explain these regions and permissions, beginning with a vanilla TrustZone-enabled platform, and then extending it with \project's protections.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/rezone-arch.pdf}
    \caption{\project architecture: Its software components are colored in dark shade and consist of secure monitor (which includes the trampoline) and gatekeeper. Secure monitor runs on the main processor cores; gatekeeper runs on the ACU. \project software controls memory accesses via the PPC.}
    \vspace{-0.2cm}
    \label{fig:rezone_arch}
    \vspace{-0.3cm}
\end{figure}

\begin{figure*}[!ht]
    \centering
        \includegraphics[width=0.95\linewidth]{images/rezone-execution.pdf}
    \caption{\project execution model, memory access permissions, and memory layout: \project ensures that the code running inside zone 1 -- i.e., at S.EL$_\textrm{0/1}$ -- can only access zone 1's private memory region (M$_\textrm{Z1}$). This protection is achieved by reconfiguring the PPC to restrict the processor's access permissions when entering zone 1 (steps 3\&4), and reverting these configurations when exiting zone 1 (steps 5\&6). The PPC is used only to restrict the secure accesses.}
    \vspace{-0.2cm}
    \label{fig:HZ-exec-model}
    \vspace{-0.2cm}
\end{figure*}

Just like in a typical TrustZone setup, in \project, the normal world includes regions for the REE OS (M$_\texttt{OS}$) and shared memory (M$_\texttt{SH}$). The secure world has independent regions for the TEE software. The TZASC is then configured accordingly to enforce memory protection based on the state of the NS bit, preventing the normal world software from accessing secure world regions. The first line in the permissions table (see Figure~\ref{fig:HZ-exec-model}) shows how the normal world has only read/write access permissions to normal world memory regions.

Then, in \project we further separate the secure world memory into independent regions for the secure monitor (M$_\texttt{SM}$) and for each zone $i$, e.g., zone 1 (M$_\texttt{Z1}$). We need to ensure that the secure monitor software (EL3) continues enjoying full access permissions, but the code running at S.EL$_\textrm{0/1}$ is confined to (i) the zone's private memory M$_\texttt{Z1}$ and (ii) the REE shared memory for enabling data exchanges during TA calls. To this end, we leverage the PPC to restrict secure world accesses. However, given that the PPC cannot distinguish secure accesses coming from EL3 or from S.EL$_\textrm{0/1}$ code, these permissions need to be dynamically changed by the monitor when entering a zone (i.e., reprogramming the PPC to remove \texttt{RW} access permissions to M$_\texttt{OS}$ and to secure world memory as per line three in the permissions table) and when leaving a zone (i.e., reverting to the permissions in line two of the table).

At this point, a subtle difficulty arises in order to accommodate the processor transition from S.EL1 to EL3 when exiting a zone. If the S.EL1 code running in the context of a zone is wholly prevented from accessing the secure monitor memory, this protection will still be in place by the time the zone's trusted OS traps into the secure monitor when exiting the zone. This means that, although the secure monitor is trusted, it will still be blocked by PCC resulting in memory access aborts and a system crash. To solve this problem, we create a dedicated secure memory region containing code and data that are necessary only to facilitate this transition securely. This code is part of the trampoline. The trampoline still belongs to the secure monitor because it runs in SL3. We then segregate a region of the trampoline's memory  (M$_\texttt{T}$) from the rest of the secure monitor memory (M$_\texttt{SM}$) because these regions need to be configured with different memory access permissions. M$_\texttt{SM}$ is always denied access from S.EL$_\textrm{0/1}$. In contrast, M$_\texttt{T}$ is marked read-only by the PPC therefore allowing the processor to both execute trampoline code from M$_\texttt{T}$ and load context data also from M$_\texttt{T}$ while still running in S.EL1. The trampoline code will then engage the AUC to remove the PPC memory access restrictions to M$_\texttt{SM}$ therefore allowing the secure monitor to freely run at S.EL3 and restore the normal world execution. These reasons justify the permissions displayed in the last two rows of the table in Figure~\ref{fig:HZ-exec-model}, which are enforced by the PPC.


\subsection{Securing the PPC Memory Access Permissions }
\label{sec:memory_restrictions}

To guarantee the enforcement of the memory access permissions as described above, the PPC must be (re)configured exclusively by a trusted component. In \project, this component is the  gatekeeper/AUC ensemble. We configure the PPC so that only the AUC is authorized to perform this operation. Since the PPC can differentiate requests based on the bus master ID, we program the PPC to accept configuration requests only by a bus master identified with the AUC's MID. Requests originating from other bus masters, e.g., the processor, will be denied. The AUC runs the gatekeeper code and dynamically updates the PPC permissions when entering or leaving a zone by serving the specific requests send by the trampoline, e.g., to enable M$_\textrm{SM}$ \texttt{RW} permissions at zone exits.

\project also needs to defend against a potential attack. The communication between processor and AUC is facilitated by a message queue unit (MQ in Figure~\ref{fig:rezone_arch}) which is agnostic to the current exception level of the processor. Therefore, when the processor sends a permission reconfiguration request via the MQ to the AUC, the gatekeeper cannot distinguish whether this request was generated by trusted EL3 code or by untrusted S.EL1 code. As a result, an attacker running at S.EL1 within a zone could craft a request to disable the memory access restrictions enforced by the PPC. To thwart this threat, the gatekeeper must be able to foretell that this request is malicious and therefore must be refused. To this end, trampoline and gatekeeper share a secret token initialized at boot time and copied to their private memory regions. This token is then used by the trampoline for authenticating PPC reconfiguration requests sent to the gatekeeper. Since the secret token is not accessible at EL3, an attacker can no longer spoof legitimate requests, making the system robust againt these attacks.


\subsection{Preventing Cross-zone Interference at the Processor Level }
\label{sec:memory_restrictions}

The mechanisms discussed so far ensure that all memory transactions observed outside the processor cluster are controlled according to the permissions matrix specified in Figure~\ref{fig:HZ-exec-model}. These mechanisms need to be complemented with additional measures to safeguard against potential attacks within the processor itself. We address two concrete concerns.

First, the PPC acts only at the system bus level. Therefore, its memory access protections do not extend to the internal caches of the processor cluster. For this reason, if the private L1 cache contains cached data that a given zone is not authorized to read or write, if the core enters that particular zone, this content will be accessible to that zone, which constitutes a security violation. Likewise, a similar problem may occur for the shared L2 cache, where cached content could be available for other cores. To prevent these problems, the private cache of the core executing the zone and shared caches must be flushed.

Second, the PPC cannot differentiate between single cores within a cluster. This is because the PPC observes requests as being from a single bus master: the cluster's shared cache. As a result, \project's memory restrictions enforced by the PPC are collectively applied across all cores of the same cluster. However, blocking access to the normal world memory when a core enters a zone, will also prevent other co-located cluster cores from accessing normal world memory, which may lead to crashes if they are currently executing REE code. To prevent this problem, upon zone entry, \project must halt other co-located cluster cores running in normal world until the core exists the zone. Despite the non-negligible performance overheads potentially introduced by these measures, our experiments show that these overheads can be tolerated due to the infrequent TEE invocation patterns and short TA execution times inside the secure world (see $\S$\ref{sec:eval}), essentially trading some performance degradation for increased TEE security.


\subsection{Zone Entry and Exit Workflows}
\label{sec:key_mechanism}

The protection mechanisms described above act together whenever a REE application invokes a TA hosted in a zone. This invocation triggers \project's world-switch mechanisms responsible for entering and leaving a zone (see \autoref{fig:HZ-exec-model}).

A zone entry begins when the normal-world OS issues a request through the invocation of the \texttt{smc} instruction (1), causing the execution to be handed over to the secure monitor. If the request needs to be handled by the trusted OS, \project will first differentiate to which zone the requests to that particular TA have been statically assigned. Then it forwards the request to the respective zone, i.e., zone in the figure. For this, the secure monitor starts by notifying all other cores in that cluster. The other cores will then enter an idle state. The trampoline continues by issuing a request (2) to the gatekeeper to block PPC access to the application core. To authenticate the request as coming from the secure monitor processor mode, the gatekeeper expects to receive the secret token it handed to the monitor during boot. After a successful reply from the gatekeeper (3), the trampoline will first flush its own cache content and then (4) jump to the trusted OS.

A zone exit occurs once the trusted OS returns execution to the secure monitor (5). At this point, the trampoline issues a new request to the gatekeeper (6) to unblock secure memory accesses from the processor core. The gatekeeper ensues by reconfiguring the PPC to disable the zone's protection policies, i.e., granting \texttt{RW} for all memory regions. The secure monitor will then (7) resume execution, notify other cluster cores to, finally, return to the normal world context (8) executing under traditional TrustZone restrictions enforced by the TZASC.


\newcounter{problem}
\newenvironment{problem}[1]{\refstepcounter{problem}\par\medskip
   \textbf{Problem~\theproblem. #1: } \rmfamily}{\medskip}
   
%=======================================================================
%> [IMPLEMENTATION]
%=======================================================================	
\section{Implementation}
\label{sec:impl}

We implemented a full-fledged prototype of \project on a real-world hardware platform. After presenting an overview of our prototype's hardware and software, we discuss the most interesting technical challenges of our implementation. %, from synchronizing cores before executing the trusted OS, to securely performing a context switch to the S.EL1 and correctly handling normal world and trusted world exceptions.

\if0
In this section we focus on the implementation challenges of deploying \project in a real world platform. Challenges arise in various aspects of the implementation. From synchronizing cores before executing the Trusted OS, to securely performing a context switch to the s.EL1 and correctly handling normal world and trusted world exceptions. 
In our implementation, we take advantage of the Resource Domain Controller (RDC), and a programmable MCU present in the iMX8MQ platform.
One of the main challenges in our implementation is that, although part of our model, the RDC only performs access control to main memory and not at a cache level. This means that accesses can only be controlled at a cluster level granularity, because it's the last level cache of the cluster which performs the memory accesses. This forces us to perform cache maintenance operations to guarantee that a zone does not access memory outside of the sandbox. Another insidious consequence of this, is that using the RDC to establish read-only memory regions still allows a core to make changes of memory contents at a cache level. This will result in CPUs in same cluster retrieving potentially manipulated values, given that the memory accesses will result in cache hits. Solutions for these problems are presented in this section. 

After discussing which software stack we use to prototype \project, we start by explaining the RDC programming model, then we explain how we boot the system, after which we explain how we tackle core synchronization challenges before executing a Trusted OS. Next, we explain how we guarantee secure RDC configuration, and the steps required to safely exit to s.EL1 and to handle its exceptions in the trampoline. Finally, we explain how we can restrict accesses to peripherals to the AP while, allowing other bus masters to access them.
\fi




\subsection{Hardware Specification and Security Configurations}
\label{imp:hw_sec}

The implementation of \project is tightly dependent on the targeted hardware. We used the i.MX 8MQuad Evaluation Kit (EVK), which features an i.MX8MQ SoC by NXP. This SoC is powered by (i) an application processor consisting of one cluster of four Cortex-A53 cores (@1.5 GHz) and (ii) one microcontroller, a Cortex-M4 (@266 MHz). The Cortex-A53 cluster has 32KiB level-1 (L1) instruction and data caches per core and a shared 2MiB level-2 (L2) cache. The Cortex-M4 has a 16KiB code bus cache and a 16KiB system bus cache.

We use the Cortex-M4 to act as \project's ACU, and an SoC-embedded hardware controller named Resource Domain Controller (RDC) to play the role of PPC. This controller is present in the i.MX 8M family of processors and enables fine-grained control of access permissions in platforms with multiple bus masters. This PPC offers this service through the creation of security domains. There are at most four domains, each being identified by an ID (DID$_i$). A domain represents a collection of platform resources (e.g., memory regions, peripherals), and it is tagged with a set of access permissions (e.g., read/write, read only). Bus masters, such as application processor, microcontroller, DMA, GPU, etc., can be associated with one or multiple domains. A bus master in DID$_i$ can only access a resource, if the resource is also associated to the bus master's domain, and its access privileges will be determined by the permissions of DID$_i$.

Based on the security domain scheme provided by the PPC, we use the following insight to implement the memory partitioning and access permissions described in $\S$~\ref{sec:memory_restrictions}. To create domains, assign/remove resources and/or bus masters to domains, and set permissions it is necessary to configure PPC's registers. Since the PPC is itself a platform resource, by reserving a domain (e.g., DID$_1$) with full read/write permissions to the PPC and associating the ACU as the single bus master to DID$_1$, we ensure that no other bus master in the system -- namely the processor -- will be able to tamper with PPC's security permissions. If DID$_1$ can be specified on the system prior to any interference from an adversary, we ensure that the ACU remains in full and exclusive control of the PPC. To achieve this, we can rely on the secure boot to run a customized initialization routine that will fully initialize the ACU before starting the zones' untrusted trusted OS. This initialization will be performed by the gatekeeper code that will then set up DID$_1$ and other necessary domains in the PPC.

More specifically, our implementation configures three security domains when booting the system: DID$_\textrm{0}$, DID$_\textrm{1}$, and DID$_\textrm{2}$. Domain DID$_\textrm{0}$ contains all memory (and other) resources exposed to the processor. DID$_\textrm{1}$ mainly contains the PPC and the gatekeeper's private memory region. The processor is associated to DID$_\textrm{0}$, and the ACU to DID$_\textrm{1}$. This configuration ensures that the software running on the processor has no privilege to read or write neither ACU's private memory, nor the PPC's configurations. As a result only the ACU can reconfigure the RDC, which it does to reflect the access permission matrix depicted in Figure~\ref{fig:HZ-exec-model} (last two rows). In the i.MX 8M family, Cortex-A CPU clusters are assigned a unique master ID. This means that DID$_\textrm{0}$'s permissions apply indistinguishably to every Cortex-A53 core of the processor.

Domain DID$_\textrm{2}$ allows other bus masters to function properly while the processor executes code inside a zone. In these occasions, other bus masters may need access to certain peripherals, for example to play audio asynchronously. If these bus masters are configured to be in DID$_\textrm{0}$, the PCC will apply the same permissions to them as the processor, which may cause disruptions. To prevent this problem, we create DID$_\textrm{2}$ for all other masters and give DID$_\textrm{2}$ access to all peripherals and memory regions at all times. These permissions will enable all masters from DID$_\textrm{2}$ to access the required peripherals even if the processor cannot occasionally access them. A side-effect of this approach is that a attacker controlling a zone's trusted OS may attempt to leverage one such bus masters as stepping stone to bypass the zone sandbox. In other words, the attacker may try to interfere with the behavior of a peripheral being used by some bus master to access a memory regions disallowed to the processor but permitted if performed by the bus master. To limit these attacks, zones can be configured with a white list of platform peripherals based on the requirements of legitimate trusted OSes like OPTEE2. Thus, when entering or leaving a zone, the PPC is re-configured to include the peripherals' zone-specific access permissions. In our prototype, zones block access to all 115 of our SoC's peripherals, excepting five\footnote{OPTEE2 needs access to 5 peripherals: a UART for debugging, a secure non-volatile storage device, a cryptographic hardware accelerator (CAAM), an analog phase lock loop, and an on-chip one-time-programmable controller.}.

Another peripheral-related aspect involves establishing a secure channel between processor and ACU. Upon zone entry/exit events, they exchange message reconfiguration requests via the platform's MU (see Figure~\ref{fig:rezone_arch}). In the iMX8MQ SoC, the MU is composed of two peripherals MU\_A and MU\_B, implementing the MU interface. The PPC assigns MU\_A exclusively to DID$_\textrm{0}$, and MU\_B to DID$_\textrm{1}$, ensuring that only the processor and ACU can communicate with each other through the local MU interfaces. To authenticate the requests sent by the processor, trampoline and gatekeeper share a secret token. Given that trampoline's memory is set as read-only for untrusted S.EL1 code (see the permissions table in Figure~\ref{fig:HZ-exec-model}), the trampoline cannot store the token in memory, otherwise it could be read by a compromised trusted OS. To preserve the secrecy of the token, the trampoline stores it in the \texttt{TPIDR\_EL3} 64-bit register, which is exclusively available to EL3 code --- not even S.EL1 code can read this register -- leaving the adversary a 1 in $2^{64}$ chance of guessing its value correctly. The token is randomly generated at boot time.

Given that the ACU runs at a clock speed 5.6$\times$ slower than processor cores, we implemented an important optimization aimed at offloading as much as possible critical-path workload from the gatekeeper running on the ACU to the trampoline executing on the processor at EL3 upon zone switch. Originally, the gatekeeper's mission is to reconfigure the PPC's permissions of DDI$_\textrm{0}$ resources which we experimentally verified to become sensibly slower as the number of resources grows (especially as we included the platform's peripherals). To shift most work to the trampoline, the gatekeeper temporarily associates the PPC to DDI$_\textrm{0}$, allowing the trampoline to update PPC's permissions on the gatekeeper's behalf, running this logic on a fast Cortex-A53 rather than on the slow Cortex-M. Once finished, the gatekeeper removes the PPC from DDI$_\textrm{0}$, reacquiring its former condition of sole guardian of the PPC.



% Because TrustZone design is the enabler for the severity of vulnerabilities found in TrustZone, TrustZone enforcing hardware is not enough to address this problems. Lately, several platforms have came up with hardware mechanisms to create domains within the SoC. These domains are independent of TrustZone and aim to control access to subsets of system resources for the various masters of the platform (e.g., Application Processor, microcontroller, GPU, etc).
% Chip designers provide hardware based mechanisms to validate memory accesses. They are generally called protection units. Here we provide some examples:
% \begin{itemize}
    % \item Xilinx - Xilinx Memory Protection Units (XMPU) and Xilinx Peripheral Protection Unit (XPPU)
    % \item NXP - Resource Domain Controller (RDC), Extended Resource Domain Controller (xRDC) and xRDC2
    % \item Qualcomm - xPU "This means the XPU registers are only one mean to secure peripherals and/or memory, all of which can be protected by other technology like TrustZone isolation." %https://blog.quarkslab.com/analysis-of-qualcomm-secure-boot-chains.html
    % \item Qualcomm - SPU memory controller "The TSF shall be implemented to restrict the ability to [modify and define] the memory areas shared with other components of the SoC to SP-ExtMM controlled by the SP-CPU." %https://www.commoncriteriaportal.org/files/epfiles/1045b_pdf.pdf
    % \item ? Apple - Hardware “filter” to prevent AP to SEP memory access -Only SEP’s KF core has this filter %https://www.blackhat.com/docs/us-16/materials/us-16-Mandt-Demystifying-The-Secure-Enclave-Processor.pdf https://www.theiphonewiki.com/wiki/Secure_Enclave_Processor
% \end{itemize}


%There is an ongoing trend in the SoC industry to embedded an increasing number of processing units and bus masters in the same chip and to provide additional mechanisms to isolate them. In response, we start seeing an increasing number of platforms which implement, at the system level, additional hardware access control mechanisms orthogonal to TrustZone. In the following, we describe a few examples implemented in the NXP iMX8 and the Xilinx Zynq UltraScale+ families. 

%  On final aspect of these platforms is that each cluster is a master. This means that memory regions cannot be assigned to a single core, but may be assigned per cluster, allowing for memory access policies to be granular at the cluster level.
%\david{Note: In the iMX8MQ, the upper 1GB is not protectable by RDC. This is not really problem as long as that space is dedicate to non-critical applications. Not sure how feasible doing this though.}

\subsection{Cross-core Synchronization When Running Inside a Zone}
\label{sec:synch}

When a single core enters a zone and executes the trusted OS, given that the PPC removes access of the whole processor cluster to several memory regions (e.g., normal world memory), we must take care to prevent situations where the software running on another core of the cluster would execute while the first core is still actively running inside the zone. Otherwise, a second core would simply crash as it cannot access neither the data nor the code from blocked memory regions. Below are the instances where such scenarios might occur (for the sake of simplicity we consider only two cores):

\begin{enumerate}
  \setlength\itemsep{0em}
    \item\label{sync1} Two cores $c_1$ and $c_2$ execute secure monitor code at EL3, and $c_1$ issues a zone entry, requesting a shift to S.EL1 while $c_2$ still runs at EL3. This can be a problem, because if $c_1$'s request is attended without proper synchronization, $c_2$ will not be able to access secure monitor memory.
    
    \item\label{sync2} One core ($c_1$) is executing the trusted OS at S.EL1 while another ($c_2$) is sleeping. Meanwhile the sleeping core $c_2$ awakens into monitor code (e.g. due to an interrupt). Again this is a problem, because $c_2$ will not be able to access monitor memory while $c_1$ executes the trusted OS.
    
    \item\label{sync3} Two cores $c_1$ and $c_2$ are executing normal world code, and $c_2$ requires a service from a TA hosted inside a zone. This is a problem because, when $c_2$ enters the zone, $c_1$ will be denied access to normal world memory.
\end{enumerate}

We solve this problem by properly synchronizing the cores using spin locks and FIQ interrupts. To address scenario \ref{sync1}, the monitor tracks which CPU cores are currently executing the secure monitor. If a core intends to enter a zone, they all wait on a barrier. At that point, $c_2$ sits on a spin lock while $c_1$ is allowed to jump into the trusted OS. Once $c_1$ concludes the zone call and returns to EL3, $c_2$ can continue. We solve scenario \ref{sync2} by waking the CPU core $c_2$ into an a trampoline's read-only memory region (not-writable by the running trusted OS) and waiting for the trusted OS in $c_1$ to cease execution by using a spin lock (\texttt{rz\_lock}). 
To solve scenario \ref{sync3}, we use an FIQ interrupt and a spin lock (\texttt{rz\_lock}).  First, when $c_1$ issues a request from normal world to enter a zone, it traps into the monitor (EL3) where it fires an FIQ interrupt and grabs a the \texttt{rz\_lock}. The goal of this interrupt is to notify other cores (i.e., $c_2$) that $c_1$ wishes to enter a zone. Core $c_2$ is then interrupted and jumps into trampoline code, an exception handler running in S.EL1, where it unlocks $c_1$ letting it continue to enter the zone; $c_2$ now waits on the spin lock until $c_1$ exists the zone, allowing $c_2$ to resume its execution in the normal world. To implement these synchronization techniques, the trampoline code executes partly in EL3, partly in S.EL1 exception levels.


\subsection{Micro-Architectural Maintenance in EL3-S.EL1 Switches}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-ContextSwitch.pdf}
    \caption{Context-switch between EL3-S.EL1 requires micro-architectural maintenance operations (A, B, E). Entering a zone (EL3$\rightarrow$S.EL1) requires A, B, C, D and E. Exiting a zone (S.EL1$\rightarrow$EL3) requires C, D, E and F.}
	\vspace{-0.2cm}
    \label{fig:scr_ctx_hw}
	\vspace{-0.3cm}
\end{figure}

Triggered by some zone entry/exit event, context switching between EL3-S.EL1 requires the trampoline to coordinate not only PPC reconfiguration and cross-core synchronization, but also important cleanup tasks as illustrated in Figure~\ref{fig:scr_ctx_hw}. Having extensively discussed operations C and D above, we now focus on micro-architectural maintenance that needs to be performed.

When entering a zone (EL3$\rightarrow$S.EL1), the trampoline running on the core needs to ensure that the trusted OS (after the switch is finished) cannot access resources outside of the zone. After taking all measures to prevent interference from other cores ($\S$\ref{sec:synch}), the trampoline needs in addition to invalidate the L1 instruction and data caches and the L2 cache (A). Unless this operation is performed, data or instructions left in the cached will be accessible to the trusted OS, therefore violation the isolation properties of a zone's sandbox. Also, right before jumping into the trustedOS, the trampoline disables SMP coherency. Recall, that at this point, all other cores in the cluster are suspended. Each core has data and instruction in their own L1 caches. With SMP coherency enabled, a request to access data present in these caches would cause a cache hit, and data could be accessed by the present core, again violating the zone's isolation properties. Disabling SMP coherency prevents this from happening. Without support to disable SMP coherency, we need to flush the L1 caches of all other cores as part of the synchronization mechanism to ensure that cached data on other cores is not be accessible to them.

In addition to cache maintenance, when switching between the trusted OSes of different zones, the trampoline needs to also perform TLB maintenance (i.e., TLB invalidation) for the current core (B). The main reason is not due to concerns about violation of memory isolation across zones, as this isolation is already enforced by the PPC which sets each zone's memory region to be private. However, given that (i) the TLB for S.EL1 is shared by the trusted OSs of active zones, and (ii) the TLB has no way to tell which of the cached page table entries belong to each zone, unless a TLB invalidation is performed, a TLB lookup by the trusted OS could translate into a physical address that belongs to another zone, thus causing unexpected faults. As an optimization, we perform TLB maintenance only if the last invoked trusted OS is different from the one currently executing. Therefore, in practice, TLB invalidation is only necessary when switching between zones. With all micro-architectural maintenance done, the trampoline will restore the general purpose register state, and exit to the Trusted OS.


\subsection{Handling Exceptions at S.EL1 Exits}

In contrast to zone entries, exiting a zone by returning from S.EL1 to EL3 no longer requires the steps A and B shown in Figure~\ref{fig:scr_ctx_hw}. However, we need especial precautions in dealing with exceptions from S.EL1. Two problems may arise: %It not handled properly, an attacker hijacking the zone's trusted OS may be able to escalate privileges to the monitor or attack the normal world. %There are two problems taking the following naive approaches to handling exceptions from S.EL1:

\if0
\mypara{MMU TLB-Miss on Handling Exceptions in EL3}
Upon entering the vector table, it may be the case that there's no TLB Entry that maps the region of code. In this case the MMU will fetch the PTE that maps it to perform a page table walk, which will result in the TLB issue memory accesses. Because we've flushed page tables from the caches as part of the secure exit to s.EL1, a main memory access must be performed. However, the memory will be inaccessible as established by the trampoline. This would result in the system hanging, as the code for handling the exception would not be accessible. The issue is depicted \autoref{fig:p}~a).

\mypara{EL3 Code Injection from sEL1}
The code on the vector table must be readable from main memory, and thus marked as readable by the processor on the RDC. 
However, this will also give the TrustedOS the ability to read the code.
Due to the memory hierarchy, the vector table code will now also reside in cache, and write operations are now allowed (as long as they do not reach main memory). A TrustedOS can maliciously modify the exception handling code (e.g., modify SMC handling code), to its own advantage. Upon an SMC, the Monitor would then execute malicious code which is obtained from \emph{hitting} the cache, i.e., from not obtaining from main memory. The issue is depicted \autoref{fig:p}~b).
\fi

\begin{enumerate}
  \setlength\itemsep{0em}
    \item\label{prob1} \textit{TLB-miss:} Upon entering the vector table to handle an S.EL1 exception in EL3, if the TLB misses a page table entry that maps to the memory region of the exception handler, then the MMU must perform a page table walk. As the caches have been flushed prior to entering S.EL1, this operation will trigger an access to main memory in order to load the missed page table entry. However, since the EL3 page tables are stored in the secure monitor's memory region, whose access by EL3 code is still blocked by the PPC at this stage (recall that only the trampoline memory is marked read-only), the code for handling the exception cannot be loaded and the system will hang.
    
    \item\label{prob2} \textit{EL3 code injection from S.EL1}: From 1) it follows that the code on the L3 vector table must be marked as read-only by the PPC, allowing also the trusted OS to read the handler code from memory. However, since the vector table code will now be cached in the L1/L2 caches, write operations are still permitted to cache lines tagged as secure world memory as long as they do not reach main memory. (Note that the PPC acts only at the bus level.) An attacker with S.EL1 privileges can use this feature to modify the exception handler code to its own advantage, e.g., by modifying the SMC handler, an \texttt{smc} call can trigger the secure monitor to load malware from cache.
\end{enumerate}

To solve both problems, we disable the MMU for EL3 code (F in Figure~\ref{fig:scr_ctx_hw}). We do this in the last steps of exiting EL3 to S.EL1 when entering a zone. Note that this measure only applies to the MMU for EL3 code: we do not disable the MMU for S.EL1 code. This separation is possible because EL3 and S.EL1 have different address spaces and can be disabled/enabled individually. Given that, the virtual memory addresses are identity-mapped to physical memory addresses in the secure monitor, disabling the MMU will not disrupt the secure monitor execution. This solves problem 1, as from that point on, memory accesses at EL3 will not be subject to MMU translation; thus, no page table accesses are needed, and the exception handler can be executed without crashing. Disabling the MMU will also disable L1 and L2 caches for EL3 address spaces, and this will partially solve problem 2 as the exception handling code will always be fetched from main memory. This memory is protected read-only by the PPC, hence no modifications will be possible. However, this solution does not entirely solve the whole problem. Note that during the switch from EL3 to S.EL1, after flushing all caches, the trampoline still executes with caches turned on. This will inevitably leave some traces of trampoline data and instructions in the caches, which a malicious trusted OS can try to leverage for an attack by modifying them locally while running in S.EL1 as described above. To clean up potentially tampered cache content and avoid these attacks, we invalidate on-cache trampoline-related memory when the exception handler in EL3 is executed on an S.EL3 exit (E in Figure~\ref{fig:scr_ctx_hw}). After this cache management operation completes, the exception can be handled securely.

%%
%% NS: BACKUP => don't delete yet
%%

\if0
\mypara{Multi Cluster Scenario}\label{sec:mult}
%Our test platforms provide the necessary mechanisms for deploying a system with multiple TEEs. \nuno{TEE software, each one inside an IEE, right?} To implement multiple TEEs in the platform featuring a single cluster, the iMX8MQ, it's necessary to make only the current TEE's program memory available to EL-1. This is achieved in a similar way that secure-monitor program memory is protected; the RDC is used to prevent access to the required memory regions (i.e. other TEEs). When handling trusted service requests the secure-monitor will enable, by interacting with the micro-controller, only the required TEE to execute the service. Figure \ref{fig:multi-tee-same-cluster} illustrates the process. 
%
To implement multiple TEEs in the platform featuring more than one cluster, in addition to the techniques mentioned above, we can also leverage the fact that memory access policies can be defined per cluster. This enables simultaneously running one TEE per cluster while benefiting from mutual isolation. 
%Figure \ref{fig:multi-tee-multi-cluster} illustrates memory configuration for achieving this. 
There are many ways to employ this idea, one might be to have as many TEEs as clusters, and statically assign a TEE per cluster. This allows for a straightforward implementation of protection mechanisms, while allowing multiple TEEs to serve trusted service requests parallel to each other. More complex implementations might optimize TEE distribution base on available clusters, to run any TEE on any cluster while clusters are available to execute as many trusted services concurrently as possible.
Given that it's possible to run different TEEs on different clusters, one problem arises. Which TEE should run an each cluster. Nowadays it is common for CPUs to be implemented in a BIG.little configuration. So it is intuitive to assign performance sensitive workloads to high performance cores. System designers may define what services are to run on each cluster as to provide the best user experience. \david{These points could go to the design}

\fi


\subsection{Software Implementation}

The \project software itself is a firmware bundle based on TF-A (v2.0). TF-A implements basic bootstrapping and secure monitor functionality. We modified TF-A to incorporate the \textit{trampoline}, which we implemented in 139 and 1220 SLOC of C and assembly code, respectively. We also used the TF-A to bootstrap the \textit{gatekeeper}. The gatekeeper is implemented as a bare-metal application that runs on the Cortex-M4. It was written in 417 SLOC of C code and packaged with essential drivers to interface with our platform's PPC (i.e., the RDC). The system image was compiled with the GNU Arm toolchain for the A-profile Architecture (v9.2.1) and GNU Arm Embedded Toolchain (v9.3.1), and the final bootable image was produced with the imx-mkimage (branch imx\_5.4.3\_2.0.0).

We also changed the TF-A's context management routines and data structures to support independent zones for hosting two trusted OS instances based on OP-TEE (v3.7.0). To run OP-TEE inside a zone, no intrusive modifications were necessary; we have disabled only the support for dynamic shared memory. We create the second OP-TEE instance in a different address space, and updated the values of SMC IDs to be uniquely attributed to each OP-TEE instance.

We created two full-blown stack builds featuring different REE software: one running the Linux kernel (5.4.24) and the second the Android OS, compiled from AOSP 10.0. It was not necessary to modify REE code to support \project, however, because we added support to run multiple trusted OSs, we added drivers to interface with both of them. In our prototype we duplicate the OP-TEE Linux kernel driver, and modified the SMC\_IDs used to make calls to the second OP-TEE instance. There are two tee-supplicant services, one for each OP-TEE.



\if0
To implement \project we modified and used several open source secure world components. For monitor we used Trusted Firmware-A (TF-A) and made modifications to the Trusted OS services to make them issue the rezone\_suspend interrupt, and also modified EL3 exiting code, and vector table code, to implement the trampoline. Additionally, to support multiple Trusted OSs we made the necessary changes to TF-A's context management routines and data structures, while duplicating the OPTEE service, to handle requests to the second OPTEE instance.
To safely run Trusted OSes without them being able to thwart the established access policies \project controller takes ownership of the RDC. To implement it we make use of the provided board support package, including drivers to interface with the RDC and perform initialization routines. Although the platform supports true random number generation, in our prototype we do not make use of this feature due to lack of support for it for both the monitor and micro-controller. A developer with access to the appropriate documentation should use the features available in the platform to securely generate the secret token.
No intrusive modifications are necessary to execute OPTEE in a secure world zone. However, a deployed OPTEE build will not support dynamic shared memory, and so the configuration parameter must be set do disabled. Additionally to support running multiple Trusted OSs, we create a second OPTEE instance in a different address space, which required specifying the designated address space. Additionally, we updated the values of SMC IDs to be uniquely attributed the second OPTEE instance.
It is not necessary to modify REE code to support \project, however, because we added support to run multiple Trusted OSs, it is necessary to add drivers to interface with both of them. In our prototype we duplicate the OPTEE Linux kernel driver, and modified the SMC\_IDs used to make calls to the second OPTEE instance. Additionally we also have two tee-supplicant services, one for each OPTEE instance.
\fi


%Because the trampoline is shared between the monitor and the untrusted zones, this software component must be tailored to be as minimal as possible and encompass mostly read-only memory to avoid corruption from a rogue Trusted OS. All writable data used by the trampoline must be non-critical and can't be re-used upon a zone exit.

%\mypara{System Initialization and Multi-zone Support: moved from design section} To setup the system, the normal world's and all zones' domains must be statially defined at design-time. This includes defining access privileges to memory and peripherals address ranges, and explicitly  identify shared-memory regions between each zone and the REE. A user must also disable dynamic shared memory allocation in the Trusted OSs. This feature allows any normal-world address to be used as shared memory but, given that shared memory regions are defined statically, it cannot be used. From our experience, mainstream Trusted OSs such as OPTEE or ??? allow turning it off at compile-time. For each defined zone, the corresponding Trusted OS must be be associated with an unique range of SMC (Secure-Monitor Call) IDs. Trusted OSs originating from different vendors use the same SMC ID ranges as defined by the SMC Calling Convention (SMCCC) \cite{}. Since \project allows different Trusted OSs, or event the multiple instances of the same Trusted OS, in the same system, the issue arises of conflicting SMC IDs. To solve it, our current design mandates that a user must manually modify both the normal-world drivers and Trusted OS handlers to offset the SMC IDs of each Trusted OS instance so that each falls in a mutually exclusive range. We believe the range defined by the SMCC is sufficiently large to host all possible SMC IDs in a realistic system configuration. All this information is directly compiled into the monitor image. At system initialization, the monitor creates an RPC configuration for each zone as well as a map of SMC to zone IDs. It then activates each zone in a sequential fashion so that each trusted OS can perform its initialization, before handing control to the REE OS. At runtime, when the normal-world OS issues a request to the secure world passing it a given SMC ID, the monitor will translate the SMC ID into a zone ID, fetch the zone's RPC configuration and commit it to the hardware before jumping to the Trusted OS.


%\subsection{%Implementation Overview}

%The implementation of \project is tightly dependent on the targeted hardware. Next, we start by presenting our target platform, and then the details of our software implementation. 

%To implement \project we take advantage of a programmable MCU present in both our test platforms, iMX8MQ and iMX8QM, and in the flexibility both this platforms provide in assigning memory resources to different processing elements while excluding others.
%\david{Mention that we modify TF-A.} 
%make sure a reader could reconstruct the implementation


%=======================================================================
%> [EVALUATION]
%=======================================================================
%\newpage
\section{Performance Evaluation}
\label{sec:eval}

%We evaluated \project on an i.MX 8MQuad Evaluation Kit (EVK). The platform features an i.MX8MQ SoC, powered by four Cortex-A53 (@1.5 GHz) and one Cortex-M4 (@266 MHz). The Cortex-A53 cluster features 32KiB level-1 (L1) instruction and data, per core, caches, and a shared 2MiB level-2 (L2) cache. The Cortex-M4 features a 16KiB code bus cache and a 16KiB system bus cache

We evaluated \project for the i.MX8 platform described in $\S$\ref{imp:hw_sec}. The software stack includes the TF-A (v2.0), OP-TEE kernel (v3.7.0), client library and supplicant (v3.7.0), Linux kernel (v5.4.24), and Android 10. The system image was compiled with the GNU Arm toolchain for the A-profile Architecture (v9.2.1) and GNU Arm Embedded Toolchain (v9.3.1), and the final bootable image was produced with the imx-mkimage (branch imx\_5.4.3\_2.0.0). Our performance evaluation focused on microbenchmarks ($\S$\ref{sec:eval_micro}) and real-world TAs ($\S$\ref{sec:eval_TAs}). We have also evaluated the impact of \project on the normal world execution ($\S$\ref{sec:eval_NW}) and on supporting multiple TEEs ($\S$\ref{sec:eval_mTEE}). While evaluating the performance overhead for the microbenchmarks and real-world TAs, we compare three different system configurations: (i) the standard OP-TEE deployment (No RZ); (ii) the \project deployment (RZ); and (iii) the \project deployment with no trusted OS preemption from the REE (RZ no IRQ).   

%In this section we evaluate the prototype \project implementation by measuring performance overhead and analyzing security aspects. 
%The overhead evaluation is performed on the iMX8MQ which provides four Arm Cortex-A53, one Arm Cortex-M4. 

%We base our work on TF-A (version 2.0), OPTEE-OS (version 3.7.0), and other components (OPTEE client library and OPTEE supplicant (version 3.7.0) , OPTEE test (branch imx\_5.4.3\_2.0.0), Linux kernel (5.4.24), imx mkimage (branch imx\_5.4.3\_2.0.0) ) on Code Aurora IMX repositories~\cite{imxaurora}. For Android we follow NXP provided steps for building Android 10.
%We compare three cases: No \project, is a typical TrustZone deployment; \project, where a system is configured with \project; and \project no IRQ, which is a system deployed with \project but with no Trusted OS preemption, meaning normal world interrupts do not interrupt the Trusted OS. Preventing the Trusted OS from beeing preempted by the normal-world is an optimization we evaluate, due to the high cost of context switching between worlds.






\subsection{Microbenchmarks}
\label{sec:eval_micro}

From a micro perspective, we measured (i) the world switch time and (ii) the GlobalPlatform API invocation time, and we ran (iii) the OP-TEE sanity testsuite (a.k.a. xtest).  

\mypara{World Switch Time.}
We measure the the world switch time, i.e., the amount of time since the SMC call in the normal world till the execution of first instruction on the trusted OS. To measure the world switch time, we used the AArch64 generic timer, which features a 64-bit cycle counter running at 8.33MHz. We measured the context switch time for the the standard OP-TEE deployment and compared with \project. Reported results translate the average of 1000 collected samples. At the end of each iteration, we flush the caches, so that each sample does not translate the hot-cache effect of the previous running. We observed an average 13x increase due to \project, i.e., the world switch time increased from an average of 47.5 clock cycles (5.7 microseconds @ 8.33 MHz) to 624.1 clock cycles (74.9 microseconds @ 8.33 MHz). This significant increase translates the cumulative penalty of: (i) the additional \project trampoline and gatekeeper execution time; (ii) the AP-MCU requests; (ii) the penalty of running a portion of the trampoline with caches disabled; (iii) the time of the cache maintenance operations; and finally, (iv) the cold cache effect on the trusted OS while fetching the first instructions. Although, at a first glance, a 13x penalty may suggest a prohibitive performance cost for a system, we will see, in the remaining of this section, that the \project overhead gets considerably smaller (till the point of becoming negligible) while we flow to a macro perspective.    
% No_RZ	47.5 ticks	5.70 us	2.9 std_dev
% RZ	624.1 ticks	74.90 us 11.0 std_dev 13x slower

%We first measure the impact on world switching, in particular we measure the time it takes for a call issued by the normal world to reach the Trusted OS. 
%With No \project, we observe almost one 0.91us, with \project the time to switch context between the normal world and the Trusted OS increases to 50.29us, a 55x increase. This significant increase is a natural consequence of the amount of time of cache maintenance operations as well as the cold cache effect on the different pieces of software.

\if0
The results are presented in \autoref{tab:ctx}.
%
%
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{ccc}
& Time & Overhead\\
\toprule
No \project & 85.49us & - \\
\project & 420.86us & 4.92x \\
\bottomrule
\end{tabular} 
\caption{Context-switch overhead with \project}
\label{tab:ctx}
\end{table}
\fi

\mypara{GlobalPlatform API.}
We also measure the round-trip time of calling some of the most used GlobalPlatform client APIs. The execution time accounts for the time spent since issuing the API call on the normal world client application till receiving the reply from the TA. This process includes a full round-trip world switch as well as the execution of the trusted OS and TA for handling the request. To measure the execution time, we used the Linux time API with the CLOCK\_REALTIME parameter enabled (i.e., Linux uses the AArch64 generic timer). We collected 1000 samples, while for each sample the APIs were invoked in sequence, following the order in which they are presented in \autoref{fig:api}. While calling the APIs in a particular order impose a cause-consequence effect at the microarchitecture (e.g., hot-cache), we believe this is the most realistic setup, per the standard behaviour of real-world applications. Between each collected sample, i.e., full execution of the nine APIs, we flush the microarchitectural state, so that there is no cumulative effect of the microarchitectural state between samples. According to \autoref{fig:api}, we can build four takeway points. First, the geometric mean of the normalized performance overhead for the nine API benchmarks is 2.32x, i.e., a significant decrease comparing to the 13x overhead imposed at the world switch. Second, we can observe that the three APIs (i.e., \textit{OpenSession}, \textit{InvokeCommand}, and \textit{CloseSession}) that explicitly call the trusted world has a larger penalty, ranging from 2.33x to 4.08x. The \textit{InvokeCommand} and \textit{CloseSession} APIs are the ones that take less time to execute, and thus the ones with the bigger overhead, due to the over-penalty of cache-related operations. Third, from the remaining six APIs, three have almost no penalty. Notable exceptions encompass the two pair of APIs related to shared memory. This is related to the configuration of the shared memory on OP-TEE, i.e., disable dynamic shared memory. Because dynamic shared memory is disabled, the \textit{AllocateSharedMemory} implementation is identical to the \textit{RegisterSharedMemory}. While running the \textit{RegisterSharedMemory} API, there is no explicit call to the trusted world, and so the code and data is already cached. The same applies for the release operation. Finally, we can observe that the preemption of the trusted OS from the REE (RZ No IRQ) slightly decreases the overhead, i.e., the geometric mean reduces from 2.32x to 2.28x.
%RZ: 2.32;       RZ_No_IRQ: 2.28;



%\david{geometric mean results: RZ: 2.00; RZ\_No\_IRQ: 2.01;}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/api_barchart.pdf}
    \vspace{-0.6cm}
    \caption{\project overhead and duration of main GlobalPlatform APIs}
    \vspace{-1.5em}
    \label{fig:api}
\end{figure}

%\david{Surprisingly we observe overheads in calls which do not invoke the the secure world. This is caused by the sequential nature of the test when combined with the cache-maintenance operations. For example TEEC\_Invoke command, performs a Trusted OS call which will clear all caches, while TEEC\_Allocate\_Shared\_Memory does not invoke the Trusted OS, but suffers from the cache maintenance operations performed prior, and the same is true for TEEC\_ReleaseAllocatedSharedMemory. These functions will not invoke the OS because we've disabled dynamic shared memory in OPTEE. The following two API calls essentially perform the same operations as before, again, due to disabling dynamic shared memory, and thus do not call the Trusted OS.}

\if0
\begin{verbatim}
TEEC inti ctx -> no TOS call
open session -> TOS call
invoke -> TOS call
allocate shmem -> no TOS call (porque disabilitamos dyn. shmem) suffers from cache misses fro mbefore
release allocated shmem -> no TOS call (porque disabilitamos dyn. shmem) suffers from cache misses fro mbefore
register shmem -> no TOS call (porque disabilitamos dyn. shmem) same operation has allocate shmem, already in cache
release registered shmem -> no TOS call (porque disabilitamos dyn. shmem) same operations as release allocated mem already in cache
close session -> TOS call
finit ctx -> no TOS call
\end{verbatim}
\fi



\if0
Measure xtest testsuite overheads. These are the categories pros authors used
\begin{itemize}
    \item storage-stress benchmark\_ 1001 + 1002 + 1003
    \item sha-stress - benchmark\_ 2001 + 2002
    \item aes-stress - benchmark\_ 2011 + 2012
    \item os - 1001 + 1002 + 1003 + 1004 + 1005 + 1006 + 1007 + 1008 + 1009 + 1010 + 1011 + 1012 + 1015 + 1016 + 1017 + 1018 + 1019 + 1020 + 1021 + 1022
    \item - shared memory - \_7000
    \item concurrency - 1013
    \item SDP - 1014
    \item socket - \_2
    \item crypto - \_4
    \item global platform - \_5
    \item storage - \_6
    \item keymanager + derivation + certificates - 800x, 810x
    \item average
\end{itemize}
\fi


\mypara{xtest test suite} OPTEE provides a suite of regression tests, called xtest, to verify the correct implementation of the trusted OS and related APIs. We used xtest (branch imx\_5.4.3\_2.0.0) to evaluate the impact of \project on the execution of different TEE functionality, i.e., trusted OS core features, cryptographic operations, secure storage, key management, etc. The suite encompasses a total of 95 test, grouped into nine groups. The suits also provides seven benchmarks aiming at assessing the performance of cryptographic- and storage-related operations (trusted storage, AES, SHA). Each individual test exercise a set of the Global Platform APIs, i.e., open and closes a session and invoke specific commands. We measure the execution time for the complete run of each test/benchmark, which includes a call in the REE, running the test in the trusted world, and returning to the normal world. We measure the time by using the Linux time API. We collected 1000 samples for each test/benchmark. \autoref{fig:xtest} presents a summarized view of the results, represented by the geometric mean of all test for the same group. Unit tests are represented in nine groups on the left, while benchmarks are represented into three groups on the right. {\color{orange}A detailed view of the results per test/benchmark can also be found in Appendix XPTO.} The first conclusion that can be taken is that geometric mean of the performance overhead for all tests and benchmarks is 1.71x. The group of tests that has a bigger impact are the TEE Internal API and Global Platform API, i.e., 2.96x and 2.37x, respectively. These group of tests are the ones with smaller execution time and simpler trusted world operations. Interestingly, the geometric mean of the performance overhead for the Global Platform API tests is very similar to the ones presented before. The deviation can be justified by the higher number of APIs that is tested in xtest. On the other hand, tests such as mbed TLS and key derivation perform fewer but complex operations on the trusted world. This results in a smaller overall penalty. The network socket group corresponds to the implementation of secure sockets in OP-TEE, which leverage a normal world client application (i.e., tee-supplicant) to securely communicate through a socket. Naturally these tests required a large number of world switches, from sock management to retrieving data. Notwithstanding, because the complexity of the operations performed in the trusted world is significant, the performance overhead is relatively lower when compared to the TEE API groups.

To validate our conclusions, we performed a small experiment aiming at modifying one particular unit test (i.e., 4007 symmetric). The test consists in performing different symmetric encryption schemes (e.g., AES, DES, HMAC-MDS, etc) for incremental key sizes (e.g., 64-, 128-, 512-bit). The standard implementation encompasses a total of 3978 trusted world calls per run. We modified the implementation to perform all iterations in a single TA call. By simply batching all operations and processing them in a one-time trusted operation, we reduced the number of calls to the trusted to 96, and were able to decrease the performance overhead from 3.6x to 1.08x. In summary, we identified two main factors impacting the performance overhead, i.e., (i) the number of trusted OS calls and (ii) the complexity/duration of the operation running in the trusted world (mainly the logic of the TA). Workloads encompassing simple TA operations/logic with higher number of world switches will translate in a significant performance overhead. In contrast, workloads encompassing complex TA operations with small number of world switches will translate in a negligible performance overhead.



\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/xtest_simple_barchart.pdf}
    \vspace{-0.8cm}
    \caption{Geometric mean of \project's overhead in xtest test suite.}
    \label{fig:xtest}
\end{figure}
% linha a tracejado com a média
% máximo percentil 5\% 95\%
% Escala de 0% a 100%
% TODO: Expirementar as mesmas escalas

%Overall \project affects xtest the most, the shorter the code they execute in the trusted world is and the higher the number of trusted OS and TA calls. For example four of the most affected groups of tests, Cryptographic algorithms, TEE Internal Arithmetic API, GLobal Platform API, and storage perform a large number of quick operations on the secure world in their individual tests. On the other hand tests such as mbed TLS and key derivation, perform fewer but complex operations on the secure world. The network socket tests is the OPTEE implementation of secure sockets which leverage a normal world service (i.e., tee-supplicant) to securely communicate through a socket. Naturally these tests required a large number of context switches between world, from sock management to retrieving data. However because the amount of processing in OPTEE is significant, overheads are relatively low compared to other tests. Tests for OS core features, perform a plethora of tests within the OPTEE itself. The tests most responsible for the overhead are test 1001 and 1020. 1001 is a quick tests (less then 150us without \project) which will naturally be largely affected by the cache maintenance operations. Test 1020 tests a specific synchronization algorithm which is affected by the hard sequentialism \project imposes on trusted OS workloads. The last regression test, test for shared memory. Because we’ve disabled dynamic shared memory in OPTEE shared memory related tests will not invoke OPTEE, however in this group there are two tests which test that OPTEE correctly handles request for opening non-existant or invalid TAs. The benchmark suite of tests will exercise OPTEE in storage, SHA and AES performance with large number of calls to OPTEE.



\if0
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{images/benchmarks/migration_barchart.pdf}
    \caption{xtest 4007\_symmetric test with normal world code migrate to execute in a TA, and in its original form.}
    \label{fig:migration}
\end{figure}
\fi

\subsection{Real-world Applications}
\label{sec:eval_TAs}

%\sandro{Change order between bitcoin wallet and DRM player. I would change the title to "Secure Applications Overhead" ou qualquer coisa assim... }

To understand the performance overhead of \project in real-world use cases, we evaluated two different TAs: (i) a Bitcoin wallet; and (ii) a DRM Player. We believe this two TAs are representative of completely different profiles with regard to the frequency the trusted world is invoked. The bitcoin wallet represents a TA invoked with a low-frequency pattern, similar to cryptographic key management (e.g., keymaster) or biometric authentication (e.g., fingerprint service), while the DRM player represents a use case requiring high-frequency interaction between the normal and trusted world.

\mypara{Bitcoin wallet.}
To evaluate the crypto wallet TA, we leveraged an open source Bitcoin wallet implementation \cite{bitcoinwallet}. The Bitcoin wallet TA provides a set of services which includes the creation and deletion of a master key, access the mnemonic for a master key, sign a transaction, and get the address of the wallet. We believe these services are the ones that represent common operations performed by TAs with a similar profile. To measure the execution time, we also leveraged the Linux time API. \autoref{fig:bitcoinwallet} depicts the normalized performance overhead for the average of 1000 samples. The geometric mean of the performance overhead stands for 1.50x for the vanilla \project implementation, and 1.48x for a non-preemptible zone configuration. The wallet services that presents the higher overhead are related to simple one-time operations. For instance, the absolute execution time of the operation responsible for checking if a master key exists is considerable smaller (11.9ms for the standard OP-TEE deployment) than the other services, and thus the penalty is higher. Notwithstanding, the results clearly demonstrate that the impact of \project in longer time-consuming operations, e.g., Bitcoin sign transaction (the one likely to be executed more frequently) is low (1.2x) and one order of magnitude smaller than the overhead observed in the raw world switch. This highlights that the expected performance penalty for workloads with a similar TA profile is reasonable and will not affect the overall user experience. 
%Furthermore, disabling the preemption on the trusted OS presents a marginal improvement.
%We narrowed our evaluation to the \textit{sign transaction} and \textit{get wallet address} services. ... , while services such as \textit{create master key} and \textit{delete master key} are seen as one-time operations

%     1 check key -> open secure storage -> will cause multiple calls to normal world as the OS accesses the ree fs
%     2 generate mnemonic/key -> generate mnemonic, store key in the ree fs (various calls to supplicant) 
%     3 generate mnemonic/key -> same as above, but mnemonic is an argument
%     4 delete mnemonic/key -> open object (ree fs), delete it (ree fs)
%     5 sign transaction -> get master key from ree fs, do many cryptographic operations
%     5 get address -> get master key from ree fs, derive public key (wallet address)
%     
%     every open, read, and close will invoke the normal world
%\david{command 1 being the simplest (and shortest running) is the most affected by \project. this command tries to open a file (holding the master key) from the REE, and thus will perform calls to the normal world. Similarly, command 4 is also a simple command which accesses the master key storage in the REE fs, and will delete it the key if it exists. By doing more work than command 1, the relative runtime execution of the command will have lower overheads. Other commands do significant amounts of cryptographic operations, and the penalties involved from context switching, and this cache maintenance, are less pronounced.}

%We use a previous implementation of a bitcoin wallet~\cite{bitcoinwallet} to be executed as a TA in a Trusted OS. We measure the time to execute with the \emph{time} Linux utility, and observe the \emph{real time} component of the output. Overhead for TA operations goes up to 2.2x for the command that executes in least amount of time, however for other commands the overhead is smaller, as low as 1.2x. Overall, disabling interrupts in the Trusted OS achieves modest performance improvements. The results are presented in \autoref{fig:bitcoinwallet}.

\if11
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/benchmarks/wallet_barchart.pdf}
    \vspace{-0.6cm}
    \caption{\project overheads on a bitcoin wallet use case.}
	\vspace{-0.3cm}
    \label{fig:bitcoinwallet}
\end{figure}
\fi

\mypara{DRM Player.}
To implement the DRM player service, we leveraged the open source OP-TEE Clearkey plugin~\cite{opteeclearkey} and the media player ExoPlayer~\cite{exoplayer}. This systems approximates to a security level 2 (L2) DRM compatible setup~\cite{widevinelevels}, where video is decrypted within the TEE, but processed/decoded in the normal world. For instance, with the Clearkey plugin, video content is split into subsamples, which are decrypted within the TEE; after decryption, subsamples are decoded in the normal world and the content is presented to the user. Among the three security levels, the L2 DRM configuration translates the worst-case scenario for performance, since the process is split among the two worlds. To evaluate the DRM service performance we measured the (i) execution time for decrypting one subsample for three different resolutions and frame rates (\autoref{fig:drm_macro}, left) and (ii) the time elapsed between decoded content (\autoref{fig:drm_macro}, right). According to \autoref{fig:drm_macro}, three main conclusions can be drawn. First, the geometric mean of the normalized performance overhead for the DRM subsample decryption is 1.64x. Intuitively, the higher the frame rate, the bigger the penalty, i.e., for the 1920x1080@60 configuration the expected performance penalty is 2x. Second, the \project configuration which lacks preemption (RZ No IRQ) slightly improves the performance of the decryption process, reducing the geometric mean of the normalized performance overhead to 1.4x. This benefit is also noticeable in the the processing of the decoded frames and the rendering of the final image (\autoref{fig:drm_macro}, right). Third, although there is a penalty in the decryption process, this penalty is not noticeable in the playback of the video and does not impact the user experience.    

%{\color{orange}
%Although we observed 1.5x increase in subsample decryption times, this falls well bellow the ~16ms mark for 60fps content and 41ms for 24fps content.
%We also observe a slight improvement in performance, to around 1.4x, by disabling TEE interrupts. }

%{\color{orange}Although \project causes overheads in decrypting subsamples, the smooth playback of media is not compromised. In ExoPlayer, processing decoded frames for rendering the final image occurs at periodic intervals. We measure the time elapsed between decoded content. The results are presented in \autoref{fig:drm_macro}. Although the period between processing frames increases slightly the overhead is not perceptible to the end-user. Each subsample is decrypted individually, and due to the costs incurred by context switching, we believe that playing DRM content in a \project enabled system can be significantly optimized by increasing the number of subsamples decrypted per TEE call.}

%\david{geometric mean DRM subsample decryption: RZ: 1.64; RZ\_No\_IRQ: 1.43;}
%\david{geometric mean DRM elapsed time: RZ: 1.01; RZ\_No\_IRQ: 1.00}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\columnwidth]{images/benchmarks/drm_barchart.pdf}
    \includegraphics[width=0.49\columnwidth]{images/benchmarks/drm_macro_barchart.pdf}
    \vspace{-0.6cm}
    \caption{DRM use case test subsample decryption (center), processing interval (right).
    }
    \label{fig:drm_macro}
	\vspace{-0.3cm}
\end{figure}


\subsection{Normal world impact}
\label{sec:eval_NW}

To measure the impact of \project on the overall normal world execution, we ran the PCMark (v3.0) for Android benchmark. The benchmark is mainly used to measure the performance of smartphones and tablets, by using tests based on everyday activities. The suite consists of five real applications (e.g., web browsing, data and video editing), with the Work 3.0 benchmark translating the performance of the whole system. Running PCMark produces a score with higher numbers indicating better performance. Running PCMark on a typical smartphone takes around 10 minutes. We compared five different system configurations: (i) the standard OP-TEE deployment, with no trusted world calls while running PCMark (No RZ); (ii) the \project deployment, with no trusted world calls while running PCMark (RZ); and the \project deployment with explicit trusted world calls every (iii) one, (iv) ten, and (v) twenty seconds, while running PCMark. At the trusted world, one toy TA performs a simple sum operation and returns to the normal world. Results are depicted in \autoref{fig:PCMarkv3}. The main takeway from \autoref{fig:PCMarkv3}, is that if the trusted world is not stressed, \project has no almost no penalty in the overall performance picture of the system.  


%{\color{orange}The final test result is represented by \emph{Work 3.0 performance score}. We perform measurements on a setup configured without \project, configured with \project without periodic invocation, configured with \project and with periodic invocations to a Trusted OS in 1s, 10s, and 20s intervals. The more frequent the invocation to Trusted OSes the more performance is affected, as can be observed in \autoref{fig:PCMarkv2}. However, \project does not significantly degrade performance of the normal world if a Trusted OS is not invoked. }

%\david{PCMark Work 3.0, is a benchmark suite that performs tests that mimic common, everyday tasks. Instead of evaluating individual units, the result is a measurement of the performance of a device as a complete unit. The Work 3.0 Performance Score reflects this, as it uses web browsing, photo editing, video editing, data manipulation and writing scenarios to achieve a score of the system's performance.}

\if10
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/benchmarks/nw_barchart.pdf}
    \caption{\project normal world impact measured as impact on PCMark (v3.0) benchmark without invoking a Trusted OS, and with periodic invocations in 1s, 10s, and 20s intervals.}
    \label{fig:PCMarkv3}
\end{figure}
\else
\begin{table}
\centering
\begin{tabular}{cccc}
\textbf{Configuration} & \textbf{Interval} & \textbf{Work 3.0 Score} & \textbf{Overhead} \\
\midrule
No RZ & - & 5020 & 0.00\% \\
RZ & - & 5018 & 0.04\% \\
RZ & 20s & 5018 & 0.04\% \\ 
RZ & 10s & 5002 & 0.36\% \\
RZ & 1s & 4971 & 0.99\% \\

\toprule
\end{tabular} 
    \caption{\project normal world impact measured as impact on PCMark (v3.0) benchmark without invoking a Trusted OS, and with periodic invocations in 1s, 10s, and 20s intervals.}
  \vspace{-2.7em}
    \label{fig:PCMarkv3}
\end{table}
\fi

%\david{Use the Work 3.0 performance benchmark to test the performance of your device. This test takes around 10 minutes on a typical smartphone.}


\subsection{Multiple zones penalty}
\label{sec:eval_mTEE}

To understand the performance penalty of supporting multiple zones, we built two specific test case scenarios. The main difference, implementation-wise, in the trampoline, to schedule a different zone (i.e., trusted OS), is the extra operation required to invalidate the TLB. Thus, in the first case scenario, we measured the execution time of running xtest 4001 on trusted OS 2, while the previous running zone were also running trusted OS 2. In the second test case scenario, we measured the execution time since of running xtest 4001 on trusted OS 2, while the previous running zone were running trusted OS 1. To measure the execution time, we also used the Linux time API. We collected 1000 samples for each test case scenario. For the first test case scenario, it takes, on average, 75.7ms to complete. For the second test case scenario, it takes, on average, 77.5ms to complete, i.e., a 1.8ms (2.6\%) increase. Overall, we believe the extra penalty to provide multiple zones is really small and negligible for the overall performance of the system.     

\if0
\begin{verbatim}
    Ao termos multi-TEEs temos um factor extra de penalização de performance, TLBI invalidate.
    
    é necessário fazer TLBI quando executamos o TrustedOS 2 depois de ter executado o Trusted OS 2 (isto porque fazemos TLBI quando sabemos que o último TEE a executar é diferente do que queremos executar a seguir)
    
    portanto temos dois cenários:
    1) TEE executa "sozinho", onde nõa haverá TLBI
    2) TEE é executado depois de outro (haverá um TLBI)
    
    portanto para avaliarmos fazemos
    Scenário 1:
        TOS2 -> executa uma TA (escolhemos o 4001, mas na verdade poderia ser outro exemplo qualquer)
    
    scenários 2:
        TOS1 -> xtest 1001 (isto chama só TOS, nãoi invoca TAs, na verdade não itneressa. o nosso interesse é que o próximo TOS seja diferente)
        TOS2 -> executa uma TA (escolhemos o 4001, mas na verdade poderia ser outro exemplo qualquer)
\end{verbatim}
\fi
 
%{\color{orange}To measure the impact multiple zones might have in performance, we compare two scenarios. In the first scenario we invoke Trusted OS 2, we use xtest regression test 4001, which will invoke a TA to perform cryptographic operations. On scenario 2, we first invoke a simple operation on Trusted OS1, before calling Truste OS2. This is done by invoking xtest regression test 1001, a simple test which only invokes the Trusted OS. Invoking the trusted OS1 first will result in a TLBI being performed upon a call to Trusted OS2. After Trusted OS1 is invoked, we execute the same xtest test as in scenario 1, regression test 4001, on Trusted OS2. 
%We observe an overhead of 2.6\% corresponding to an average of 1.8ms in a test which takes 77.5ms to execute without invalidating the TLB. We consider this overhead to be negligible, particularly in light of the overhead already incurred by the cache maintenance operations.}


%=======================================================================
%> [SECURITY ANALYSIS]
%=======================================================================

\section{Security Analysis}
\label{sec:sec_analysis}
In this section we present our security analysis. We measure the TCB size and compare to alternative solutions. We also survey 80 CVE vulnerability reports aiming at understanding the number of attacks \project could prevent. 
\if0
\begin{itemize}
    \item Address how CVEs are solved by applying \project (See TFence for a paper that does the same)
    \item Scheme detailing how vulnerabilities are prevented
\end{itemize}
\fi


\subsection{TCB Size}
\label{sec:eval_tcb}


To assess the TCB size, we counted the number of source lines of code (SLOC) using the SLOCCount tool. We evaluated the TCB size for a typical OP-TEE deployment, i.e., the TF-A and OP-TEE kernel, and compared with \project. We have also calculated the full TCB size for a set of systems representative of the three main classes of works offering multiple isolated environments, i.e., (i) normal world virtualization (NW-Virt), (ii) normal world enclaves (NW-E), and (iii) trusted world same privilege isolation (TW-SPI). To assess the full TCB size for the related work, we collected evidence about the additional TCB changes from the papers and calculated the total TCB by adding those values to reference values for TF-A or TF-A plus OP-TEE kernel, depending on the system.     

%\project enables the creation Zones, sandboxes for trusted OSes running in s-EL1. With this, the runtime system TCB is reduced considerably, as a malicious trustedOS can no longer compromise the system.

The results are presented in \autoref{tab:tcb_comparision}. We can drawn three main conclusions. First, we can claim that \project reduces the TCB size of a typical TrustZone-assisted TEE system by 88.2\%. It is a significant decrease that is intuitively linked to the removal of the OP-TEE kernel as part of the TCB. Second, we can argue that \project adds a total of 5345 SLOC to the privileged software, which includes the addition of the \project Trampoline code to the secure monitor (1523 SLOC) and the \project Gatekeeper (3,822 SLOC) running in the MCU. Although the \project Gatekeeper code may seem significantly large for the simplicity of the component, it is a consequence of leveraging ready-available board support package (BSP) code from NXP for the current PoC implementation. We believe that a clean-slate assembly implementation (which we strive to implement in the future) would reduce these numbers further to a few hundred SLOC. Finally, comparing \project with alternative designs, we can conclude that \project presents non-negligible advantages. For both the NW-Virt and NW-E class of solutions, it is clear that \project presents a much smaller TCB, which results from building atop less privileged software components. Comparing to TEEv and PrOS, \project also presents non-intuitive security advantages: first, we highlight that a clean-slate implementation of the \project Gatekeeper would push the \project TCB reduction further to +90\%; second, the values represented in \autoref{tab:tcb_comparision} does not account either for (i) the manual engineering effort for removing privilege memory management instructions or (ii) the TCB of binary instrumentation tools used to automate such process (reason to mark those values with an \textbf{*}); and third, the isolation imposed by \project in the trusted world is hardware-enforced while TW-SIP solutions rely on software.

%, which may be not intuitively gathered from \autoref{tab:tcb_comparision}

%, a feature-full open-source TrustedOS, with support for many different platforms, from the TCB. With \project we add 5,345 LoC, spanning both monitor (1523 LoC) and \project controller code (3,822 LoC), when compared against a typical secure monitor deployment. The \project controller large number of LoC is due to our use of readily available board support code, we could optimize the implementation, and due to its simplicity it could be coded in assembly. This would further reduce the TCB as measured in LoC, and make \project controller code formally verifiable.

%We compare \project with similar works that aim to reduce the system TCB, \autoref{tab:tcb_comparision}.
%\project demonstrates significantly reduced TCB as compared to most other works. Comparing to works with similar TCB size, \project makes stronger security guarantees, by not relying on software techniques to establish a sandbox. Instead, \project uses hardware mechanisms to establish zones.

\begin{table}[!t]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.5}
\centering
\footnotesize
\scalebox{0.77}{%
\begin{tabular}{ccccccc}
& & \begin{tabular}[x]{@{}c@{}} Monitor\\TCB\end{tabular} &
\begin{tabular}[x]{@{}c@{}} Trusted OS \\ TCB \end{tabular} & 
\begin{tabular}[x]{@{}c@{}} Add. Priv. \\ Software (SLoC) \end{tabular} & 
\begin{tabular}[x]{@{}c@{}} Total TCB \\ (kSLoC) \end{tabular} &
\begin{tabular}[x]{@{}c@{}} Change in \\ TCB (\%) \end{tabular}\\
\toprule
& Typical & TF-A & OPTEE & - & 255 & - \\
& \textbf{\project} & \textbf{TF-A} & - & \textbf{5345} & \textbf{30} & \textbf{-88.2\%} \\
\midrule
\multirow{2}{*}{ NW-Virt } & PrivateZone \cite{Jang2018} & TF-A & OPTEE & 5,206 & 260 & 2.0\% \\
& OSP \cite{Cho2016} & TF-A & OPTEE & 800 & 256 & 0.3\% \\ \hdashline
\multirow{2}{*}{ NW-E } & Sanctuary \cite{Brasser2019} & TF-A & OPTEE & 656 & 255 & 0.3\% \\
& TrustICE \cite{Sun2015}& TF-A & OPTEE & 283 & 255 & 0.1\% \\ \hdashline
\multirow{2}{*}{ TW-SPI } & TEEv \cite{Li2019} & TF-A & - & 3,800 & 28\textbf{*} & -88.8\%\textbf{*} \\
& PrOS \cite{Kwon19} & TF-A & - & 3,000 & 28\textbf{*} & -89.2\%\textbf{*} \\ 

\bottomrule
\end{tabular}  
}
\vspace{5pt}
\caption{SLOC of the TCB for a typical TrustZone-assisted TEE system, \project, and related work. The reference value for the SLOC for the TF-A secure monitor is 24,607 and the OP-TEE kernel is 230,094.  }
 \vspace{-1.5em}
\label{tab:tcb_comparision}
\end{table}
%Additional privileged software includes additions to the secure monitor code and other software components; in the case of \project it includes the \project Trampoline and Gatekeeper code.
%NW-Virt: Normal World Virtualization; NW-E: Normal World Enclave; TW-SPI: Trusted World Same Privilege Isolation.



\if0
\subsection{Attack Mitigation}
TrustZone-based TEEs have been the target of multiples attacks, which exploit software flaws to obtain privileged execution, extract secrets, or twarth security functionality. We next analyze how these attacks would fare in a system deployed with \project.

\mypara{Attack 1. } By compromising a TA, it is possible to exploit a flaw in a secure driver~\cite{BreakingArmTZ, DeepDive}. Secure drivers have access to mmap, which allows them to map physical memory. The Secure Monitor can then be mapped by the now malicious secure driver, and the attacker can do anything on the platform, including exposing secrets. A master key is one of such secrets. In the Samsung ..., the master key is used by the drcrypto driver for cryptographic operations.
There are two ways in which the master key can be obtained: a) obtaining access to EL3 memory and reading the master key location, b) or via an SMC to the secure monitor.

\mypara{Mitigation 1. } \project mitigates against obtaining the Master Key by preventing the Trusted OS from accessing monitor memory. Because malicious software can longer map the Secure Monitor it can no longer obtain the master key directly. This solves problem 1.a). However, the attacker can still obtain the master key through a Secure Monitor Call (SMC), problem 1.b). To mitigate this, with \project, we argue for implementing cryptographic primitives requiring platform keys, and other system critical features, in a separate Zone which will not reveal the key being used. 

\mypara{Attack 2.} An attacker can compromise a system TA  through the Trusted OS, by first obtaining execution privileges in the Trusted OS \cite{BreakFDE,shen-trustedcore}. This can be used to thwart security functionality. For example, an attacker can obtain the secret key used to encrypt the file system~\cite{BreakFDE} or effectively compromise the fingerprint authentication mechanism~\cite{shen-trustedcore}. 
%The secret key is encrypted by the user password, however it is possible to bruteforce the password on a powerful PC. 

\mypara{Mitigation 2.} \project allows for the secure deployment of multiple OSes. It is possible to prevent a compromised component from zone$_{1}$ from obtaining secrets from other zones, provided that zone$_{1}$ is bug free. Securely developing zone$_{1}$ is easier than doing the some for a single TEE domain hosting all trusted applications. Thus, by using \project to allow more than one TEE to execute in the secure world, a vulnerability in one zone can not be used to obtain secrets from another.
 
\mypara{Attack 3.} By leveraging a TA's access to normal world memory, it is possible to access all memory in the normal world~\cite{gb-exploit6, Aravind2017}. This is possible because the Trusted OS can map the normal world physical memory at will, and in certain scenarios can map this memory unto a TAs address space. With access to normal world memory an attacker can compromise the Linux kernel, for example by creating a back door within seldom used kernel modules. This gives the attacker arbitrary code execution at kernel level of privilege.

\mypara{Mitigation 3.} In \project we can restrict the normal world memory accessible to a Trusted OS. This requires knowledge of what memory is dedicated for sharing memory between the TEE and REE, however, on some platforms TF~-~A already supports modifying an in-memory device tree. This means that TF-A can specify to the kernel which memory is available for sharing information between worlds. Fixing the shared memory space makes it possible for secure monitor to enforce secure-world zones, although, at a cost of not supporting dynamic shared memory, which allows a normal world process to mark part of its memory as shareable with the TEE.

\mypara{Attack 4.} Code reuse attacks. An attacker can leverage control highjacking to compromise the Trusted OS~\cite{gb-exploit4}. In particular the attacker might leverage the presence of privileged operations, for example in the case for Armv7-A or Armv8-A\_aarch32 the DACR registers, which when set to zero disable MMU based memory protection.

\mypara{Mitigation 4.} In \project, we use platform level access control mechanisms to enforce zone access permissions to memory. Even with access to privileged instructions in the Trusted OS, an attacker can not modified these policies, and thus is confined to the specified sandbox. 
\fi

\subsection{Vulnerability Analysis}
% \david{Objectivo. Perceber como CVEs reais quais os ataques que podem ser mitigados}
% \david{Metodologia, 80 CVEs, critério usado para classificação, relacionar com os vetores de ataque. Se o exploit é mitigado ...}
% \david{takeways, main findings, insights - TOs, }
% \david{Component -> ataque vector}
% \david{bullet -> check - unknown}

We next evaluate how deploying \project in real world systems can help mitigate the impact of vulnerabilities present in the various trusted world components. In particular, in light of the fact that we can now contain vulnerabilities inside zones, thus preventing vulnerabilities in one zone from affecting another zone, the normal world, or monitor software.

As part of the the evaluation, we analyze 80 TEE related CVEs reported as critical, and group them based on the affected component: Trusted OS, TA, Cryptographic Implementation, Hardware Issue and Bootloader.
For vulnerabilities that affect the TEE, but present insufficient information to determine if the affected component is Trusted OS or TA, we label them as TO/TA.
In our analysis we consider a \project deployment model where TAs are deployed with a dedicated trusted OS (e.g., a library OS) in dedicated zones.
A vulnerability is considered mitigated if it only affects these components but cannot be used to attack other system components. \autoref{tab:security-table} summarizes our analysis. 

\input{secure_analysis_table}

\mypara{Trusted OS and Trusted Applications Vulnerabilities.}
%Trusted OS and Trusted TA vulnerabilities, are related in that often times a vulnerability in a TA can be leveraged to exploit vulnerabilities and flaws in the Trusted OS~\cite{Cerdeira2020}. 
With \project, vulnerabilities and flaws in the Trusted OS and TAs are mitigated in as much as the vulnerability now affects only the Trusted OS and corresponding TAs. 
%Most of the vulnerabilities in \autoref{tab:security-table} pertain Trusted OS and TA, and the impact of a vulnerability in them can be substantially reduced. 
However, there are cases in which compromising a TA is enough to allow attackers to meet their goals. One example of this is \href{https://www.cvedetails.com/cve/CVE-2018-5210}{2018-5210}, a vulnerability which allows an attacker to gains TEE privilege execution, and incidentally allows the attacker to retrieve device unlocking information, which can then further be used to obtain the device unlocking code. We consider this vulnerability mitigated, because an attacker can not affect other system components. 
Another problem is miss-configuration. For example, \href{https://www.cvedetails.com/cve/CVE-2017-18311}{2017-18311}, pertains a miss-configuration vulnerability where a custom implementation of a TrustZone controller allows other masters to escalate privileges. Because \project is orthogonal to TrustZone and we only aim to reduce Trusted OS privileges, and because the attack is a misconfiguration of TrustZone related access control policies, an attack leveraging this vulnerability would not be prevented. However, \project could be extended to consider other bus masters in protecting both normal world, and trusted world software, provided that the platform's PPC is flexible enough to do so.

\mypara{Hardware Vulnerabilities.} 
The \href{https://www.cvedetails.com/cve/CVE-2017-18282}{2017-18282} CVE, is a hardware issue where a hardware component of the system can be manipulated by a malicious agent from the normal world into performing secure data accesses. These types of issues are not prevented by \project, as we only protect against secure accesses while the Trusted OS is executing.

\mypara{Cryptographic Vulnerabilities.} 
Cryptographic issues are beyond the scope of \project, even without common software vulnerabilities in Trusted OSes and Trusted Applications, the security functionality provided by these components is still dependent on the correct and careful implementation of cryptographic primitives and schemes.

\mypara{Bootloader Vulnerabilities.} 
The bootloading stage occurs before the secure monitor starts execution. At this stage the CPU executes in the secure world and flaws at this point may enable attackers to load arbitrary code at the highest privilege level. We consider these types of problems out of the scope of \project as the mechanism used to load the runtime TCB are the root of all trust in the system.


%\mypara{2016-2431} This vulnerability refers to a lack of system calls parameter validation on the Trusted OS. It assumes code execution privileges in a TA, and enables attackers to build read and write gadgets to the Trusted OS. This vulnerability fits the attack scenario where an attacker gains Trusted OS level privileges. With Trusted OS level of privileges an attacker can access any memory and every resource available to the CPU. Although \project does not address the vulnerability directly is prevents a compromised Trusted OS from attacking the normal world and the secure monitor, thus reducing the impact of this vulnerability.


% \david{TODO: escolher 4 ou 5 vulnerabilidades}
\if0
2016-2431	"The Qualcomm TrustZone component in Android before 2016-05-01 on Nexus 5, Nexus 6, Nexus 7 (2013), and Android One devices allows attackers to gain privileges via a crafted application, aka internal bug 249688009.

This vulnerability assumes code execution privileges in QSEE TA.
TrustZone kernel does not perform any validation on QSEE-supplied arguments (more specifically, it freely uses any given pointers), meaning that at the time all syscalls were vulnerable. Vulnerable syscalls allow for building read and write gadgets to the Trusted OS.
"


2017-17176	The hardware security module of Mate 9 and Mate 9 Pro Huawei smart phones with the versions earlier before MHA-AL00BC00B156, versions earlier before MHA-CL00BC00B156, versions earlier before MHA-DL00BC00B156, versions earlier before MHA-TL00BC00B156, versions earlier before LON-AL00BC00B156, versions earlier before LON-CL00BC00B156, versions earlier before LON-DL00BC00B156, versions earlier before LON-TL00BC00B156 has a arbitrary memory read/write vulnerability due to the input parameters validation. An attacker with the root privilege of the Android system could exploit this vulnerability to read and write memory data anywhere or execute arbitrary code in the TrustZone.


2017-6294	"In Android before the 2018-06-05 security patch level, NVIDIA Tegra X1 TZ contains a possible out of bounds write due to missing bounds check which could lead to escalation of privilege from the kernel to the TZ. User interaction is not needed for exploitation. This issue is rated as high. Version: N/A. Android: A-69316825. Reference: N-CVE-2017-6294. 

NVIDIA TLK TrustZone OS contains a potential vulnerability in the logging driver where the software writes data after the end or before the beginning of the intended buffer, which may lead to arbitrary code execution, denial of service, or escalation of privileges. - buffer overflow may lead to arbitray code execution within the TEE"


2015-4422	"The TEEOS module of Huawei Mate 7 smartphone which is used to realize the function of fingerprint identification has an input check error, which enables the attackers with the root permission to modify kernel-mode memory data of TEEOS module, which could make system break down, TEEOS be tampered or malicious code execution. (Vulnerability ID: HWPSIRT-2015-03012)

There is a arbitrary memory read/write vulnerability in the hardware security module of some Huawei smart phones due to the input parameters validation. An attacker with the root privilege of the Android system could exploit this vulnerability to read and write memory data anywhere or execute arbitrary code in the TrustZone. (Vulnerability ID: HWPSIRT-2017-01060)
http://www.huawei.com/en/psirt/security-advisories/huawei-sa-20170306-01-smartphone-en - An attacker can write arbitrary code to TEE global task memory, this allows him to obtain execution wiithin the global task by provoking a crash and forcing code execution to an attacker controlled address
 - a system call vulnerability allows an attacker to arbitrarily write to any memory address within the TEE, which allows him for example to bypass security checks for accessing fingerprint images

Security Advisory - Arbitrary Memory Read Write Vulnerability in Huawei Smart Phones
"
\fi

\if0

\subsection{Attack Surface}
%\david{Mitigations are also attack surface}

The attack surface for a typical TrustZone assisted TEE system includes all the SMCs and interfaces the secure monitor, Trusted OS and Trusted Applications provide to the normal world.

Attack surface becomes:
\begin{itemize}
    \item Guessing the authentication token
    \item Connection with the micro-controller
    \item SMC calls (calls to the monitor)
    \item Interfaces TAs provide
    \item Trusted OS syscalls
\end{itemize}

\fi

Although \project cannot prevent vulnerabilities from occurring in TAs and in Trusted OS, cannot protect against system miss-configurations, poor cryptographic implementations or defective bootloaders, overall \project mitigates against 86.5\% of the analyzed critical vulnerabilities by preventing vulnerabilities from reaching outside of their dedicate Zone.

%=======================================================================
%> [DISCUSSION]
%=======================================================================
%\newpage
\section{Discussion}
\label{sec:discussion}

\mypara{Available hardware to implement \project.} 
To implement \project, we leveraged an OEM-specific platform partition controller, i.e., NXP's RDC. However, in \ref{sec:plat_req}, we have abstractly modeled the PPC so that \project would be ported to other platforms offering similar custom facilities. For example, the Zynq UltraScale+ MPSoC provides a Xilinx-specific memory protection unit and peripheral protection unit (XMPU and XPPU, respectively) \cite{xilinxisol} while Qualcomm Snapdragon SoCs feature the External Protection Unit (XPU) \cite{qualcommxpu}. Both fulfill all PPC requirements. Besides vendor-specific components, the Arm System MMU (SMMU) is an architectural standard and widely available component that would also be able to fill the same role, although with the increased performance penalty of page-table walks. Platform management cores are also a clear trend in modern platforms, which due to the hardware complexity tend to embedded an increasing number of ACUs for power management and security operations.

%\jose{is it necessary to mention management cores?} \david{as we are pressed for space, I dont' think it's worth it really. Maybe say somehting like, platform mangement cores are already present in various platforms to perform, power mangement or serving as a senser hub, In \project we require a dedicate security one (qualcomm has one in their latest flagships)}

\mypara{Performance vs Security Trade-Off.}  
To guarantee the correct sandboxing of zones, \project requires extreme measures, i.e., on a world-switch, a core must flush the full cache hierarchy and halt the other cores from the cluster. As shown in $\S$\ref{sec:eval}, although, at the micro view, there are a non-negligible overhead, from a macro perspective, real-world applications does not impact the user experience. These performance impact might still be further minimized. As described in $\S$\ref{sec:mult}, \project will benefit from multi-cluster platforms, where one cluster might continue executing in the normal world while the other runs a zone. Also, optimizations such as batching of a zone's invocations would amortize the costs of world-switching. On the other hand, \project's approach can contain or even fully mitigate a large number of attacks (see $\S$\ref{sec:sec_analysis}). In essence, we believe \project is trading a small decrease in performance for huge security benefits. 

\if0
\subsection{Deployment In Other Platforms}\label{sec:otherplat}
\mypara{Xilinx Protection Units.} Xilinx has also developed and included in their Zynq UltraScale+ MPSoC portfolio a set of protection units complementary to TrustZone~\cite{}. The Xilinx memory protection unit (XMPU) and the Xilinx peripheral protection unit (XPPU) are system-level controllers that verify if a particular bus master is explicitly allowed to access a specific address (memories and peripherals). There are a total of eight XMPUs for protecting transactions into the DDR, the OCM, and the interconnect (e.g., SATA and PCIe). There is one XPPU, which allows for protecting peripherals, message buffers, and inter-subsystem communication channels. A master ID list is used to define the masters that are allowed to access peripherals. Similarly to the i.MX8 families, in Zynq UltraScale+ devices the quad Cortex-A53 cluster has the same master ID for all of its cores, making it impossible to use the XMPU and XPPU to create security domains per core.
\fi

\mypara{\project vs ArmV8.4 vs Armv9.} In Armv8.4 and Armv9, Arm introduced architectural features that are able to provide similar security properties to \project's. In particular, the protection of the REE and monitor from the trusted OS, as well as hosting multiple isolated trusted OSes. In Armv8.4, the S.EL2 \cite{armv84sel2} enables the execution of an hypervisor in the secure world. The Armv9 confidential computing architecture extends the number of worlds, introducing the concept of realms \cite{armv9realms}. Realms are essentially virtual machines that execute isolated from their own hypervisor, which itself is hosted in the normal world. Notably, in Armv9, the monitor is completely isolated from the secure world. %While in this architecture, the secure world is targeted to deploy static security services and firmware, the realm world is meant to host dynamically instantiated realms that contain either full-blown OSs or small TA unikernels. 
%Realm interactions with the hypervisor must be mediated by the Realm Manager running in EL2 of the realm world.
While both approaches seem promising, to our best knowledge, there is only a small number of Armv8.4 hardware implementations available to date, and none of Armv9. Given the long hardware development and manufacturing cycles, widespread availability of these platforms probably still lies many years ahead. In contrast, \project can be deployed in readily and widely available COTS SoCs. Furthermore, both approaches enlarge the TCB by requiring a privileged software component to manage VMs, either the secure hypervisor or the Realm Manager. \project maintains the traditional TrustZone model and only slightly modifies it to achieve its security properties. This allows it to maintain a minimal and immutable TCB.
% Arm foresees these to be developed to the highest standards of software engineering to achieve minimal, correct and impervious implementations. However, one cannot completely rely on this, as it was also the initial promise of TrustZone software itself. The evolution of requirements and services will likely bloat both software stacks.
%from all others, in particular, 
%: non-secure/normal, secure, monitor and realm \cite{armv9realms}.

%{\color{orange} ... Starting from ArmV8.4, TrustZone features a secure world hypervisor designed to provide different execution environments within the secure world itself, and which will also enable the protection of normal world, and monitor memory. However, platforms featuring the new architecture are not yet widespread, meaning that there is a lack hardware solutions for achieving the goals we propose. Additionally ReZone can be applied to already existing platforms which meet the necessary hardware requirements as discussed in ($\S$\ref{sec:plat_req}) ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... Here we are going to discuss Armv8.4 and Armv9 ... }

%=======================================================================
%> [RELATED WORK]
%=======================================================================
\section{Related Work}
\label{sec:related}

\par There are several security-oriented hardware architectures that have been devised to provide basic underlying primitives for the creation of TEE systems~\cite{Maene2018, Pinto2019, Cerdeira2020}. These TEE-enabler hardware technologies include: \textbf{CPU extensions} such as Intel SGX~\cite{Costan2016_2}, Arm TrustZone~\cite{Pinto2019}, and Sanctum~\cite{Costan2016}; separate \textbf{co-processors} such as the Apple SEP~\cite{Tarjei2016} and the Qualcomm SPU~\cite{SPU2019}; dedicated \textbf{security chips} such as the TPM~\cite{TPM2019}; and hardware support for \textbf{secure virtualization} such as AMD SEV~\cite{SEV2019} and Arm Realms~\cite{armv9realms}. Recently, academia has been focused in exploring RISC-V to propose novel TEE hardware architectures~\cite{Nasahl2020, Bahmani2021}, e.g., CURE~\cite{Bahmani2021} and HECTOR-V~\cite{Nasahl2020}. In our work, we leverage COTS hardware primitives to provide augmented isolation within the TEE.

% proposes a secure TEE design strategy using a heterogeneous CPU architecture

%TyTAN~\cite{} and TrustLite~\cite{} are preeminent examples of hardware TEE architectures for resource-constrained embedded devices. 

%\par Contextualize TEE hardware with systems... In the following, we describe different approaches aiming at ... 

\mypara{Hardware-enforced TEE systems.} There are a plethora of augmented TEE systems aiming at offering additional security guarantees. Komodo~\cite{Ferraiuolo2017} implements a small TEE monitor which provide sealed storage and remote attestation as originally specified for SGX enclaves. TLR \cite{Santos2014} and TrustShadow \cite{Guan2017} implement lightweight runtimes within the trusted world aiming at shielding security-critical applications from untrusted OSes. TrustICE~\cite{Sun2015} and Sanctuary~\cite{Brasser2019} leverage the TZASC to create enclaves within the normal world. These enclaves are isolated and cannot access the REE, but the trusted OS has full access to the system. TrustICE has multi-core limitations, while Sanctuary falls short on depending on TZASC features not available in any COTS SoC release to date. CaSe~\cite{Zhang2016_3} and SecTEE~\cite{Zhao2019}  allows TAs to run entirely from the cache and and on-chip memory, respectively. CaSe~\cite{Zhang2016_3} ensures that TA state is encrypted while written back to main memory. Ginseng~\cite{Yun2019} protects variables tagged as "sensitive", by allocating them on CPU registers and encrypting them before saving in memory. Keystone~\cite{Lee2020} and MultiZone~\cite{Garlati2020} leverage the hardware primitives available on the standard RISC-V ISA, i.e. physical memory protection (PMP) to isolate individual enclaves.  
%SKEE~\cite{Azab2016} ...



\mypara{Virtualization-aided TEE systems.} Overshadow~\cite{Xiaoxin2008}, Trustvisor~\cite{mccune2010trustvisor}, and Inktag~\cite{McCune2010} implement hypervisor-based security architectures for Intel and AMD. In the context of TrustZone-based systems, vTZ~\cite{Hua2017}, OSP~\cite{Cho2016}, and PrivateZone~\cite{Jang2018} leverages the virtualization extensions available in the normal world (NS.EL2) to implement isolated environments. These approaches have some drawbacks, which includes TCB augmentation, performance decrease, and intrusive design. OSP~\cite{Cho2016} tries to minimize the performance impact by activating the hypervisor on-demand. With Armv8.4-A, Arm introduced the secure hypervisor mode (S.EL2) and the Hafnium hypervisor~\cite{hafnium}. Our solution does not rely on any hardware virtualization support, and thus can be used in combination with existing hypervisors and support legacy systems.
%The idea of leveraging hardware virtualization support to implement isolated environments is not a new endeavour.
%, while providing additional security guarantees.


\mypara{Same-privileged Isolation.} Same-privileged isolation, also referred to as \textit{intra-level} isolation~\cite{Yeongpil2017}, is a well-established software technique to harden monolithic OS (e.g., \textit{nested kernel}~\cite{Dautenhahn2015}), hypervisors (e.g., \textit{Nexen}~\cite{Shi2017}), and TEEs~\cite{Li2019, Kwon19}, typically by interposing on all updates to virtual memory translations to assert protections on physical memory. TEEv~\cite{Li2019} and PrOS~\cite{Kwon19} use same-privilege isolation to secure a minimalist hypervisor from trusted guest OSes, due to the lack of hardware virtualization support in the trusted world before Armv8.4-A. Both solutions rely on manual engineering effort or binary instrumentation tools for removing privilege memory management instructions. 

%Our solution don't include a secure hypervisor as part of the TCB and we do not use same-privileged isolation but rather ... (\textit{page table mediation}) ... to harden the secure OS from accessing the REE.   




%OSP~\cite{Cho2016}: Their work enables TAs to run on the normal world by using an hypervisor. 2 stage translation overheads are mitigated by only activating the hypervisor when TAs need to run. Our work does not require an hypervisor to be dedicated to the TAs, freeing that privilege level for other applications.

%TrustICE~\cite{Sun2015}: Their work enables TAs to run on the normal world by suspending the REE-OS on all cores while the TA is running. Non-running TAs are protected by marking their memory as secure. Biggest disadvantage is suspending the REE-OS to run TAs, our approach does not require this to provide multiple runtime environments.

%Sanctuary~\cite{sun2015trustice}: Their work enables TAs to run on the normal world by taking advantage of non-common platform features and hardware. Their work relies on each CPU core having its own master ID and this ID being used in bus accesses. It is unknown how widely available this feature realy is. For example the platform they use to test it, the hikey960 does not support it. Further it requires the presence of the TZC-400 which enables each core to have a differente view of what is normal-world memory. Wide use of the TZC unlikely. Going by the Arm-Trusted-Firmware repository, very few platforms actually use the TZC. Our solution is deployable to real world platforms.

%TEEv~\cite{Li2019}: Their work does not provide hardware enforced isolation, rather, it relies on same privilege isolation techniques, as such removing privileged instructions. With this they implement an hypervisor in EL1 to run multiple TEEs on the secure world. In our solution we only require trap and emulation techniques to protect the normal world, which is already "vulnerable" today. To protect environments between one another we achieve hardware enforced access control.

%PrOS~\cite{Kwon19}: Their work does not provide invariant isolation properties rather, they make calls to the monitor in a paravirtualizated-fashion. With this they implement an hypervisor in EL3 and are able to run multiple TEEs on sEL1. In our solution we only require trap and emulation techniques to protect the normal world, which is already "vulnerable" today. To protect environments between one another we achieve hardware enforced access control.

%vTZ~\cite{Hua2017}: Their work provides a TEE environment for each virtual machine, with aid of an hypervisor. They do this by emulating TrustZone features in software.




%=======================================================================	
%> [CONC]
%=======================================================================
\section{Conclusion}
\label{sec:conclusion}

In this paper, we presented \project, a new security architecture that can effectively reduce the privileges of a TrustZone-assisted TEE by leveraging specific hardware primitives available in modern hardware platforms. We have fully implemented and evaluated \project for the i.MX 8MQuad EVK, and the results demonstrated that the performance of real-world applications such as DRM is not affected. We have also surveyed 80 CVE vulnerability reports and estimate that \project could mitigate 86.5\% of them.

%to restrict the privileges of the trusted OS
%creating sandboxed domains (\textit{zones}) inside the trusted world. The key idea behind the \project design relies on



%\section*{Acknowledgments}
%We thank... David Cerdeira was supported by FCT grant SFRH/BD/146231/2019. - Algoritmi project reference: UIDB/00319/2020 -


\newpage
%\section*{Availability}
%-------------------------------------------------------------------------------

%USENIX program committees give extra points to submissions that are backed by artifacts that are publicly available. If you made your code or data available, it's worth mentioning this fact in a dedicated section.

\section*{Check before submission}
\begin{verbatim}
Uniformizar:
    RPC (Resource Platform Controller) -> PPC? RZASC?
    secure world -> trusted world
    IEE (isolated environments) -> Zone
    capitalization: Zone or zone?
    trusted OS/Trusted OS/TOS
    trusted App/Trusted App/TA
    OSes/OSs
    ReZone Controller -> Zone Controller
    micro-controller/microcontroller/MCU
    S-EL(0|1) -> s.EL, sEL?
    ATF -> TFA
    iMX8M / i.MX8M
\end{verbatim}

==> backups/main_body-back-2-3-4.tex <==
%=======================================================================
%> [BACKGROUND]
%=======================================================================	
%\section{Background and Attacks}

\section{Background and Motivation}

%This section provides context on TrustZone-assisted TEEs, attacks, and hardware access control filters.

\subsection{TrustZone-assisted TEE}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/tz-SW-HW.pdf}
    \caption{TrustZone-assisted TEE: hardware-software architecture}
    \label{fig:tz_sw_overview}
\end{figure}

% \textbf{NS: Please turn this into paragraphs. Tell a story. See how we do it in the S\&P paper to introduce the reader to TrustZone technology. First present the overall architecture showing NW/SW separation, say that each core can run in each world. Maybe at this point talk about the TZAC and the system-wide memory protection mechanisms to conclude the description of the hardware architecture. Then, on a second paragraph, present the typical software stack comprising the rich OS then the Trusted OS running in the SW (EL-1 ring) along with the monitor (in EL-3) (which is necessary to present here because you will talk about that later). Say that the software in SW have full access to the whole memory, both NW and NW. Then proceed to explaining that there are unprivileged trusted applications (TAs) running in EL-0. Some of these are geral purpose, others are system TAs, etc. As it is now, everything is mixed up.}
% \begin{itemize}
%     \item Trusted OS - Vendor dependent software
%     \item System TAs - 2 factor auth data; keychain data (banking, password management...); private keys (gpg, signing certificates, electronic IDs, device encryption...); biometric data (ie: fingerprint), etc...
%     \item General Purpose TAs - Vendor software, and partners software: Disney, Paramount, Sony Pictures, 20th Century Fox, Universal Studios, Warner Bros
%     \item Monitor - Commonly implemented by customizing Arm-Trusted-Firmware
%     \item .
% \end{itemize}

%\nuno{The whole text of this section is very good, but I it's quite long and too full of details. I think we should shorten it and present only the bare minimum that allows the reader to understand the attacks that will be introduced in the next section. Many of the low level details presented here can be briefed in latter sections as we present the design and implementation of our system. The takeaway point from this background section is that the SW software is almighty.}

%\sandro{I would suggest to reduce the intro para and merge the SW Architecture together into the intro paragraph. We need to discuss if the full TZASC paragraph can be removed.. I'm not 100\% convinced.. }



TrustZone is a System-on-Chip (SoC) and CPU system-wide security solution available in a broad range of Arm processors. The technology has been pivotal for the materialization of TEEs in mobile devices by providing an isolated environment for secure processing of sensitive data and programs (i.e., trusted applications). TrustZone is built upon the concept of protection domains, i.e., the {\em secure world} (SW) and the {\em normal world} (NW). The SW shields critical functionality from the NW, which is used for running an untrusted operating system (OS) and its applications. 
%In the TrustZone hardware architecture, each physical processor provides two virtual cores and a set of well-defined mechanisms (e.g., {\em monitor mode}, SMC instruction) to switch between secure and non-secure states. At a given point in time, the world where the processor currently executes is based on the state of the Non-Secure (NS) bit. There is additional hardware logic in a TrustZone-enabled SoC that extends the security state of the processor to other system components, i.e., bus, interrupt controller, memory hierarchy, and peripherals. 
%ensuring that SW resources cannot be accessed by NW components.
%\mypara{Software Architecture}. 
\autoref{fig:tz_sw_overview} depicts the software architecture of a TrustZone-assisted TEE. Inside the SW runs the TEE software, while in the NW run the Rich Execution Environment (REE) and untrusted applications. The TEE software has three fundamental building blocks: the {\em secure monitor}, the {\em trusted OS}, and {\em trusted Applications}. The secure monitor, running at the higher level of privilege (i.e., S-EL3), provides basic mechanisms for secure context switching and platform-specific management (e.g., power management). The trusted OS runs in S-EL1 and provides an underlying infrastructure for sustaining the lifecycle of TAs. TAs execute in unprivileged S-EL0 and are typically developed by platform vendors and OEMs. 
%Core components of the trusted OS encompass (i) the trusted kernel, which provides the basic OS primitives for managing TAs, (ii) device drivers for accessing trusted peripherals, (iii) low-level code for cross-world interactions, and (iv) shared libraries (e.g., cryptographic) and TEE primitives, such as remote attestation, trusted I/O, and secure storage. 


%Trusted applications are unprivileged programs that make use of the Trusted OS services to implement a wide range of features, which serve mainly two purposes. One is providing trusted services to the system and the OS. This includes handling biometric identification, cryptographic key management and trusted random number generation, to name a few. This is software developed by the platform vendor or OEMs. The other purpose of TAs is implementing application specific services whose compromised functionality affects the company who developed them or the user, but not the system directly. Examples of this are TAs part of DRM solutions, and TAs implementing part of electronic payments systems. Some applications require efficient cross-world communication mechanisms. To enable this, trusted OSs often allow TAs to map physical memory. The Trusted OS manages the physical memory available to each TA, some Trusted OS implementations enable TAs to map any normal-world address, while others only enable the mapping of specific shared memory regions. The last piece of a running TEE, is the {\em secure monitor}, which implements mechanisms for secure context switching between worlds and runs with highest privilege, in protection ring EL3. 


%The {\em TEE bootloader} bootstraps the TEE system into a secure state, and it is critical to implement the trusted boot primitive. Together, trusted applications, trusted OS, secure monitor, and TEE bootloader constitute the software TCB of a typical TEE system. For this reason, TEE designers aim for small and bug-free implementations. Nonetheless, vulnerabilities exist and attacks are successful.

%\mypara{TrustZone Address Space Controller.}
%The TrustZone Address Space Controller (TZASC) enforces physical memory protection in TrustZone-based systems. The TZASC allows the partition of external memory on secure and non-secure regions. To date, Arm has publicly released two TZASC specifications, i.e., the Arm CoreLink TZC-380~\cite{} and TZC-400~\cite{}. Both controllers share similar high-level features, i.e., the ability to configure the security access permissions for memory regions (contiguous areas in the address space), but, at the low-level, there are slight differences. For instance, the TZC-380 provides a \textit{security inversion} option (disabled by default), which allow non-secure memory regions to not be accessible to masters in a secure state. This feature is not available in the TZC-400. The TZC-400 introduces a set of prime mechanisms for fine-grain isolation, in particular, the \textit{identity-based filtering of non-secure accesses}, which allows per bus master (e.g., CPU cluster, MCU, DMA controller) partition. Despite the existence of TZC-380 and TZC-400 specifications, OEM manufacturers typically embedded their own proprietary controllers into their SoCs (e.g., Rockchip RK3399, \textcolor{red}{????}, \textcolor{red}{...}), which just provides coarse-grained configuration. Worst, there are SoCs used in well-established Arm-based platforms, e.g., Raspberry Pi 4, which do not feature a TZASC-like controller at all~\cite{}. 
%This results in a significant heterogeneity and fragmentation ...        


%At its core TrustZone extends the processor to enable CPU cores to operate in one of two states, secure and non-secure. Memory and resource access are made aware of the current security state of the processor through the NS bit (non-secure bit). The NS bit is then used to bar access to a resource according to the security state. Additionally, secure-world can map the memory as being non-secure, which results in secure-world memory accesses being performed as normal-world accesses. This way, the secure-world can access normal-world as if normal-world is the one accessing the resource. This design decisions makes it hard to prevent secure-world from accessing normal-world memory. For example, TZC-380 is a TrustZone controller developed by Arm which has a feature enabling memory accesses performed in a secure state to not being able to access normal-word memory (priority inversion), however given that secure-world software can map memory as being normal, this does not prevent the secure-world from accessing normal-world memory, it just has to do so intentionally.
%As alluded to earlier, to enforce the access control of each security state it is necessary to use dedicated hardware. Arm sells two TrustZone controllers TZC-380 and TZC-400 to this end. They differ in the features they provide, but both allow for specifying a hierarchy of memory regions with r/w privileges and secure and non-secure access. Although feature-full, Arm's TrustZone controllers are not deployed in every TrustZone-enabled system. It is common for SoC vendors to design and implement their own TrustZone controllers. This enables SoC vendors to tailor the hardware to their specific needs, but also results in less features and in a fragmentation of TrustZone-enabled systems. For example the rk3399 from Rockchip only allows the configuration of memory regions security state, and not other access control mechanism is present (e.g., R/W). Another example, is Zynq xxx, which only allows the configuration of all SRAM as either secure or non-secure. The broadcom SoCs used in the RPi don't feature a TrustZone controller of any sort[...], although the CPU cores themselves implement the TrustZone specification.



\subsection{Exploiting Overprivileged SW Software}\label{sec:attacks}

%\subsection{Attacks}\label{sec:attacks}

\if0
\begin{itemize}
    \item Agrupar classes de ataques
    \item explicar que o modelo actual não funciona
\end{itemize}
\fi

%Modelos dos ataques à TZ, some of which \project resolves.
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/TZ-Attacks.pdf}
    \caption{
    High-level view of the major class of attacks targeting TrustZone-assisted TEEs described in the literature that \project aims at mitigating.
    %Flow of attacks on TrustZone-based systems. Boomerang~\cite{Aravind2017}, QSEE Privilege Escalation and Exploit~\cite{gb-exploit4}, Exploiting TrustZone on Android~\cite{shen-trustedcore}, Breaking Android Full Disk Encryption~\cite{BreakFDE},  Hijacking the Linux Kernel from QSEE~\cite{gb-exploit6}, EL3 tour~\cite{EL3Tour}, A Deep Dive Into Samsung's TrustZone (Part 3)~\cite{DeepDive}, Breaking Samsung's Arm TrustZone~\cite{BreakingArmTZ}.
    }
    \label{fig:tz_attacks}
\end{figure}

%\nuno{I suggest that we change the title to something more insightful; but it hasn't necessarily need to be this one. The text of this section is all very good. I simply suggest that we emphasize more the root problem, i.e., the fact that SW is overprivileged and because of that even rather simple vulnerabilities in different components of the SW software can be catastrophic. I'd stress this in the first paragraph, and them continue on to explain each of the several attack vectors in its own paragraph. To make it easier to parse the rest of this section, each of these paragraphs could start with a bold title.}

%\sandro{I 100\% agree with Nuno. Going straight to the point into an initial paragraph and then split the discuss the three attack vectors (complementing with concrete CVEs from reported attacks) in specific paragraphs: (i) "Trusted OS can access the secure monitor.", (ii) "Trusted OS can access all TAs memory", (iii) "Trusted OS can access normal world memory"}

In the Armv7-A/Armv8-A architecture, monitor and trusted OS enjoy similar privileges with regard to read-write operations over secure and non-secure memory. Thus, the trusted OS has a complete view and full access to all system resources, including the secure monitor, TAs, and NW software. ... There are a plethora of successful attacks deriving from ... . David et all.~\cite{} has recently highlighted the extent of the problem, ... A complete tour on how to compromise the (i) REE kernel and the (ii) TEE kernel from a NSW application is detailed in the paper, but the logical ... 
\autoref{fig:tz_attacks} depicts the three main class of issues existing in TrustZone-assisted TEE deriving from 

%To begin their attack on the secure world, an attacker may start compromise a TA first. There are numerous reports on vulnerabilities in TAs (e.g.,~\cite{gb-exploit4}). These attacks depend on the software quality of the TAs, and as history tells us: writing bug free software is hard. After compromising a TA an attacker may try to compromise the Trusted OS, or the Trusted OS itself may have some vulnerability that may be exploited without exploiting a TA~\cite{shen-trustedcore}, and he may be successful. At this point, an attacker is in a high privileged position, as they can access any resource in the system. If not available to them until now, an attacker may create a backdoor in the normal-world kernel~\cite{gb-exploit6}. It's also possible to compromise TAs from the Trusted OS kernel~\cite{BreakFDE}. Additionally, an attacker may even compromise the secure monitor~\cite{DeepDive} giving them full control of the platform.
%These attacks are depicted in \autoref{fig:tz_attacks}.


\mypara{SW software can access normal world memory.}~\cite{gb-exploit6, gb-exploit7, Aravind2017} First, the Trusted OS can not practically be restricted from accessing all normal-world memory. As we will see below in ($\S$\ref{sec:hwmp}), even though TrustZone controllers such as TZC-380 and TZC-400, feature the possibility to define various memory regions, including the ability to prevent secure-world from accessing the normal-world, Trusted OSes can map memory as \emph{normal}, enabling them to perform normal world accesses from secure world. Even though ultimately this features are a non-issue to a compromised Trusted OS, they may raise the bar in preventing attacks such as boomerang attacks~\cite{Aravind2017} and in cases where the Trusted OS is not fully compromised. For this to be true, the cross-world shared memory regions must be grouped into a few memory regions enforceable by the TrustZone controller. This is a limitation of the TrustZone controller which features limited number of regions.

\mypara{Trusted OS can access the secure monitor.}~\cite{DeepDive},~\cite{BreakingArmTZ} Second, a Trusted OS can access secure monitor memory. In case a Trusted OS is compromised, a secure monitor could still regain control execution, detect the security breach and handle it in some way, if there was an effective privilege separation between the two pieces of software. However the Trusted OS can high-jack the secure monitor by modifying the code and data of the secure monitor, and gaining access to every resource in the platform, while executing at the highest privilege level. This is possible again due to coarse dual nature of TrustZone, privileged software (i.e., Trusted OS and secure monitor) in the secure-world cannot partitioned.

\mypara{Trusted OS can access all TAs memory}. Third, with a Trusted OS having access to all TAs' memory, an attacker may compromise any other TA without requiring them to be vulnerable~\cite{BreakFDE, DeepDive, shen-trustedcore}. If TrustZone TEE systems were to provide multiple isolated environments, it would be easier to contain vulnerabilities, and in particular Trusted OS vulnerabilities. This also requires additional hardware features to prevent Trusted OSes from accessing each other resources. Some researchers have proposed software based solutions which rely on same privilege isolation techniques~\cite{teev, ...}, but, although we believe these techniques may raise the bar for attackers, we argue they are not sufficient in the presence of a fully compromised Trusted OS.
\david{All TAs shared the same security domain.}


\subsection{Known Defenses and Their Limitations}\label{sec:defenses}

%\nuno{I think we should add a brief section here that explains the different defensive approaches that exist today for thwarting these attacks and explain the weaknesses of these approaches. Come up with three or four categories of existing defense techniques and briefly present them in individual paragraphs. It is in the measure of how compelling our criticism is that we will persuade the reviewers about the benefits of our approach. We should try to criticize the existing approaches in such a way that we find our sweet spot.}

%\sandro{I agree. We have such knowledge from our SOK paper. We can organize this subsection with three paragraphs, each one describing the defense (giving examples with papers) and highlighting existing limitations...}

%\david{usar fraquezas dos trabalhos para justificar o design point}
%\david{objectivos de segurança, portabilidade, performance aceitável}

We highlight two main class of defenses aiming at ...   

\mypara{Isolated compartments within the NW}. A major class of works focused in ... While one line of works, e.g., TrustICE~\cite{} and SANCTUARY~\cite{}, leverages the TZASC ..., a second line of works, e.g., OSP~\cite{}, PrivateZone~\cite{}, and vTZ~\cite{}, explore the hardware virtualization extensions available in the NW. While the latter can incur in a slight performance degradation, due to the lack of a two-stage translation, the former ... Notwithstanding, both approaches can only protect compromised TAs from accessing the normal world OS, with the caveat ... TAs with access to Trusted OS syscalls ... In all these works, a compromised Trusted OS is still able to access all TAs, the REE kernel, and the monitor, and bring the full system down. 

\mypara{Secure hypervisor within the SW}. Write something here ...





%\subsection{Leveraging Platform-Specific Hardware}\label{sec:approach}

\subsection{The need for reduced SW privileges}

%\nuno{I'm a little bit changing my mind with respect to what I mentioned in our last meeting about moving the description of the new hardware features to latter sections of the paper -- although not entirely because here we should not be so detailed in the description. So, I think it might flow nicely to give the reviewer an intuition of what new hardware features are available our there that we could use to try to overcome all the limitations we highlighted in the section above. Then, after introducing these features point to Figure 3 and say that we aim to investigate how these new features can be leveraged in such a way that we can reduce the privileges in the SW, and proactively prevent the attack vectors described above. I think this is also the place were we should present the general platform features as currently described in Section 4.2; besides the description of the threat model will also require a previous introduction of the platform's features that we're going to use. Then, the next section will orderly clarify our goals and threat model.}


%\sandro{I agree with giving an hint about what we are going to do, but without to much detail. I would suggest the title of this section to be more generic, and not completely focused in the hardware itself, e.g., "The need to reduce Secure World privileges"}

%\jose{I think it would make more sense to move the section here, but simplify it, and leave section 4.2 as is.}

%=======================================================================
%> [Goals and Threat Model]
%=======================================================================	
\section{Threat Model and Goals}

%\sandro{I believe we should present the threat model first and then our goals...}

\subsection{Threat Model}\label{sec:threat_model}

%\nuno{The threat model is supposed to describe the attacks that are within scope and attacks that are not in scope. I think most of the following text must be fixed to describe this information. Note that these are the attacks that the adversary may try to launch to subvert the defense mechanisms of \project.}

\sandro{I personally do not like the 1st paragraph. The 2nd paragraph needs strong polishing. The bullet points are good but need some minor touches. The last paragraph needs to be polished - straight to the point.}
\david{Done. Please check.}

The TrustZone threat model, establishes the normal world as untrusted, while trusting the secure world. The trusted secure world components are the secure monitor, the Trusted OS, and to a lesser extent TAs. However, the prevalence of attacks and flaws targeting secure world software shows the inadequacies of this model~\cite{Cerdeira2020}.  
%However, TAs can often be targets for privilege escalation, with their compromise leading to powerful attacks~\cite{Cerdeira2020}. For this reason we consider that TAs are also trusted in the typical TrustZone-assisted TEE.

With \project we aim first to remove privileges from Trusted OS and its applications, and second to create additional secure-world environments to minimize the impact a single vulnerability may have on the system. To this end, our threat model considers mutual distrustful domains between the normal world and the Trusted OS, and between Trusted OSes in the secure world. In practice, a malicious agent with control over a running TA or Trusted OS can try to mount software attacks against the secure monitor, the normal world, and other Trusted OSes. We also benefit from TrustZone features to prevent the normal world from accessing secure world memory (i.e., secure monitor and Trusted OSes). In \project we require the use of an auxiliary processor which we consider to be flawless, and thus trusted. Additionally we require a secure boot process to guarantee that the TCB is correctly initialized.
%We distinguish between two types of TCB. There is the system TCB, which includes the system components whose compromise allow an attacker to successfully attack all system components (e.g., compromised bootloader), and there's the functional TCB, which includes the system components whose compromise affect not the system security but the security of the applications relying on their correct operation (e.g., secure random number generator). In this work we focus on the system TCB, and the components are either trusted or untrusted in relation their role in participating in the system TCB. 
%
In summary:
\begin{itemize}
  \setlength\itemsep{0em}
    \item The normal world (i.e., normal world kernel and hypervisor) is untrusted;
    \item The sEL1 and sEL0 (i.e., Trusted OS(es) and corresponding TAs) are untrusted;
    \item The EL3 (i.e., secure monitor) is trusted;
    \item The auxiliary processor and the software executing on it are trusted; and
    \item The platform's secure boot initializes the system to a known state.
\end{itemize}

%By effectively sandboxing the Trusted OS, \project diminishes the system TCB to include only the secure monitor, and an auxiliary processor.
We do not consider physical attacks that tamper with hardware, e.g., fault injection. Similarly to a typical TrustZone deployment, we do not consider Denial-of-Service (DoS) attacks including those caused, for example, by a malicious Trusted OS not relinquishing control to the normal world.
Our solution has the side-effect of providing cache side-channel protection between Zones, and between Zones and normal world. However, micro-architectural side-channels are out of the scope of our work.

\subsection{Goals}
With \project, we aim at building a novel design that improves the security guarantees of TrustZone based systems, by effectively reducing the secure world privileges and thus minimizing the system's Trusted Computing Base (TCB). This mechanism should be deployed in real world hardware platforms and shall incur acceptable overheads for typical TrustZone-based TEEs workloads. \project main goals can be summarized as follows:

%\nuno{IMO the goals can be stated in a much more assertive way; we're digressing a bit and being somewhat imprecise, e.g., ``It is essential to prevent a compromised trusted OS from tampering with the secure-monitor and thus making it the sole system's TCB.'', this doesn't mean what we want: we want S-EL1 software to be blocked from reading and writing memory owned by EL3, unless explicit access privileges are granted to well-defined EL3 memory regions. Same comment for the others. The third goal says something like: ``it's possible to etc.'', this does not read like a goal but something hypothetical: do we want to provide this in \project?}

%\sandro{I agree 100\% with Nuno. Straight to the point and without possibilities/doubts...}

\mypara{Goal I: Reduce Secure-World Privileges.} 
\sandro{This paragraph is too big. This initial paragraph shall be straight to the point, explaining that the main goal is to reduce the secure world privileges and then let each objective in a bullet or number describe how we can accomplish that.}
\david{Done. Please check.}

We develop \project with the goal of sandboxing Trusted OSs in the secure world, preventing them from accessing arbitrary platform resources including the normal world and secure monitor memory regions, and devices.
The high level system model achieved by following the proposed objectives is depicted in \autoref{fig:rezone_vhl}.
We call this sandboxes secure-world zones. This high-level goal can be mapped into three main objectives:

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/ReZone_VHL.pdf}
    \caption{High level goals for the \project design.}
    \label{fig:rezone_vhl}
\end{figure}


\begin{enumerate}

  \item \textbf{Secure-Monitor Isolation.}\label{goal:secmon} The first objective is to provide a secure environment for monitor to execute. This way even in the presence of a malicious Trusted OS, the secure monitor can still be trusted as the system root of trust. Traditional hardware memory and peripheral protection mechanisms in TrustZone are limited in that they do not provide an effective privilege separation between EL3 and sEL1.
  %The first issue we tackle is secure-monitor isolation. We leverage the hardware features highlighted in section \ref{sec:hwmp}.In particular, the key-feature required to protect secure-monitor code is the ability to define a memory region as inaccessible to the CPU. We use this feature to prevent a Trusted OS from tampering with the secure-monitor. Traditional methods of hardware memory control in TrustZone (i.e. TrustZone controllers) are not sufficient. As we've explained earlier, TrustZone controllers are equally accessible to secure-monitor and Trusted OS. This makes configurations put in place to protect the system futile in a situation where the Trusted OS is compromised.
  
  \item \textbf{Normal world protection.}\label{goal:secnorm} The second objective is to provide normal world protection, in order to prevent malicious Trusted OSs from accessing arbitrary normal world memory. Currently, TrustZone offers an asymmetrical protection scheme where the secure world cannot be prevented from accessing normal world memory. This, in combination with other flaws, leads to attacks such as those we discussed in ($\S$\ref{sec:attacks}).
  %The TrustZone specification gives full access memory and peripheral access to the Trusted OS. However, in reality, the Trusted OS can perform all it's typical operations without requiring access to all platform resources, and in fact, the resources available to the Trusted OS have often times been used against the normal-world OS ~\cite{} \ref{} .%For this reason, we implement mechanisms that add a layer of protection to the normal world. This way the normal-world can be better protected from the Trusted OS, preventing attacks such as~\cite{}. %The mechanisms we employ is partially based on previous works~\cite{} with the added feature of an asynchronous minimal page-table introspection mechanism.
  
  \item \textbf{Multiple Isolated Environments.}\label{goal:multtee} The third objective is enabling the use of different environments for multiple Trusted OSs. Decomposing the current deployment of TEEs in more than one environment improves the overall security of the system, due to lower impact of TEE related flaws and vulnerabilities~\cite{Brasser2019,Li2019,Kwon19}.
  %With a mechanism that is able to mark memory as inaccessible from a high privilege-level can be leveraged to implement multiple lower privilege-level execution environments. %In \project this allows us to implement multiple TEEs which are not able to interfere with one-another.Similarly to other works ~\cite{Aravind2017}, we argue that decomposing current deployment of TEEs in more than one environment improves the overall security of the system. This is mainly due to preventing flaws affecting one TA from affecting another. %As a result, it's possible to either create different environments for each type of TA (e.g., System TAs) or create environments for each developer, so that developers do not need to rely on the correctness of other developers code. %This allows us to implement multiple TEEs which are not able to interfere with one-another. %However, short of new hardware implementing the Armv8.4(?) specification and up, there are still no solutions to providing hardware based multiple environments in TrustZone.
  
\end{enumerate}



\mypara{Goal II: Minimize the (secure world) TCB.}
\sandro{Text needs a strong refinement.}
\david{This goal is a consequence of Goal I, or Goal I is a consequence of this. I don't see a situation where we could minimize the TCB without also reducing privileges, or reducing privileges without reducing the TCB. I'd say we can remove this point. Please check.}
TrustZone-assisted TEEs suffer from large TCBs. To address this we set a goal of excluding Trusted OSes and TAs from the TCB. This way, a security flaw in a Trusted OS or TA will not enable an attacker to fully compromise other parts of the system.

\mypara{Goal III: Portability.}
\sandro{I'm not sure the description is good with regard to the goal. I'm not convinced.} \david{done. Please check.}
Another goal we aim for is portability. Specifically, we intend to create a design that is not tied to a singular platform. This goal is achieved by making use of real-world hardware as a testbed for \project, while not relying on the specific hardware mechanisms, but rather on the ability to create security domains orthogonal to TrustZone.

\mypara{Goal IV: Acceptable Performance.}
\sandro{We shall elaborate a bit more. I'm not convinced.} \david{Done. Please check.}
Our last goal is that the overheads incurred by our solution, should not significantly affect common TrustZone-based TEE workloads. In other words, we are willing to trade a performance penalty, as long as not detrimental to the user experience, for some much improved security guarantees.


%=======================================================================
%> [DESIGN]
%=======================================================================	
\section{Design}
\label{sec:overview}

\david{TODO: como surgem as sandboxes?}


%\textbf{NS: Introduce the section and provide a roadmap for it. This is very helpful because it gives structure to your through process.}

%\textbf{NS: Previously, the list below was stated as design goals, but I think in this context, since we are building a system that wants to leverage a few hardware primitives to provide additional protections, you can basically provide a high level description of what the system does, and what its components are with respect to the traditional TEE architecture presented in the previous sections. How different will it be? What new components are introduced into the picture? And finally briefly say that with our system, it will be possible to configure the system to operate with four or five new partitioning schemes which we will describe in detail in each of the next sections.}

\project's design focuses on providing the ability to create multiple isolated security domains inside TrustZone's secure world. Essentially, it sandboxes secure world's EL1/EL0 execution modes in isolated domains called zones, reducing its privilege, thus protecting both normal world and the secure monitor from rogue Trusted OSes or TAs, and also enabling the monitor to multiplex the secure-world by context-switching multiple TEEs. To achieve this, the design is centered on a custom world switch mechanism which leverages hardware security primitives orthogonal to TrustZone, including memory and peripheral protection controllers as well as a system management microcontroller unit (MCU) \jose{Nuno thinks we need to contrast this with related work based on Trustzone standard features ie. TZASC, normal-world procted domains}. In this section, before detailing \project's architecture depicted in Figure \ref{fig:rezone_overview}, we start by defining a platform model which defines the hardware requirements for implementing it, and finish by describing its key mechanism and full system operation.

\sandro{Still in this first paragraph I believe we should have a reference to a Figure supporting this high-level design description. Suggestion:}
\newline
{\color{red}Figure X depicts an abstract view / high-level perspective of \project's design. Below, we explain the expected platform model, we overview the \project architecture, detail the key mechanism, and describe the full system operation.}

\jose{done. check if it is okay with you.}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/rezone-hw.pdf}
    \caption{\project enabling hardware components and typical components of platform featuring Trustzone.}
    \label{fig:RZ_HW}
\end{figure}


%Our system aims at deprivileging the trusted OS, effectively crating multiple security domains as oposed to the dual-world model of traditional TrustZone.Our system creates an effective privilege separation between the Trusted OS and the secure-monitor. This is a feature which enables the secure-monitor to be trusted as the system root-of-trust whether the trusted OS is compromised or not. In addition, with our system it's possible to remove the asymmetry in privileges between the trusted OS and the REE, by protecting all but explicitly allowed normal world memory regions to be accessed by the trusted OS. The mechanisms that enable this also enable the creation of multiple execution environments in sEL1, allowing for secure deployment of multiple TEEs.


\subsection{Platform Model}\label{sec:plat_req}

\nuno{As I mentioned in my previous comments, I think this text should be moved (and adapted) to Section 2.4.}

\jose{I think the section should be here. From my perspective, the platform requirements we define here are part of the design.}

\project's design makes a set of assumptions regarding the features offered by the underlying platform, which are the basic primitives needed to implement the key protection mechanism described throughout this section. These include:

\jose{Nuno needs to see a diagram/figure of bus masters, mcu, etc... (similar to trustzone for armv8-a pag18})

\begin{enumerate}

    \item \textbf{Platform-level resource protection controller (RPC)}, i.e., a dynamically configurable memory and peripheral protection controller, orthogonal Trustzone's protection mechanisms (e.g., TZASC) \jose{confusing: tzasc is an rpc? split multiple sentences.}. The RPC shall be capable of (i) setting fine-grained access control attributes (e.g., RO, RW) for a each defined memory region; (ii) differentiating between multiple bus-masters; and (iii) protecting memory-mapped input/output (MMIO) \sandro{(acronym needs to be defined)}\jose{done} regions, including their own; %to, but including,

    \item \textbf{Programmable system management core(s)}, i.e., independent processor(s) and bus master(s), distinct from the main and powerful application processors. Typically, these cores are added for housekeeping purposes and implemented as small MCUs (e.g., Cortex-M4); \sandro{(Martins, I slightly extended this point, so please check if you are comfortable with changes)}\jose{made a minor change. i think now it's ok.}

    \item \textbf{Secure boot process} that is able to guarantee a management core is in full control of the system's protection controllers, while their access is blocked to the main application cores.

\end{enumerate}

These requirements are modeled on the platforms described in ($\S$\ref{sec:hwmp}) and ($\S$\ref{sec:otherplat}). Although we did not carry out an extensive survey, we believe many other current and future platforms will meet these requirements, especially those targeting the high-end embedded markets such as automotive. \sandro{We need to be more confident in this message.} \jose{need to discuss} %Also, there is an increasing trend to include similar mechanisms in mobile SoCs. For example, Qualcomm's SPU (secure processing unit)~\cite{Qualcomm2019} provides many, if not all, of the aforedescribed features.

\sandro{I like this paragraph but I strongly believe it should be moved to the Implementation or Discussion section. At this point, a reader/reviewer without much knowledge cannot understand what is being discussed.} \jose{need to discuss}
\newline
{\color{red}We designed \project assuming that, w.r.t. application cores, the protection controllers act only on a per-cluster basis. Typically an RPC cannot differentiate between the multiple cluster cores as it observes requests as being from a single bus master, the shared cache. All accesses to the internal cluster caches will not be subject to RPC restrictions, only to TrustZone's. Despite being a limitation and not actually a model requirement, we make this assumption given that both platforms we model these design requirements on have this characteristic. If a similar platform fulfills all of the aforementioned requirements and, in addition, provides per-core isolation, this would allow for the system to be more flexible, scalable and performant.}

%\textbf{NS: the next paragraph was formerly named ``\project'' but I don't quite follow if this is common across all the protection modes that we can support, or if this is in itself a specific protection mode. Can you please clarify that? And also describe what benefits it can bring?}
% In TrustZone systems, secure-world has access to all system resources. One way we can protect resources is to have a separate processor mediate the configuration of memory region security attributes.
% Attributes are: secure-world read/write and normal world read/write. All of these privileges can be removed creating a grey-area, which we call \project.

\subsection{Architecure}

%\nuno{I think this section should be renamed ``Architecture'' and you should introduce all the components of the \project system, both software and hardware components.}

\sandro{In our document, we still cannot clearly communicate "what is \project". A design, and architecture, a mechanism ?! Furthermore, I do believe we have agreed we shall have specific names for the sandboxes - Zones if I'm not wrong?!} \jose{need to discuss}

\jose{I think \project is the overall system (architecture, mechanism, etc) which allows us to create the secure-world zones to achieve the goals.}

\jose{Modified "sandbox" to "zone" or "secure-world zone" in most of the text.}

\project can be understood as providing a set of security domains, each with a well defined set of memory and peripheral resources it can access, 
effectively increasing the number of security domains of a typical TrustZone system. A security domain is activated according to the execution context (\sandro{I honestly don't like this first sentence.}\jose{can you be more specific?}). As shown in Figure \ref{fig:rezone_overview}, in the main application processors, there are four execution contexts types: (i) \textbf{\textit{the normal-world}}, (ii) the \textbf{\textit{secure-monitor}}, (iii) the \textbf{\textit{monitor trampoline}}, and (iv) \textbf{\textit{multiple secure-world zones}}, or just, \textbf{\textit{zones}}, (\sandro{update the naming per the agreed term for sandboxes}\jose{done}). The normal-world, the monitor and different zones all have a single dedicated security domain. The monitor trampoline, however, executes either in the the monitor of the zones' security domains.
An additional execution context, (v) the \textbf{\textit{\project controller}}, hosted on a dedicated programmable management core (\sandro{I think we should call the names we have defined in the platform model, i.e., "programmable system management MCU"}\jose{done}) is itself encapsulated in its own security domain, which is isolated from the main processor cores at all times. On a world switch, it coordinates with the monitor trampoline to dynamically reconfigure the platform-level protection controllers to enable the secure-world zones. 

\sandro{I believe the use of "mypara" for the descritpion of each context keeps easier for the reader. I have restructured, accordingly.} 

\jose{thanks. it looks better.}
 
\mypara{Normal-world context.} The \textit{normal-world context} corresponds to the normal-world state of a typical TrustZone system. In this case, the security domain boundaries are enforced by the standard TrustZone mechanisms (e.g., TZASC). It comprises the rich OS and REE Apps (\sandro{rich OS and REE Apps, per Figure 1 - Btw naming in Figures are not kept coherent / uniform - compare Figure 1 and Figure 4})\jose{done}, and it can not access neither the secure monitor, trampoline, \project controller, nor the zones domains' resources.
%The \textbf{\textit{secure-monitor context}} executes in a domain created by leveraging a hardware based memory-arbiter, in a way as to prevent the Trusted OS from accessing secure-monitor context. The secure monitor is the system's root-of-trust and can access any of the system resources.

\mypara{Secure monitor context.} The \textit{secure monitor context} executes in a security domain akin to the typical TrustZone's secure world (\sandro{I think a bit of detail with regard to EL3 vs sEL1 shall be given} \jose{don't understand why. this is just referring to the secure-world permissions }). Therefore, it can access all platform resources except the \project controller's. This constraint is ensured (\sandro{limitation?! assured or "ensured/guaranteed"}\jose{done. check.}) by the RPC.

\mypara{Trampoline context.} The component responsible for issuing requests to the \project Controller to switch the currently active security domain is the \textit{trampoline context}. Because of this, it has a special property in that it executes in two security domains at different points in time. Upon a Rich OS request to a zone, it executes in monitor mode enjoying monitor domain access privileges. After issuing a \project Controller command to activate the target zone, it starts running inside that zone's security domain. It then hands execution to the trusted OS. Later, when the trusted OS issues an SMC, the trampoline executing in monitor mode, still under the zone's security domain, issues a request to the RDC to deactivate it. At this stage, it will resume execution under the monitor's security domain and finally hand execution to the monitor context. This idea is pivotal to \project's design as it is not possible to atomically enable a zone's domain and jump to the trusted OS in sEL1, or atomically disable a zone's domain on a trusted OS SMC call. 
Because the trampoline is shared between the monitor and the untrusted zones, this software component must be tailored to be as minimal as possible and encompass mostly read-only memory to avoid corruption from a rogue Trusted OS. All writable data used by the trampoline must be non-critical. 
(\sandro{The description of the trampoline context is not clear and is a bit confusing, in particular the description related to the execution in two security domains. I'm sure a reader without much knowledge will not understand much. Furthermore, at this point, juts Figure 4 was referenced; however, it is not clear in Figure 4 were the trampoline context runs.} \jose{i've rewritten it to try to make it clearer. feedback? as for the last point, i think we discussed this, David was supposed to label the figure.})

\mypara{Secure-world zone contexts.} Each \textit{secure-world zone context} (\sandro{Do not forget to update naming})\jose{done}, encompassing a Trusted OS and respective TAs, has its own dedicated security domain which excludes all other domains' resources with the exception of pre-established shared memory regions. As the traditional TrustZone resource protection primitives do not distinguish between secure-world privilege modes (i.e., between EL3 and secure EL1/EL0) and are asymmetrical in the sense that they are able to protect the secure world from the normal world, but not the other way around, zone domain boundaries are enforced by the RPC. 

\mypara{\project Controller context.} The \textit{\project Controller context} executes in an isolated system management MCU (\sandro{we should name microcontroller and use the acronym MCU}\jose{done}) and its security domain encompasses a small private memory region and the platform-level resource protection controller (\sandro{platform-level \textbf{resource} protection controller - per naming of section 4.1} \jose{done}). Its main role is to dynamically reconfigure the RPC to activate/deactivate secure-world zone domains (\sandro{Do not forget to update naming}\jose{done}). The need for this component is intrinsically connected with the fact it is the single domain with RPC access privileges. If application processors were allowed to directly reconfigure the RDC for the monitor to enable or disable secure zone domains, there would be no way to guarantee that the Trusted OS would not also do the same. This would allow it to gain access to monitor or normal world resources, breaking the system security proprieties. (\sandro{Sentence is long and confusing. Split in simple messages, maybe 2 sentences} \jose{done. check if it is okay with you}). Therefore it is only the \project controller that directly activates and deactivates secure zone domains by configuring the RDC to only allow accesses according to the predefined system policies. It does so in response to requests issued by the application cores via a secure channel which, at each request, authenticates the client as being  the secure monitor to avoid spoofing by a malicious trusted OS (see $\S$\ref{sec:key_mechanism}).

\mypara{}(\sandro{There is a change in the flow that contexts are being described. Per the initial paragraph, the \textbf{\textit{trampoline context}} is just executed in the application processors, and is enumerated as (iii). Here, it appears as the last, after describing the \textbf{\textit{\project controller context}}, which changes the order / flow. I believe we shall keep the samer order and coherency.})

\jose{done}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/ReZone.pdf}
    \caption{\project overview}
    \label{fig:rezone_overview}
\end{figure}

\subsection{Key Mechanism}\label{sec:key_mechanism}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/ReZone-ExecModel.pdf}
    \caption{\project Execution Model \jose{David please update Domain Controller to \project Controller}}
    \label{fig:HZ-exec-model}
\end{figure*}

The key idea of our design is centered around the creation of multiple secure-world zones which sandbox TrustZone's sEL1 and sEL0 privilege levels and that can be activated on-demand by EL3 software. To this end, our design includes (\sandro{the design "implements"?!?! confusing}\jose{done}) a custom world-switch mechanism which leverages: (i) the hardware primitives detailed in ($\S$\ref{sec:plat_req}); and (ii) the fact that, although TrustZone does not provide EL3/sEL1 address space isolation, there is actually strong privilege isolation at the register level since the latter cannot access the former's system registers (\sandro{This sentence is confusing because is too long, and and some point the reader loses track which is in fact leveraged to provide such secure-world domains isolation.}\jose{rewrote it. check it.}). \project takes full control (\sandro{I don't like much the way is phrased with "we"}\jose{done. check it.}) of all protection mechanisms by, at boot time, configuring them to allow accesses coming only from the \textit{\project Controller} running in the management MCU (\sandro{programmable system managment core - per naming of section 4.1}\jose{done}). Also at boot time, (\sandro{I don't like much the way is phrased with "we"}\jose{done}) a secure communication channel is established between the secure monitor and the \textit{\project Controller} based on a secret-key that is kept private to the monitor by storing it in an EL3 register (\sandro{Kind of scratchpad reg?!} \jose{not scrachtpad since all EL3 registers are being used}). The \textit{\project Controller} authenticates the secure monitor, at each request, to modify RPC configuration. The monitor can then enable and disable protection via request to the \textit{\project Controller} upon Trusted OS entry and exit. 

(\sandro{In my opinion, and aligned to what I have said before, we shouldn't be focused in this per-cluster limitation in the design. We should describe in a generic way, and let the problem arise in the implementation and discuss how we see benefits in having per-CPU control in the Discussion Section. I think it's possible to describe this part in a generic way. It's just my view, that we should discuss in the next meeting.}\jose{to discuss}) 
As described in ($\S$\ref{sec:plat_req}), RPC protection acts only at a per-cluster basis and is is not enforced on accesses to the cluster internal caches. For this reasons two actions must be taken when a zone context is activated in one of the cores. First, all cache contents must be flushed so that the trusted OS cannot access or modify other domain's in-cache data. Beyond the cache, protection is enforced by RPC. Secondly, all other cores within the cluster must be halted to prevent other cores executing in the normal world from fetching their data to cache. Although these are extreme actions that, at first sight, might suggest prohibitive performance overhead (\sandro{prohibitive performance overhead}\jose{done}) and UX impacts, our experiment shows it not so critical due to the sporadic invocation patterns and reduced execution times of secure world services (see $\S$\ref{sec:eval}), essentially trading-off huge security benefits by moderate performance hits. \jose{Nuno and David, this last point on trade-offs needs to be polished. Any ideas? Maybe mention that we can still run other cluster in parallel which is very common in today's big little architectures?}

The key world-switch mechanism is depicted in \autoref{fig:HZ-exec-model}. After the normal-world issues a request (1), the execution is handed to the monitor context (\sandro{\textit{secure monitor context } per naming in subsection 4.1}\jose{in my opinion we don't need to be that verbose all the time.}). If the request needs to be handles by the Trusted OS (\sandro{suggestion: needs to be handled by the Trusted OS}\jose{done.}), \project will activate the target zone's security domain and hand it execution \nuno{what you mean by ``activate its domain''?} \jose{I've added a definition of secure-sandbox activation in section 4.2}. For this, the secure monitor starts by notifying all other cores in that cluster (\sandro{The part of the IPIs is not an implementation detail?!}\jose{removed}). The other cores will then flush their caches and enter an idle state. After all other cluster cores are idling, the trampoline (2) issues a request to the \textit{\project Controller} (\sandro{Please note the image has no reference to "\project Controller"}\jose{noted}) to activate the target zone domain (\sandro{Do not forget to update naming}). To authenticate the request as coming from a secure monitor context (\sandro(\textit{secure monitor context} per naming in subsection 4.1?!)\jose{done})), the \textit{\project Controller} expects to receive a secret token it handed to the monitor during boot and protected during zone execution by storing it in an EL3 register (\sandro{\textit{\project Controller} twice and another reference to the token in the EL3 register - i think is not needed}\jose{done}). After a successful reply from the \textit{\project Controller} (3), the trampoline (\sandro{Shall we introduce as \textit{Trampoline} ?!}) will first flush its own cache content (\sandro{suggestion: microarchitectural state!?}\jose{is it more than cache?}) and then (4) jump to the Trusted OS. After the Trusted OS returns execution to the \textit{secure monitor} (5), the trampoline (\sandro{Shall we introduce as \textit{Trampoline} ?!}) issues a new request (6) so that the \project controller (\sandro{domain controller now!? I'm confused}\jose{old nomenclature. done}) deactivates the zone domain (\sandro{Do not forget to update naming}\jose{done}) and reestablished the secure-monitor domain. The monitor will then resume normal-world execution (7), notify other cluster cores to, finally, return to the normal world context (8) executing under traditional TrustZone restrictions. 
\nuno{This paragraph is describing how we do things, but I feel it's important to explain why we do them in this way. In particular, I feel that we need to explain the permission privileges that result from combining the security mechanisms from RDC and TZC, and talk about the technical restrictions involved in setting them up that justify our solution and the steps above (e.g., the need to have a trampoline, etc.).}
\jose{Nuno, please check the 4.2 architecture section. I've added the justification for the need of the trampoline code there. Also that section also clearly describes what protection is enforced by the TZC vs the RDC.}

This key mechanism by itself ensures Goal I's objective I and II by enabling the protection of monitor and normal-world memory while a trusted OS executes inside a secure-world zone. Using the mechanism as a bedrock, the secure monitor is able to easily restore the context and activate the security domain of multiple TEEs depending on the request of the secure achieving objective III. As each TEE is sandboxed in a zone, it will also not be capable to access other TEEs' resources.

% Our platform model assumes that protections have cluster granularity. Because of the need block monitor memory after while one of the cores is executing a trusted OS, another core cannot execute in the monitor context while the trusted is executing. The trampoline our design essentially serializes secure world requests.

\nuno{Another big question I have is: if we're going to implement IEE, which enforces full isolation from the normal world, how are they going to be able to share memory with each other? What's \project's mechanism to enable that?}

\jose{ Sections  4.4. to 4.6 and partially 4.7 are already described in section 4.3. But I agree we can maybe highlight or detail some of these main points a bit more.}

\subsection{Full System Operation}

(\sandro{I would recomend to split this text among several "mypara", each one for a part of the lifecycle. When this is done, I can give you a strong opinion on how to improve this subsection. I believe still something is missing...} \jose{to discuss})

\jose{Each OS SMCID range is offseted}
To setup the system, all zone domains and their respective access privileges to memory and peripherals must be statically defined at design-time in a manifest file. For each defined zone (\sandro{Do not forget to update naming}), the provided services (\sandro{Which services?! It's not clear to me}) must be listed, and each service shall be associated with an unique SMC (Secure-Monitor Call) ID. This information is directly compiled into the monitor image. At system initialization, the monitor creates zones (\sandro{Do not forget to update naming}) by relaying this information to the \textit{\project Controller} which saves this information in its private memory and acknowledges the success of the operation by returning a zone (\sandro{Do not forget to update naming}) ID to the monitor. The monitor then creates a map of SMC to zone IDs (\sandro{Do not forget to update naming}). It would be possible to directly fetch these configurations in the domain controller (\sandro{This term was never introduced before, and it's not linked to any context described in 4.2}) itself. However, this interface will seamlessly allow the dynamic instantiation of zones (\sandro{Do not forget to update naming}) in future iterations of our design.

At runtime, when the normal-world OS issues a request to the secure world passing it a given SMC ID, the monitor will translate the SMC ID into a zone (\sandro{Do not forget to update naming}) ID, and pass this ID to the \textit{\project Controller} to activate the target zone (\sandro{Do not forget to update naming}). The controller (\sandro{which one?! the \textit{\project Controller}?!}) will then use this ID to get the RPC configurations for the target zone (\sandro{Do not forget to update naming}). This makes the segregation of the Trusted OS into multiple isolated zones (\sandro{Do not forget to update naming}) transparent to the normal-world client, and therefore there's no need for modifications of normal-world drivers.


\nuno{After we explain how \project is able to protect the monitor and the normal world, then it's time to give a complete explanation of the entire system operation: i) installation, ii) bootstapping, iii) runtime. I think most of the text from ``Key Mechanism'' could come here.}

\jose{Don't really understand what is meant by "instalation". Boostraping and runtime are somewhat described in section 4.3. Now that David  has multiple TEEs executing, we could maybe also explain how we envision the changes in the different software layers and programming model needed for this functionality.}

\jose{Maybe we should also address the problems arising with shared memory management.}



\if0
\subsection{Normal-World Trusted Service Request}
On a request for a trusted service, made through a Secure Monitor Call (SMC) instruction, if there's no trusted service request pending, the secure-monitor handles the request by looking at the SMC function identifier (smc\_fid). If the smc\_fid corresponds to a service provided by the secure-monitor (e.g., PSCI calls), the secure-monitor serves the request and resumes normal-world operation. This is no different to how these services are service typically. If, on another hand, the smc\_fid identifies a request for the Trusted OS, the monitor must protect itself. \nuno{because?... it's not clear at this point how is the secure world memory configured so as to justify the need for the monitor to protect itself when a request is made to the trusted os.} This is done by interacting with the MCU. The secure-monitor enters the trampoline and issues a SEC\_MON\_PROTECT command to the MCU. If the MCU identifies the secure-monitor successfully, the MCU will enforce the secure policy established during boot \nuno{somewhere before this point we need to clearly state what this security policy is.}. The secure-monitor will wait for a response from the MCU before executing the Trusted OS. The Trusted OS will then schedule a TA to service the normal-world request. Upon completion, the Trusted OS will return execution to the secure-monitor by issuing a SMC instruction. The SMC is handled in the previously established trampoline. The secure monitor will then interact with the MCU once again to re-allow access to the secure-monitor program memory, wait for the MCU response and resume normal execution, including returning to the normal-world. Figure \ref{fig:monitor_prot_seq} illustrates this process. \nuno{please update this reference; maybe refer to the figure earlier in this paragraph to help the reader understand the execution flow.}
\fi



\if0
\subsection{Secure-Monitor Isolation}\label{sec:secure_monitor_isolation}
The MCU acts as a mediator for the memory access controller configuration, and only acts on requests from the secure monitor, this enables us to make secure-monitor code inaccessible to a running Trusted OS \nuno{I think it might flow better if you first explain the problem, then the solution. Question: what prevents the trusted OS from tampering with the memory reserved to the MCU?}. 
Two things we must consider are the context switch from Trusted OS to secure-monitor, and a context-switch issued by the normal-world. \nuno{What about the steady state when the core is running with sEL1 privileges, i.e. Trusted OS code? what prevents it from accessing the monitor's reserved memory?}
We implement a small region of code written in assembly, that performs the necessary operations to handle both of these cases, which we call trampoline. 
The trampoline authenticates itself with the MCU, by sending a secret token with a request for an operation. \nuno{why does the trampoline need to authenticate itself?}
This token is made secret by storing it in system registers only available to secure-monitor level privilege (i.e. EL3) while the Trusted OS is execugin. We next explain the various phases of secure-monitor isolation operation.
\fi



\if0
\subsection{Normal-world Protection}\label{sec:normal}
Protecting the normal-world from a Trusted OS protects the executing REE from malicious TEEs from compromising the normal-world OS operations. This is particularly useful when attacks to TEEs can be made from the normal-world's user space applications, as opposed to attacks requiring an already compromised operating systems. TrustZone specification allows a Trusted OS to access any memory available to a given CPU, which enables some useful security features such as TZRKP [], but also the potential to compromise the normal-world OS. More insidiously, to effectively restrict secure-world access to a memory region is also to restrict it for the normal-world. Preventing the secure-world from accessing certain memory-regions while allowing normal-world to access them requires a per-core memory access control, which has been proposed in~\cite{Brasser2019} by leveraging non-standard features of a \textbf{barely used} TrustZone controller: the TZASC-400, and which even their test platform did not feature. Another solution is the introduction of virtualization in the secure-world as proposed in ARMv8.4-A specification. But hardware featuring the functionality may be still be a few years away from mass commercialization, as it tends to with new Arm architecture specifications~\cite{}. We propose a solution leveraging the RDC present in the iMX8MQ.

In TrustZone there are two mechanisms controlling memory accesses, virtual memory and TrustZone controllers. In addition to virtual memory mappings, virtual memory may be used to implement memory access security policies: read, write, executable. The policies are put in place by configuring the permission bits in each page table entry or page table directory. A Trusted OS may change this permissions or create new memory mappings during its execution, a feature which may be abused by attackers to compromise the system [bits please write zero primitive allows disabling domain enforcement (armv7)]. It's also possible for a Trusted OS to set the TTBR register, a pointer to active page table. Further, an attacker could also hypothetically disable virtual memory altogether to access system memory without restrictions~\cite{}. 
\david{Should this paragraph go to background?}

The mechanisms provided by TrustZone hardware are not sufficient to create meaningful isolation between the secure monitor and the Trusted OS. Because of this, we required orthogonal access control systems. In our implementation we configure the RDC to mark normal world memory as inaccessible while the Trusted OS is executing. This approach prevents all unintended accesses to the normal world memory (e.g., only allow shared-memory to be accessed), however it comes at the cost of having to perform cache maintenance on every context switch to the Trusted OS, and having to suspend all the cores on the cluster. By relying on hardware mechanisms on not on software approaches such as same privilege isolation techniques, we are able to relax the threat model to include completely compromised (i.e., untrusted) Trusted OSes.

\nuno{I think some parts of this paragraph are too verbose, and a part of our solution has already been mentioned in Section 5.3 when we talked about context switching.}
\fi

\newcounter{problem}
\newenvironment{problem}[1]{\refstepcounter{problem}\par\medskip
   \textbf{Problem~\theproblem. #1: } \rmfamily}{\medskip}
   

==> extra/intro-old-nuno.tex <==
%=======================================================================
%> [INTRO]
%=======================================================================	
\section{Introduction}

% [Para1] TrustZone is widely available for securing sensitive applications, both user-level and kernel-level applications.
Arm TrustZone is a technology embedded into Arm processors. It is presently found in millions of mobile phones and low-end devices equipped with application processors, such as Infotainment centers in automotive products, and SmartTVs. Vendors and OEMs rely on TrustZone for the creation of so-called Trusted Execution Environments (TEEs) which can be used for protecting the execution of sensitive programs named Trusted Applications (TAs). Some TAs implement security-sensitive operating system (OS) functions; for example, Android OS relies on dedicated TAs for authentication purposes, generation of cryptographic keys, or file disk encryption. Other TAs implement user-level functionality that can be shared across several applications, e.g., DRM media decoders, electronic payment systems, crypto-wallets, etc. TEEs are rooted on TrustZone and consist of a trusted software stack that offers APIs and runtime support for the execution of TAs. Examples of TEEs include OP-TEE and Qualcomm's QSEE. TEEs' goal is to ensure that even if the OS is compromised by an attacker (e.g., through a rootkit), the execution state of the TAs running inside a TEE cannot be inspected or tampered with, thus offering strong confidentiality and integrity protection.

% [Para2] For protecting sensitive applications it typically relies on a privileged execution environment named secure world.
To protect the execution state of TAs, TEEs leverage some essential hardware mechanisms provided by TrustZone. In Armv8-A, TrustZone provides two execution environments named \textit{normal world} and \textit{trusted world}. The normal world runs a rich software stack comprised of full blown OS and applications; often named Rich Execution Environment (REE), it is normally considered untrusted. The trusted world runs a smaller and simpler software stack consisting of the TEE and a set of TAs. In the Arm architecture, the system can be in one of two possible states: \textit{non-secure} and \textit{secure}. These security states map onto the normal and trusted worlds respectively. TrustZone enforces system-wide isolation between both worlds and provides controlled entry-points that enable the system to switch across states. A typical world switch occurs when an application in the REE needs to invoke the services of a specific TA. This case begins with the processor running the REE in non-secure state. The application issues a call to the local OS, which in turn leverages a driver to request a state switch to enter the trusted world. This request is performed via the invocation of an instruction that causes the processor state to change (to secure state), and run a TEE service which in turn will forward the request to the respective TA. When the TA finishes serving the request, the processor changes state back to non-secure state, and resumes the execution of the application in the normal world. Importantly, the Arm architecture provides two physical address spaces -- non-secure and secure. This means that software in non-secure state can only see non-secure resources (e.g., memory), but never secure resources. This is the basic mechanism that TEEs use to shield the memory regions in the trusted world (including TAs' memory) from an untrusted OS running in normal world.

% [Para3] However, in most cases, the secure world operates with overly elevated privileges which is a source of potential threats
However, an important limitation of TrustZone is its lack of defenses against attacks that manage to compromise certain critical components of the TEE software. To understand why, Figure~\ref{fig:intro_trustzone} depicts the internals of a TEE/TA software stack. Different components run at different exception levels. From the bottom up, the secure monitor runs in S-EL3 -- i.e., at the highest privilege level -- and provides basic mechanisms for world context switching and platform-specific management (e.g., power management). The trusted OS runs in S-EL1 -- i.e., kernel mode -- and implements essential memory management,  scheduling, IPC, and common services for TAs. TAs run in S-EL0 -- i.e., user mode -- and run with the least privileges of all. If a TA gets compromised, e.g., after exploiting a vulnerability, the attacker will be restricted only to accessing the memory address space of that particular TA. However, if an attacker can hijack the trusted OS he can immediately fully control the system, including (a) the REE in the normal world, (b) all guest TAs, and (c) the secure monitor -- both latter in the trusted world. This level of control is possible because S-EL1 gives full permission to access and configure both secure and non-secure memory regions. For similar reasons, this level of control would also be obtained by hijacking the secure monitor.

Unfortunately, many devices today face serious risks of being compromised by attacks of this nature. In the past, security researchers have demonstrated how an attacker, operating from the normal world, can escalate privileges into S-EL1 mode by chaining a sequence of two exploits~\cite{gb-exploit4,gb-exploit5}. First, exploiting a vulnerable DRM media decoding TA, and then a vulnerability in the trusted OS. From there, security researchers have shown how to (a) gain control of the Linux kernel, (b) retrieve decryption keys from Android KeyStore TA, or (c) access platform cryptographic keys controlled by the secure monitor. Notably, recent studies~\cite{Cerdeira2020} have shown that commercial TEE systems are plagued with a large number of vulnerabilities, most of them affecting TA and trusted OS software. This suggests that the current attack surface for TEE systems is seriously enlarged, being TA and trusted OS highly attractive vectors for launching critical attacks. Currently, TrustZone offers no protection against such a catastrophic breach of security that results from compromising the trusted OS. %which can considered to be catastrophic. %Given the proliferation of many Armv8-A devices featuring TrustZone technology, providing effective defenses against these attacks is fundamental. 

% [Para4] Despite the large body of work on TrustZone and TEE, there are limited solutions for reducing privileges in the secure world for mitigating these threats.

Despite the abundant research on securing TrustZone-assisted TEEs, not many systems can offer practical defenses for thwarting privilege escalation attacks in the case where the trusted OS has been compromised as described above. In one line of work, we find systems like Sanctuary~\cite{Brasser2019} that aim to reduce the attack surface of the trusted OS by shifting TAs from the trusted world into user-level enclaves in the normal world. In practice, however, due to portability reasons and the existence of legacy code, vendors and OEMs continue deploying TAs in the secure world for many devices making them vulnerable to attacks. Other works propose techniques to verify the code of the trusted OS. While this is an extremely important direction, it forces the replacement of pre-existing TEE software making this solution not yet ready for widespread adoption. A third approach is to confine individual instances of TEE/TA stacks inside sandboxes in the trusted world, e.g., by leveraging a hypervisor~\cite{hafnium} or same-privilege isolation~\cite{Kwon19,Li2019}. This is an interesting direction as it would prevent a compromised trusted OS from further escalating privileges across its own sandbox. However, these approaches tend to depend on large trusted computing bases, which may include a hypervisor or a binary-code rewriting tool, respectively.

% [Para5] In this paper, we present \project, a system that effectively reduces the privileges of the secure world by creating isolated (untrusted) sandboxed domains named \textit{zones}. Show the idea in the figure clearly stating how it allows for memory protection in three dimensions: (a) preventing code from accessing monitor code, (b) from accessing normal world OS, and (c) from access memory of other zones. This effectively thwarts the attacks illustrated in figure x.
In this paper, we present \project, a new security architecture that effectively reduces the privileges of a potentially compromised trusted OS so as to counter ongoing privilege escalation attacks in the system. This is achieved by creating isolated (untrusted) sandboxed domains named \textit{zones} inside the trusted world. Zones have access to private memory regions, and provide an execution environment for S-EL1/S-EL0 code, covering trusted OS and TAs, respectively. \project restricts the memory access privileges of the code running inside a zone (including S-EL1, trusted OS code), preventing it from arbitrarily accessing memory allocated for: (i) the normal world REE software, (ii) the secure monitor, and (iii) other zones. The only way for a given zone to communicate with an external memory protection domain is through mutually shared memory regions. In \project, the monitor still belongs to the trusted computing base. Using \project, a typical, monolithic TEE stack can then be restructured and partitioned into multiple zones, for instance, as depicted in Figure~\ref{fig:intro_rezone}. Each zone contains its own trusted OS instance effectively playing the role of a libOS. Then, we associate user-level TAs and kernel-level TAs to independent zones. With this configuration, an attacker that hijacks the trusted OS in zone 1 (by exploiting the vulnerabilities as described in Figure~\ref{xxx}), will not be able to further escalate its privileges to access secure monitor or normal world memory. This separation of TAs across zones, further prevents attackers from using user-level TAs -- which are more commonly plagued with vulnerabilities -- as stepping stones for interfering with kernel-level TAs, which implement critical system functions. To give vendors and OEMs maximal flexibility, \project can be configured differently, allowing the TEE stack to be partitioned into additional zones, and different trusted OSes to be deployed in different zones.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/intro-trustzone.pdf}
    \caption{Privilege escalation attack in a TrustZone-assisted TEE: (1) hijack a user-level TA, e.g., exploiting vulnerability in the Widevine TA (CVE-2015-6639)~\cite{gb-exploit4}, (2) hijack the trusted OS, e.g., exploiting vulnerability in syscall interface of Qualcomm's QSEOS (CVE-2016-2431)~\cite{gb-exploit5}. Once in control of the trusted OS, other attacks can be launched: (a) control the rich OS, e.g., by deploying a backdoor in the Linux kernel~\cite{gb-exploit6}, (b) control a kernel-level TA, e.g., to extract full disk encryption keys of Android's KeyMaster service~\cite{gb-keymaster}, or (c) control the secure monitor, e.g., to unblock the device bootloader~\cite{gb-bootloader}.}
    \label{fig:intro_trustzone}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/intro-rezone.pdf}
    \caption{\project setup enforcing TEE privilege reduction: after compromising user-level TA$_\textrm{U}$ and trusted OS in Zone U, an attacker cannot escalate privileges to (a) rich OS, (b) kernel-level TA$_\textrm{K}$ in Zone K, or (c) secure monitor.}
    \label{fig:intro_rezone}
\end{figure}

% [Para6] In contrast to alternative sandboxing systems for the secure world, \project does not require hypervisor or same-privilege isolation. Instead, it leverages new hardware mechanisms that allow us to implement memory-protection while (1) preserving retro-compatibility with existing TEE software, and (2) adding only a few lines of code to the ATF monitor software. Specifically, \project leverages two bus masters and a dedicated microcontroller available on modern platforms. One bus master 
A central technical novelty of \project's design is that we take advantage of a hardware address space controller available in modern platforms to restrict the privileges of S-EL1 (trusted OS) code. Existing systems such as Sanctuary~\cite{Brasser2019} have already leveraged a TrustZone address space controller named TZASC for protecting user-level enclaves in the normal world. TZASC controllers, such as the TZC-400, feature the possibility to specify access permissions to various physical memory regions, including the ability to prevent trusted world code from accessing normal world memory. However, these configurations can be reverted by S-EL1 code, rendering the TZASC ineffective for enforcing zone isolation. Instead, we use a TrustZone-agnostic address space controller that can allow only a specific bus master to reconfigure memory access permissions. An example of such a controller is the RDC, available in iMX8MQ and iMX8QM boards. In \project, we harness this feature and reserve a low-end micro-controller available in the SoC to be exclusively responsible for setting these permissions, e.g., specifying the private memory regions of each zone. Given that the platform's main cores cannot override these permissions (not even when running in S-EL1), RDC and micro-controller can then be used as building blocks for restricting the memory access privileges of (a potentially compromised) trusted OS, and enforce strong zone isolation.

% [Para7] Although the key insight is simple, the design of \project is not straightforward. From the security standpoint, we need to cover several corner cases involving the behavior of L1 and L2 caches that could lead to security breaches. Moreover, preventing some of these breaches inevitably requires cache flushes upon transitioning between zones which pays a performance toll. \project also has to cope with less efficient microcontroller which may lead to additional overheads. In our design, we propose several techniques that both (1) guarantee the memory isolation of each zone, and (2) can reduce the system overheads and costs of zone switching.
% [Para8] We have implemented \project on real hardware boards featuring Mxxx. Tested with OP-TEE. We will open source our prototype. We have extensively evaluated our system with several benchmarks and use case applications. 
Based on this insight, we have built \project. Our system includes multiple non-trivial optimizations and mechanisms to manage the life-cycle of zones and guarantee system-wide security (e.g., avoiding cache-based data leaks). To make our design generally applicable to various hardware platforms, we specify the general properties of TrustZone-agnostic address space controllers that satisfy \project's requirements. We have fully implemented \project for the iMX8MQ platform, and integrated \project with Android OS and OP-TEE -- i.e., REE and TEE, respectively. Our code will be made open source.

% [Para9] Our evaluation results show that despite the existence of sensible performance overheads in microbenchmarks, in full blown applicaitons, \project does not meaningfully degrade the performance of applications such as Wallet or even DRM. In particular, a DRM application -- which requires frequent transitions between normal world OS and the zone where the DRM application runs, has an overhead of only X%. The overall performance of the system is not affected. We have also surveyed 50 CVE vulnerability reports and estimate that \project will be able to thwart 80% of potential privilege escalation attacks that could result from exploiting these bugs.
We have extensively evaluated \project using various benchmarks and real-world applications. Our evaluation results show that despite the existence of sensible performance overheads in microbenchmarks, in full blown applications, \project does not meaningfully degrade the performance of applications such as Wallet or even DRM. In particular, a DRM application -- which requires frequent transitions between normal world OS and the zone where the DRM application runs, has an overhead of only X\%. The overall performance of the system is not affected. We have also surveyed 50 CVE vulnerability reports and estimate that \project will be able to thwart 80\% of potential privilege escalation attacks that could result from exploiting these bugs.

% [Para3] However, for protecting sensitive applications, it relies on a protection domain that often operates with overly elevated privileges and this is a source of potential threats




% What problem do we address
%There have been numerous reports of vulnerabilities in TrustZone-based TEEs. In particular in trusted applications and in Trusted OSs, with some trusted applications vulnerabilities having been used as a stepping stone to exploit the Trusted OS. Although, the Trusted OS is not the highest privileged piece of software, TrustZone design provides it with enough tools to become as privilege as the secure monitor.

\if0

TrustZone design gives control of most of the platform to the Trusted OS. There are still some features which are configured by the secure monitor only (e.g., debugging \textit{, anything else?}), and a strong register separation, however a malicous Trusted OS can inject code into the secure monitor. This is a direct consequence of having all secure-world accesses be treated as the same, which prevents the secure monitor from accessing secure devices which the trustOS cannot access. Additionally, because a Trusted OS can access physical memory arbitrarily, it could also modify secure monitor code. This prevents a clear-cut privilege separation between EL3 and sEL1, and enables attackers who can compromise sEL1, to also compromise EL3.
A Trusted OS having access to all physical memory can also compromise the normal-world OS, for example to create backdoors [ref to escalating privileges to linux kernel from QSEE], or compromise the trusted applications [ref to breaking FDE in Android]. Furthermore because Trusted OS attacks are often launched from trusted applications, it may be possible that by exploiting a vulnerability in a trusted application an attacker can compromise another trusted application.
This design aspect of TrustZone, allows exploited vulnerabilities in Trusted OS to potentially compromise the system as whole.
\textit{Sidenote: platforms which feature lock bits are less prone to this. For example the iMX8M allows establishing and locking domains until a hardware reset, but the application processor, and associated domain is still fully compromised.}



% What's the solution
To solve for these issues, the following should be possible:
\begin{enumerate}
    \item\label{priv_monitor} secure monitor and normal world code and data (excl. shared memory) should be inaccessible to the Trusted OS
    \item\label{mult} vulnerabilities in one trusted application should not affect another trusted application
    \item\label{normal} only shared memory regions of the normal-world, should be accessible to the Trusted OS
\end{enumerate}

By protecting the secure monitor from possibly malicious interference of the trustOS, it is possible to minimize the impact of attacks on the Trusted OS. The secure monitor will always be able to regain control of the platform, and it may implement functionality to detect a compromised Trusted OS. To implement \ref{priv_monitor}), we devised the solution described in ($\S$\ref{sec:scheme}). This solution leverages TrustZone independent hardware enforced isolation and a context switching scheme relying on an additional processing unit.

To prevent vulnerabilities in one application from affecting another, we propose the creation of multiple environments. These environments encompass a Trusted OS and a collection of trusted applications which may be related. For example we consider the case for a system environment which supports all trusted applications providing services to the OS. Additional environments might be created for each vendor so that their apps are not susceptible to vulnerabilities from another vendor, and it allows to open the environment for developer trusted applications as long as the Trusted OS supporting them is without flaws, or \ref{normal}) is true.
For addressing \ref{mult}), we implemented a Trusted OS context switching scheme, which protects all the involved Trusted OSs, and relies on assumption \ref{priv_monitor}), as described in ($\S$\ref{sec:mult}).

Only allowing specific normal-world memory regions to be accessed by the Trusted OS, protects the normal-world against a rogue Trusted OS and limits the impact of vulnerabilities or flaws Trusted OS may have. For example it prevents a compromised Trusted OS from installing a backdoor in the normal-world kernel.
To address \ref{normal}), we perform cache maintenance operations, leverage the onboard memory access controller, and suspend cores running in the normal world as described in ($\S$\ref{sec:normal}). 

We implement these mechanisms in two platforms, iMX8MQ and iMX8QM. These platforms feature different hardware and hardware architectures which shows that our solution is not dependent on a single platform, and that it works in real deployable systems.

\fi



\if0

\begin{itemize}
    \item Secure monitor fully isolated from Trusted OS
    \item No same privilege isolation for separating TEEs
    \item Normal world protection
\end{itemize}
\nuno{Scratch: begin}

1. TrustZone everywhere for securing mobile and IoT devices.

2. However, lots of vulnerabilities

3. A fundamental problem remains despite multiple proposed solutions: trusted OS is more privileged than the OS. Insight: today normal world OS and secure world OS are highly uneven in terms of privileges: why does the secure world OS need to have so much privileges in the system? By exploiting a single bug in the trusted OS an adversary can gain full control over the system. We investigate how these privileges can be balanced out and enforce the principle of least privilege.

4. We propose hardware-enforced {\em secure realms}, where we break up the privileges of the secure world attributed to the trusted OS into multiple isolated environments that can host the trusted OS with the following reduction of privileges: i) isolation from the normal world, ii) isolation from the monitor. Possibility to create multiple secure realm instances allowing for multiple TEEs to exist thereby separating user-level applications from OS-level applications. Does not preclude the use of virtualization inside a secure realm (?). Can be used in conjunction with other TEE architectures, e.g., that shift the TA execution to the normal world such as Sanctuary (?).

\nuno{Scratch: end}

%\textbf{NS: I suggest that you try to write a proper intro :) It's good to help you organize the ideas. There are four main questions any good paper must answer: (a) what's the problem you're concerned about? (b) why is that problem interesting? (c) what's the solution you propose? (d) how does your solution solve the entirely of the problem? Naturally, the intro doesn't need to be written entirely in this order, but these points must somehow be explained there.}

% Why is the problem interesting
TrustZone is a technology embedded into Arm processors present in mobile phones, and other platforms with application processors, such as Infotainment centers in automotive products, and SmartTVs in our living rooms. Vendors and OEMs rely on TrustZone for two main different use cases. One is assisting the operating system in ensuring authentication, generating secure cryptographic keys, or providing the means for implementing file disk encryption for example. The other is to provide vendors with an environment for securely processing and obtaining data, the most representative of these are DRM solutions, and electronic payments.
Both these cases require an environment inaccessible to the operating system. The goal being that even if the OS is compromised, as is often the case [ref to android kernel vulnerabilities], it still is not possible to retrieve secrets or compromise operation within the secure environment.

% What problem do we address
There have been numerous reports of vulnerabilities in TrustZone-based TEEs. In particular in trusted applications and in Trusted OSs, with some trusted applications vulnerabilities having been used as a stepping stone to exploit the Trusted OS.
Although, the Trusted OS is not the highest privileged piece of software, TrustZone design provides it with enough tools to become as privilege as the secure monitor.

TrustZone design gives control of most of the platform to the Trusted OS. There are still some features which are configured by the secure monitor only (e.g., debugging \textit{, anything else?}), and a strong register separation, however a malicous Trusted OS can inject code into the secure monitor. This is a direct consequence of having all secure-world accesses be treated as the same, which prevents the secure monitor from accessing secure devices which the trustOS cannot access. Additionally, because a Trusted OS can access physical memory arbitrarily, it could also modify secure monitor code. This prevents a clear-cut privilege separation between EL3 and sEL1, and enables attackers who can compromise sEL1, to also compromise EL3.
A Trusted OS having access to all physical memory can also compromise the normal-world OS, for example to create backdoors [ref to escalating privileges to linux kernel from QSEE], or compromise the trusted applications [ref to breaking FDE in Android]. Furthermore because Trusted OS attacks are often launched from trusted applications, it may be possible that by exploiting a vulnerability in a trusted application an attacker can compromise another trusted application.
This design aspect of TrustZone, allows exploited vulnerabilities in Trusted OS to potentially compromise the system as whole.
\textit{Sidenote: platforms which feature lock bits are less prone to this. For example the iMX8M allows establishing and locking domains until a hardware reset, but the application processor, and associated domain is still fully compromised.}



% What's the solution
To solve for these issues, the following should be possible:
\begin{enumerate}
    \item\label{priv_monitor} secure monitor and normal world code and data (excl. shared memory) should be inaccessible to the Trusted OS
    \item\label{mult} vulnerabilities in one trusted application should not affect another trusted application
    \item\label{normal} only shared memory regions of the normal-world, should be accessible to the Trusted OS
\end{enumerate}

By protecting the secure monitor from possibly malicious interference of the trustOS, it is possible to minimize the impact of attacks on the Trusted OS. The secure monitor will always be able to regain control of the platform, and it may implement functionality to detect a compromised Trusted OS. To implement \ref{priv_monitor}), we devised the solution described in ($\S$\ref{sec:scheme}). This solution leverages TrustZone independent hardware enforced isolation and a context switching scheme relying on an additional processing unit.

To prevent vulnerabilities in one application from affecting another, we propose the creation of multiple environments. These environments encompass a Trusted OS and a collection of trusted applications which may be related. For example we consider the case for a system environment which supports all trusted applications providing services to the OS. Additional environments might be created for each vendor so that their apps are not susceptible to vulnerabilities from another vendor, and it allows to open the environment for developer trusted applications as long as the Trusted OS supporting them is without flaws, or \ref{normal}) is true.
For addressing \ref{mult}), we implemented a Trusted OS context switching scheme, which protects all the involved Trusted OSs, and relies on assumption \ref{priv_monitor}), as described in ($\S$\ref{sec:mult}).

Only allowing specific normal-world memory regions to be accessed by the Trusted OS, protects the normal-world against a rogue Trusted OS and limits the impact of vulnerabilities or flaws Trusted OS may have. For example it prevents a compromised Trusted OS from installing a backdoor in the normal-world kernel.
To address \ref{normal}), we perform cache maintenance operations, leverage the onboard memory access controller, and suspend cores running in the normal world as described in ($\S$\ref{sec:normal}). 

We implement these mechanisms in two platforms, iMX8MQ and iMX8QM. These platforms feature different hardware and hardware architectures which shows that our solution is not dependent on a single platform, and that it works in real deployable systems.


\fi

% Does the solution solve the problem entirely



==> extra/main_body-bak.tex <==
%=======================================================================
%> [INTRO]
%=======================================================================	
\section{Introduction}

% [Para1] TrustZone is widely available for securing sensitive applications, both user-level and kernel-level applications.


% [Para2] For protecting sensitive applications it typically relies on a privileged execution environment named secure world.

% [Para3] However, in most cases, the secure world operates with overly elevated privileges which is a source of potential threats

% [Para4] Despite the large body of work on TrustZone and TEE, there are limited solutions for reducing privileges in the secure world for mitigating these threats.

% [Para5] In this paper, we present ReZone, a system that effectively reduces the privileges of the secure world by creating isolated (untrusted) sandboxed domains named \textit{zones}. Show the idea in the figure clearly stating how it allows for memory protection in three dimensions: (a) preventing code from accessing monitor code, (b) from accessing normal world OS, and (c) from access memory of other zones. This effectively thwarts the attacks illustrated in figure x.

% [Para6] In contrast to alternative sandboxing systems for the secure world, ReZone does not require hypervisor or same-privilege isolation. Instead, it leverages new hardware mechanisms that allow us to implement memory-protection while (1) preserving retro-compatibility with existing TEE software, and (2) adding only a few lines of code to the ATF monitor software. Specifically, ReZone leverages two bus masters and a dedicated microcontroller available on modern platforms. One bus master 

% [Para7] Although the key insight is simple, the design of ReZone is not straightforward. From the security standpoint, we need to cover several corner cases involving the behavior of L1 and L2 caches that could lead to security breaches. Moreover, preventing some of these breaches inevitably requires cache flushes upon transitioning between zones which pays a performance toll. ReZone also has to cope with less efficient microcontroller which may lead to additional overheads. In our design, we propose several techniques that both (1) guarantee the memory isolation of each zone, and (2) can reduce the system overheads and costs of zone switching.

% [Para8] We have implemented ReZone on real hardware boards featuring Mxxx. Tested with OP-TEE. We will open source our prototype. We have extensively evaluated our system with several benchmarks and use case applications. 

% [Para9] Our evaluation results show that despite the existence of sensible performance overheads in microbenchmarks, in full blown applicaitons, ReZone does not meaningfully degrade the performance of applications such as Wallet or even DRM. In particular, a DRM application -- which requires frequent transitions between normal world OS and the zone where the DRM application runs, has an overhead of only X%. The overall performance of the system is not affected. We have also surveyed 50 CVE vulnerability reports and estimate that ReZone will be able to thwart 80% of potential privilege escalation attacks that could result from exploiting these bugs.


% [Para3] However, for protecting sensitive applications, it relies on a protection domain that often operates with overly elevated privileges and this is a source of potential threats


TrustZone is a technology embedded into Arm processors present in mobile phones, and other platforms with application processors, such as Infotainment centers in automotive products, and SmartTVs in our living rooms. Vendors and OEMs rely on TrustZone for two main different use cases. One is assisting the operating system in ensuring authentication, generating secure cryptographic keys, or providing the means for implementing file disk encryption for example. The other is to provide vendors with an environment for securely processing and obtaining data, the most representative of these are DRM solutions, and electronic payments.
Both these cases require an environment inaccessible to the operating system. The goal being that even if the OS is compromised, as is often the case~\cite{xxx}, it still is not possible to retrieve secrets or compromise security-sensitive operations.

% What problem do we address
There have been numerous reports of vulnerabilities in TrustZone-based TEEs. In particular in trusted applications and in Trusted OSs, with some trusted applications vulnerabilities having been used as a stepping stone to exploit the Trusted OS.
Although, the Trusted OS is not the highest privileged piece of software, TrustZone design provides it with enough tools to become as privilege as the secure monitor.

TrustZone design gives control of most of the platform to the Trusted OS. There are still some features which are configured by the secure monitor only (e.g., debugging \textit{, anything else?}), and a strong register separation, however a malicous Trusted OS can inject code into the secure monitor. This is a direct consequence of having all secure-world accesses be treated as the same, which prevents the secure monitor from accessing secure devices which the trustOS cannot access. Additionally, because a Trusted OS can access physical memory arbitrarily, it could also modify secure monitor code. This prevents a clear-cut privilege separation between EL3 and sEL1, and enables attackers who can compromise sEL1, to also compromise EL3.
A Trusted OS having access to all physical memory can also compromise the normal-world OS, for example to create backdoors [ref to escalating privileges to linux kernel from QSEE], or compromise the trusted applications [ref to breaking FDE in Android]. Furthermore because Trusted OS attacks are often launched from trusted applications, it may be possible that by exploiting a vulnerability in a trusted application an attacker can compromise another trusted application.
This design aspect of TrustZone, allows exploited vulnerabilities in Trusted OS to potentially compromise the system as whole.
\textit{Sidenote: platforms which feature lock bits are less prone to this. For example the iMX8M allows establishing and locking domains until a hardware reset, but the application processor, and associated domain is still fully compromised.}



% What's the solution
To solve for these issues, the following should be possible:
\begin{enumerate}
    \item\label{priv_monitor} secure monitor and normal world code and data (excl. shared memory) should be inaccessible to the Trusted OS
    \item\label{mult} vulnerabilities in one trusted application should not affect another trusted application
    \item\label{normal} only shared memory regions of the normal-world, should be accessible to the Trusted OS
\end{enumerate}

By protecting the secure monitor from possibly malicious interference of the trustOS, it is possible to minimize the impact of attacks on the Trusted OS. The secure monitor will always be able to regain control of the platform, and it may implement functionality to detect a compromised Trusted OS. To implement \ref{priv_monitor}), we devised the solution described in ($\S$\ref{sec:scheme}). This solution leverages TrustZone independent hardware enforced isolation and a context switching scheme relying on an additional processing unit.

To prevent vulnerabilities in one application from affecting another, we propose the creation of multiple environments. These environments encompass a Trusted OS and a collection of trusted applications which may be related. For example we consider the case for a system environment which supports all trusted applications providing services to the OS. Additional environments might be created for each vendor so that their apps are not susceptible to vulnerabilities from another vendor, and it allows to open the environment for developer trusted applications as long as the Trusted OS supporting them is without flaws, or \ref{normal}) is true.
For addressing \ref{mult}), we implemented a Trusted OS context switching scheme, which protects all the involved Trusted OSs, and relies on assumption \ref{priv_monitor}), as described in ($\S$\ref{sec:mult}).

Only allowing specific normal-world memory regions to be accessed by the Trusted OS, protects the normal-world against a rogue Trusted OS and limits the impact of vulnerabilities or flaws Trusted OS may have. For example it prevents a compromised Trusted OS from installing a backdoor in the normal-world kernel.
To address \ref{normal}), we perform cache maintenance operations, leverage the onboard memory access controller, and suspend cores running in the normal world as described in ($\S$\ref{sec:normal}). 

We implement these mechanisms in two platforms, iMX8MQ and iMX8QM. These platforms feature different hardware and hardware architectures which shows that our solution is not dependent on a single platform, and that it works in real deployable systems.




\if0

\begin{itemize}
    \item Secure monitor fully isolated from Trusted OS
    \item No same privilege isolation for separating TEEs
    \item Normal world protection
\end{itemize}
\nuno{Scratch: begin}

1. TrustZone everywhere for securing mobile and IoT devices.

2. However, lots of vulnerabilities

3. A fundamental problem remains despite multiple proposed solutions: trusted OS is more privileged than the OS. Insight: today normal world OS and secure world OS are highly uneven in terms of privileges: why does the secure world OS need to have so much privileges in the system? By exploiting a single bug in the trusted OS an adversary can gain full control over the system. We investigate how these privileges can be balanced out and enforce the principle of least privilege.

4. We propose hardware-enforced {\em secure realms}, where we break up the privileges of the secure world attributed to the trusted OS into multiple isolated environments that can host the trusted OS with the following reduction of privileges: i) isolation from the normal world, ii) isolation from the monitor. Possibility to create multiple secure realm instances allowing for multiple TEEs to exist thereby separating user-level applications from OS-level applications. Does not preclude the use of virtualization inside a secure realm (?). Can be used in conjunction with other TEE architectures, e.g., that shift the TA execution to the normal world such as Sanctuary (?).

\nuno{Scratch: end}

%\textbf{NS: I suggest that you try to write a proper intro :) It's good to help you organize the ideas. There are four main questions any good paper must answer: (a) what's the problem you're concerned about? (b) why is that problem interesting? (c) what's the solution you propose? (d) how does your solution solve the entirely of the problem? Naturally, the intro doesn't need to be written entirely in this order, but these points must somehow be explained there.}

% Why is the problem interesting
TrustZone is a technology embedded into Arm processors present in mobile phones, and other platforms with application processors, such as Infotainment centers in automotive products, and SmartTVs in our living rooms. Vendors and OEMs rely on TrustZone for two main different use cases. One is assisting the operating system in ensuring authentication, generating secure cryptographic keys, or providing the means for implementing file disk encryption for example. The other is to provide vendors with an environment for securely processing and obtaining data, the most representative of these are DRM solutions, and electronic payments.
Both these cases require an environment inaccessible to the operating system. The goal being that even if the OS is compromised, as is often the case [ref to android kernel vulnerabilities], it still is not possible to retrieve secrets or compromise operation within the secure environment.

% What problem do we address
There have been numerous reports of vulnerabilities in TrustZone-based TEEs. In particular in trusted applications and in Trusted OSs, with some trusted applications vulnerabilities having been used as a stepping stone to exploit the Trusted OS.
Although, the Trusted OS is not the highest privileged piece of software, TrustZone design provides it with enough tools to become as privilege as the secure monitor.

TrustZone design gives control of most of the platform to the Trusted OS. There are still some features which are configured by the secure monitor only (e.g., debugging \textit{, anything else?}), and a strong register separation, however a malicous Trusted OS can inject code into the secure monitor. This is a direct consequence of having all secure-world accesses be treated as the same, which prevents the secure monitor from accessing secure devices which the trustOS cannot access. Additionally, because a Trusted OS can access physical memory arbitrarily, it could also modify secure monitor code. This prevents a clear-cut privilege separation between EL3 and sEL1, and enables attackers who can compromise sEL1, to also compromise EL3.
A Trusted OS having access to all physical memory can also compromise the normal-world OS, for example to create backdoors [ref to escalating privileges to linux kernel from QSEE], or compromise the trusted applications [ref to breaking FDE in Android]. Furthermore because Trusted OS attacks are often launched from trusted applications, it may be possible that by exploiting a vulnerability in a trusted application an attacker can compromise another trusted application.
This design aspect of TrustZone, allows exploited vulnerabilities in Trusted OS to potentially compromise the system as whole.
\textit{Sidenote: platforms which feature lock bits are less prone to this. For example the iMX8M allows establishing and locking domains until a hardware reset, but the application processor, and associated domain is still fully compromised.}



% What's the solution
To solve for these issues, the following should be possible:
\begin{enumerate}
    \item\label{priv_monitor} secure monitor and normal world code and data (excl. shared memory) should be inaccessible to the Trusted OS
    \item\label{mult} vulnerabilities in one trusted application should not affect another trusted application
    \item\label{normal} only shared memory regions of the normal-world, should be accessible to the Trusted OS
\end{enumerate}

By protecting the secure monitor from possibly malicious interference of the trustOS, it is possible to minimize the impact of attacks on the Trusted OS. The secure monitor will always be able to regain control of the platform, and it may implement functionality to detect a compromised Trusted OS. To implement \ref{priv_monitor}), we devised the solution described in ($\S$\ref{sec:scheme}). This solution leverages TrustZone independent hardware enforced isolation and a context switching scheme relying on an additional processing unit.

To prevent vulnerabilities in one application from affecting another, we propose the creation of multiple environments. These environments encompass a Trusted OS and a collection of trusted applications which may be related. For example we consider the case for a system environment which supports all trusted applications providing services to the OS. Additional environments might be created for each vendor so that their apps are not susceptible to vulnerabilities from another vendor, and it allows to open the environment for developer trusted applications as long as the Trusted OS supporting them is without flaws, or \ref{normal}) is true.
For addressing \ref{mult}), we implemented a Trusted OS context switching scheme, which protects all the involved Trusted OSs, and relies on assumption \ref{priv_monitor}), as described in ($\S$\ref{sec:mult}).

Only allowing specific normal-world memory regions to be accessed by the Trusted OS, protects the normal-world against a rogue Trusted OS and limits the impact of vulnerabilities or flaws Trusted OS may have. For example it prevents a compromised Trusted OS from installing a backdoor in the normal-world kernel.
To address \ref{normal}), we perform cache maintenance operations, leverage the onboard memory access controller, and suspend cores running in the normal world as described in ($\S$\ref{sec:normal}). 

We implement these mechanisms in two platforms, iMX8MQ and iMX8QM. These platforms feature different hardware and hardware architectures which shows that our solution is not dependent on a single platform, and that it works in real deployable systems.


\fi

% Does the solution solve the problem entirely




%=======================================================================
%> [BACKGROUND]
%=======================================================================	
%\section{Background and Attacks}

\section{Background and Motivation}

%This section provides context on TrustZone-assisted TEEs, attacks, and hardware access control filters.

\subsection{TrustZone-assisted TEE}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/tz-SW-HW.pdf}
    \caption{TrustZone-assisted TEE: hardware-software architecture}
    \label{fig:tz_sw_overview}
\end{figure}

% \textbf{NS: Please turn this into paragraphs. Tell a story. See how we do it in the S\&P paper to introduce the reader to TrustZone technology. First present the overall architecture showing NW/SW separation, say that each core can run in each world. Maybe at this point talk about the TZAC and the system-wide memory protection mechanisms to conclude the description of the hardware architecture. Then, on a second paragraph, present the typical software stack comprising the rich OS then the Trusted OS running in the SW (EL-1 ring) along with the monitor (in EL-3) (which is necessary to present here because you will talk about that later). Say that the software in SW have full access to the whole memory, both NW and NW. Then proceed to explaining that there are unprivileged trusted applications (TAs) running in EL-0. Some of these are geral purpose, others are system TAs, etc. As it is now, everything is mixed up.}
% \begin{itemize}
%     \item Trusted OS - Vendor dependent software
%     \item System TAs - 2 factor auth data; keychain data (banking, password management...); private keys (gpg, signing certificates, electronic IDs, device encryption...); biometric data (ie: fingerprint), etc...
%     \item General Purpose TAs - Vendor software, and partners software: Disney, Paramount, Sony Pictures, 20th Century Fox, Universal Studios, Warner Bros
%     \item Monitor - Commonly implemented by customizing Arm-Trusted-Firmware
%     \item .
% \end{itemize}

%\nuno{The whole text of this section is very good, but I it's quite long and too full of details. I think we should shorten it and present only the bare minimum that allows the reader to understand the attacks that will be introduced in the next section. Many of the low level details presented here can be briefed in latter sections as we present the design and implementation of our system. The takeaway point from this background section is that the SW software is almighty.}

%\sandro{I would suggest to reduce the intro para and merge the SW Architecture together into the intro paragraph. We need to discuss if the full TZASC paragraph can be removed.. I'm not 100\% convinced.. }



TrustZone is a System-on-Chip (SoC) and CPU system-wide security solution available in a broad range of Arm processors. The technology has been pivotal for the materialization of TEEs in mobile devices by providing an isolated environment for secure processing of sensitive data and programs (i.e., trusted applications). TrustZone is built upon the concept of protection domains, i.e., the {\em secure world} (SW) and the {\em normal world} (NW). The SW shields critical functionality from the NW, which is used for running an untrusted operating system (OS) and its applications. 
%In the TrustZone hardware architecture, each physical processor provides two virtual cores and a set of well-defined mechanisms (e.g., {\em monitor mode}, SMC instruction) to switch between secure and non-secure states. At a given point in time, the world where the processor currently executes is based on the state of the Non-Secure (NS) bit. There is additional hardware logic in a TrustZone-enabled SoC that extends the security state of the processor to other system components, i.e., bus, interrupt controller, memory hierarchy, and peripherals. 
%ensuring that SW resources cannot be accessed by NW components.
%\mypara{Software Architecture}. 
\autoref{fig:tz_sw_overview} depicts the software architecture of a TrustZone-assisted TEE. Inside the SW runs the TEE software, while in the NW run the Rich Execution Environment (REE) and untrusted applications. The TEE software has three fundamental building blocks: the {\em secure monitor}, the {\em trusted OS}, and {\em trusted Applications}. The secure monitor, running at the higher level of privilege (i.e., S-EL3), provides basic mechanisms for secure context switching and platform-specific management (e.g., power management). The trusted OS runs in S-EL1 and provides an underlying infrastructure for sustaining the lifecycle of TAs. TAs execute in unprivileged S-EL0 and are typically developed by platform vendors and OEMs. 
%Core components of the trusted OS encompass (i) the trusted kernel, which provides the basic OS primitives for managing TAs, (ii) device drivers for accessing trusted peripherals, (iii) low-level code for cross-world interactions, and (iv) shared libraries (e.g., cryptographic) and TEE primitives, such as remote attestation, trusted I/O, and secure storage. 


%Trusted applications are unprivileged programs that make use of the Trusted OS services to implement a wide range of features, which serve mainly two purposes. One is providing trusted services to the system and the OS. This includes handling biometric identification, cryptographic key management and trusted random number generation, to name a few. This is software developed by the platform vendor or OEMs. The other purpose of TAs is implementing application specific services whose compromised functionality affects the company who developed them or the user, but not the system directly. Examples of this are TAs part of DRM solutions, and TAs implementing part of electronic payments systems. Some applications require efficient cross-world communication mechanisms. To enable this, trusted OSs often allow TAs to map physical memory. The Trusted OS manages the physical memory available to each TA, some Trusted OS implementations enable TAs to map any normal-world address, while others only enable the mapping of specific shared memory regions. The last piece of a running TEE, is the {\em secure monitor}, which implements mechanisms for secure context switching between worlds and runs with highest privilege, in protection ring EL3. 


%The {\em TEE bootloader} bootstraps the TEE system into a secure state, and it is critical to implement the trusted boot primitive. Together, trusted applications, trusted OS, secure monitor, and TEE bootloader constitute the software TCB of a typical TEE system. For this reason, TEE designers aim for small and bug-free implementations. Nonetheless, vulnerabilities exist and attacks are successful.

%\mypara{TrustZone Address Space Controller.}
%The TrustZone Address Space Controller (TZASC) enforces physical memory protection in TrustZone-based systems. The TZASC allows the partition of external memory on secure and non-secure regions. To date, Arm has publicly released two TZASC specifications, i.e., the Arm CoreLink TZC-380~\cite{} and TZC-400~\cite{}. Both controllers share similar high-level features, i.e., the ability to configure the security access permissions for memory regions (contiguous areas in the address space), but, at the low-level, there are slight differences. For instance, the TZC-380 provides a \textit{security inversion} option (disabled by default), which allow non-secure memory regions to not be accessible to masters in a secure state. This feature is not available in the TZC-400. The TZC-400 introduces a set of prime mechanisms for fine-grain isolation, in particular, the \textit{identity-based filtering of non-secure accesses}, which allows per bus master (e.g., CPU cluster, MCU, DMA controller) partition. Despite the existence of TZC-380 and TZC-400 specifications, OEM manufacturers typically embedded their own proprietary controllers into their SoCs (e.g., Rockchip RK3399, \textcolor{red}{????}, \textcolor{red}{...}), which just provides coarse-grained configuration. Worst, there are SoCs used in well-established Arm-based platforms, e.g., Raspberry Pi 4, which do not feature a TZASC-like controller at all \cite{}. 
%This results in a significant heterogeneity and fragmentation ...        


%At its core TrustZone extends the processor to enable CPU cores to operate in one of two states, secure and non-secure. Memory and resource access are made aware of the current security state of the processor through the NS bit (non-secure bit). The NS bit is then used to bar access to a resource according to the security state. Additionally, secure-world can map the memory as being non-secure, which results in secure-world memory accesses being performed as normal-world accesses. This way, the secure-world can access normal-world as if normal-world is the one accessing the resource. This design decisions makes it hard to prevent secure-world from accessing normal-world memory. For example, TZC-380 is a TrustZone controller developed by Arm which has a feature enabling memory accesses performed in a secure state to not being able to access normal-word memory (priority inversion), however given that secure-world software can map memory as being normal, this does not prevent the secure-world from accessing normal-world memory, it just has to do so intentionally.
%As alluded to earlier, to enforce the access control of each security state it is necessary to use dedicated hardware. Arm sells two TrustZone controllers TZC-380 and TZC-400 to this end. They differ in the features they provide, but both allow for specifying a hierarchy of memory regions with r/w privileges and secure and non-secure access. Although feature-full, Arm's TrustZone controllers are not deployed in every TrustZone-enabled system. It is common for SoC vendors to design and implement their own TrustZone controllers. This enables SoC vendors to tailor the hardware to their specific needs, but also results in less features and in a fragmentation of TrustZone-enabled systems. For example the rk3399 from Rockchip only allows the configuration of memory regions security state, and not other access control mechanism is present (e.g., R/W). Another example, is Zynq xxx, which only allows the configuration of all SRAM as either secure or non-secure. The broadcom SoCs used in the RPi don't feature a TrustZone controller of any sort[...], although the CPU cores themselves implement the TrustZone specification.



\subsection{Exploiting Overprivileged SW Software}\label{sec:attacks}

%\subsection{Attacks}\label{sec:attacks}

\if0
\begin{itemize}
    \item Agrupar classes de ataques
    \item explicar que o modelo actual não funciona
\end{itemize}
\fi

%Modelos dos ataques à TZ, some of which ReZone resolves.
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/TZ-Attacks.pdf}
    \caption{
    High-level view of the major class of attacks targeting TrustZone-assisted TEEs described in the literature that ReZone aims at mitigating.
    %Flow of attacks on TrustZone-based systems. Boomerang~\cite{Aravind2017}, QSEE Privilege Escalation and Exploit~\cite{gb-exploit4}, Exploiting TrustZone on Android~\cite{shen-trustedcore}, Breaking Android Full Disk Encryption~\cite{BreakFDE},  Hijacking the Linux Kernel from QSEE~\cite{gb-exploit6}, EL3 tour~\cite{EL3Tour}, A Deep Dive Into Samsung's TrustZone (Part 3)~\cite{DeepDive}, Breaking Samsung's Arm TrustZone~\cite{BreakingArmTZ}.
    }
    \label{fig:tz_attacks}
\end{figure}

%\nuno{I suggest that we change the title to something more insightful; but it hasn't necessarily need to be this one. The text of this section is all very good. I simply suggest that we emphasize more the root problem, i.e., the fact that SW is overprivileged and because of that even rather simple vulnerabilities in different components of the SW software can be catastrophic. I'd stress this in the first paragraph, and them continue on to explain each of the several attack vectors in its own paragraph. To make it easier to parse the rest of this section, each of these paragraphs could start with a bold title.}

%\sandro{I 100\% agree with Nuno. Going straight to the point into an initial paragraph and then split the discuss the three attack vectors (complementing with concrete CVEs from reported attacks) in specific paragraphs: (i) "Trusted OS can access the secure monitor.", (ii) "Trusted OS can access all TAs memory", (iii) "Trusted OS can access normal world memory"}

In the Armv7-A/Armv8-A architecture, monitor and trusted OS enjoy similar privileges with regard to read-write operations over secure and non-secure memory. Thus, the trusted OS has a complete view and full access to all system resources, including the secure monitor, TAs, and NW software. ... There are a plethora of successful attacks deriving from ... . David et all. \cite{} has recently highlighted the extent of the problem, ... A complete tour on how to compromise the (i) REE kernel and the (ii) TEE kernel from a NSW application is detailed in the paper, but the logical ... 
\autoref{fig:tz_attacks} depicts the three main class of issues existing in TrustZone-assisted TEE deriving from 

%To begin their attack on the secure world, an attacker may start compromise a TA first. There are numerous reports on vulnerabilities in TAs (e.g.,~\cite{gb-exploit4}). These attacks depend on the software quality of the TAs, and as history tells us: writing bug free software is hard. After compromising a TA an attacker may try to compromise the Trusted OS, or the Trusted OS itself may have some vulnerability that may be exploited without exploiting a TA~\cite{shen-trustedcore}, and he may be successful. At this point, an attacker is in a high privileged position, as they can access any resource in the system. If not available to them until now, an attacker may create a backdoor in the normal-world kernel~\cite{gb-exploit6}. It's also possible to compromise TAs from the Trusted OS kernel~\cite{BreakFDE}. Additionally, an attacker may even compromise the secure monitor~\cite{DeepDive} giving them full control of the platform.
%These attacks are depicted in \autoref{fig:tz_attacks}.


\mypara{SW software can access normal world memory.} \cite{gb-exploit6, gb-exploit7, Aravind2017} First, the Trusted OS can not practically be restricted from accessing all normal-world memory. As we will see below in ($\S$\ref{sec:hwmp}), even though TrustZone controllers such as TZC-380 and TZC-400, feature the possibility to define various memory regions, including the ability to prevent secure-world from accessing the normal-world, Trusted OSes can map memory as \emph{normal}, enabling them to perform normal world accesses from secure world. Even though ultimately this features are a non-issue to a compromised Trusted OS, they may raise the bar in preventing attacks such as boomerang attacks~\cite{Aravind2017} and in cases where the Trusted OS is not fully compromised. For this to be true, the cross-world shared memory regions must be grouped into a few memory regions enforceable by the TrustZone controller. This is a limitation of the TrustZone controller which features limited number of regions.

\mypara{Trusted OS can access the secure monitor.} \cite{DeepDive}, \cite{BreakingArmTZ} Second, a Trusted OS can access secure monitor memory. In case a Trusted OS is compromised, a secure monitor could still regain control execution, detect the security breach and handle it in some way, if there was an effective privilege separation between the two pieces of software. However the Trusted OS can high-jack the secure monitor by modifying the code and data of the secure monitor, and gaining access to every resource in the platform, while executing at the highest privilege level. This is possible again due to coarse dual nature of TrustZone, privileged software (i.e., Trusted OS and secure monitor) in the secure-world cannot partitioned.

\mypara{Trusted OS can access all TAs memory}. Third, with a Trusted OS having access to all TAs' memory, an attacker may compromise any other TA without requiring them to be vulnerable~\cite{BreakFDE, DeepDive, shen-trustedcore}. If TrustZone TEE systems were to provide multiple isolated environments, it would be easier to contain vulnerabilities, and in particular Trusted OS vulnerabilities. This also requires additional hardware features to prevent Trusted OSes from accessing each other resources. Some researchers have proposed software based solutions which rely on same privilege isolation techniques~\cite{teev, ...}, but, although we believe these techniques may raise the bar for attackers, we argue they are not sufficient in the presence of a fully compromised Trusted OS.
\david{All TAs shared the same security domain.}


\subsection{Known Defenses and Their Limitations}\label{sec:defenses}

%\nuno{I think we should add a brief section here that explains the different defensive approaches that exist today for thwarting these attacks and explain the weaknesses of these approaches. Come up with three or four categories of existing defense techniques and briefly present them in individual paragraphs. It is in the measure of how compelling our criticism is that we will persuade the reviewers about the benefits of our approach. We should try to criticize the existing approaches in such a way that we find our sweet spot.}

%\sandro{I agree. We have such knowledge from our SOK paper. We can organize this subsection with three paragraphs, each one describing the defense (giving examples with papers) and highlighting existing limitations...}

%\david{usar fraquezas dos trabalhos para justificar o design point}
%\david{objectivos de segurança, portabilidade, performance aceitável}

We highlight two main class of defenses aiming at ...   

\mypara{Isolated compartments within the NW}. A major class of works focused in ... While one line of works, e.g., TrustICE \cite{} and SANCTUARY \cite{}, leverages the TZASC ..., a second line of works, e.g., OSP \cite{}, PrivateZone \cite{}, and vTZ \cite{}, explore the hardware virtualization extensions available in the NW. While the latter can incur in a slight performance degradation, due to the lack of a two-stage translation, the former ... Notwithstanding, both approaches can only protect compromised TAs from accessing the normal world OS, with the caveat ... TAs with access to Trusted OS syscalls ... In all these works, a compromised Trusted OS is still able to access all TAs, the REE kernel, and the monitor, and bring the full system down. 

\mypara{Secure hypervisor within the SW}. Write something here ...





%\subsection{Leveraging Platform-Specific Hardware}\label{sec:approach}

\subsection{The need for reduced SW privileges}

%\nuno{I'm a little bit changing my mind with respect to what I mentioned in our last meeting about moving the description of the new hardware features to latter sections of the paper -- although not entirely because here we should not be so detailed in the description. So, I think it might flow nicely to give the reviewer an intuition of what new hardware features are available our there that we could use to try to overcome all the limitations we highlighted in the section above. Then, after introducing these features point to Figure 3 and say that we aim to investigate how these new features can be leveraged in such a way that we can reduce the privileges in the SW, and proactively prevent the attack vectors described above. I think this is also the place were we should present the general platform features as currently described in Section 4.2; besides the description of the threat model will also require a previous introduction of the platform's features that we're going to use. Then, the next section will orderly clarify our goals and threat model.}


%\sandro{I agree with giving an hint about what we are going to do, but without to much detail. I would suggest the title of this section to be more generic, and not completely focused in the hardware itself, e.g., "The need to reduce Secure World privileges"}

%\jose{I think it would make more sense to move the section here, but simplify it, and leave section 4.2 as is.}

%=======================================================================
%> [Goals and Threat Model]
%=======================================================================	
\section{Threat Model and Goals}

%\sandro{I believe we should present the threat model first and then our goals...}

\subsection{Threat Model}\label{sec:threat_model}

%\nuno{The threat model is supposed to describe the attacks that are within scope and attacks that are not in scope. I think most of the following text must be fixed to describe this information. Note that these are the attacks that the adversary may try to launch to subvert the defense mechanisms of ReZone.}

\sandro{I personally do not like the 1st paragraph. The 2nd paragraph needs strong polishing. The bullet points are good but need some minor touches. The last paragraph needs to be polished - straight to the point.}

The TrustZone threat model, establishes the normal world as untrusted, while trusting the secure world. Namely, the trusted secure world components are the secure monitor, the Trusted OS, and to a lesser extent TAs. However, the prevalence of attacks and flaws targeting secure world shows the inadequacies of this model \cite{Cerdeira2020}.  
%However, TAs can often be targets for privilege escalation, with their compromise leading to powerful attacks \cite{Cerdeira2020}. For this reason we consider that TAs are also trusted in the typical TrustZone-assisted TEE.

With ReZone we aim first to lower the level of trust an end-user must concede to the Trusted OS and its applications, and second to reduce trust between TAs executing in different execution domains. To this end, our threat model considers mutual distrustful domains between the normal world and the Trusted OS, and between Trusted OSes. In practice, a malicious agent with control over a running  TA or Trusted OS can try to mount software attacks against the secure monitor, the normal world, and other Trusted OSes. We also use TrustZone to prevent the normal world accessing secure world memory (i.e., secure monitor and Trusted OSes). Our threat model does not prevent a malicious agent from exploiting flaws in those software components. In ReZone we require the use of an auxiliary processor which we consider to be flawless, and thus trusted.
%We distinguish between two types of TCB. There is the system TCB, which includes the system components whose compromise allow an attacker to successfully attack all system components (e.g., compromised bootloader), and there's the functional TCB, which includes the system components whose compromise affect not the system security but the security of the applications relying on their correct operation (e.g., secure random number generator). In this work we focus on the system TCB, and the components are either trusted or untrusted in relation their role in participating in the system TCB. 
%
In summary:
\begin{itemize}
  \setlength\itemsep{0em}
    \item The normal world (i.e., all user space, kernel, and hypervisor code) is untrusted;
    \item The sEL1 and sEL0 (i.e., Trusted OS(es) and corresponding TAs) are untrusted;
    \item The EL3 (i.e., secure monitor) is trusted;
    \item The auxiliary processor and the software executing on it are trusted; and
    \item The platform's secure boot initializes the system in a known state
\end{itemize}

%By effectively sandboxing the Trusted OS, ReZone diminishes the system TCB to include only the secure monitor, and an auxiliary processor.
We do not consider physical attacks that tamper with hardware, e.g., fault injection. And, as in 
a typical TrustZone deployment, we do we do not consider Denial-of-Service (DoS) attacks including those caused by a malicious Trusted OS, for example, by not relinquishing control to the normal world or malicious manipulation of system interrupts.
Our solution has the side-effect of providing cache-sidechannel protection, however micro-architectural side-channels are not our focus and we do not make claims of protecting against them.

\subsection{Goals}
With ReZone, we aim at building a novel design / architecture / mechanism (\sandro{select the one that fits better}) that improves the security guarantees of TrustZone based systems, by effectively reducing the secure world privileges and thus minimizing the system's Trusted Computing Base (TCB). This mechanism should be deployable in real world hardware platforms and shall incur acceptable overheads for typical TrustZone-based TEEs workloads. The ReZone main goals can be sumarized as follows:

%\nuno{IMO the goals can be stated in a much more assertive way; we're digressing a bit and being somewhat imprecise, e.g., ``It is essential to prevent a compromised trusted OS from tampering with the secure-monitor and thus making it the sole system's TCB.'', this doesn't mean what we want: we want S-EL1 software to be blocked from reading and writing memory owned by EL3, unless explicit access privileges are granted to well-defined EL3 memory regions. Same comment for the others. The third goal says something like: ``it's possible to etc.'', this does not read like a goal but something hypothetical: do we want to provide this in ReZone?}

%\sandro{I agree 100\% with Nuno. Straight to the point and without possibilities/doubts...}

\mypara{Goal I: Reduce Secure-World Privileges.} 
\sandro{This paragraph is too big. This initial paragraph shall be straight to the point, explaining that the main goal is to reduce the secure world privileges and then let each objective in a bullet or number describe how we can acomplish that.}
We develop ReZone with the goal of building a mechanism which serves three objectives: secure-monitor isolation, normal world protection, and multiple isolated environments. These are achieved using a combination of hardware and software mechanisms and techniques to improve the overall security of the system. The high level system model achieved by following the proposed goals is depicted in \autoref{fig:rezone_vhl}.
Achieving these goals enables the sandboxing of multiple Trusted OSs in the secure world, preventing them from accessing arbitrary platform resources including the normal world, and secure monitor memory regions, and devices. We call this sandboxes secure world sandboxes. \david{isolated environemnt -> zone}. This high-level goal can be mapped into three main objectives:

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/ReZone_VHL.pdf}
    \caption{High level goals for the ReZone design.}
    \label{fig:rezone_vhl}
\end{figure}


\begin{enumerate}

  \item \textbf{Secure-Monitor Isolation.}\label{goal:secmon} The first objective is to provide a secure environment for monitor to execute. This way even in the presence of a malicious Trusted OS, the secure monitor can still be trusted as the system root of trust. Traditional hardware memory and peripheral protection mechanisms in TrustZone are limited in that they do not provide an effective privilege separation between EL3 and sEL1.
  %The first issue we tackle is secure-monitor isolation. We leverage the hardware features highlighted in section \ref{sec:hwmp}.In particular, the key-feature required to protect secure-monitor code is the ability to define a memory region as inaccessible to the CPU. We use this feature to prevent a Trusted OS from tampering with the secure-monitor. Traditional methods of hardware memory control in TrustZone (i.e. TrustZone controllers) are not sufficient. As we've explained earlier, TrustZone controllers are equally accessible to secure-monitor and Trusted OS. This makes configurations put in place to protect the system futile in a situation where the Trusted OS is compromised.
  
  \item \textbf{Normal world protection.}\label{goal:secnorm} The second objective is to provide normal world protection, in order to prevent malicious Trusted OSs from accessing arbitrary normal world memory. Currently, TrustZone offers an asymmetrical protection scheme where the secure world cannot be prevented from accessing normal world memory. This, in combination with other flaws, leads to attacks such as those we discussed in ($\S$\ref{sec:attacks}).
  %The TrustZone specification gives full access memory and peripheral access to the Trusted OS. However, in reality, the Trusted OS can perform all it's typical operations without requiring access to all platform resources, and in fact, the resources available to the Trusted OS have often times been used against the normal-world OS ~\cite{} \ref{} .%For this reason, we implement mechanisms that add a layer of protection to the normal world. This way the normal-world can be better protected from the Trusted OS, preventing attacks such as~\cite{}. %The mechanisms we employ is partially based on previous works~\cite{} with the added feature of an asynchronous minimal page-table introspection mechanism.
  
  \item \textbf{Multiple Isolated Environments.}\label{goal:multtee} The third objective is enabling the use of different environments for multiple Trusted OSs. Decomposing the current deployment of TEEs in more than one environment improves the overall security of the system, due to lower impact of TEE related flaws and vulnerabilities~\cite{Brasser2019,Li2019,Kwon19}.
  %With a mechanism that is able to mark memory as inaccessible from a high privilege-level can be leveraged to implement multiple lower privilege-level execution environments. %In ReZone this allows us to implement multiple TEEs which are not able to interfere with one-another.Similarly to other works ~\cite{Aravind2017}, we argue that decomposing current deployment of TEEs in more than one environment improves the overall security of the system. This is mainly due to preventing flaws affecting one TA from affecting another. %As a result, it's possible to either create different environments for each type of TA (e.g., System TAs) or create environments for each developer, so that developers do not need to rely on the correctness of other developers code. %This allows us to implement multiple TEEs which are not able to interfere with one-another. %However, short of new hardware implementing the Armv8.4(?) specification and up, there are still no solutions to providing hardware based multiple environments in TrustZone.
  
\end{enumerate}


\sandro{I do believe this paragraph shall not be here! I added the strikethrough} \st{Starting from ArmV8.4, TrustZone features a secure world hypervisor designed to provide different execution environments within the secure world itself, and which will also enable the protection of normal world, and monitor memory. However, platforms featuring the new architecture are not yet widespread, meaning that there is a lack hardware solutions for achieving the goals we propose. Additionally ReZone can be applied to already existing platforms which meet the necessary hardware requirements as discussed in} ($\S$\ref{sec:plat_req}).
\newline

\mypara{Goal II: Minimize the (secure world) TCB.}
\sandro{Text needs a strong refinement.}
TrustZone assited TEEs, suffer from large TCBs when considering the impact a single vulnerability can have of the system. To address this we set a goal of minimizing the TCB of TrustZone base systems, excluding Trusted OSes and TAs from it. This way, a security flaw in a Trusted OS or TAs will not enable an attacker to fully compromise other parts of the system, or even the full device.

\mypara{Goal III: Enhance Portability.}
\sandro{I'm not sure the description is good with regard to the goal. I'm not convinced.}
Another goal we aim for is portability. This goal is achieved by making use of real-world hardware and platforms as a testbed for ReZone. In particular we target platforms which enable the creating of security domains orthogonal to TrustZone.

\mypara{Goal IV: Acceptable Performance.}
\sandro{We shall elaborate a bit more. I'm not convinced.}
Our last goal is that performance should significantly affect common TrustZone base TEE workflows. In other words, we are willing to trade some performance penalty, as long as not deterimental to user experience, for some much improved security benifits.


%=======================================================================
%> [DESIGN]
%=======================================================================	
\section{Design}
\label{sec:overview}

\david{TODO: como surgem as sandboxes?}


%\textbf{NS: Introduce the section and provide a roadmap for it. This is very helpful because it gives structure to your through process.}

%\textbf{NS: Previously, the list below was stated as design goals, but I think in this context, since we are building a system that wants to leverage a few hardware primitives to provide additional protections, you can basically provide a high level description of what the system does, and what its components are with respect to the traditional TEE architecture presented in the previous sections. How different will it be? What new components are introduced into the picture? And finally briefly say that with our system, it will be possible to configure the system to operate with four or five new partitioning schemes which we will describe in detail in each of the next sections.}

Rezone's design focuses on providing the ability to create multiple security domains inside TrustZone's secure world. Essentially, it sandboxes secure world's EL1/EL0 execution modes, reducing its privilege, thus protecting both normal world and the secure monitor from rogue Trusted OSes or TAs, and also enabling the monitor to multiplex the secure-world by context-switching multiple TEEs. To achieve this, the design is centered on a custom world switch mechanism which leverages hardware security primitives orthogonal to TrustZone, including memory and peripheral protection controllers as well as a system management microcontroller.

\sandro{Still in this first paragraph I believe we should have a reference to a Figure supporting this high-level design description. Suggestion:}
\newline
{\color{red}Figure X depicts an abstract view / high-level perspective of \textsc{ReZone}'s design. Below, we explain the expected platform model, we overview the \textsc{ReZone} architecture, detail the key mechanism, and describe the full system operation.}


%Our system aims at deprivileging the trusted OS, effectively crating multiple security domains as oposed to the dual-world model of traditional TrustZone.Our system creates an effective privilege separation between the Trusted OS and the secure-monitor. This is a feature which enables the secure-monitor to be trusted as the system root-of-trust whether the trusted OS is compromised or not. In addition, with our system it's possible to remove the asymmetry in privileges between the trusted OS and the REE, by protecting all but explicitly allowed normal world memory regions to be accessed by the trusted OS. The mechanisms that enable this also enable the creation of multiple execution environments in sEL1, allowing for secure deployment of multiple TEEs.


\subsection{Platform Model}\label{sec:plat_req}

\nuno{As I mentioned in my previous comments, I think this text should be moved (and adapted) to Section 2.4.}

\jose{I think the section should be here. From my perspective, the platform requirements we define here are part of the design.}

ReZone's design makes a set of assumptions regarding the features offered by the underlying platform, which are the basic primitives needed to implement the key protection mechanism described throughout this section. These include:

\begin{enumerate}

    \item \textbf{Platform-level resource protection controller (RPC)}, i.e., a dynamically configurable memory and peripheral protection controller, orthogonal Trustzone's protection mechanisms (e.g., TZASC). The RPC shall be capable of (i) setting fine-grained access control attributes (e.g., RO, RW) for a each defined memory region; (ii) differentiating between multiple bus-masters; and (iii) protecting MMIO \sandro{(acronym needs to be defined)} interfaces, including their own; %to, but including,

    \item \textbf{Programmable system management core(s)}, i.e., independent processor(s) and bus master(s), distinct from the main and powerful application processors. Typically, these cores are know as housekeeping cores and implemented as small microcontrollers (e.g., Cortex-M4); \sandro{(Martins, I slightly extended this point, so please check if you are comfortable with changes)}

    \item \textbf{Secure boot process} that is able to guarantee a management core is in full control of the system's protection controllers, while their access is blocked to the main application cores.

\end{enumerate}

These requirements are modeled on the platforms described in ($\S$\ref{sec:hwmp}) and ($\S$\ref{sec:otherplat}). Although we did not carry out an extensive survey, we believe many other current and future platforms will meet these requirements, especially those targeting the high-end embedded markets such as automotive. \sandro{We need to be more confident in this message.}%Also, there is an increasing trend to include similar mechanisms in mobile SoCs. For example, Qualcomm's SPU (secure processing unit)~\cite{Qualcomm2019} provides many, if not all, of the aforedescribed features.

\sandro{I like this paragraph but I strongly believe it should be moved to the Implementation or Discussion section. At this point, a reader/reviewer without much knowledge cannot understand what is being discussed.}
\newline
{\color{red}We designed Rezone assuming that, w.r.t. application cores, the protection controllers act only on a per-cluster basis. Typically an RPC cannot differentiate between the multiple cluster cores as it observes requests as being from a single bus master, the shared cache. All accesses to the internal cluster caches will not be subject to RPC restrictions, only to TrustZone's. Despite being a limitation and not actually a model requirement, we make this assumption given that both platforms we model these design requirements on have this characteristic. If a similar platform fulfills all of the aforementioned requirements and, in addition, provides per-core isolation, this would allow for the system to be more flexible, scalable and performant.}

%\textbf{NS: the next paragraph was formerly named ``ReZone'' but I don't quite follow if this is common across all the protection modes that we can support, or if this is in itself a specific protection mode. Can you please clarify that? And also describe what benefits it can bring?}
% In TrustZone systems, secure-world has access to all system resources. One way we can protect resources is to have a separate processor mediate the configuration of memory region security attributes.
% Attributes are: secure-world read/write and normal world read/write. All of these privileges can be removed creating a grey-area, which we call ReZone.

\subsection{Architecure}

%\nuno{I think this section should be renamed ``Architecture'' and you should introduce all the components of the ReZone system, both software and hardware components.}

\sandro{In our document, we still cannot clearly communicate "what is ReZone". A design, and architecture, a mechanism ?! Furthermore, I do believe we have agreed we shall have specific names for the sandboxes - Zones if I'm not wrong?!}

ReZone can be understood as providing a set of security domains, each with a well defined set of memory and peripheral resources it can access, 
effectively increasing the number of security domains of a typical TrustZone system. A security domain is activated according to the execution context (\sandro{I honestly don't like this first sentence.}). As shown in Figure \ref{fig:rezone_overview}, in the main application processors, there are four execution contexts: (i) \textbf{\textit{the normal-world}}, (ii) the \textbf{\textit{secure-monitor}}, (iii) the \textbf{\textit{monitor trampoline}}, and (iv) \textbf{\textit{multiple secure-world sandboxes}} (\sandro{update the naming per the agreed term for sandboxes}).
An additional execution context, (v) the \textbf{\textit{ReZone controller}}, hosted on a dedicated processor (\sandro{I think we should call the names we have defined in the platform model, i.e., "programmable system management MCU"}) is itself encapsulated in its own security domain, which is isolated from the main processor cores at all times. On a world switch, it coordinates with the monitor trampoline to dynamically reconfigure the platform-level protection controllers to enable the secure world sandboxes. 

\sandro{I believe the use of "mypara" for the descritpion of each context keeps easier for the reader. I have restructured, accordingly.}
 
\mypara{Normal-world context.} The \textit{normal-world context} corresponds to the normal-world state of a typical TrustZone system. In this case, the security domain boundaries are enforced by the standard TrustZone mechanisms (e.g., TZASC). It comprises the untrusted OS and untrusted Apps (\sandro{rich OS and REE Apps, per Figure 1 - Btw naming in Figures are not kept coherent / uniform - compare Figure 1 and Figure 4}), and it can not access neither the secure monitor, trampoline, Rezone controller, nor the secure sandbox domains resources.
%The \textbf{\textit{secure-monitor context}} executes in a domain created by leveraging a hardware based memory-arbiter, in a way as to prevent the Trusted OS from accessing secure-monitor context. The secure monitor is the system's root-of-trust and can access any of the system resources.

\mypara{Secure monitor context.} The \textit{secure monitor context} executes in a security domain akin to the typical TrustZone's secure world (\sandro{I think a bit of detail with regard to EL3 vs sEL1 shall be given}). Therefore, it can access all platform resources except the ReZone controller's. This limitation is assured (\sandro{limitation?! assured or "ensured/guaranteed"}) by the RPC.


\mypara{Secure-world sandbox context.} Each \textit{secure-world sandbox context} (\sandro{Do not forget to update naming}), encompassing a Trusted OS and respective TAs, has its own dedicated security domain which excludes all other domains' resources with the exception of pre-established shared memory regions. As the traditional TrustZone resource protection primitives do not distinguish between secure-world privilege modes (i.e., between EL3 and secure EL1/EL0) and are asymmetrical in the sense that they are able to protect the secure world from the normal world, but not the other way around, sandbox domain boundaries are enforced by the RPC. 

\mypara{ReZone Controller context.} The \textit{ReZone Controller context} executes in an isolated microprocessor (\sandro{we should name microcontroller and use the acronym MCU}) and its security domain encompasses a small private memory region and the platform-level memory protection controller (\sandro{platform-level \textbf{resource} protection controller - per naming of section 4.1}). Its main role is to dynamically reconfigure the RPC to activate/deactivate secure-world sandbox domains (\sandro{Do not forget to update naming}). The need for this component is intrisically connected with the single domain with access to the RPC, because if application processors were given access to the RPC so that the monitor could directly reconfigure resource access policies to enable secure sandbox domains, there would be no way to guarantee that the Trusted OS would not also do the same to gain access to monitor or normal world resources (\sandro{Sentence is long and confusing. Split in simple messages, maybe 2 sentences}). Therefore it is only the ReZone controller that directly activates and deactivates secure sandbox domains by configuring the RDC to only allow accesses according to the predefined system policies. It does so in response to requests issued by the application cores via a secure channel which, at each request, authenticates the client as being  the secure monitor to avoid spoofing by a malicious trusted OS (see $\S$\ref{sec:key_mechanism}).


\mypara{}(\sandro{There is a change in the flow that contexts are being described. Per the initial paragraph, the \textbf{\textit{trampoline context}} is just executed in the application processors, and is enumerated as (iii). Here, it appears as the last, after describing the \textbf{\textit{ReZone controller context}}, which changes the order / flow. I believe we shall keep the samer order and coherency.})

\mypara{Trampoline context.} The component responsible for issuing this requests is the \textit{trampoline context} which has a special property in that it executes in two security domains at different points in time. First it runs with secure monitor domain privileges, but when a secure sandbox is activated, it runs on that sandbox's domain. This is pivotal as it is not possible atomically enable a secure sandbox domain and jump to sEL1. Therefore, there needs to be a part of monitor code still visible from sandboxes' domain, that issues the requests that enable the security domain before jumping to the trusted OS, as well as the inverse operation, when the trusted OS finishes execution. This software component must be tailored to be as minimal as possible and encompass mostly read-only memory to avoid corruption from a rogue Trusted OS. All writable data used by the trampoline must be non-critical. 
(\sandro{The description of the trampoline context is not clear and is a bit confusing, in particular the description related to the execution in two security domains. I'm sure a reader without much knowledge will not understand much. Furthermore, at this point, juts Figure 4 was referenced; however, it is not clear in Figure 4 were the trampoline context runs.})

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/ReZone.pdf}
    \caption{ReZone overview}
    \label{fig:rezone_overview}
\end{figure}
\david{nome do componente de software no monitor}
\david{caixa verde na sandbox}

\subsection{Key Mechanism}\label{sec:key_mechanism}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/ReZone-ExecModel.pdf}
    \caption{ReZone Execution Model}
    \label{fig:HZ-exec-model}
\end{figure*}

The key idea of our design is centered around the creation of multiple secure-world domains which sandbox TrustZone's sEL1 and sEL0 privilege levels and that can be reconfigured on-demand by EL3 software. To this end, our design implements (\sandro{the design "implements"?!?! confusing}) a custom world-switch mechanism by leveraging the hardware primitives detailed in ($\S$\ref{sec:plat_req}) and the fact that, although TrustZone does not provide physical address space isolation, there is actually strong EL3/sEL1 privilege separation at the register level, as the latter cannot access the former's system registers (\sandro{This sentence is confusing because is too long, and and some point the reader loses track which is in fact leveraged to provide such secure-world domains isolation. }). We take full control (\sandro{I don't like much the way is phrased with "we"}) of all protection mechanisms by, at boot time, configuring them to allow accesses coming only from the \textit{ReZone Controller} running in an isolated management processor (\sandro{programmable system managment core - per naming of section 4.1}). Also at boot time, we establish (\sandro{I don't like much the way is phrased with "we"}) a secure communication channel between the secure monitor and the \textit{ReZone Controller} based on a secret-key that is kept private to the monitor by storing it in an EL3 register (\sandro{Kind of scratchpad reg?!}). The \textit{ReZone Controller} authenticates the secure monitor, at each request, to modify RPC configuration. The monitor can then enable and disable protection via request to the \textit{ReZone Controller} upon Trusted OS entry and exit. 

(\sandro{In my opinion, and aligned to what I have said before, we shouldn't be focused in this per-cluster limitation in the design. We should describe in a generic way, and let the problem arise in the implementation and discuss how we see benefits in having per-CPU control in the Discussion Section. I think it's possible to describe this part in a generic way. It's just my view, that we should discuss in the next meeting.}) As described in ($\S$\ref{sec:plat_req}), RPC protection acts only at a per-cluster basis and is is not enforced on accesses to the cluster internal caches. For this reasons two actions must be taken when a secure-sandbox context is activated in one of the cores. First, all cache contents must be flushed so that the trusted OS cannot access or modify other domain's in-cache data. Beyond the cache, protection is enforced by RPC. Secondly, all other cores within the cluster must be halted to prevent other cores executing in the normal world from fetching their data to cache. Although these are extreme actions that, at first sight, might suggest inadmissible high performance (\sandro{prohibitive performance overhead}) and UX impacts, our experiment shows it not so critical due to the sporadic invocation patterns and reduced execution times of secure world services (see $\S$\ref{sec:eval}), essentially trading-off huge security benefits by moderate performance hits. \jose{Nuno and David, this last point on trade-offs needs to be polished. Any ideas? Maybe mention that we can still run other cluster in parallel which is very common in today's big little architectures?}

The key world-switch mechanism is depicted in \autoref{fig:HZ-exec-model}. After the normal-world issues a request (1), the execution is handed to the monitor context (\sandro{\textit{secure monitor context } per naming in subsection 4.1}). If the request requires a Trusted OS running in a secure-world sandbox to handle it (\sandro{suggestion: needs to be handled by the Trusted OS}), ReZone will activate the target sandbox's security domain and hand it execution \nuno{what you mean by ``activate its domain''?} \jose{I've added a definition of secure-sandbox activation in section 4.2}. For this, the secure monitor starts by notifying all other cores in that cluster via IPIs (\sandro{The part of the IPIs is not an implementation detail?!}). The other cores will then flush their caches and enter an idle state. After all other cluster cores are idling, the trampoline (2) issues a request to the \textit{ReZone Controller} (\sandro{Please note the image has no reference to "Rezone Controller"}) to activate the target secure-sandbox domain (\sandro{Do not forget to update naming}). To authenticate the request as coming from a monitor mode context (\sandro(\textit{secure monitor context} per naming in subsection 4.1?!)), the \textit{ReZone Controller} expects to receive a secret token issued by the ReZone Controller during boot and protected during secure-sanbox execution by storing it in an EL3 register (\sandro{\textit{ReZone Controller} twice and another reference to the token in the EL3 register - i think is not needed}). After a successful reply from the \textit{ReZone Controller} (3), the trampoline (\sandro{Shall we introduce as \textit{Trampoline} ?!}) will first flush its own cache content (\sandro{suggestion: microarchitectural state!?}) and then (4) jump to the Trusted OS. After the Trusted OS returns execution to the \textit{secure monitor} (5), the trampoline (\sandro{Shall we introduce as \textit{Trampoline} ?!}) issues a new request (6) so that the domain controller (\sandro{domain controller now!? I'm confused}) deactivates the secure-sandbox domain (\sandro{Do not forget to update naming}) and reestablished the secure-monitor domain. The monitor will then resume normal-world execution (7), notify other cluster cores to, finally, return to the normal world context (8) executing under traditional TrustZone restrictions. 
\nuno{This paragraph is describing how we do things, but I feel it's important to explain why we do them in this way. In particular, I feel that we need to explain the permission privileges that result from combining the security mechanisms from RDC and TZC, and talk about the technical restrictions involved in setting them up that justify our solution and the steps above (e.g., the need to have a trampoline, etc.).}
\jose{Nuno, please check the 4.2 architecture section. I've added the justification for the need of the trampoline code there. Also that section also clearly describes what protection is enforced by the TZC vs the RDC.}

This key mechanism by itself ensures Goal I's objective I and II by enabling the protection of monitor and normal-world memory while a trusted OS executes inside a secure-world sandbox. Using the mechanism as a bedrock, the secure monitor is able to easily restore the context and activate the security domain of multiple TEEs depending on the request of the secure achieving objective III. As each TEE is sandboxed, it will also not be capable to access other TEEs' resources.

% Our platform model assumes that protections have cluster granularity. Because of the need block monitor memory after while one of the cores is executing a trusted OS, another core cannot execute in the monitor context while the trusted is executing. The trampoline our design essentially serializes secure world requests.

\nuno{Another big question I have is: if we're going to implement IEE, which enforces full isolation from the normal world, how are they going to be able to share memory with each other? What's ReZone's mechanism to enable that?}

\jose{ Sections  4.4. to 4.6 and partially 4.7 are already described in section 4.3. But I agree we can maybe highlight or detail some of these main points a bit more.}

\subsection{Full System Operation}

(\sandro{I would recomend to split this text among several "mypara", each one for a part of the lifecycle. When this is done, I can give you a strong opinion on how to improve this subsection. I believe still something is missing...})

\jose{Each OS SMCID range is offseted}
To setup the system, all secure sandboxes and their respective access privileges to memory and peripherals must be statically defined at design-time in a manifest file. For each defined sandbox (\sandro{Do not forget to update naming}), the provided services (\sandro{Which services?! It's not clear to me}) must be listed, and each service shall be associated with an unique SMC (Secure-Monitor Call) ID. This information is directly compiled into the monitor image. At system initialization, the monitor creates sandboxes (\sandro{Do not forget to update naming}) by relaying this information to the \textit{ReZone Controller} which saves this information in its private memory and acknowledges the success of the operation by returning a sandbox (\sandro{Do not forget to update naming}) ID to the monitor. The monitor then creates a map of SMC to sandbox IDs (\sandro{Do not forget to update naming}). It would be possible to directly fetch these configurations in the domain controller (\sandro{This term was never introduced before, and it's not linked to any context described in 4.2}) itself. However, this interface will seamlessly allow the dynamic instantiation of sandboxes (\sandro{Do not forget to update naming}) in future iterations of our design.

At runtime, when the normal-world OS issues a request to the secure world passing it a given SMC ID, the monitor will translate the SMC ID into a sandbox (\sandro{Do not forget to update naming}) ID, and pass this ID to the \textit{ReZone Controller} to activate the target sandbox (\sandro{Do not forget to update naming}). The controller (\sandro{which one?! the \textit{ReZone Controller}?!}) will then use this ID to get the RPC configurations for the target sandbox (\sandro{Do not forget to update naming}). This makes the segregation of the Trusted OS into multiple isolated sandboxes (\sandro{Do not forget to update naming}) transparent to the normal-world client, and therefore there's no need for modifications of normal-world drivers.


\nuno{After we explain how ReZone is able to protect the monitor and the normal world, then it's time to give a complete explanation of the entire system operation: i) installation, ii) bootstapping, iii) runtime. I think most of the text from ``Key Mechanism'' could come here.}

\jose{Don't really understand what is meant by "instalation". Boostraping and runtime are somewhat described in section 4.3. Now that David  has multiple TEEs executing, we could maybe also explain how we envision the changes in the different software layers and programming model needed for this functionality.}

\jose{Maybe we should also address the problems arising with shared memory management.}



\if0
\subsection{Normal-World Trusted Service Request}
On a request for a trusted service, made through a Secure Monitor Call (SMC) instruction, if there's no trusted service request pending, the secure-monitor handles the request by looking at the SMC function identifier (smc\_fid). If the smc\_fid corresponds to a service provided by the secure-monitor (e.g., PSCI calls), the secure-monitor serves the request and resumes normal-world operation. This is no different to how these services are service typically. If, on another hand, the smc\_fid identifies a request for the Trusted OS, the monitor must protect itself. \nuno{because?... it's not clear at this point how is the secure world memory configured so as to justify the need for the monitor to protect itself when a request is made to the trusted os.} This is done by interacting with the micro-controller. The secure-monitor enters the trampoline and issues a SEC\_MON\_PROTECT command to the micro-controller. If the micro-controller identifies the secure-monitor successfully, the micro-controller will enforce the secure policy established during boot \nuno{somewhere before this point we need to clearly state what this security policy is.}. The secure-monitor will wait for a response from the micro-controller before executing the Trusted OS. The Trusted OS will then schedule a TA to service the normal-world request. Upon completion, the Trusted OS will return execution to the secure-monitor by issuing a SMC instruction. The SMC is handled in the previously established trampoline. The secure monitor will then interact with the micro-controller once again to re-allow access to the secure-monitor program memory, wait for the micro-controller response and resume normal execution, including returning to the normal-world. Figure \ref{fig:monitor_prot_seq} illustrates this process. \nuno{please update this reference; maybe refer to the figure earlier in this paragraph to help the reader understand the execution flow.}
\fi



\if0
\subsection{Secure-Monitor Isolation}\label{sec:secure_monitor_isolation}
The micro-controller acts as a mediator for the memory access controller configuration, and only acts on requests from the secure monitor, this enables us to make secure-monitor code inaccessible to a running Trusted OS \nuno{I think it might flow better if you first explain the problem, then the solution. Question: what prevents the trusted OS from tampering with the memory reserved to the micro-controller?}. 
Two things we must consider are the context switch from Trusted OS to secure-monitor, and a context-switch issued by the normal-world. \nuno{What about the steady state when the core is running with sEL1 privileges, i.e. Trusted OS code? what prevents it from accessing the monitor's reserved memory?}
We implement a small region of code written in assembly, that performs the necessary operations to handle both of these cases, which we call trampoline. 
The trampoline authenticates itself with the micro-controller, by sending a secret token with a request for an operation. \nuno{why does the trampoline need to authenticate itself?}
This token is made secret by storing it in system registers only available to secure-monitor level privilege (i.e. EL3) while the Trusted OS is execugin. We next explain the various phases of secure-monitor isolation operation.
\fi



\if0
\subsection{Normal-world Protection}\label{sec:normal}
Protecting the normal-world from a Trusted OS protects the executing REE from malicious TEEs from compromising the normal-world OS operations. This is particularly useful when attacks to TEEs can be made from the normal-world's user space applications, as opposed to attacks requiring an already compromised operating systems. TrustZone specification allows a Trusted OS to access any memory available to a given CPU, which enables some useful security features such as TZRKP [], but also the potential to compromise the normal-world OS. More insidiously, to effectively restrict secure-world access to a memory region is also to restrict it for the normal-world. Preventing the secure-world from accessing certain memory-regions while allowing normal-world to access them requires a per-core memory access control, which has been proposed in \cite{Brasser2019} by leveraging non-standard features of a \textbf{barely used} TrustZone controller: the TZASC-400, and which even their test platform did not feature. Another solution is the introduction of virtualization in the secure-world as proposed in ARMv8.4-A specification. But hardware featuring the functionality may be still be a few years away from mass commercialization, as it tends to with new Arm architecture specifications \cite{}. We propose a solution leveraging the RDC present in the iMX8MQ.

In TrustZone there are two mechanisms controlling memory accesses, virtual memory and TrustZone controllers. In addition to virtual memory mappings, virtual memory may be used to implement memory access security policies: read, write, executable. The policies are put in place by configuring the permission bits in each page table entry or page table directory. A Trusted OS may change this permissions or create new memory mappings during its execution, a feature which may be abused by attackers to compromise the system [bits please write zero primitive allows disabling domain enforcement (armv7)]. It's also possible for a Trusted OS to set the TTBR register, a pointer to active page table. Further, an attacker could also hypothetically disable virtual memory altogether to access system memory without restrictions \cite{}. 
\david{Should this paragraph go to background?}

The mechanisms provided by TrustZone hardware are not sufficient to create meaningful isolation between the secure monitor and the Trusted OS. Because of this, we required orthogonal access control systems. In our implementation we configure the RDC to mark normal world memory as inaccessible while the Trusted OS is executing. This approach prevents all unintended accesses to the normal world memory (e.g., only allow shared-memory to be accessed), however it comes at the cost of having to perform cache maintenance on every context switch to the Trusted OS, and having to suspend all the cores on the cluster. By relying on hardware mechanisms on not on software approaches such as same privilege isolation techniques, we are able to relax the threat model to include completely compromised (i.e., untrusted) Trusted OSes.

\nuno{I think some parts of this paragraph are too verbose, and a part of our solution has already been mentioned in Section 5.3 when we talked about context switching.}
\fi

\newcounter{problem}
\newenvironment{problem}[1]{\refstepcounter{problem}\par\medskip
   \textbf{Problem~\theproblem. #1: } \rmfamily}{\medskip}
   
%=======================================================================
%> [IMPLEMENTATION]
%=======================================================================	
\section{Implementation}
\label{sec:impl}

%\david{sections orientadas ao challenge, interface}


%\nuno{I think it might flow better to have the organization in terms of ``monitor / nw / SW domains'' moved into the design section because it's mostly directly related with the goals we want to achieve. Then here we can restructure the implementation section around the implementation challenges and the respective solutions -- possibly, some of the titled (bold) paragraphs currently in this section.}

To implement ReZone we take advantage of a programmable micro-controller present in both our test platforms, iMX8MQ and iMX8QM, and in the flexibility both this platforms provide in assigning memory resources to different processing elements while excluding others.
\david{Mention that we modify TF-A.}
%make sure a reader could reconstruct the implementation
%don't forget loc

% \begin{itemize}
%     \item TZASC na tabela
%     \item imagem a ocupar duas colunas
%     \item layout de memória com endereços fisicos
% \end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-overall.pdf}
    \caption{Hardware achitecture and components of a ReZone enabled system}
    \label{fig:my_label}
\end{figure}


\begin{problem}{Lack of access control in the cache}
Having access control only being performed on accesses to main memory is a challenge, as it forces us to perform cache maintenance operations to ensure that the access control policy acts as intended.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-Problem1-Cache.pdf}
    \caption{RDC only performs access control to main memory.}
    \label{fig:p1}
\end{figure}
\david{desenhar multicluster}

\end{problem}

\begin{problem}{MMU TLB-Miss on Handling Exceptions in EL3}
Upon entry unto the vector table, it may be the case that there's no TLB Entry that maps the region of code. In this case the MMU will fetch the PTE that maps it, which results on an access to the memory subsystem to perform a page table walk. Because we've flushed page tables from the caches, a main memory access must be performed. However, if the exception is taken from sEL1 (e.g., TrustedOS performed an SMC), the memory will be protected. This will result in the system hanging, as the exception cannot be dealt with.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-Problem2-PageTable.pdf}
    \caption{A TLB miss may occur while page table memory is protected}
    \label{fig:p2}
\end{figure}
\end{problem}

\begin{problem}{Code Injection Into EL3 from sEL1}
The code on the vector table must be readable from main memory, and thus marked as readable by the processor on the RDC. 
However, this will also give the TrustedOS the ability to read the code.
Due to the memory hierarchy, the vector table code will now also reside in cache, and write operations are now allowed (as long as it they do not reach main memory). A TrustedOS can maliciously modify the exception handling code (e.g., modify SMC handling code), to its own advantage. Upon an SMC, the Monitor will then execute malicious code which is obtained from \emph{hitting} the cache, and not from obtaining from main memory.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-Problem3-CodeInjection.pdf}
    \caption{A malicious TrustedOS can inject code into the the secure monitor, even if RDC is marks the code memory region as read-only.}
    \label{fig:p3}
\end{figure}
\end{problem}


\subsection{Hardware Memory Protection}\label{sec:hwmp}


%\subsection{\color{red} System Hardware Protection Controllers}\label{sec:hwmp}

%\textbf{NS: Once you've set the stage to the problem we want to tackle -- i.e., the coarse level of isolation featuring the current TEE hw/sw architectures -- then it's time to talk about the new hardware features available in emerging boards and talk about the potential they have to increase that granularity and as a result increase the security of TEEs. I confess that the current text is somewhat confusing. I'd prefer to have some structure where you start off by saying that our goal is to design a new architecture that increases the granularity of privilege separation using these new cool hardware features, then have one paragraph to talk about each feature; then maybe a table or something else were to present the specific features of each board. The cool feature could be something like: a) protection units for fine-grained memory partitioning, b) per-cluster policy enforcement, etc. For each, describe what it is, and explain how it could be leveraged to increase the state of affairs presented in the section above.}
%TZASC / TZASC-like and TZPC / TZPC-like hardware. Hardware which enforces security-state policies. Such which memory is marked as secure. TrustZone is a specification, TZASC and TZPC are not. They are a proprietary solution whose use Arm charges money for. Vendors often develop their own hardware security-enforcement IP, which has different, and often less, features than those of Arm


% Because TrustZone design is the enabler for the severity of vulnerabilities found in TrustZone, TrustZone enforcing hardware is not enough to address this problems. Lately, several platforms have came up with hardware mechanisms to create domains within the SoC. These domains are independent of TrustZone and aim to control access to subsets of system resources for the various masters of the platform (e.g., Application Processor, micro-controller, GPU, etc).
% Chip designers provide hardware based mechanisms to validate memory accesses. They are generally called protection units. Here we provide some examples:
% \begin{itemize}
    % \item Xilinx - Xilinx Memory Protection Units (XMPU) and Xilinx Peripheral Protection Unit (XPPU)
    % \item NXP - Resource Domain Controller (RDC), Extended Resource Domain Controller (xRDC) and xRDC2
    % \item Qualcomm - xPU "This means the XPU registers are only one mean to secure peripherals and/or memory, all of which can be protected by other technology like TrustZone isolation." %https://blog.quarkslab.com/analysis-of-qualcomm-secure-boot-chains.html
    % \item Qualcomm - SPU memory controller "The TSF shall be implemented to restrict the ability to [modify and define] the memory areas shared with other components of the SoC to SP-ExtMM controlled by the SP-CPU." %https://www.commoncriteriaportal.org/files/epfiles/1045b_pdf.pdf
    % \item ? Apple - Hardware “filter” to prevent AP to SEP memory access -Only SEP’s KF core has this filter %https://www.blackhat.com/docs/us-16/materials/us-16-Mandt-Demystifying-The-Secure-Enclave-Processor.pdf https://www.theiphonewiki.com/wiki/Secure_Enclave_Processor
% \end{itemize}


%There is an ongoing trend in the SoC industry to embedded an increasing number of processing units and bus masters in the same chip and to provide additional mechanisms to isolate them. In response, we start seeing an increasing number of platforms which implement, at the system level, additional hardware access control mechanisms orthogonal to TrustZone. In the following, we describe a few examples implemented in the NXP iMX8 and the Xilinx Zynq UltraScale+ families. 

There is an ongoing trend in the SoC industry to embedded an increasing number of processing units and bus masters into the same chip. In response, we start seeing an increasing number of platforms that implement, at the system level, additional hardware access control mechanisms orthogonal to TrustZone.% In the following, we describe a few examples implemented in the NXP i.MX8 and Xilinx Zynq UltraScale+ families. 

NXP has developed an hardware controller which aims to create multiple security domains within the SoC by allowing chip resources to be separated into partitions or domains. The i.MX 8M family features the \textit{Resource Domain Controller (RDC)} while the i.MX 8QuadMax family features the \textit{Extended Resource Domain Controller (XRDC)}. Both controllers have similar high-level features, but the XRDC module is a new iteration which incorporates TrustZone controller features, not requiring two separate onboard controllers. The RDC is hardware embedded in the SoC that enables the creation of multiple platform domains. A domain is a collection of resources and respective access permissions. Access permission specify the access privileges each master in the platform has over a specific resource. This enables fine grained control of access permissions in platforms that feature multiple processing elements. For example the iMX8M features a GPU, Arm application processor (4 cores), one microcontroller (cortex-M4), etc. Each master can be attributed with exclusive rights to a given resource, expanding on the TrustZone dual-world model of system security to multi-domain platform control. 
%Note that in both families, Cortex-A CPU clusters are assigned with a unique master ID, which means policies cannot be enforced per core. 

%  On final aspect of these platforms is that each cluster is a master. This means that memory regions cannot be assigned to a single core, but may be assigned per cluster, allowing for memory access policies to be granular at the cluster level.


\subsection{Hardware Controller Related Challenges}
We leverage the Resource Domain Controller (RDC) to enable more secure TrustZone-base TEEs as explained further in this section. However both the iMX8QM and iMX8MQ platforms limit the execution of our design in significant ways.
%\textbf{David: Don't really know where to put this: the RDC also allows us to prevent DMA attacks against the greyzoned secure-monitor (but not the normal-world)}

\mypara{No private CPU core memory} 
The first limitation is that memory accesses cannot be controlled per core. This is because accesses to main memory are performed by the L2 cache, and because L2 caches are shared by the entire cluster. Having per core access control implies being able to control accesses to L2 cache. With the ability to specify memory control access per core it would be simpler to implement ReZone, there would be no need to perform synchronization between cores, and cache flushes would be limited to L1 caches instead of all L1 e and L2 caches, diminishing overheads.
%The first limitation is that secure-world memory access cannot be controlled per core. Having control per core, would enable easily deploying multiple TEEs where a TEE running in one core could not access the memory of a TEE running in a second core, when paired with our first mechanism \ref{sec:impl}. \nuno{Please be concrete about what's the first mechanism. Also, does this only limit the ability to have multiple TEEs/IEEs? How does it affect the other security properties we're interested in?} However, we use the available control per cluster in the iMX8QM (the iMX8MQ features a single cluster), to similar effect.

\mypara{Secure-world may always access normal-world memory} None of the features in the platform enable the secure-world to be truly restricted in accessing the normal-world memory. This is mainly due to the ability of the secure-world to map memory in a way that the CPU core performs non-secure accesses when running in the secure world.

\mypara{TrusteOS can access secure-world resources} Another limitation is that there is no enforceable memory separation between the secure-monitor and the Trusted OS although they execute in different privilege levels, secure-monitor executes at EL3 and Trusted OS executes at secure-EL1. 
%Additionally any configuration made by the secure monitor to hardware controllers (e.g., TZC-380) can be unmade by the Trusted OS. 
%not entirely true, see tzc380 lock bit
The kernel of the problem is that TrustZone access control only considers the security state of the processor, and not its privileged level. This lowers overall system security. 
Additionally, because we aim to have multiple Trusted OSes in the secure world, with TrustZone only features, a Trusted OS can also access other Trusted OSes' resources.
%\nuno{This last part reads a little bit vague. Are we only concerned that a compromised Trusted OS can access the monitor's memory? Or that it may also undermine isolation between IEEs' memory? Or that it also affects the peripherals?}


\subsection{Boot}\label{sec:boot}
When booting, the system must ensure that the micro-controller has exclusive access to its program memory by creating a dedicated domain for it, including dedicated memory regions and the required peripherals, such as the hardware-based interface used to communicate with the application processor. To do this in our test platform, which first boots the application processor, the monitor starts the micro-controller before initializing the Trusted OSes. After starting, the microcontroller sets up it's own domain. From then on the micro-controller can establish access control policies over memory and peripherals available to the application processor. 
%\nuno{what's exactly this ``system configuration''? how do we set this up securely? do we need to ensure that the microcontroller boots up first and before the other cores? if so, how do we guarantee that?} 
%
To initialize the Trusted OSes, the boot process already preloaded unto memory the respective images.
On the first Trusted OS execution, the secure monitor is already protected by following the steps 2 through 7 described in ($\S$\ref{sec:key_mechanism}).
%by issuing the SEC\_MON\_PROTECT command to the micro-controller, and establishing the trampoline before handling execution to the Trusted OS. \nuno{sorry, don't quite understand this step: ``can already'' or ``is already''? don't we need to hard-guarantee this?} 
%The trampoline is small region of code, that is marked as non-writable by TrustZone independent mechanisms present in the platform (i.e. the RDC). \nuno{the trampoline is part of the monitor, right? doesn't it also need to be protected against reading? otherwise can't the trusted os read the auth token from memory?}

\david{todo: peripheral protection}

\david{Limited regions configuration}

\subsection{Secure-Monitor Authentication}\label{sec:mon_auth}
Effectively, ReZone makes the secure monitor in charge of setting up memory access control policies, however it does not have direct access to the RDC. The component which has access to the RDC is the micro-controller, and because the means used to communicate with the micro-controller are available to both the secure-monitor and Trusted OS, it is necessary for the secure-monitor to authenticate itself when issuing commands to the micro-controller. If no authentication is performed, a Trusted OS could use the hardware-based interface between the application processor and micro-controller to issue commands to undo the established memory access policies.
%\nuno{This is very interesting but needs a more thorough explanation. If I understand correctly, we need to explain that the monitor is still in charge of setting up all the memory protection domains in the system. However, to enforce these memory protection policies, it needs to send specific instructions to the microntroller. But since the microcontroller could also receive spoofed instructions from a potentially compromized trusted OS, then we need to ensure that the monitor authenticates itself toward the microcontroller. Is my understanding correct?}
%
The authentication is simple, but effective. ReZone requires a secret token. The token is 64 bit wide, and is stored in a CPU register inaccessible to a Trusted OS. 
The content of this register is inaccessible to a Trusted OS due to the EL3 level of privilege having exclusive access to it. This results in any attempt to access these registers from EL1 leading to an exception handled by the monitor.
A compromised Trusted OS has a 1 in $2^{64}$ chances of guessing the secret token. Any token mismatch signals the presence of a compromised Trusted OS to the micro-controller, and steps may be taken accordingly.
%\nuno{what's the communication channel between the monitor and the microcontroller? what prevents the trusted os from accessing the token? how is the token (which is a secret) securely loaded into both the monitor and the microcontroller?}
%
To establish its identity, the first command the secure-monitor issues to the micro-controller is a request for the generation of the secret token used in authentication requests. Implicitly the micro-controller will trust the first request after booting is from the secure monitor. This holds true because the token exchange is done before a Trusted OS begins execution, giving a Trusted OS no opportunity to interfere with this step.
%\nuno{why can we trust that this request comes from the secure monitor and not from the trusted os? is it because you assume that the system will first boot into EL3 code? in other words, you always assume that the first request is trusted by the microcontroller?}
%
In the first command, the micro-controller generates and stores the token in its dedicated memory, and issues the token to the secure monitor. 
%\nuno{how can we ensure that it's not intercepted, e.g., by another core running already in sEL1?}
%
To create the token, a sufficiently high-entropy source must be used, as is standard practice. It is common for platforms to be equipped with hardware designed for such cases. Such is the case with our test platform.

\subsection{Secure Context Switch}\label{sec:securectxswitch}

%\nuno{wasn't a part of this already explained in the section above?} 
Secure context switching is done by interacting with the micro-controller while on a particular memory region, suspending cluster cores and performing micro-architectural maintenance.


\mypara{Micro-Architectural Maintenance}\label{sec:cachemaintenance}
Upon checking that an SMC is for the Trusted OS, the monitor will suspend the other cores in the same cluster. 
We must suspend the cores, because it's not possible to allow the normal world to access normal world resources, and preventing the Trusted OS from accessing them at the same time. After suspending all cores in the cluster, we mark normal world memory and peripherals, as inaccessible. This prevents a Trusted OS from accessing them.
As part of the suspend routine, each core will evict all of its data from the caches (see $\S$\ref{sec:cachemaintenance}). We must flush all caches. There are two reasons for this. The first is that a malicious OS could manipulate data and instructions in the cache by mapping the physical memory as accessible, which could enable the Trusted OS to perform control flow hijacking. The third is that flushing all data from L2 caches requires also flushing L1 caches, due to autolocking \cite{green2017autolock} caused by cache allocation policies.
Performing these operations is only required at a cluster level, due to the RDC, the PRC in our test platform, being able to distinguish between memory accesses of each cluster.
%This step is skipped when using ReZone to only protect the secure monitor.
In addition to performing cache flushes, when switching between Trusted OSes, TLB maintenance (i.e., TLB invalidation) for the current core is required for switching between Trusted OSes. Not due to security concerns, since both Trusted OSes are in a sandbox and can only access memory directly assigned to them, but because otherwise a Trusted OS could be addressing parts of the the other Trusted OS address space, causing unexpected faults. As an optimization, we only perform TLB maintenance if the last invoked Trusted OS is different from the one we are currently going to execute. In practice this prevents TLB maintenance operations when the system is making use of a single Trusted OS, as invalidating the TLB is only necessary when switching between Trusted OSes.

TrustZone extends memory accesses with one bit. This bit informs whether the access is mode from a secure context or a normal context. This information extends to the cache, and with each cache line a bit is stored to keeps track of whether the line was fetched has secure or normal. This allows for efficiently separating normal world accesses from secure world accesses, but not without flaws~\cite{armageddon, truspy}. We make standard use of this feature, using it to prevent the normal world from accessing secure memory.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-ContextSwitch.pdf}
    \caption{Context-Switch to and from a TrustedOS requires micro-architectural maintenance operations including cache and TLB maintenance.}
    \label{fig:scr_ctx_hw}
\end{figure*}

\david{peripheral reconfiguration}

\nuno{maybe this is the place where we could discuss other alternative approaches that we explored before converging on the cash flush strategy.}

\mypara{ReZone Trampoline} 
% \nuno{the text is good, but it's too descriptive: it doesn't explain why we do things the way we do.
% For instance, these are some of the questions I had after reading this first paragraph. 
% Why do we need to suspend the cores? 
% Why is this only be done at the cluster level? 
% Why are we evicting the caches? 
% Why is cache evicting skipped when protecting the secure monitor?
% }
%
Before reconfiguring memory access control policies, the secure monitor enters the ReZone Trampoline region.
This region is marked as readonly while a Trusted OS is executing, to enable code execution by the monitor. This is required to prevent the memory reconfiguration from causing causing execution errors. 
We mark it as readonly because the application processor still needs to be able to read this region instructions to be able to execute them. By marking it readonly we guarantee that even the presence of a malicious Trusted OS, the region is unmodified, and thus the code cannot be bypassed.
If the ReZone Trampoline would be marked as non-accessbile, it could lead to a crash after reconfiguring memory access control policies, due to the secure monitor trying to fetch instruction which could be not retrieved from memory. In the same vein, a readonly ReZone Trampoline also enables secure exception handling, because it allows immutable code to handle exceptions.
It is in the ReZone Trampoline that the ReZone Sandbox is activated. 
%\nuno{I'm confused: isn't the trampoline part of ReZone? what you mean by disabling ReZone?}
A Trusted OS could try to run code from the ReZone Trampoline to deactivate the ReZone Sandbox, however this code relies on access to EL3 only registers, as described in ($\S$\ref{sec:mon_auth}), thus any such attempts to bypass ReZone will be unsuccessful.

In the ReZone Trampoline the ReZone Sandbox is activated by issuing a SEC\_MON\_PROTECT command to the micro-controller. If the micro-controller identifies the secure-monitor successfully, the micro-controller will enforce the configured access control policy. The secure-monitor will wait for a response from the micro-controller, after which it performs core micro-architectural maintenance (see $\S$\ref{sec:cachemaintenance}). After this, execution control can safely be transferred to the Trusted OS.

The trusted OS will execute, and will likely schedule a TA to service the normal-world request. Upon completion, the Trusted OS will return execution to the secure-monitor by issuing a SMC instruction. The SMC is handled in the previously established ReZone Trampoline. The secure monitor will then interact with the micro-controller once again to re-allow access to the secure monitor program memory, and wait for the micro-controller response and resume execution on all cluster cores, including returning to the normal-world. 
%\nuno{Part of this has been explained in the section above.}

\david{readonly RDC problem}


\mypara{Multi Cluster Scenario}\label{sec:mult}
%Our test platforms provide the necessary mechanisms for deploying a system with multiple TEEs. \nuno{TEE software, each one inside an IEE, right?} To implement multiple TEEs in the platform featuring a single cluster, the iMX8MQ, it's necessary to make only the current TEE's program memory available to EL-1. This is achieved in a similar way that secure-monitor program memory is protected; the RDC is used to prevent access to the required memory regions (i.e. other TEEs). When handling trusted service requests the secure-monitor will enable, by interacting with the micro-controller, only the required TEE to execute the service. Figure \ref{fig:multi-tee-same-cluster} illustrates the process. 
%
To implement multiple TEEs in the platform featuring more than one cluster, in addition to the techniques mentioned above, we can also leverage the fact that memory access policies can be defined per cluster. This enables simultaneously running one TEE per cluster while benefiting from mutual isolation. 
%Figure \ref{fig:multi-tee-multi-cluster} illustrates memory configuration for achieving this. 
There are many ways to employ this idea, one might be to have as many TEEs as clusters, and statically assign a TEE per cluster. This allows for a straightforward implementation of protection mechanisms, while allowing multiple TEEs to serve trusted service requests parallel to each other. More complex implementations might optimize TEE distribution base on available clusters, to run any TEE on any cluster while clusters are available to execute as many trusted services concurrently as possible.


\subsection{Concurrent Normal-World Trusted Service Requests}\label{sec:concurrent_nw}
Because we suspend all cluster cores, we do not support concurrent requests in the single cluster of the iMX8MQ platform.
%\nuno{why having a single cluster prevents the execution of concurrent requests? is it something that we prevent for safety reasons? or is it something that is intrinsically disallowed by the platform's hardware?} 
Calls to the Trusted OS are, therefore, inherently serialized.
%\textbf{David: We have two options, either stall the request, until the executing is concluded, or return a busy state. The latter is probably more compatible but less user-friendly, the former may require Linux driver modifications}.
On the iMX8QM, which features two CPU clusters, it's possible to serve up to two simultaneous trusted service requests if they are executed on different clusters, otherwise they'll have to be serialized. 
%\nuno{again, similar questions.}
Issuing the service request to the correct cluster, may require Linux driver modifications.


\subsection{Synchronization}\label{sec:synch}
Because the cpu loses access to the secure monitor program memory when the Trusted OS is executing \nuno{loses access because it's something enforced by ReZone?}, we must take care to prevent situations where the monitor would execute while the Trusted OS is active \nuno{why? I don't get this. make it explicit what can go wrong}. These are the instances where such scenarios might occur (for the sake of simplicity we only consider two cores):
\begin{enumerate}
  \setlength\itemsep{0em}
    \item\label{sync1} Two cores are executing monitor code and one of them starts executing the Trusted OS \nuno{so? what needs to happen?}
    \item\label{sync2} Two cores are executing monitor code and it is required of the Trusted OS to execute some code, so the core must wait for Trusted OS to resume execution before continuing execution
    \item\label{sync3} One core is executing the Trusted OS while another is sleeping, meanwhile the sleeping core awakens (e.g. due to an interrupt) \nuno{awakens to execute monitor code?}
\if0
    \item\label{sync4} One core is executing the Trusted OS and the other core executes an SMC while in the normal-world
    \david{Suspendendo os cores, deixamos de ter o caso 4}
\fi
\end{enumerate}

To address problem \ref{sync1}, we \nuno{who does this? which component of ReZone and how is this done?} track which cpu's cores are currently executing the secure monitor, and only jump to the Trusted OS when none of the cores are executing the secure monitor.
Problem \ref{sync2}, is solved by perform waiting operations in a read-only memory region, which the Trusted OS can not modify. \nuno{I think all of this is really interesting and should be explained in much more detail, possibly even with some figure explaining each of these scenarios.}
To solve problem \ref{sync3}, we wake the core in a read-only memory region, and wait for the Trusted OS to stop executing before jumping to the actual entry point for the core. Knowledge of the active state of the Trusted OS is maintained by a mutex (rz\_lock) which is locked when jumping to the Trusted OS and released when the Trusted OS is no longer executing.
\if0
Problem \ref{sync4} can be solved by making sure that exceptions are first handled in a read-only memory region, and execution of the exception handler only continues after the rz\_lock mutex is released.
\fi
An additional problem arising from marking secure monitor program memory inaccessible to the CPU is sudden loss of a program stack for performing operations \nuno{please explain this better}. We solve this issue by having a separate stack used during memory reconfiguration, and before evaluating whether the Trusted OS is executing.


\if0
Thus, the ways in which a Trusted OS can manipulate memory accesses are two: privileged instructions (disabling virtual memory, setting the page table register), and page table manipulation (e.g., setting permission bits in a page table entry). Our proposed solutions tackles these two mechanisms. To prevent the execution of privileged instruction we use same privilege isolation techniques, removing the ability for the Trusted OS to execute them by removing them from the code, while making sure that ROP gadgets cannot be mounted to execute them [bits please use of thumb mode to mount a rop chain; vTZ; TEEv, PrOS]. To address page table modification we take advantage of the already required companion micro-processor, and use it as a page table sentinel. The Sentinel periodically inspects the Trusted OS page tables to make sure no mappings outside of the allowed ones exist.
\fi

%\subsection{Hardware Memory Access Control}\label{sec:rdc}
%The RDC present in the iMX8MQ is an hardware component external the CPU. By configuring it, it's possible to establish up to four domains. Domains are a collection of resources and corresponding access policies enforced the domain processing elements access them. Access to resources can be controlled by setting read and write permission access for each domain.
%
%
%\subsection{Sentinel and Application Processor}\label{sec:sentinel}
% To implement ReZone we leverage two domains. The application processor is bound to one domain. For normal world and monitor operations the processor can access the resources without restriction except for the RDC itself and the second domain. The microprocessor which executes the sentinel program is bound to the second domain. This domains is configured to be more privileged, having direct access to the RDC, and hence can configure the access policies affecting all other domains.
%
%\subsection{ReZone Trampoline and Exception Interposition}\label{sec:trampoline}
%We modified the context switching logic to be able to activate greyzone every time the Trusted OS executes. Furthermore, we need to interpose every event which returns control back the secure monitor. To achieve this we install our own vector table that uppon an event first waits for monitor protection to be disabled, and only then proceeds with typical execution.
%
%\subsection{Context Switching and Cache Maintenance}\label{sec:ctx_switching}
%Due to the external nature of the component described in \ref{sec:rdc}, accesses are only validated when data is either fetched or written to main memory. This means that memory access control is not performed at cache level, and special care must be taken to remove security sensitive data from cache before performing a context switch from monitor to Trusted OS.
%
%We must syncronize memory accesses when performing cache maintenance operations. In particular we must be certain that all outstanding memory accesses required by a flush operation are complete, before activating monitor protection. Arm provides a DSB to this effect.
% arm cortex a8 programmers guide
% Data Synchronization Barrier ( DSB ). All pending loads and stores, cache maintenance instructions, and all TLB maintenance instructions, are completed before program execution continues. A DSB behaves like a DMB , but with additional properties. 

\david{Note: In the iMX8MQ, the upper 1GB is not protectable by RDC}

\if0
\subsection{Design Alternatives}
Experiments and alternative decisions we tried.

\subsubsection{Clear cache state before jumping to Trusted OS}
\david{This would only make sense if we are trying to protect monitor only. However maybe we could present this section as \textit{assuming same priviliege isolation techniques on Trusted OS}}
Perform combinations (instruction and data maintenance) of the following from non-cached memory:
\begin{itemize}
    \item invalidate instructions (remove instructions from cache)
    \begin{itemize}
        \item by virtual address
        \item single instruction (clears instruction cache)
    \end{itemize}
    \item flush (clean+invalidate) data
    \begin{itemize}
        \item Try to identify commonly used data before jumping to Trusted OS by (by virtual address)
        \item flush all monitor data (by virtual address)
    \end{itemize}
\end{itemize}

\subsubsection{Clear only writable data before jumping to Trusted OS}
\david{This would only make sense if we are trying to protect monitor only}
Only flush RW data, and invalidate vector table instructions.
With intact vector table code, we can safely perform invalidation operations while RDC is still active to prevent undue writes to main memory.
After clearing all monitor data we can safely disable RDC.


\subsubsection{Using same privilege techniques + ReZone}
Use same privilege isolation techniques + the rezone mechanism to prevent updates to pagetables.
We marked Trusted OS pagetables as uncacheable, so that they benefit from RDC protection.


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/xtest_simple_barchart_mon.pdf}
    \caption{Secure monitor isolation tests.}
    \label{fig:xtest_mon}
\end{figure*}
\fi

\subsection{\textcolor{red}{Performance}}
Given that we are now able to run different TEEs on different clusters, one problem arises. Which TEE should run an each cluster. Nowadays it is common for CPUs to be implemented in a BIG.little configuration. So it is intuitive to assign performance sensitive workloads to high performance cores. System designers may define what services are to run on each cluster as to provide the best user experience. One important limitation of our solution is that in order to provide isolation between TEEs, only one TEE should be active on a given cluster. This prevents vulnerabilities in one TEE from affecting another. For example, this prevents a DRM application vulnerability from affecting the cryptographic key management.

\subsection{Communication infrastructure}
\david{shared memory}
\david{Maybe this should go unto the design section}

\subsection{Deployment In Other Platforms}\label{sec:otherplat}
\mypara{Xilinx Protection Units.} Xilinx has also developed and included in their Zynq UltraScale+ MPSoC portfolio a set of protection units complementary to TrustZone~\cite{}. The Xilinx memory protection unit (XMPU) and the Xilinx peripheral protection unit (XPPU) are system-level controllers that verify if a particular bus master is explicitly allowed to access a specific address (memories and peripherals). There are a total of eight XMPUs for protecting transactions into the DDR, the OCM, and the interconnect (e.g., SATA and PCIe). There is one XPPU, which allows for protecting peripherals, message buffers, and inter-subsystem communication channels. A master ID list is used to define the masters that are allowed to access peripherals. Similarly to the i.MX8 families, in Zynq UltraScale+ devices the quad Cortex-A53 cluster has the same master ID for all of its cores, making it impossible to use the XMPU and XPPU to create security domains per core.

\david{demonstrate that there are platforms which are rezone compatible.}
\david{automotive, smartTVs, mobile, industrial control systems (xillinx)}

\mypara{SMMU ReZone Implementation}

%=======================================================================
%> [EVALUATION]
%=======================================================================	
\section{Evaluation}
\label{sec:eval}

In this section we evaluate the prototype ReZone implementation by measuring performance overhead and analyzing security aspects. The overhead evaluation is performed on the iMX8MQ which provides four Arm Cortex-A53, one Arm Cortex-M4. The Cortex-A53 cluster features 32KB L1 instruction, and 32KB L1 data caches per core, and 2MB L2 cache shared by the four cores. Each core's clock frequency can go up to 1.5GHz. The Cortex-M4 runs at 266MHz and features 16KB code bus cache and 16KB system bus cache. We base our work on ATF, OPTEE-OS, and other repositories on Code Aurora IMX repositories \cite{imxaurora}. For all relevant repositories we used the branch imx\_5.4.3\_2.0.0 branches, or similar. For Android we follow NXP provided steps for building Android 10.
We compare three cases: No ReZone, is a typical TrustZone deployment; ReZone, where a system is configured with ReZone; and ReZone no IRQ, which is a system deployed with ReZone but with no Trusted OS preemption, meaning normal world interrupts do not interrupt the Trusted OS. Preventing the Trusted OS from beeing preempted by the normal-world is an optimization we evaluate, due to the high cost of context switching between worlds.

\subsection{Microbenchmarks}

%We evaluate the performance of ReZone by measuring the overhead on small building blocks of normal world-secure world interaction.

\sandro{Go straight to the point on the descriptions. Please see vTZ paper. Write clear takeways and conclusions from results. English is bad..}

\mypara{World switching}
We first measure the impact on world switching, in particular we measure the time it takes for a normal world SMC to reach the Trusted OS. 
With No Rezone, we observe 85.49us between the SMC and handling by the OPTEE. With ReZone the time to switch context between the normal world and the Trusted OS increases to 420.89us, a 4.92x increase.
%\david{Should we measure roundtrip?}
%\david{Should we just write the results in text?}
\if0
The results are presented in \autoref{tab:ctx}.
%
%
\begin{table}[!htb]
\centering
\footnotesize
\begin{tabular}{ccc}
& Time & Overhead\\
\toprule
No ReZone & 85.49us & - \\
ReZone & 420.86us & 4.92x \\
\bottomrule
\end{tabular} 
\caption{Context-switch overhead with \project}
\label{tab:ctx}
\end{table}
\fi

\mypara{GlobalPlatform API}
As baseline for understanding the performance penalties incurred by ReZone, we evaluate the costs of invoking the basic API used for interacting with a TEE.
To do this, we measured the time lapsed for the invocation of this APIs by a client application. 
%The application is executed once, and all test iterations are performed from within the application. 
The results, presented in \autoref{fig:api}, show a significant overhead increase. Surprisingly we observe overheads in calls which do not invoke the the secure world. We believe this is caused by the sequential nature of the test when combined with the cache-maintenance operations. For example TEEC\_Register\_Shared\_memory, performs a Trusted OS call which will clear all caches, while TEEC\_Release\_Registered\_Shared\_Memory does not invoke the Trusted OS, but suffers from the cache maintenance operations performed prior, and the same is true for subsequent requests. Overall, preventing the Trusted OS from being preempted by the normal world slightly improves the overhead.

\if0
\begin{itemize}
    \item InitializeContext
    \item FinalizedContext
    \item OpenSession
    \item CloseSession
    \item AllocateSharedMemory
    \item ReleaseAllocatedSharedMemory
    \item RegisterSharedMemory
    \item ReleaseRegisteredSharedMemory
    \item InvokeCommand
\end{itemize}
\fi

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/api_barchart.pdf}
    \caption{ReZone overhead for main GlobalPlatform APIs}
    \label{fig:api}
\end{figure}

\if0
Measure xtest testsuite overheads. These are the categories pros authors used
\begin{itemize}
    \item storage-stress benchmark\_ 1001 + 1002 + 1003
    \item sha-stress - benchmark\_ 2001 + 2002
    \item aes-stress - benchmark\_ 2011 + 2012
    \item os - 1001 + 1002 + 1003 + 1004 + 1005 + 1006 + 1007 + 1008 + 1009 + 1010 + 1011 + 1012 + 1015 + 1016 + 1017 + 1018 + 1019 + 1020 + 1021 + 1022
    \item - shared memory - \_7000
    \item concurrency - 1013
    \item SDP - 1014
    \item socket - \_2
    \item crypto - \_4
    \item global platform - \_5
    \item storage - \_6
    \item keymanager + derivation + certificates - 800x, 810x
    \item average
\end{itemize}
\fi

\if0
Because cache maintenance is required for both effective monitor protection and correct system behavior, we studied the effect various cache maintenance tactics have one the context switch time of ReZone to determine the best one overall.
Our first approach was to invalidate the instruction cache, and flush all data caches.
In our experiments this provide the best overall results when compared to the other tactics.
The other tactics were invalidating the instructions cache by virtual address, in combination with selectively flushing previously access monitor data structures and function pointers, and invalidating all instruction cache
with selective data flush.
The best overhead results are provided in~\autoref{fig:xtest}. It's worth nothing that the characteristics of the different test suites vary largely. Small quick tests such as the the Global Platform API test exhibit a few additional milliseconds in test duration but cause a high relative overhead increase.

We speculate that the reason flushing all caches is more efficient than most tactics is due to two main reasons.
First invalidating the instruction cache will result in successive faults in monitor protection activation code, which must be performed after caches are flushed. This will cause increased overheads present in whichever tactic we tried. Another reason is that invalidating the instruction cache by virtual address requires a non-neglible amount of computation, due to having to iterate over every single address including the invalidation code itself.
On the other hand selective flushing data .
\fi

\mypara{xtest test suite} OPTEE provides a suite of regression tests, called xtest, to verify the correct implementation of Trusted OS and related APIs. We measure the execution time of these tests to evaluate how ReZone affects the execution of the plethora of TEE functionality. %We execute the xtest program for each test as opposed to having the program execute all tests in one sitting. 
We modify the xtest program to measure the elapsed time of each unit test. The geometric mean of the overheads in each test within a group of tests is presented in \autoref{fig:xtest}.
We warn the reader to not interpret the results of these tests at face value, as these tests are not intended as benchmarks, except for the benchmark suite which includes storage, and cryptographic benchmarks.
However, analyzing the unit tests with higher overheads provides insight into the impact ReZone has on a system. For example we observed significantly higher overheads in some regression tests than in others.
The main factor is the number of context switches.
Taking this into account we modified one of the most affected tests to be executed almost entirely in a TA.
The modification decreased the incurred overheads from more than 4x to less than 0.05x, as can be seen in \autoref{fig:migration}.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/xtest_simple_barchart.pdf}
    \caption{Geometric mean of ReZone's overhead in xtest test suite.}
    \label{fig:xtest}
\end{figure*}
% linha a tracejado com a média
% máximo percentil 5\% 95\%
% Escala de 0% a 100%
% TODO: Expirementar as mesmas escalas

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/benchmarks/migration_barchart.pdf}
    \caption{xtest 4007\_symmetric test with normal world code migrate to execute in a TA, and in its original form.}
    \label{fig:migration}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/nw_barchart.pdf}
    \caption{ReZone normal world impact measured as impact on PCMarkv2 benchmark without invoking a Trusted OS, and with periodic invocations in 1s, 10s, and 20s intervals.}
    \label{fig:PCMarkv2}
\end{figure}


\subsection{Overhead in Secure Applications}

%\sandro{Change order between bitcoin wallet and DRM player. I would change the title to "Secure Applications Overhead" ou qualquer coisa assim... }

In this section we evaluate two real-world use cases to measure performance overhead of ReZone. These two use cases represent the two main workloads of TrustZone. The bitcoin wallet represents an infrequently invoked service such as cryptographic key management (e.g., keymaster) or biometric authentication (e.g., fingerprint service), while the DRM player represents a use case requiring frequent Trusted OS interaction (several times per second).

\mypara{Bitcoin wallet}
To evaluate the performance of infrequent secure world operations, typical of TEE client-applications, we setup a bitcoin-wallet to be executed as a TA in a Trusted OS. We use a previous implementation  of a bitcoin wallet~\cite{bitcoinwallet}, and slightly modified it to measure the execution times of each operation. We measure the time to execute with the \emph{time} linux utility, and observe the \emph{real time} component of the output. Overheads go as high as 1.7x, for the command that executes in least ammount of time, however for other commands the overhead is smaller, as low as 1.16x. Overall, disabling interrupts in the Trusted OS achieves modest performance improvements. The results are presented in \autoref{fig:bitcoinwallet}.
%https://github.com/Jamie-Cui/bitcoin-wallet

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/benchmarks/wallet_barchart.pdf}
    \caption{ReZone overheads on a bitcoin wallet use case.}
    \label{fig:bitcoinwallet}
\end{figure}

\mypara{DRM Player}
To test overheads incurred in playing DRM video content, we based our setup on OPTEE Clearkey plugin \cite{opteeclearkey} and in the reference media player ExoPlayer \cite{exoplayer}. By doing this we approximate a Level 2 DRM compatible setup \cite{widevinelevels}, where content is decrypted in the TEE, but decoded elsewhere (in our setup, in the normal world). With the Clearkey plugin, video content is split into subsamples. To take advantage of the TEE, subsamples are decrypted by the TEE. After decryption, subsamples are decoded by the normal world and the content presented to the user. To measure DRM performance we take the average time to decrypt a single subsample. 
%\autoref{fig:drm} presents the results. 
Although we observed more than 12x increase in subsample decryption, decryption times fall well bellow the ~16ms mark for 60fps content and 41ms for 24fps content.
We also observe a slight improvement in performance by disabling TEE interrupts. 
\if0
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/benchmarks/drm_barchart.pdf}
    \caption{DRM use case test overhead per subsample overhead.}
    \label{fig:drm}
\end{figure}
\fi

Although ReZone causes significant overheads, the smooth playback of media is not compromised. In ExoPlayer, processing decoded frames for rendering the final image occurs at periodic intervals. We measure the time elapsed between decoded content. The results are presented in \autoref{fig:drm_macro}. Although the period between processing frames increases, because the value is still lower than the content framerate, the overhead is not perceptible to the end-user.
%\david{honestamente deixa-me desconfortável dizer isto para a resolução de 1080... Apesar de sentir que é verdade o facto de o player dar mal deixa-me reticente. Mas na parte em que ele funciona bem, acredito que isto seja verdade.}

Each subsample is decrypted individually, and due to the costs incurred by context switching, we believe that playing DRM content in a ReZone enabled system can be significantly optimized by increasing the number of subsamples decrypted per TEE call. Furthermore as pointed out in \cite{Kwon19}, in a platform featuring heterogeneous CPUs DRM performance can be improved by leveraging the highest performance cores.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/benchmarks/drm_barchart_macro.pdf}
    \caption{DRM use case test timelapse between processing output buffer.}
    \label{fig:drm_macro}
\end{figure}

% Apresentar valores das barras em milisegundos
% Medir frame drops
% tempo de execução do video
% gráfico com linha temporal com tempo de chamadas ao mundo seguro e apresentaão de cada frame
% QML inspector (?) like
% medir macro-processing
% limite da percepão para latência
% https://source.android.com/devices/tech/debug/systrace 

\subsection{TCB Reduction}
\david{show reduction in lines of code and binary size, from monitor + optee, to monitor}

\david{We should mention, how the multiple TEEs affects the TCB (i.e., secure monitor), specially if we consider "dynamic" TEEs (for all developers for instance).}

\david{comparar com a TCB de outros trabalhos}

\subsection{Normal-world impact}
To measure the impact of ReZone on normal world we execute PCMarkV2 benchmark in AOSP built for our test platform. The benchmark tests various aspects of a devices performance on real world scenarios. The final test result is represented by \emph{Work 2.0 performance score}. We perform measurements on a setup configured without ReZone, configured with ReZone without periodic invocation, configured with Rezone and with periodic invocations to a Trusted OS in 1s, 10s, and 20s intervals. The more frequent the invocation to Trusted OSes the more performance is affected, as can be observed in \autoref{fig:PCMarkv2}. However, ReZone does not degrade performance of the normal world if Trusted OSes are not invoked. 


\subsection{Multiple TEEs}
To measure the impact multiple ReZone Sandboxes might have in performance, we create two scenarios. In the first scenario we perform a TA invocation on Trusted OS 2, we use xtest regression test 1006, due to its simplicity and because it invokes TA. On scenario 2, we first invoke a simple operation on Trusted OS1. This is done by invoking xtest regression test 1001, which will only invoke the Trusted OS, and not a TA. Invoking the trusted OS1 first will create a situation in which a TLBI is performed before the first call to Trusted OS2. After Trusted OS1 is invoked we invoke a TA, the same xtest regression test 1006, on Trusted OS2. 
We observe an overhead of 1.31\% corresponding to an average of 27µs in a test which takes 205µs to execute without invalidating the TLB. We consider this overhead to be negligible, in particular in light of the overhead already incurred by the cache maintenance operations.
\david{multicluster scenario}

\subsection{Cache hierarchy}
In platforms with L3 cache it may be possible to use the hardware controller to validate accesses to it.

\section{Security Analysis}
In this section we analyze how well ReZone can prevent known TrustZone-based TEE attacks, and analyze how known vulnerabilities, out of a set of CVEs ranked as critical to system security, are mitigated by our design.
\if0
\begin{itemize}
    \item Address how CVEs are solved by applying ReZone (See TFence for a paper that does the same)
    \item Scheme detailing how vulnerabilities are prevented
\end{itemize}
\fi


\subsection{Attack Mitigation}
\mypara{Attack 1. } By compromising a TA, the authors were able to exploit a flaw in a secure driver~\cite{BreakingArmTZ, DeepDive}. Secure drivers have access to mmap, which allows them to map physical memory. The Secure Monitor can be mapped by the now malicious secure driver. 
By being able to map the Secure Monitor the attacker can do anything on the platform, including exposing secrets such as secret keys.
The master key is one of such secrets. In the Samsung ... it is loaded by the drcrypto drive and is used in cryptographic operations.
There are two ways in which the master key can be obtained: a) obtaining execution in EL3 and reading the master key location, b) or via an SMC to the secure monitor.

\mypara{Mitigation 1. } \project mitigates against obtaining the Master Key by preventing the Trusted OS from accessing monitor memory. Because malicious software can longer map the Secure Monitor it can no longer obtain the master key directly. This solves problem 1.a). However it can still obtain the master key through a Secure Monitor Call (SMC), problem 1.b). To mitigate this, with \project, it might make sense to implement cryptographic primitives in the secure monitor, so as to prevent secret key material being exposed to Trusted OSes and TAs.

\mypara{Attack 2.} An attacker can compromise a system TA (see $\S$\ref{sec:attacks}) through the Trusted OS. An attacker obtains execution in the Trusted OS. With Trusted OS privileges, it becomes possible to comprise system TAs. For example by obtain the secret key used to encrypt the file system~\cite{BreakFDE} or by effectively disabling the fingerprint mechanism~\cite{shen-trustedcore}. 
%The secret key is encrypted by the user password, however it is possible to bruteforce the password on a powerful PC. 

\mypara{Mitigation 2.} \project allows for the secure deployment of multiple OSes. It is possible to prevent a compromised component from the Application-TEE domain from obtaining secrets from the System-TEE domain, provided that the System-TEE is bug free, which is easier than doing the some for a single TEE domain. Thus, by using \project to create more than one TEE domain, a vulnerability in one domain can not obtain the secrets from another.
 
\mypara{Attack 3.} By leveraging a malicious TA access to normal world memory, it is possible to access all memory in the normal world~\cite{gb-exploit6, Aravind2017}. This is possible because the Trusted OS can map the normal world physical memory at will, and can map this memory unto a TAs address space. With access to normal world memory an attacker can compromise the Linux kernel, for example by creating a back door within seldom used kernel modules. This gives the attacker arbitrary code at kernel level of privilege.

\mypara{Mitigation 3.} In \project we can restrict the normal world memory available to a Trusted OS (see $\S$~\ref{sec:secure_monitor_isolation}). 
The secure monitor can enforce a memory layout previously established according to where the rest of the system images are loaded. This requires knowledge of what memory is dedicated for sharing memory between the TEE and REE, however, TF~-~A already support modifying an in-memory device tree. This means that TF-A can specify to the kernel which memory is available for sharing information between worlds. Fixing the shared memory space makes it easier for secure monitor to validate Trusted OS mappings, and consequentially its memory, although at a cost of not supporting dynamic shared memory, which allows a normal world process to mark part of its memory as shareable with the TEE.

\mypara{Attack 4.} Code reuse attacks. An attacker can leverages control highkacking to compromise the Trusted OS~\cite{gb-exploit4}. In particular the attacker might leverage the presence of privileged operations, for example in the case for Armv7-A or Armv8-A\_aarch32 the DACR registers, which when set to zero disable MMU based memory protection.

\mypara{Mitigation 4.} In \project, by removing privileged instructions from the Trusted OS, an attacker would be required to either modify executable memory regions, which can be easily thwarted by using PXN features, or make a request to the secure monitor for performing them. The secure monitor can have strict policies on the validity of performing this operations. For example it might make sense to allow this operations at boot time, but not after. Although this does not prevent attacks completely it raises the bar significantly for an attacker.

\mypara{Attack 5.} Boomerang attacks~\cite{Aravind2017}.

\mypara{Mitigation} Boomerangs attacks are mitigated by specifying which region of main memory is going to be used for shared memory. This can be communicated trough the device tree. The disadvantage is that it prevents normal world from dynamically allocating shared memory, since it must be allocated in a specific memory region.

\subsection{Vulnerability Analysis}

We analyze 80 CVEs reported as critical to evaluate how \project lowers the impact of high impact vulnerabilities in TEE systems, see \autoref{tab:security-table}.

\input{secure_analysis_table}

\mypara{Trusted OS and Trusted Applications Vulnerabilities}
Trusted OS and Trusted TA vulnerabilities, are related in that often times a vulnerability in a TA can be leveraged to exploit vulnerabilities and flaws in the Trusted OS ~\cite{Cerdeira2020}. As we have exemplified earlier in this section, this results in fully compromised systems for an attacker. With \project, vulnerabilities and flaws in these components are mitigated in as much as the vulnerability affects only the Trusted OS and corresponding TAs domain. Most of the vulnerabilities in \autoref{tab:security-table} pertain Trusted OS and TA, and the impact of a vulnerability in them can be substantially reduced.

\mypara{General SW Vulnerabilities} We describe as SW vulnerabilities those that do not provide sufficient detail as to the affected component. All 80 of the presented CVEs in \autoref{tab:security-table} are described to completely compromise integrity, confidentiality and availability of the system. In light of this we considered that \project mitigates this vulnerabilities according the same rationale provided for the mitigation of Trusted OS and Trusted Application vulnerabilities.

\mypara{Hardware Vulnerabilities} The \href{https://www.cvedetails.com/cve/CVE-2017-18282}{2017-18282} CVE, is a hardware issue where a hardware component of the system can be manipulated by a malicious agent from the normal world into performing secure data accesses. These types of issues could be prevented by \project, by preventing a BUS master from accessing critical memory (e.g., monitor and trusted OS).

\mypara{Cryptographic Vulnerabilities} Cryptographic issues are well beyond the scope of \project, even without common software vulnerabilities in Trusted OSes and Trusted Applications, the security functionality provided by these components is still dependent on the correct and careful implementation of cryptographic primitives and schemes.

\mypara{Bootloader Vulnerabilities} The bootloading stage occurs even before the secure monitor starts execution. At this stage the CPU executes in the secure world and flaws at this stage enable attackers to load arbitrary code at the highest privilege level. We consider these types of problems out of the scope of \project as the mechanism used to load the runtime TCB are the root of all trust in the system.


%\mypara{2016-2431} This vulnerability refers to a lack of system calls parameter validation on the Trusted OS. It assumes code execution privileges in a TA, and enables attackers to build read and write gadgets to the Trusted OS. This vulnerability fits the attack scenario where an attacker gains Trusted OS level privileges. With Trusted OS level of privileges an attacker can access any memory and every resource available to the CPU. Although \project does not address the vulnerability directly is prevents a compromised Trusted OS from attacking the normal world and the secure monitor, thus reducing the impact of this vulnerability.


% \david{TODO: escolher 4 ou 5 vulnerabilidades}
\if0
2016-2431	"The Qualcomm TrustZone component in Android before 2016-05-01 on Nexus 5, Nexus 6, Nexus 7 (2013), and Android One devices allows attackers to gain privileges via a crafted application, aka internal bug 249688009.

This vulnerability assumes code execution privileges in QSEE TA.
TrustZone kernel does not perform any validation on QSEE-supplied arguments (more specifically, it freely uses any given pointers), meaning that at the time all syscalls were vulnerable. Vulnerable syscalls allow for building read and write gadgets to the Trusted OS.
"


2017-17176	The hardware security module of Mate 9 and Mate 9 Pro Huawei smart phones with the versions earlier before MHA-AL00BC00B156, versions earlier before MHA-CL00BC00B156, versions earlier before MHA-DL00BC00B156, versions earlier before MHA-TL00BC00B156, versions earlier before LON-AL00BC00B156, versions earlier before LON-CL00BC00B156, versions earlier before LON-DL00BC00B156, versions earlier before LON-TL00BC00B156 has a arbitrary memory read/write vulnerability due to the input parameters validation. An attacker with the root privilege of the Android system could exploit this vulnerability to read and write memory data anywhere or execute arbitrary code in the TrustZone.


2017-6294	"In Android before the 2018-06-05 security patch level, NVIDIA Tegra X1 TZ contains a possible out of bounds write due to missing bounds check which could lead to escalation of privilege from the kernel to the TZ. User interaction is not needed for exploitation. This issue is rated as high. Version: N/A. Android: A-69316825. Reference: N-CVE-2017-6294. 

NVIDIA TLK TrustZone OS contains a potential vulnerability in the logging driver where the software writes data after the end or before the beginning of the intended buffer, which may lead to arbitrary code execution, denial of service, or escalation of privileges. - buffer overflow may lead to arbitray code execution within the TEE"


2015-4422	"The TEEOS module of Huawei Mate 7 smartphone which is used to realize the function of fingerprint identification has an input check error, which enables the attackers with the root permission to modify kernel-mode memory data of TEEOS module, which could make system break down, TEEOS be tampered or malicious code execution. (Vulnerability ID: HWPSIRT-2015-03012)

There is a arbitrary memory read/write vulnerability in the hardware security module of some Huawei smart phones due to the input parameters validation. An attacker with the root privilege of the Android system could exploit this vulnerability to read and write memory data anywhere or execute arbitrary code in the TrustZone. (Vulnerability ID: HWPSIRT-2017-01060)
http://www.huawei.com/en/psirt/security-advisories/huawei-sa-20170306-01-smartphone-en - An attacker can write arbitrary code to TEE global task memory, this allows him to obtain execution wiithin the global task by provoking a crash and forcing code execution to an attacker controlled address
 - a system call vulnerability allows an attacker to arbitrarily write to any memory address within the TEE, which allows him for example to bypass security checks for accessing fingerprint images

Security Advisory - Arbitrary Memory Read Write Vulnerability in Huawei Smart Phones
"
\fi

\if0

\subsection{Attack Surface}
%\david{Mitigations are also attack surface}

The attack surface for a typical TrustZone assisted TEE system includes all the SMCs and interfaces the secure monitor, Trusted OS and Trusted Applications provide to the normal world.

Attack surface becomes:
\begin{itemize}
    \item Guessing the authentication token
    \item Connection with the micro-controller
    \item SMC calls (calls to the monitor)
    \item Interfaces TAs provide
    \item Trusted OS syscalls
\end{itemize}

\fi

%=======================================================================
%> [DISCUSSION]
%=======================================================================	
\section{Discussion}
\label{sec:discussion}

\mypara{ReZone vs ArmV8.2 vs Armv9.} ...

\mypara{Per-CPU isolation / control.} ...

%=======================================================================
%> [RELATED WORK]
%=======================================================================	
\section{Related Work}
\label{sec:related}

\par There are several security-oriented hardware architectures that have been devised to provide basic underlying primitives for the creation of TEE systems~\cite{Maene2018, Pinto2019, Cerdeira2020}. These TEE-enabler hardware technologies includes \textbf{CPU extensions} such as Intel SGX~\cite{}, Arm TrustZone~\cite{Pinto2019}, and Sanctum~\cite{Costan2016}, separate \textbf{co-processors} such as the Apple SEP~\cite{} and the Qualcomm SPU~\cite{}, dedicated \textbf{security chips} such as the TPM~\cite{}, and hardware support for \textbf{secure virtualization} such as AMD SEV~\cite{}. Recently, academia has been focused in exploring RISC-V to propose novel TEE hardware architectures~\cite{Nasahl2020, Nasahl2020}. CURE~\cite{Bahmani2021} proposes ... offering different types of enclaves... and HECTOR-V~\cite{Nasahl2020} proposes a secure TEE design strategy using a heterogeneous CPU architecture. In our work, we leverage an MCU in combination with a resource controller within commercial off-the-shelf (COTS) SoC to provide augmented isolation for the TrustZone hardware architecture.

%TyTAN~\cite{} and TrustLite~\cite{} are preeminent examples of hardware TEE architectures for resource-constrained embedded devices. 

%\par Contextualize TEE hardware with systems... In the following, we describe different approaches aiming at ... 

\mypara{Hardware-enforced TEE systems.} Write hardware-enforced TEE with augmented capabilities aiming at offering additional security guarantees ... Komodo~\cite{Ferraiuolo2017} ...  \david{refer TLR e TrustShadow} ... SKEE~\cite{Azab2016} ... TrustICE~\cite{Sun2015} and Sanctuary~\cite{Brasser2019} leverages the TZASC to create enclaves within the normal world. These enclaves are isolated and cannot access the REE, but the secure OS has full access to the system. TrustICE has severe multi-core limitations, while Sanctuary falls short on depending on TZASC features not available in any COTS SoC release to date. Our solution provides isolation ... and rely on a mechanism ... SecTEE~\cite{} ... Keystone~\cite{Lee2020} and MultiZone~\cite{Garlati2020} leverage the hardware primitives available on the standard RISC-V ISA, i.e. physical memory protection (PMP) to isolate individual enclaves. While our system can be implemented ..., the  


\mypara{Virtualization-aided TEE systems.} The idea of leveraging hardware virtualization support to implement isolated environments is not a new endeavour. Overshadow~\cite{Xiaoxin2008}, Trustvisor~\cite{McCune2010}, and Inktag~\cite{Hofmann2013} implement hypervisor-based architectures and mechanisms for Intel and AMD. In the context of TrustZone-based systems, vTZ~\cite{Hua2017}, OSP~\cite{Cho2016}, and PrivateZone~\cite{Jang2018} leverages the hardware virtualization extensions available in the NW to implement isolated environments. These approaches have some drawbacks, which typically includes TCB augment, performance decrease, and intrusive design. OSP~\cite{Cho2016} tries to minimize the performance impact by activating the hypervisor only when the TEE is demanded. Our solution does not rely on any hardware virtualization support, and so can be used in combination with existing hypervisors and support legacy systems.
%, while providing additional security guarantees.


\mypara{Same-privileged Isolation.} Same-privileged isolation, also referred to as \textit{intra-level} isolation~\cite{Yeongpil2017}, is a well-established software technique to harden monolithic OS (e.g., \textit{nested kernel}~\cite{Dautenhahn2015}), hypervisors (e.g., \textit{Nexen}~\cite{Shi2017}), and TEEs~\cite{Li2019, Kwon19}, typically by interposing on all updates to virtual memory translations to assert protections on physical memory. TEEv~\cite{Li2019} and PrOS~\cite{Kwon19} use same-privilege isolation to secure a minimalist hypervisor from secure guest OSes, due to the current lack of hardware virtualization support in the SW\footnote{S-EL2 was introduced in Armv8.4, but no silicon was released to date}. Our solution don't include a secure hypervisor as part of the TCB and we do not use same-privileged isolation but rather ... (\textit{page table mediation}) ... to harden the secure OS from accessing the REE.   




%OSP~\cite{Cho2016}: Their work enables TAs to run on the normal world by using an hypervisor. 2 stage translation overheads are mitigated by only activating the hypervisor when TAs need to run. Our work does not require an hypervisor to be dedicated to the TAs, freeing that privilege level for other applications.

%TrustICE~\cite{Sun2015}: Their work enables TAs to run on the normal world by suspending the REE-OS on all cores while the TA is running. Non-running TAs are protected by marking their memory as secure. Biggest disadvantage is suspending the REE-OS to run TAs, our approach does not require this to provide multiple runtime environments.

%Sanctuary~\cite{sun2015trustice}: Their work enables TAs to run on the normal world by taking advantage of non-common platform features and hardware. Their work relies on each CPU core having its own master ID and this ID being used in bus accesses. It is unknown how widely available this feature realy is. For example the platform they use to test it, the hikey960 does not support it. Further it requires the presence of the TZC-400 which enables each core to have a differente view of what is normal-world memory. Wide use of the TZC unlikely. Going by the Arm-Trusted-Firmware repository, very few platforms actually use the TZC. Our solution is deployable to real world platforms.

%TEEv~\cite{Li2019}: Their work does not provide hardware enforced isolation, rather, it relies on same privilege isolation techniques, as such removing privileged instructions. With this they implement an hypervisor in EL1 to run multiple TEEs on the secure world. In our solution we only require trap and emulation techniques to protect the normal world, which is already "vulnerable" today. To protect environments between one another we achieve hardware enforced access control.

%PrOS~\cite{Kwon19}: Their work does not provide invariant isolation properties rather, they make calls to the monitor in a paravirtualizated-fashion. With this they implement an hypervisor in EL3 and are able to run multiple TEEs on sEL1. In our solution we only require trap and emulation techniques to protect the normal world, which is already "vulnerable" today. To protect environments between one another we achieve hardware enforced access control.

%vTZ~\cite{Hua2017}: Their work provides a TEE environment for each virtual machine, with aid of an hypervisor. They do this by emulating TrustZone features in software.




%=======================================================================	
%> [CONC]
%=======================================================================
\section{Conclusion}
\label{sec:conclusion}

\section*{Acknowledgments}
We thank... David Cerdeira was supported by FCT grant SFRH/BD/146231/2019. - Algoritmi project reference: UIDB/00319/2020 -


\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.


==> extra/sec2-nuno.tex <==
\subsection{Standard TrustZone Security Mechanisms}

We focus on TrustZone extensions for Armv7-A/Armv8-A architectures. TrustZone enables CPU cores to operate in one of two states: \textit{secure} and \textit{non-secure}. At exception levels EL0, EL1, and EL2, a processor core can execute in either of these states. For instance, the processor is in non-secure exception level 1 (N.EL1) when running REE kernel code, and in secure EL1 (S.EL1) for executing the trusted OS. The security state is controlled by the \texttt{SCR\_EL3.NS} bit in the processor. Regardless of the value of \texttt{SCR\_EL3.NS}, EL3 is always in secure state. To change security states, the execution must pass through EL3.

TrustZone extends the memory system by means of an additional bit called NS bit that accompanies the address of memory and peripherals (see Figure~\ref{fig:RZ_HW}). This additional bit gives independent physical address spaces for the normal world and for the secure world. Software running in the normal world can only make \textit{non-secure accesses} to physical memory because the core always sets the NS bit to 1 in any memory transaction generated by the normal world. Software running in the secure world usually makes only \textit{secure accesses} (i.e., NS=0), but can also make non-secure accesses (NS=1) for specific memory mappings using the NS flags in its page table entries. The processor maintains separate virtual address spaces for the secure and non-secure states. For instance, it does not use a NS.EL1 translation while in secure state, or a S.EL1 translation while in non-secure state. %Each translation is supported by independent page tables. 
The page table entries contain an NS bit that allow the trusted OS (or the secure monitor) to map virtual addresses to non-secure physical addresses by setting NS to 1. %Otherwise, setting this bit to 0 will translate into the secure physical address space. 
%The page table entries also contain an NS bit that is interpreted differently according to the current processor state.
In non-secure state, that bit is ignored: the virtual address will always be translated to non-secure physical address (NS=0). %Otherwise, the NS in the page table entry determines which physical address space the virtual memory address translates to, i.e., the access will be non-secure or secure if the NS bit in the page table entry is 1 or 0, respectively.
The NS bit of the translated physical memory address is propagated onto the data cache tags. Trying to perform a non-secure access to cached data marked as secure causes a cache miss. Accessing cached non-secure or secure memory in secure state causes a hit.


%TrustZone also extends the memory system by means of an additional bit called NS bit that accompanies the address of memory and peripherals. This bit is added to all memory system transactions, including cache tags and access to system memory and peripherals (colored in brown in Figure~\ref{fig:RZ_HW}). This additional bit gives a physical address space for the secure world and a completely separate physical address space for the normal world. Software running in the normal world can only make no-secure accesses to memory because the core always sets the NS bit to 1 in any memory transaction generated by the normal world. Software running in the secure world usually makes only secure memory accesses, but can also make non-secure accesses for specific memory mappings using the NS flags in its page table entries. 

%Memory and resource access are made aware of the current security state of the processor through the NS bit (non-secure bit). The NS bit is then used to bar access to a resource according to the security state. Additionally, secure-world can map the memory as being non-secure, which results in secure-world memory accesses being performed as normal-world accesses. This way, the secure-world can access normal-world as if normal-world is the one accessing the resource. This design decisions makes it hard to prevent secure-world from accessing normal-world memory. For example, TZC-380 is a TrustZone controller developed by Arm which has a feature enabling memory accesses performed in a secure state to not being able to access normal-word memory (priority inversion), however given that secure-world software can map memory as being normal, this does not prevent the secure-world from accessing normal-world memory. 

%TrustZone also extends the memory system by means of an additional bit that accompanies the address of memory and peripherals. This bit is called the NS bit, indicates whether the access is performed in security state secure or non-secure. This bit is added to all memory system transactions, including cache tags and access to system memory and peripherals (colored in brown in Figure~\ref{fig:RZ_HW}). This additional bit gives a physical address space for the secure world and a completely separate physical address space for the normal world. Software running in the normal world can only make no-secure accesses to memory because the core always sets the NS bit to 1 in any memory transaction generated by the normal world. Software running in the secure world usually makes only secure memory accesses, but can also make non-secure accesses for specific memory mappings using the NS flags in its page table entries. 

%There are separate virtual address translation schemes for the secure and non-secure states. For instance, the processor does not use a NS.EL1 translation while in secure state, or a S.EL1 translation while in non-secure state. Each translation is supported by independent page tables. The page table entries contain an NS bit that is interpreted differently according to the current processor state. If the processor is in non-secure state, that bit is ignored: the virtual address will be always translated to non-secure physical address (NS=0). Otherwise, if the processor is in secure state, the NS bit in the page table entry determines which physical address space the virtual memory address translates to, i.e., the physical address will be non-secure or secure if the NS bit in the page table entry is 0 or 1, respectively. The NS bit of the translated physical memory address is included in the data cache tags. Trying to perform a non-secure access to cached data marked as secure causes a cache miss. Accessing cached non-secure or secure memory in secure state causes a hit.

%If a cache miss occurs, the system sends a request to external memory, which includes the physical memory address along with the respective NS bit. 
TrustZone-aware memory and address space controllers are usually configured to map non-secure/secure physical address spaces to different physical memory regions. Typically, the non-secure address space is mapped to a subset of the existing physical memory. In contrast, the secure address space covers the entire existing physical memory, including the regions that are mapped to non-secure address space. In the Arm architecture, the TZASC enforces physical memory protection by allowing the partitioning of external memory on secure and non-secure regions. To date, Arm has publicly released two TZASC specifications, i.e., the Arm CoreLink TZC-380 and TZC-400. Both controllers share similar high-level features, i.e., the ability to configure the security access permissions for memory regions (contiguous areas in the address space).

%, but, at the low-level, there are slight differences. For instance, the TZC-380 provides a \textit{security inversion} option (disabled by default), which allow non-secure memory regions to not be accessible to masters in a secure state. This feature is not available in the TZC-400. The TZC-400 introduces a set of prime mechanisms for fine-grain isolation, in particular, the \textit{identity-based filtering of non-secure accesses}, which allows per bus master (e.g., CPU cluster, MCU, DMA controller) partition. Despite the existence of TZC-380 and TZC-400 specifications, OEM manufacturers typically embedded their own proprietary controllers into their SoCs (e.g., Rockchip RK3399), which just provides coarse-grained configuration. There are SoCs used in well-established Arm-based platforms, e.g., Raspberry Pi 4, which do not feature a TZASC-like controller at all~\cite{}. 


\subsection{Challenges of Reducing S.EL3 Privileges}

The TrustZone mechanisms described above were designed under the assumption that the S.EL1 (trusted OS) and EL3 (secure monitor) are trusted. However, if the trusted OS is hijacked, the attacks described Figure~\ref{fig:intro_trustzone} can be trivially mounted. For illustration purposes, suppose that the physical memory addresses PA$_\textrm{OS}$, PA$_\textrm{TK}$, and PA$_\textrm{SM}$ are allocated to rich OS, TA$_\textrm{K}$, and secure monitor, respectively. The attacker could mount said attacks by creating virtual address mappings in the S.EL1 page tables as indicated bellow, and use the virtual addresses VA$_i$ to access (read/write) the memory pages of the rich OS, TA$_\textrm{K}$, or secure monitor. Notation VA$\rightarrow\langle$PA, NS$\rangle$ denotes a page table entry translating virtual address VA to the physical address PA and associated NS bit value:

\noindent VA$_\textrm{OS}\rightarrow\langle$PA$_\textrm{OS}$, 1$\rangle$, VA$_\textrm{TK}\rightarrow\langle$PA$_\textrm{TK}$, 0$\rangle$, VA$_\textrm{SM}\rightarrow\langle$PA$_\textrm{SM}$, 0$\rangle$

Preventing these memory accesses by reducing the privileges of S.EL1 code is currently not possible using standard TrustZone mechanisms. Even though TZASC controllers such as TZC-380 and TZC-400 include the ability to prevent secure accesses from accessing non-secure physical memory regions, trusted OSes can map memory as normal (VA$_\textrm{OS}$), enabling them to perform normal world accesses from secure world. Moreover, since S.EL1 software has the privilege to reconfigure the TZASC, the trusted OS can always override any permissions that might have been set by the secure monitor for blocking the trusted OS's access to certain memory regions. Access to the secure monitor (VA$_\textrm{SM}$) and TAs (VA$_\textrm{TK}$) can also not be restricted. In Armv7-A/Armv8-A, trusted OS and secure monitor enjoy the highest privileges with regard to read-write operations over secure and non-secure memory. %Thus, the trusted OS has a complete view and full access to all secure world resources.

%, including the secure monitor (VA$_\textrm{SM}$) and TAs (VA$_\textrm{TK}$). The trusted OS can not practically be restricted from accessing all normal-world memory. Even though TZASC controllers such as TZC-380 and TZC-400, feature the possibility to define various memory regions, including the ability to prevent secure-world from accessing the normal-world, Trusted OSes can map memory as normal (VA$_\textrm{OS}$), enabling them to perform normal world accesses from secure world. Moreover, S.EL1 software has also the privileges to reconfigure the TZASC, which means that the standard TrustZone security mechanisms are insufficient for reducing the privileges of S.EL1 code.

%TrustZone is a System-on-Chip (SoC) and CPU system-wide security solution available in a broad range of Arm processors. %The technology has been pivotal for the materialization of TEEs in mobile devices by providing an isolated environment for secure processing of sensitive data and programs (i.e., trusted applications). TrustZone is built upon the concept of protection domains, i.e., the {\em secure world} (SW) and the {\em normal world} (NW). The SW shields critical functionality from the NW, which is used for running an untrusted operating system (OS) and its applications. 
%\autoref{fig:tz_sw_overview} depicts the software architecture of a TrustZone-assisted TEE. Inside the SW runs the TEE software, while in the NW run the Rich Execution Environment (REE) and untrusted applications. The TEE software has three fundamental building blocks: the {\em secure monitor}, the {\em trusted OS}, and {\em trusted Applications}. The secure monitor, running at the higher level of privilege (i.e., S-EL3), provides basic mechanisms for secure context switching and platform-specific management (e.g., power management). The trusted OS runs in S-EL1 and provides an underlying infrastructure for sustaining the lifecycle of TAs. TAs execute in unprivileged S-EL0 and are typically developed by platform vendors and OEMs. 


%Trusted applications are unprivileged programs that make use of the Trusted OS services to implement a wide range of features, which serve mainly two purposes. One is providing trusted services to the system and the OS. This includes handling biometric identification, cryptographic key management and trusted random number generation, to name a few. This is software developed by the platform vendor or OEMs. The other purpose of TAs is implementing application specific services whose compromised functionality affects the company who developed them or the user, but not the system directly. Examples of this are TAs part of DRM solutions, and TAs implementing part of electronic payments systems. Some applications require efficient cross-world communication mechanisms. To enable this, trusted OSs often allow TAs to map physical memory. The Trusted OS manages the physical memory available to each TA, some Trusted OS implementations enable TAs to map any normal-world address, while others only enable the mapping of specific shared memory regions. The last piece of a running TEE, is the {\em secure monitor}, which implements mechanisms for secure context switching between worlds and runs with highest privilege, in protection ring EL3. 


%The {\em TEE bootloader} bootstraps the TEE system into a secure state, and it is critical to implement the trusted boot primitive. Together, trusted applications, trusted OS, secure monitor, and TEE bootloader constitute the software TCB of a typical TEE system. For this reason, TEE designers aim for small and bug-free implementations. Nonetheless, vulnerabilities exist and attacks are successful.

%\mypara{TrustZone Address Space Controller.} The TrustZone Address Space Controller (TZASC) enforces physical memory protection in TrustZone-based systems. The TZASC allows the partition of external memory on secure and non-secure regions. To date, Arm has publicly released two TZASC specifications, i.e., the Arm CoreLink TZC-380~\cite{} and TZC-400~\cite{}. Both controllers share similar high-level features, i.e., the ability to configure the security access permissions for memory regions (contiguous areas in the address space), but, at the low-level, there are slight differences. For instance, the TZC-380 provides a \textit{security inversion} option (disabled by default), which allow non-secure memory regions to not be accessible to masters in a secure state. This feature is not available in the TZC-400. The TZC-400 introduces a set of prime mechanisms for fine-grain isolation, in particular, the \textit{identity-based filtering of non-secure accesses}, which allows per bus master (e.g., CPU cluster, MCU, DMA controller) partition. Despite the existence of TZC-380 and TZC-400 specifications, OEM manufacturers typically embedded their own proprietary controllers into their SoCs (e.g., Rockchip RK3399), which just provides coarse-grained configuration. There are SoCs used in well-established Arm-based platforms, e.g., Raspberry Pi 4, which do not feature a TZASC-like controller at all~\cite{}. 
%This results in a significant heterogeneity and fragmentation ...        

%At its core TrustZone extends the processor to enable CPU cores to operate in one of two states, secure and non-secure. Memory and resource access are made aware of the current security state of the processor through the NS bit (non-secure bit). The NS bit is then used to bar access to a resource according to the security state. Additionally, secure-world can map the memory as being non-secure, which results in secure-world memory accesses being performed as normal-world accesses. This way, the secure-world can access normal-world as if normal-world is the one accessing the resource. This design decisions makes it hard to prevent secure-world from accessing normal-world memory. For example, TZC-380 is a TrustZone controller developed by Arm which has a feature enabling memory accesses performed in a secure state to not being able to access normal-word memory (priority inversion), however given that secure-world software can map memory as being normal, this does not prevent the secure-world from accessing normal-world memory. %, it just has to do so intentionally.

%As alluded to earlier, to enforce the access control of each security state it is necessary to use dedicated hardware. Arm sells two TrustZone controllers TZC-380 and TZC-400 to this end. They differ in the features they provide, but both allow for specifying a hierarchy of memory regions with r/w privileges and secure and non-secure access. Although feature-full, Arm's TrustZone controllers are not deployed in every TrustZone-enabled system. It is common for SoC vendors to design and implement their own TrustZone controllers. This enables SoC vendors to tailor the hardware to their specific needs, but also results in less features and in a fragmentation of TrustZone-enabled systems. For example the rk3399 from Rockchip only allows the configuration of memory regions security state, and not other access control mechanism is present (e.g., R/W). Another example, is Zynq xxx, which only allows the configuration of all SRAM as either secure or non-secure. The broadcom SoCs used in the RPi don't feature a TrustZone controller of any sort[...], although the CPU cores themselves implement the TrustZone specification.



\subsection{Platform Model for \project}\label{sec:plat_req}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/rezone-hw.pdf}
    \caption{\project enabling hardware components and typical components of platform featuring Trustzone. \jose{talvez fizesse mais sentido trocar a ordem do rpc e tzc. isto para seguir o raciocinio do nuno quando aos espaços de endereçamento.}}
    \label{fig:RZ_HW}
\end{figure}

\project's design makes a set of assumptions regarding the features offered by the underlying platform, which are the basic primitives needed to implement the key protection mechanism described throughout this section. These include:

\begin{enumerate}

    \item a \textbf{Platform-level resource protection controller (RPC)}, i.e., a dynamically configurable memory and peripheral protection controller. The access checks performed by the RPC must be orthogonal or additional to those provided by Trustzone's (e.g. TZASC). The RPC shall be capable of (i) setting fine-grained access control attributes (e.g., RO, RW) for a each defined memory region; (ii) differentiating between multiple bus-masters; and (iii) protecting memory-mapped input/output (MMIO) \sandro{(acronym needs to be defined)}\jose{done} regions, including their own; %to, but including,

    \item at least one \textbf{Programmable system management core}, i.e., an independent processor, distinct from the main application processors. Typically, these cores are added for housekeeping purposes and implemented as small MCUs (e.g., Cortex-M4); \sandro{(Martins, I slightly extended this point, so please check if you are comfortable with changes)}\jose{made a minor change. i think now it's ok.}

    \item \textbf{Secure boot process} that is able to guarantee a management core is in full control of the system's protection controllers, while their access is blocked to the main application cores.

\end{enumerate}

These requirements are modeled on the platforms described in ($\S$\ref{sec:hwmp}) and ($\S$\ref{sec:otherplat}). Although we did not carry out an extensive survey, we believe many other current and future platforms will meet these requirements, especially those targeting the high-end embedded markets such as automotive. \sandro{We need to be more confident in this message.} \jose{need to discuss} %Also, there is an increasing trend to include similar mechanisms in mobile SoCs. For example, Qualcomm's SPU (secure processing unit)~\cite{Qualcomm2019} provides many, if not all, of the aforedescribed features.

\sandro{I like this paragraph but I strongly believe it should be moved to the Implementation or Discussion section. At this point, a reader/reviewer without much knowledge cannot understand what is being discussed.} \jose{need to discuss}
\newline
{\color{red}We designed \project assuming that, w.r.t. application cores, the protection controllers act only on a per-cluster basis. Typically an RPC cannot differentiate between the multiple cluster cores as it observes requests as being from a single bus master, the shared cache. All accesses to the internal cluster caches will not be subject to RPC restrictions, only to TrustZone's. Despite being a limitation and not actually a model requirement, we make this assumption given that both platforms we model these design requirements on have this characteristic. If a similar platform fulfills all of the aforementioned requirements and, in addition, provides per-core isolation, this would allow for the system to be more flexible, scalable and performant.}


==> extra/sec5-nuno.tex <==
%=======================================================================
%> [IMPLEMENTATION]
%=======================================================================	
\section{Implementation}
\label{sec:impl}



%\david{sections orientadas ao challenge, interface}


%\nuno{I think it might flow better to have the organization in terms of ``monitor / nw / SW domains'' moved into the design section because it's mostly directly related with the goals we want to achieve. Then here we can restructure the implementation section around the implementation challenges and the respective solutions -- possibly, some of the titled (bold) paragraphs currently in this section.}

%\david{explain this section, otherwise subsections are too much standalone}
%To implement \project we take advantage of a programmable MCU present in both our test platforms, iMX8MQ and iMX8QM, and in the flexibility both this platforms provide in assigning memory resources to different processing elements while excluding others.
%\david{Mention that we modify TF-A.} 
%make sure a reader could reconstruct the implementation

In this section we focus on the implementation challenges of deploying \project in a real world platform. Challenges arise in various aspects of the implementation. From synchronizing cores before executing the Trusted OS, to securely performing a context switch to the s.EL1 and correctly handling normal world and trusted world exceptions. 
In our implementation, we take advantage of the Resource Domain Controller (RDC), and a programmable MCU present in the iMX8MQ platform.
One of the main challenges in our implementation is that, although part of our model, the RDC only performs access control to main memory and not at a cache level. This means that accesses can only be controlled at a cluster level granularity, because it's the last level cache of the cluster which performs the memory accesses. This forces us to perform cache maintenance operations to guarantee that a zone does not access memory outside of the sandbox. Another insidious consequence of this, is that using the RDC to establish read-only memory regions still allows a core to make changes of memory contents at a cache level. This will result in CPUs in same cluster retrieving potentially manipulated values, given that the memory accesses will result in cache hits. Solutions for these problems are presented in this section. 

After discussing which software stack we use to prototype \project, we start by explaining the RDC programming model, then we explain how we boot the system, after which we explain how we tackle core synchronization challenges before executing a Trusted OS. Next, we explain how we guarantee secure RDC configuration, and the steps required to safely exit to s.EL1 and to handle its exceptions in the trampoline. Finally, we explain how we can restrict accesses to peripherals to the AP while, allowing other bus masters to access them.

\if0 %refer to figure 3. hardware platform
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/hw-arch/rezone-overall.pdf}
%     \caption{Hardware achitecture and components of a \project enabled system}
%     \label{fig:my_label}
% \end{figure}
\fi

\subsection{Nuno's notes}

\nuno{Explain optimization of shifting logic from the gateway to the trampoline because the AUC is much slower than the main processor cores.}
...issues a request to the gatekeeper to further configure the PPC to block access to to the protection controller itself by the application cores. This prevents a zone from reconfiguring its access privileges

\nuno{Implementation of the secure channel and usage of separate registers.}
The key idea of our design is centered around the creation of multiple secure-world zones which sandbox TrustZone's sEL1 and sEL0 privilege levels and that can be activated on-demand by EL3 software. To this end, our design includes a custom world-switch mechanism which leverages: (i) the hardware primitives detailed in ($\S$\ref{sec:plat_req}); and (ii) the fact that, although TrustZone does not provide EL3/sEL1 address space isolation, there is actually strong privilege isolation at the register level since the latter cannot access the former's system registers. 
At boot time, a secure communication channel is established between the secure monitor and the \textit{\project Controller} based on a secret-key that is kept private to the monitor by storing it in an EL3 register. The \textit{\project Controller} authenticates the secure monitor, at each request to block or unblock RPC access by the application cores.

Because the trampoline is shared between the monitor and the untrusted zones, this software component must be tailored to be as minimal as possible and encompass mostly read-only memory to avoid corruption from a rogue Trusted OS. All writable data used by the trampoline must be non-critical and can't be re-used upon a zone exit.

This token is protected during zone execution by storing it in an EL3 register. 

\nuno{System Initialization and Multi-zone Support: moved from design section}
To setup the system, the normal world's and all zones' domains must be statially defined at design-time. This includes defining access privileges to memory and peripherals address ranges, and explicitly  identify shared-memory regions between each zone and the REE. A user must also disable dynamic shared memory allocation in the Trusted OSs. This feature allows any normal-world address to be used as shared memory but, given that shared memory regions are defined statically, it cannot be used. From our experience, mainstream Trusted OSs such as OPTEE or ??? allow turning it off at compile-time. For each defined zone, the corresponding Trusted OS must be be associated with an unique range of SMC (Secure-Monitor Call) IDs. Trusted OSs originating from different vendors use the same SMC ID ranges as defined by the SMC Calling Convention (SMCCC) \cite{}. Since \project allows different Trusted OSs, or event the multiple instances of the same Trusted OS, in the same system, the issue arises of conflicting SMC IDs. To solve it, our current design mandates that a user must manually modify both the normal-world drivers and Trusted OS handlers to offset the SMC IDs of each Trusted OS instance so that each falls in a mutually exclusive range. We believe the range defined by the SMCC is sufficiently large to host all possible SMC IDs in a realistic system configuration. All this information is directly compiled into the monitor image. At system initialization, the monitor creates an RPC configuration for each zone as well as a map of SMC to zone IDs. It then activates each zone in a sequential fashion so that each trusted OS can perform its initialization, before handing control to the REE OS. At runtime, when the normal-world OS issues a request to the secure world passing it a given SMC ID, the monitor will translate the SMC ID into a zone ID, fetch the zone's RPC configuration and commit it to the hardware before jumping to the Trusted OS.

\subsection{Software and Software Modifications}

To implement \project we modified and used several open source secure world components. For monitor we used Trusted Firmware-A (TF-A) and made modifications to the Trusted OS services to make them issue the rezone\_suspend interrupt, and also modified EL3 exiting code, and vector table code, to implement the trampoline. Additionally, to support multiple Trusted OSs we made the necessary changes to TF-A's context management routines and data structures, while duplicating the OPTEE service, to handle requests to the second OPTEE instance.
To safely run Trusted OSes without them being able to thwart the established access policies \project controller takes ownership of the RDC. To implement it we make use of the provided board support package, including drivers to interface with the RDC and perform initialization routines. Although the platform supports true random number generation, in our prototype we do not make use of this feature due to lack of support for it for both the monitor and micro-controller. A developer with access to the appropriate documentation should use the features available in the platform to securely generate the secret token.
No intrusive modifications are necessary to execute OPTEE in a secure world zone. However, a deployed OPTEE build will not support dynamic shared memory, and so the configuration parameter must be set do disabled. Additionally to support running multiple Trusted OSs, we create a second OPTEE instance in a different address space, which required specifying the designated address space. Additionally, we updated the values of SMC IDs to be uniquely attributed the second OPTEE instance.
It is not necessary to modify REE code to support \project, however, because we added support to run multiple Trusted OSs, it is necessary to add drivers to interface with both of them. In our prototype we duplicate the OPTEE Linux kernel driver, and modified the SMC\_IDs used to make calls to the second OPTEE instance. Additionally we also have two tee-supplicant services, one for each OPTEE instance.

\subsection{Hardware Memory Protection}\label{sec:hwmp}


%\subsection{\color{red} System Hardware Protection Controllers}\label{sec:hwmp}

%\textbf{NS: Once you've set the stage to the problem we want to tackle -- i.e., the coarse level of isolation featuring the current TEE hw/sw architectures -- then it's time to talk about the new hardware features available in emerging boards and talk about the potential they have to increase that granularity and as a result increase the security of TEEs. I confess that the current text is somewhat confusing. I'd prefer to have some structure where you start off by saying that our goal is to design a new architecture that increases the granularity of privilege separation using these new cool hardware features, then have one paragraph to talk about each feature; then maybe a table or something else were to present the specific features of each board. The cool feature could be something like: a) protection units for fine-grained memory partitioning, b) per-cluster policy enforcement, etc. For each, describe what it is, and explain how it could be leveraged to increase the state of affairs presented in the section above.}
%TZASC / TZASC-like and TZPC / TZPC-like hardware. Hardware which enforces security-state policies. Such which memory is marked as secure. TrustZone is a specification, TZASC and TZPC are not. They are a proprietary solution whose use Arm charges money for. Vendors often develop their own hardware security-enforcement IP, which has different, and often less, features than those of Arm


% Because TrustZone design is the enabler for the severity of vulnerabilities found in TrustZone, TrustZone enforcing hardware is not enough to address this problems. Lately, several platforms have came up with hardware mechanisms to create domains within the SoC. These domains are independent of TrustZone and aim to control access to subsets of system resources for the various masters of the platform (e.g., Application Processor, microcontroller, GPU, etc).
% Chip designers provide hardware based mechanisms to validate memory accesses. They are generally called protection units. Here we provide some examples:
% \begin{itemize}
    % \item Xilinx - Xilinx Memory Protection Units (XMPU) and Xilinx Peripheral Protection Unit (XPPU)
    % \item NXP - Resource Domain Controller (RDC), Extended Resource Domain Controller (xRDC) and xRDC2
    % \item Qualcomm - xPU "This means the XPU registers are only one mean to secure peripherals and/or memory, all of which can be protected by other technology like TrustZone isolation." %https://blog.quarkslab.com/analysis-of-qualcomm-secure-boot-chains.html
    % \item Qualcomm - SPU memory controller "The TSF shall be implemented to restrict the ability to [modify and define] the memory areas shared with other components of the SoC to SP-ExtMM controlled by the SP-CPU." %https://www.commoncriteriaportal.org/files/epfiles/1045b_pdf.pdf
    % \item ? Apple - Hardware “filter” to prevent AP to SEP memory access -Only SEP’s KF core has this filter %https://www.blackhat.com/docs/us-16/materials/us-16-Mandt-Demystifying-The-Secure-Enclave-Processor.pdf https://www.theiphonewiki.com/wiki/Secure_Enclave_Processor
% \end{itemize}


%There is an ongoing trend in the SoC industry to embedded an increasing number of processing units and bus masters in the same chip and to provide additional mechanisms to isolate them. In response, we start seeing an increasing number of platforms which implement, at the system level, additional hardware access control mechanisms orthogonal to TrustZone. In the following, we describe a few examples implemented in the NXP iMX8 and the Xilinx Zynq UltraScale+ families. 

There is an ongoing trend in the SoC industry to embedded an increasing number of processing units and bus masters into the same chip. In response, we start seeing an increasing number of platforms that implement, at the system level, additional hardware access control mechanisms orthogonal to TrustZone.% In the following, we describe a few examples implemented in the NXP i.MX8 and Xilinx Zynq UltraScale+ families. 

NXP has developed an hardware controller which aims to create multiple security domains within the SoC by allowing chip resources to be separated into domains. The i.MX 8M family of processors features the \textit{Resource Domain Controller (RDC)}.
%while the i.MX 8QuadMax family features the \textit{Extended Resource Domain Controller (XRDC)}. Both controllers have similar high-level features, but the XRDC module is a new iteration which incorporates TrustZone controller features, not requiring two separate onboard controllers. 
The RDC is hardware embedded in the SoC that enables the creation of multiple platform domains. A domain is a collection of resources (e.g., memory regions, peripherals) and respective access permissions. Access permission specify the access privileges each Domain ID in the platform has over a specific resource.
A Domain ID establishes a collection of masters to which access permissions for each resource applies.
This enables fine grained control of access permissions in platforms that feature multiple processing elements. For example the iMX8M features a GPU, Arm application processor (4 cores), one MCU (Cortex-M4), etc. Each Domain ID can be attributed with exclusive rights to a given resource, expanding on the TrustZone dual-world model of system security to multi-domain platform control. 

In \project we establish the the following domains using the RDC. AP domain, Domain ID 0, to which all memory and resource restrictions we intend to enforce on the AP are applied.
To allow secure execution of the \project Controller, and to allow the \project Controller to take exclusive access of the RDC we establish Domain ID 1, \project Controller domain.
Additionally we need a third domain, Domain ID 2, the reasons for which we explain in \autoref{sec:sharing_periph}.
%Note that in both families, Cortex-A CPU clusters are assigned with a unique master ID, which means policies cannot be enforced per core. 

%  On final aspect of these platforms is that each cluster is a master. This means that memory regions cannot be assigned to a single core, but may be assigned per cluster, allowing for memory access policies to be granular at the cluster level.
\david{Note: In the iMX8MQ, the upper 1GB is not protectable by RDC. This is not really problem as long as that space is dedicate to non-critical applications. Not sure how feasible doing this though.}

\if0 % this is explained in background
% \mypara{No private CPU core memory} 
% The first limitation is that memory accesses cannot be controlled per core. This is because accesses to main memory are performed by the L2 cache, and because L2 caches are shared by the entire cluster. Having per core access control implies being able to control accesses to L2 cache. With the ability to specify memory control access per core it would be simpler to implement \project, there would be no need to perform synchronization between cores, and cache flushes would be limited to L1 caches instead of all L1 e and L2 caches, diminishing overheads.
% %The first limitation is that secure-world memory access cannot be controlled per core. Having control per core, would enable easily deploying multiple TEEs where a TEE running in one core could not access the memory of a TEE running in a second core, when paired with our first mechanism \ref{sec:impl}. \nuno{Please be concrete about what's the first mechanism. Also, does this only limit the ability to have multiple TEEs/IEEs? How does it affect the other security properties we're interested in?} However, we use the available control per cluster in the iMX8QM (the iMX8MQ features a single cluster), to similar effect.
% 
% \mypara{Trusted OS may always access normal-world memory} None of the features in the platform enable the Trusted OS to be truly restricted in accessing the normal-world memory. This is mainly due to the ability of the Trusted OS to map memory in a way that the CPU core performs non-secure accesses, which the TZC will not able to identify as coming from a core executing in secure world.
% 
% \mypara{TrusteOS can access secure-world resources} Another limitation is that there is no enforceable memory separation between the secure-monitor and the Trusted OS, Although they execute in different privilege levels. 
% %Additionally any configuration made by the secure monitor to hardware controllers (e.g., TZC-380) can be unmade by the Trusted OS. 
% %not entirely true, see tzc380 lock bit
% The kernel of the problem is that TrustZone access control only considers the security state of the processor, and not its privileged level. This lowers overall system security. 
% Additionally, because we aim to have multiple Trusted OSes in the secure world, with TrustZone only features, a Trusted OS can also access other Trusted OSes' resources.
% %\nuno{This last part reads a little bit vague. Are we only concerned that a compromised Trusted OS can access the monitor's memory? Or that it may also undermine isolation between IEEs' memory? Or that it also affects the peripherals?}
\fi

\subsection{Boot}\label{sec:boot}
When booting, the system must ensure that the ACU has exclusive access to its program memory by creating a dedicated domain for it, including dedicated memory regions and the required peripherals (e.g., the MU\_B). To do this in our test platform, which first boots the application processor, as part of its initialization routine, monitor will start the ACU before initializing the Trusted OSs. After starting, the ACU will run \project Controller which will set up the Domain IDs. From then on, the ACU locks access to RDC, only unlocking it upon a request from the trampoline.
%\nuno{what's exactly this ``system configuration''? how do we set this up securely? do we need to ensure that the  boots up first and before the other cores? if so, how do we guarantee that?} 
%
%To initialize the Trusted OSes, the boot process already preloaded unto memory the respective images.
%On the first Trusted OS execution the dedicated zone is already established, leaving the Trusted OS no change to compromise other system components right from the start.
%by issuing the SEC\_MON\_PROTECT command to the micro-controller, and establishing the trampoline before handling execution to the Trusted OS. \nuno{sorry, don't quite understand this step: ``can already'' or ``is already''? don't we need to hard-guarantee this?} 
%The trampoline is small region of code, that is marked as non-writable by TrustZone independent mechanisms present in the platform (i.e. the RDC). \nuno{the trampoline is part of the monitor, right? doesn't it also need to be protected against reading? otherwise can't the trusted os read the auth token from memory?}


\subsection{Synchronization}\label{sec:synch}
In \project, because we remove access of monitor, and normal world, code and memory to the CPU while the Trusted OS is executing, we must take care to prevent situations where the software would execute while the Trusted OS is active. Otherwise, they would simply crash as they cannot access neither the data, nor the code. These are the instances where such scenarios might occur (for the sake of simplicity we only consider two cores):
\begin{enumerate}
  \setlength\itemsep{0em}
    \item\label{sync1} Two cores are executing monitor code and one of them starts executing the Trusted OS. This is a problem, because while the Trusted OS is running, other cores will not be able to access monitor memory.
    
    \item\label{sync2} One core is executing the Trusted OS while another is sleeping, meanwhile the sleeping core awakens in monitor code (e.g. due to an interrupt). Again this is a problem because other cores are not able to access monitor memory while the Trusted OS is running.
    
    \item\label{sync3} One core is executing in the normal world, while the second core requires a service from the Trusted OS or a TA. This is a problem because, when the Trusted OS is running other cores are not able to access normal world memory.
\end{enumerate}

To address scenario \ref{sync1}, the monitor tracks which CPU cores are currently executing the secure monitor, and only jump to the Trusted OS when all of them leave the monitor.
Scenario \ref{sync2}, is solved by waking the CPU in an a read-only uncached memory region, which the Trusted OS will not be able to tamper with, and waiting for Trusted OS to cease execution by using a spinlock (rz\_lock). 
To solve scenario \ref{sync3}, we use an FIQ interrupt and a spin\_lock (rz\_lock). 
Before issuing the FIQ, the current core will grab the rz\_lock, and wait until other cores leave monitor code. For the cores that exit the monitor, they will have to wait in the trampoline for the lock to be released. When the current core is the only one executing the monitor, the core will issue an FIQ interrupt.
This interrupt will cause all cores executing in the normal world to enter the trampoline. 
At this point, both the cores that were running in monitor and exited, and the cores that were executing in the normal world, are waiting in the Trampoline for the Trusted OS to complete execution. We do this by making the waiting cores wait for the release of the lock.



%\subsection{Hardware Memory Access Control}\label{sec:rdc}
%The RDC present in the iMX8MQ is an hardware component external the CPU. By configuring it, it's possible to establish up to four domains. Domains are a collection of resources and corresponding access policies enforced the domain processing elements access them. Access to resources can be controlled by setting read and write permission access for each domain.
%
%
%\subsection{Sentinel and Application Processor}\label{sec:sentinel}
% To implement \project we leverage two domains. The application processor is bound to one domain. For normal world and monitor operations the processor can access the resources without restriction except for the RDC itself and the second domain. The microprocessor which executes the sentinel program is bound to the second domain. This domains is configured to be more privileged, having direct access to the RDC, and hence can configure the access policies affecting all other domains.
%
%\subsection{\project Trampoline and Exception Interposition}\label{sec:trampoline}
%We modified the context switching logic to be able to activate greyzone every time the Trusted OS executes. Furthermore, we need to interpose every event which returns control back the secure monitor. To achieve this we install our own vector table that uppon an event first waits for monitor protection to be disabled, and only then proceeds with typical execution.
%
%\subsection{Context Switching and Cache Maintenance}\label{sec:ctx_switching}
%Due to the external nature of the component described in \ref{sec:rdc}, accesses are only validated when data is either fetched or written to main memory. This means that memory access control is not performed at cache level, and special care must be taken to remove security sensitive data from cache before performing a context switch from monitor to Trusted OS.
%
%We must syncronize memory accesses when performing cache maintenance operations. In particular we must be certain that all outstanding memory accesses required by a flush operation are complete, before activating monitor protection. Arm provides a DSB to this effect.
% arm cortex a8 programmers guide
% Data Synchronization Barrier ( DSB ). All pending loads and stores, cache maintenance instructions, and all TLB maintenance instructions, are completed before program execution continues. A DSB behaves like a DMB , but with additional properties. 

\subsection{Secure RDC Configuration}
\david{This could go to design, there aren't really any special details i think}
To securely perform an RDC configuration, only the trampoline and \project Controller, are allowed to access it. This is achieved by having the \project Controller lock the RDC, at all times except during reconfiguration in the trampoline.
This way the Trusted OS cannot tamper with the established configuration, without unlocking access to the RDC. Unlocking is only possible if the AP sends the correct secret token to the \project Controller. During Trusted OS execution this token is kept in a EL3-only register, TPIDR\_EL3, leaving the Trusted OS to guess the secret token value (a 1 in $2^{64}$ chance of guessing correctly). 
% The original value of TPIDR\_EL3, is stored in memory which will only accessbile to EL3 after RDC configuration. % To much detail?
Communication between the AP and ACU is established by using hardware communication a mechanism present in the iMX8MQ platform, the Message Unit (MU). The MU is composed of two peripherals MU\_A and MU\_B, implementing the MU interface. MU\_A is exclusively assigned to the AP, while MU\_B is exclusively assigned to the ACU, by configuring the RDC to only allow the AP and \project Controller domains to access their respective MU interface. Doing this allows the system to unambiguously establish a communication interface between the AP and the \project Controller.

\if0 % this is already mentioned in the design
Effectively, \project makes the secure monitor in charge of setting up memory access control policies, however it does not have direct access to the RDC. \david{update} The component which has access to the RDC is the ACU, and because the means used to communicate with the ACU are available to both the secure-monitor and Trusted OS, it is necessary for the secure-monitor to authenticate itself when issuing commands to the ACU. If no authentication is performed, a Trusted OS could use the hardware-based interface between the application processor and ACU to issue commands to undo the established memory access policies.
%
The authentication is simple, but effective. \project requires a secret token. The token is 64 bit wide, and is stored in a CPU register inaccessible to a Trusted OS. 
The content of this register is inaccessible to a Trusted OS due to the EL3 level of privilege having exclusive access to it. This results in any attempt to access these registers from EL1 leading to an exception handled by the monitor.
A compromised Trusted OS has a 1 in $2^{64}$ chances of guessing the secret token. Any token mismatch signals the presence of a compromised Trusted OS to the ACU, and steps may be taken accordingly.
%\nuno{what's the communication channel between the monitor and the ACU? what prevents the trusted os from accessing the token? how is the token (which is a secret) securely loaded into both the monitor and the ACU?}
%
To establish its identity, the first command the secure-monitor issues to the ACU is a request for the generation of the secret token used in authentication requests. Implicitly the ACU will trust the first request after booting is from the secure monitor. This holds true because the token exchange is done before a Trusted OS begins execution, giving a Trusted OS no opportunity to interfere with this step.
%\nuno{why can we trust that this request comes from the secure monitor and not from the trusted os? is it because you assume that the system will first boot into EL3 code? in other words, you always assume that the first request is trusted by the ACU?}
%
In the first command, the ACU generates and stores the token in its dedicated memory, and issues the token to the secure monitor. 
%\nuno{how can we ensure that it's not intercepted, e.g., by another core running already in sEL1?}
%
To create the token, a sufficiently high-entropy source must be used, as is standard practice. It is common for platforms to be equipped with hardware designed for such cases. Such is the case with our test platform.
\fi

\subsection{Secure Exit to s.EL1}
%\nuno{wasn't a part of this already explained in the section above?} 


\mypara{Micro-Architectural Maintenance}\label{sec:cachemaintenance}
Upon checking that an SMC is a Trusted OS call, the monitor will suspend the other cores in the same cluster, and enter the trampoline before exiting EL3.
% I actually don't know how to only interrupt cares in the same cluster, but I can think of "workarrounds" that implement the same effect
In the trampoline, the core will perform micro-architectural maintenance operations, to ensure that a Trusted OS cannot access resources outside of the zone. These operations include invalidating the L1 instruction and data caches, as well as the L2 cache. This is necessary, because, if data or instructions are left in the cache the Trusted OS will be able to access them. With access to this information the Trusted OS can potentially read secrets, but more importantly it can malicously modify data and instructions. Both data and instruction would then be used by unsuspecting victims, and can result and the compromise of the established isolation between domains. For example, it would possible, in principle, for a TrustedOS to modified REE kernel code to open backdoor to an attacker.

In addition to performing cache flushes, when switching between Trusted OSes, TLB maintenance (i.e., TLB invalidation) for the current core is required for switching between Trusted OSes. Not due to security concerns, since both Trusted OSes are encapsulated in a zone and can only access memory directly assigned to them, but because otherwise a Trusted OS could be addressing parts of the the other Trusted OS address space, causing unexpected faults. As an optimization, we only perform TLB maintenance if the last invoked Trusted OS is different from the one we are currently going to execute. In practice this prevents TLB maintenance operations when the system is making use of a single Trusted OS, as invalidating the TLB is only necessary when switching between Trusted OSes.

At the last step, we disable SMP coherency before jumping to the TrustedOS. Recall, that during EL3 exit to s.EL1, we have suspended all other cores in the cluster. Each core has data and instruction in their own L1 caches. With SMP coherency enabled, a request to access data present in these caches would cause a cache hit, and data could be accessed, with the same consequences previously explained. Disabling SMP coherency, prevents this from happening, thus providing a simple way to mitigate this issue. Without support to disable SMP coherency, as part of the suspending mechanism we would have to flush each cores L1 caches to ensure that data in the other cores caches would not be accessible.

With all micro-architectural maintenance done, the trampoline will restore the general purpose register state, and exit to the Trusted OS.
\autoref{fig:scr_ctx_hw} depicts the required steps to securely exit to s.EL1. \david{I don't think the picture is essential to convey these ideas}

% TrustZone extends memory accesses with one bit. This bit informs whether the access is mode from a secure context or a normal context. This information extends to the cache, and with each cache line a bit is stored to keeps track of whether the line was fetched has secure or normal. This allows for efficiently separating normal world accesses from secure world accesses, but not without flaws~\cite{armageddon, truspy}. We make standard use of this feature, using it to prevent the normal world from accessing secure memory.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/hw-arch/rezone-ContextSwitch.pdf}
    \caption{Context-Switch to and from a TrustedOS requires micro-architectural maintenance operations including cache and TLB maintenance.}
    \label{fig:scr_ctx_hw}
\end{figure*}

\subsection{Handling Exceptions from s.EL1}
Handling exceptions from s.EL1 in \project must be done carefully, otherwise a malicious Trusted OS may be able to escalate privileges to the monitor or attack the normal world. There are two problems in taking a naive approach to handle exceptions from s.EL1:

\mypara{MMU TLB-Miss on Handling Exceptions in EL3}
Upon entering the vector table, it may be the case that there's no TLB Entry that maps the region of code. In this case the MMU will fetch the PTE that maps it to perform a page table walk, which will result in the TLB issue memory accesses. Because we've flushed page tables from the caches as part of the secure exit to s.EL1, a main memory access must be performed. However, the memory will be inaccessible as established by the trampoline. This would result in the system hanging, as the code for handling the exception would not be accessible. The issue is depicted \autoref{fig:p}~a).

\mypara{EL3 Code Injection from sEL1}
The code on the vector table must be readable from main memory, and thus marked as readable by the processor on the RDC. 
However, this will also give the TrustedOS the ability to read the code.
Due to the memory hierarchy, the vector table code will now also reside in cache, and write operations are now allowed (as long as they do not reach main memory). A TrustedOS can maliciously modify the exception handling code (e.g., modify SMC handling code), to its own advantage. Upon an SMC, the Monitor would then execute malicious code which is obtained from \emph{hitting} the cache, i.e., from not obtaining from main memory. The issue is depicted \autoref{fig:p}~b).

\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{images/rezone-problems.pdf}
    \caption{a) A TLB miss may occur while page table memory is protected; b) A malicious TrustedOS can inject code into the the secure monitor, even if RDC marks the code memory region as read-only.}
    \label{fig:p}
\end{figure*}

To solve both of these problems in the last steps of exiting to s.EL1 we disable the MMU for code running in EL3. This solves problem 1, as from that point on, memory access performed by EL3 will not be subject to MMU translation, thus no access to page tables is necessary, and exception handling code will be executed. Disabling the MMU will also disable caches for the core, and this will partially solve problem 2 as the exception handling code will always be fetched from main memory, and in main memory the corresponding memory region is enforced read-only by the RDC configuration, thus no modifications will be possible. The problem is still not entirely solved, however. Note that during the secure exit to s.EL1, after flushing all caches the trampoline still executes with caches turned on. This will inevitably leave traces of data and instructions, which a malicious Trusted OS can try to leverage for an attack. To prevent this from happening we must invalidate trampoline related memory in the exception handler. As an optimization, as opposed to performing the cache maintenance operations with caches turned-off, we first invalidate a small function <function name>, still with MMU turned off. After invalidating <function name> we jump to it, and re-enable the MMU (and thus, caches). This function will then invalidate the rest of the trampoline memory. 
%Because it is not possible to only invalidate readonly memory regions, we temporarily re-enable RDC protection for the trampoline memory region, and perform a cache flush. The RDC will guarantee that no modifications reach main memory, and in effect allow the trampoline to invalidate any code and data changes. % I'm thorn on giving this much detail of the implementation
After the cache management operation the exception can be handled securely.
Due to the additional steps required to securely handle s.EL1 exceptions, we establish different vector tables for cores exiting to normal world (i.e., El1 or EL2), and for cores exiting to s.EL1, resulting in having different exception handling code for exceptions from s.EL1 and EL1/2.

\if0 % I believe this is already explained in the design
\mypara{\project Trampoline} 
% \nuno{the text is good, but it's too descriptive: it doesn't explain why we do things the way we do.
% For instance, these are some of the questions I had after reading this first paragraph. 
% Why do we need to suspend the cores? 
% Why is this only be done at the cluster level? 
% Why are we evicting the caches? 
% Why is cache evicting skipped when protecting the secure monitor?
% }
%
Before reconfiguring memory access control policies, the secure monitor enters the \project Trampoline region.
This region is marked as readonly while a Trusted OS is executing, to enable code execution by the monitor. This is required to prevent the memory reconfiguration from causing causing execution errors. 
We mark it as readonly because the application processor still needs to be able to read this region instructions to be able to execute them. By marking it readonly we guarantee that even the presence of a malicious Trusted OS, the region is unmodified, and thus the code cannot be bypassed.
If the \project Trampoline would be marked as non-accessbile, it could lead to a crash after reconfiguring memory access control policies, due to the secure monitor trying to fetch instruction which could be not retrieved from memory. In the same vein, a readonly \project Trampoline also enables secure exception handling, because it allows immutable code to handle exceptions.
It is in the \project Trampoline that the target zone is activated. 
%\nuno{I'm confused: isn't the trampoline part of \project? what you mean by disabling \project?}
A Trusted OS could try to run code from the \project Trampoline to deactivate the active zone, however this code relies on access to EL3 only registers, as described in ($\S$\ref{sec:mon_auth}), thus any such attempts to bypass \project will be unsuccessful.

In the \project Trampoline the target zone is activated by issuing a SEC\_MON\_PROTECT command to the ACU. If the ACU identifies the secure-monitor successfully, the ACU will enforce the configured access control policy. The secure-monitor will wait for a response from the ACU, after which it performs core micro-architectural maintenance (see $\S$\ref{sec:cachemaintenance}). After this, execution control can safely be transferred to the Trusted OS.

The trusted OS will execute, and will likely schedule a TA to service the normal-world request. Upon completion, the Trusted OS will return execution to the secure-monitor by issuing a SMC instruction. The SMC is handled in the previously established \project Trampoline. The secure monitor will then interact with the ACU once again to re-allow access to the secure monitor program memory, and wait for the MCU response and resume execution on all cluster cores, including returning to the normal-world. 
%\nuno{Part of this has been explained in the section above.}

An additional problem arising from marking secure monitor program memory inaccessible to the CPU is the loss of a program stack for performing operations \nuno{please explain this better}. We solve this issue by having a separate stack used during memory reconfiguration, and before evaluating whether the Trusted OS is executing. \david{where to put this?}
\fi

\subsection{Sharing Peripherals with Other Bus Masters}\label{sec:sharing_periph}
In \project we are able to give a zone access to specific devices. We use this feature to prevent non-related devices from being accessed by the Trusted OS. However, other bus masters may need access to these devices, for example to play audio asynchronously to the AP. If these masters are configured to be in the same Domain ID as the AP, they will also be prevented from accessing the devices. To solve this, we use three RDC Domain IDs, Domain ID 0 which the only participant master is AP, Domain ID 1 to which the ACU and its peripherals (e.g., RDC) belong, and Domain ID 2 for all other masters. Domain ID 2 is given access to all peripherals and memory regions at all times. This will enable the masters from this Domain ID to access the required peripherals even if the AP can't access them at a given point in time.

\subsection{Multi Cluster Scenario}\label{sec:mult}
%Our test platforms provide the necessary mechanisms for deploying a system with multiple TEEs. \nuno{TEE software, each one inside an IEE, right?} To implement multiple TEEs in the platform featuring a single cluster, the iMX8MQ, it's necessary to make only the current TEE's program memory available to EL-1. This is achieved in a similar way that secure-monitor program memory is protected; the RDC is used to prevent access to the required memory regions (i.e. other TEEs). When handling trusted service requests the secure-monitor will enable, by interacting with the micro-controller, only the required TEE to execute the service. Figure \ref{fig:multi-tee-same-cluster} illustrates the process. 
%
To implement multiple TEEs in the platform featuring more than one cluster, in addition to the techniques mentioned above, we can also leverage the fact that memory access policies can be defined per cluster. This enables simultaneously running one TEE per cluster while benefiting from mutual isolation. 
%Figure \ref{fig:multi-tee-multi-cluster} illustrates memory configuration for achieving this. 
There are many ways to employ this idea, one might be to have as many TEEs as clusters, and statically assign a TEE per cluster. This allows for a straightforward implementation of protection mechanisms, while allowing multiple TEEs to serve trusted service requests parallel to each other. More complex implementations might optimize TEE distribution base on available clusters, to run any TEE on any cluster while clusters are available to execute as many trusted services concurrently as possible.
Given that it's possible to run different TEEs on different clusters, one problem arises. Which TEE should run an each cluster. Nowadays it is common for CPUs to be implemented in a BIG.little configuration. So it is intuitive to assign performance sensitive workloads to high performance cores. System designers may define what services are to run on each cluster as to provide the best user experience. \david{These points could go to the design}

\if0 % this is clearly implied, or mentioned in the design, I don't think we need to raise this point further
% \subsection{Concurrent Normal-World Trusted Service Requests}\label{sec:concurrent_nw}
% Because we suspend all cluster cores, we do not support concurrent requests in the single cluster of the iMX8MQ platform.
% %\nuno{why having a single cluster prevents the execution of concurrent requests? is it something that we prevent for safety reasons? or is it something that is intrinsically disallowed by the platform's hardware?} 
% Calls to the Trusted OS are, therefore, inherently serialized.
% %\textbf{David: We have two options, either stall the request, until the executing is concluded, or return a busy state. The latter is probably more compatible but less user-friendly, the former may require Linux driver modifications}.
% On the iMX8QM, which features two CPU clusters, it's possible to serve up to two simultaneous trusted service requests if they are executed on different clusters, otherwise they'll have to be serialized. 
% %\nuno{again, similar questions.}
% Issuing the service request to the correct cluster, may require Linux driver modifications.
\fi 


\if0 % very old text. ignore
% \subsection{Design Alternatives}
% Experiments and alternative decisions we tried.
% 
% \subsubsection{Clear cache state before jumping to Trusted OS}
% \david{This would only make sense if we are trying to protect monitor only. However maybe we could present this section as \textit{assuming same priviliege isolation techniques on Trusted OS}}
% Perform combinations (instruction and data maintenance) of the following from non-cached memory:
% \begin{itemize}
%     \item invalidate instructions (remove instructions from cache)
%     \begin{itemize}
%         \item by virtual address
%         \item single instruction (clears instruction cache)
%     \end{itemize}
%     \item flush (clean+invalidate) data
%     \begin{itemize}
%         \item Try to identify commonly used data before jumping to Trusted OS by (by virtual address)
%         \item flush all monitor data (by virtual address)
%     \end{itemize}
% \end{itemize}
% 
% \subsubsection{Clear only writable data before jumping to Trusted OS}
% \david{This would only make sense if we are trying to protect monitor only}
% Only flush RW data, and invalidate vector table instructions.
% With intact vector table code, we can safely perform invalidation operations while RDC is still active to prevent undue writes to main memory.
% After clearing all monitor data we can safely disable RDC.
% 
% \subsubsection{Using same privilege techniques + \project}
% Use same privilege isolation techniques + the \project mechanism to prevent updates to pagetables.
% We marked Trusted OS pagetables as uncacheable, so that they benefit from RDC protection.
% 
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{images/benchmarks/xtest_simple_barchart_mon.pdf}
%     \caption{Secure monitor isolation tests.}
%     \label{fig:xtest_mon}
% \end{figure*}
\fi





==> space-tricks.test.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}

%\newcommand{\subparagraph}{}
\usepackage[small,compact,noindentafter]{titlesec} 
\usepackage[compact]{titlesec}

\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}

\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[subtle,margins=normal]{savetrees}
%\usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}
